Deep Reinforcement Learning for Joint Cruise Control and Intelligent Data Acquisition in UAVs-Assisted Sensor Networks

Unmanned aerial vehicle (UAV)-assisted sensor networks (UASNets), which play a crucial role in creating new opportunities, are experiencing significant growth in civil applications worldwide. UASNets improve disaster management through timely surveillance and advance precision agriculture with detailed crop monitoring, thereby significantly transforming the commercial economy. UASNets revolutionize the commercial sector by offering greater efficiency, safety, and cost-effectiveness, highlighting their transformative impact. A fundamental aspect of these new capabilities and changes is the collection of data from rugged and remote areas. Due to their excellent mobility and maneuverability, UAVs are employed to collect data from ground sensors in harsh environments, such as natural disaster monitoring, border surveillance, and emergency response monitoring. One major challenge in these scenarios is that the movements of UAVs affect channel conditions and result in packet loss. Fast movements of UAVs lead to poor channel conditions and rapid signal degradation, resulting in packet loss. On the other hand, slow mobility of a UAV can cause buffer overflows of the ground sensors, as newly arrived data is not promptly collected by the UAV. Our proposal to address this challenge is to minimize packet loss by jointly optimizing the velocity controls and data collection schedules of multiple UAVs.Furthermore, in UASNets, swift movements of UAVs result in poor channel conditions and fast signal attenuation, leading to an extended age of information (AoI). In contrast, slow movements of UAVs prolong flight time, thereby extending the AoI of ground sensors.To address this challenge, we propose a new mean-field flight resource allocation optimization to minimize the AoI of sensory data.

==> Mymacros.tex <==
%some macro definitions

% format
\newcommand{\class}[1]{{\normalfont\slshape #1\/}}

% School
\newcommand{\Feup}{Faculdade de Engenharia da Universidade do Porto}




\theoremstyle{definition}
\newtheorem{Def}{\textbf{Definition}}
%\newtheorem{lemma}{\textbf{Lemma}}
\newtheorem{corollary}{\textbf{Corallary}}
\newtheorem{Obs}{\textbf{Observation}}


%\newcommand{\equals}{\stackrel{\mathrm{def}}{=}}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}


==> Persistence.tex <==
\part{Implemented Design}

==> Quote.tex <==
\cleardoublepage
\thispagestyle{plain}

\vspace*{8cm}

\begin{flushright}
  \textsl{``If I have seen further it is by standing on the shoulders of giants''} \\
	\vspace*{1.5cm}
	Sir Isaac Newton
\end{flushright}


==> README <==
%% FEUPPHDTESES Style for LaTeX README
%% Document Style `FEUP PhD Teses'
%% By Mario Saenz Espinoza
%% mario.espinoza at fe.up.pt

%% General Considerations:
	%% - Uses BibTeX
	%% - Uses MakeIndex

%% Make sure to specify those properties in the "Project/Properties" section of your LaTeX editor.
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% TOP MATTER
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Package options:
	%% - prodeb/prodef/pdeqb/pdeec: choose a doctoral program
		% PRODEB: Programa Doutoral em Engenharia Biomedica
		% PRODEF: Programa Doutoral em Engenharia Fisica
		% PDEQB: Programa Doutoral em Engenharia Quimica e Biologica
		% PDEEC: Programa Doutoral em Engenharia em Electrotecnica e Computadores
	%% - libre: for any kind of work that is not the PhD thesis (e.g. monografia, workplan, etc.)
	%% - jury: copy for the Jury
	%% - final: final copy
	%% - onpaper: links are not shown (for paper versions)
	%% - linenum: to include line numbers
	%% - backrefs: include back references from bibliography to citation place
	
%% \graphicspath:
	%% - Where the "Figures" folder is located.  Save all your images in this folder
	
%% \include{mymacros}:
	%% - Save all macros in this .tex file
	
%% \hyphenation:
	%% - Set all the special hyphenation exceptions.  Shouldn't be needed, but could be useful for the "Resumo"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% GENERAL INFORMATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% \author
	%% - Your name

%% \title
	%% - Title of your thesis

%% \supervisor
	%% - Name of your Supervisor

%% \thesisdate
	%% - Date of your thesis.  Use only "month, year"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CHAPTERS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Add your chapters, each in a sepparate .tex file


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% BIBLIOGRAPHY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% This is tricky.  There is a difference between 'bibliography' and 'references'.  'Bibliography' is all the literature you used in your research, whether you cited them explictly or not.  'References' are the specific entries you have cited and your work is referred to.

%% Therefore, if you are using 'Bibliography', the whole section in the main file ('Template_EN.tex') should look like this:

% \renewcommand{\bibname}{Bibliography}
% \phantomsection
% \addcontentsline{toc}{chapter}{Bibliography}
% \begin{singlespace}
	% \nocite{*}
	% \bibliographystyle{IEEEtranSN}
	% \bibliography{References}								% Bibliography/References [.bib file]
% \end{singlespace}
% \clearemptydoublepage

%% If you are using 'References':

% \renewcommand{\bibname}{References}
% \phantomsection
% \addcontentsline{toc}{chapter}{References}
% \begin{singlespace}
	% \bibliographystyle{IEEEtranN}
	% \bibliography{References}								% Bibliography/References [.bib file]
% \end{singlespace}
% \clearemptydoublepage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% APPENDIX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%Don't do anything except adding your "Appendix.tex" file


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% OTHERS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% I hope you enjoy it!  Keep up the good work.  Bom trabalho.

==> sections/analysis/analysis.tex <==
\chapter{Worst-Case Traversal Time Analysis}
\label{chap:analysis}
% \begin{center}
% 	\fbox{\bf
% 		\centering
% 		\begin{minipage}{\linewidth}
% 			\centering
% 			The outcome of the work that has been presented in this chapter titled ``Worst-case traversal time analysis of TSN with multi-level preemption'' was accepted in the {Journal of Systems Architecture} ({JSA}), Vol. 116, 2021. \footnote{https://doi.org/10.1016/j.sysarc.2021.102079}.   
% 	\end{minipage}}
% \end{center} In Chapter~\ref{chap:feasibility} and~\ref{chap:Implementation}, we have extensively discussed the feasibility of multi-level preemption and provided implementation recommendations.

Satisfying temporal requirements is central to any real-time communication medium. As such, formal timing analyses must be conducted to provide safe temporal guarantees whenever a new feature/scheme is proposed for a real-time communication protocol. In this Chapter, we present results on the worst-case traversal time (WCTT) of frames under the multi-level preemption assumption. To this end, we extend the worst case performance analysis for one-level preemption presented by~\cite{Thiele2016Formal}, wherein the authors used Compositional Performance Analysis (CPA) to analyse the delay experienced by each frame in a switched Ethernet network. 

%
% \section{Model of computation}
% \label{sec:analysis:model}
% \input{feupphdteses/sections/analysis/sections/model.tex}
%
\section{A brief background on CPA}
\label{sec:analysis:cpa}
\input{feupphdteses/sections/analysis/sections/cpa.tex}
%
\section{Proposed analysis}
\label{sec:analysis:approach}
\input{feupphdteses/sections/analysis/sections/analysis.tex}
%
\section{Evaluation}
\label{sec:analysis:experiment}
\input{feupphdteses/sections/analysis/sections/experiment.tex}
%
% \section{Related work}
% \label{sec:analysis:related_work}
% \input{feupphdteses/sections/analysis/sections/related_work.tex}

\section{Chapter summary}
\label{sec:analysis:conclusion}
\input{feupphdteses/sections/analysis/sections/conclusion.tex}


==> sections/analysis/sections/abstract.tex <==
To achieve low latency transmission of time-sensitive flows in Ethernet networks, the IEEE introduced the IEEE~802.1Qbu~Standard, which specifies a $1$-level preemption scheme for IEEE~802.1 networks. The specification allows the suspension of a \textit{preemptable frame} prior to its completion for the speedy transmission of an \textit{express frame}; but any other preemptable frame cannot be transmitted before the completion of the already preempted frame. While this approach improves the performance of express frames, the performance is negatively impacted in scenarios where the number of express frames is high. Another limitation is the fact that preemptable frames with timing requirements can suffer long blocking periods due to the non-preemptive service of frames in the same category. This is irrespective of the individual priority level of each frame. 

Recently, a multi-level preemption scheme has been proposed to circumvent these limitations. The work focused on the feasibility and implementation requirement of such an approach, but a formal analysis of the worst-case performance guarantees under the proposed scheme was not provided. In this paper, we fill this gap by presenting the aforementioned analysis of the TSN~IEEE~802.1Qbu networks under the multi-level preemption assumption. Evaluation is performed with a realistic automotive use-case and the results showcase an improvement up to $53.07\%$ for preemptable frames with firm timing requirements.

==> sections/analysis/sections/acknowledgment.tex <==
This work was partially supported by the project Safe Cities - Inovação para Construir Cidades Seguras, ref. POCI-01-0247-FEDER-041435, co-funded by the European Regional Development Fund (ERDF), through the Operational Programme for Competitiveness and Internationalization (COMPETE 2020); also by National Funds through FCT/MCTES (Portuguese Foundation for Science and Technology), within the CISTER Research Unit (UIDB/04234/2020).


==> sections/analysis/sections/analysis.tex <==
In the multi-level preemption scheme, each frame can belong to only one of the following three categories: ($1$)~can preempt other frames and is non-preemptable, i.e., cannot be preempted by any other frame, because it is part of the highest priority class (e.g., express traffic); ($2$)~can preempt other frames and can also be preempted  and finally ($3$)~cannot preempt other frames and can be preempted by any frame in categories~($1$) and ($2$). We refer to categories ($1$), ($2$), and ($3$), as ``express flows''; ``preemptable flows with firm timing requirements'' (tpflows), and ``best effort flows'' (bpflows), respectively. With this nomenclature in mind, we have everything we need to discuss the components of the end-to-end delay of a frame, say~$f_i^q$ that arrives at time $a_i^q$. In a nutshell, there are four components, namely: ($1$)~the \textit{lower-priority blocking} -- i.e., the delay due to frame(s) with a lower priority than~$f_i$; ($2$)~the \textit{same-priority blocking} -- i.e., the delay due to frame(s) with the same priority as $f_i$; ($3$)~the \textit{higher priority interference} -- i.e., the delay associated to frame(s) with a higher priority than~$f_i$;~and finally, ($4$)~the \textit{preemption overheads}, which is the delay due to preemption overheads. 

\subsection{Lower-priority blocking}
\label{subsec:Lower-priority blocking}
In this section, we derive an upper-bound on the lower-priority blocking experienced by a frame in each flow class.
\subsubsection{Lower-priority blocking for ``express flows''}
Every express frame can experience the maximum lower-priority blocking in two scenarios: ($i$)~when it is blocked by the largest lower priority express frame since frames in the same preemption class are served in a non-preemptive manner; or ($ii$)~when it is blocked by the largest non-preemptable fragment of a preemptable frame\footnote{We recall that any preemptable frame that is less than or equal to $143$~bytes in size cannot be preempted.}. Lemma~\ref{lemma:lower-priority-express-blocking} provides an upper-bound on the blocking due to scenario~($ii$).

\begin{lemma}[$\PB^{\mathcal{E}}_i$]
\label{lemma:lower-priority-express-blocking}
For any express flow~$f_i \in \mathcal{E}$, the maximum blocking of any frame~$f_i^q$ (with $q \ge 1$) caused by a preemptable frame is given by Equation~\ref{eqn:lower-priority-blocking-lemma}.
\begin{equation}
    \label{eqn:lower-priority-blocking-lemma}
    \PB^{\mathcal{E}}_i = \min \Bigg\{ \underbrace{\max_{j\: \in \: \mathcal{P}} \left\{C_j^+\right\}}_{(a)},\: \underbrace{\dfrac{143\: bytes}{rTX}}_{(b)} \Bigg\} 
\end{equation}
\end{lemma}
 \begin{proof}
On one side, if all the preemptable frames are shorter than $143~bytes$, then the maximum blocking time to any express frame is caused by the largest of these frames. This is captured by term~($a$). On the other side, the longest non-preemptable fragment of any preemptable frame is $143$~bytes length~\citep{Thiele2016Formal}. This means a maximum blocking time of $\frac{143\: bytes}{rTX}$ (where $rTX$ is the link speed). This is captured by term ($b$). Therefore, a tight upper-bound on the blocking time caused by a preemptable frame to any express frame~$f_i^q$ (with $q \ge 1$) is given by the minimum between terms~($a$) and~($b$), and the lemma follows.
\end{proof}
 
From Lemma~\ref{lemma:lower-priority-express-blocking}, Theorem~\ref{theorem:Lower-priority-blocking-express} provides a tight upper-bound on the lower-priority blocking incurred by any express frame. 
 
 \begin{theorem}[$\LPB^{\mathcal{E}}_i$]
 \label{theorem:Lower-priority-blocking-express}
For any express flow~$f_i \in \mathcal{E}$, if $lp^{\mathcal{E}}(i)$ represents the set of express frames with a priority lower than that of $f_i$, then a tight upper-bound on the lower-priority blocking to any frame~$f_i^q$ (with $q \ge 1$)  is given by Equation~\ref{eqn:lower-priority-blocking-express}.
\begin{equation}
    \label{eqn:lower-priority-blocking-express}
    \LPB^{\mathcal{E}}_i = \max \Bigg\{ \underbrace{\max_{j\: \in \: lp^{\mathcal{E}}(i)}\left\{C_j^+\right\}}_{(a)},  \: \underbrace{ \PB^{\mathcal{E}}_i }_{(b)} \Bigg\}
\end{equation}
 \end{theorem}
 \begin{proof}
Any express frame~$f_i^q$ can suffer lower-priority blocking due either to the transmission of ($1$)~a lower-priority express frame or ($2$)~a preemptable frame. In the first case, term~($a$) captures the largest blocking time since frames in the same preemption class are served in a non-preemptive manner. On the other hand, if the blocking is caused by a preemptable frame, then  Lemma~\ref{lemma:lower-priority-express-blocking} provides an upper-bound on the lower-priority blocking, i.e., $\PB^{\mathcal{E}}_i$ (term~($b$)). Therefore, a tight upper-bound on the blocking time suffered by any express frame~$f_i^q$ (with $q \ge 1$) is given by the maximum between terms~($a$) and~($b$), and the theorem follows. 
\end{proof}
Note that Equations~\ref{eqn:lower-priority-blocking-lemma} and~\ref{eqn:lower-priority-blocking-express} are similar to Equations~5 and~7 in~\citep{Thiele2016Formal}. We explicitly address this behavior in the analysis for the sake of completeness.

\subsubsection{Lower-priority blocking for ``tpflows''}
\label{subsec:Lower-priority blocking-tp}
Every flow can preempt all flows in a lower preemption class by design, but the converse is not true. A tpflow is no exception to this rule. This means that each tpflow frame~$f_i^q$ can be blocked by ($i$)~at most the largest non-preemptable fragment of any preemptable frame in a lower preemption class or ($ii$)~a lower-priority frame of the same preemption class as $f_i$, since frames of the same class are served in a non-preemptive manner. Lemma~\ref{lemma:lower-priority-tp-blocking} computes an upper-bound on the blocking time incurred by a tpflow frame due to frame(s) in lower preemption classes.

\begin{lemma}[$\PB^{\mathcal{TP}}_i$]
\label{lemma:lower-priority-tp-blocking}
For any flow~$f_i \in \mathcal{TP}$, the maximum blocking time of any frame~$f_i^q$ (with $q \ge 1$) caused by a frame of a lower preemption class is given by Equation~\ref{eqn:lower-priority-tp-blocking-lemma}.
\begin{equation}
    \label{eqn:lower-priority-tp-blocking-lemma}
    \PB^{\mathcal{TP}}_i =  \: \min \Bigg\{ \underbrace{ \max_{j\: \in \: \{lp(i)\: \mid \:  \operatorname{PC}_j \:  > \: \operatorname{PC}_i\}} \left\{C_j^+\right\}}_{(a)},
\underbrace{\dfrac{143\: bytes}{rTX}}_{(b)} \Bigg\}
\end{equation}
\end{lemma}
 \begin{proof}
The proof of Lemma~\ref{lemma:lower-priority-tp-blocking} is similar to that of Lemma~\ref{lemma:lower-priority-express-blocking}. Given frame~$f_i^q$, if all the frames in a lower preemption class are shorter than $143~bytes$, then the maximum blocking incurred by $f_i^q$ is caused by the largest of these frames. This is captured by term~($a$). Otherwise, the longest non-preemptable fragment of any preemptable frame is $143$~bytes length~\citep{Thiele2016Formal} and this means a maximum blocking time of $\frac{143\: bytes}{rTX}$ (where $rTX$ is the link speed). This is captured by term ($b$). Therefore, a tight upper-bound on the blocking time caused by a preemptable frame of a lower preemption class to~$f_i^q$ is given by the minimum between terms~($a$) and~($b$), and the lemma follows.
\end{proof}

From Lemma~\ref{lemma:lower-priority-tp-blocking}, Theorem~\ref{theorem:Lower-priority blocking-tp} derives a tight upper-bound on the lower-priority blocking incurred by any tpflow frame.
\begin{theorem}[$\LPB^{\mathcal{TP}}_i$]
\label{theorem:Lower-priority blocking-tp}
For any tpflow flow~$f_i \in \mathcal{TP}$, the maximum lower-priority blocking of any frame~$f_i^q$ (with $q \ge 1$) is given by Equation~\ref{eqn:lower-priority-tpflow}.
\begin{equation}
    \label{eqn:lower-priority-tpflow}
\LPB^{\mathcal{TP}}_i =\max \Bigg\{ \underbrace{\max_{ j\: \in \: \{lp(i)\: \mid \: \operatorname{PC}_i\: = \: \operatorname{PC}_j\}}\left\{C_j^+\right\} }_{(a)}, \:  \underbrace{\PB^{\mathcal{TP}}_i}_{(b)} \Bigg\}
\end{equation}
 \end{theorem}
 
\begin{proof}

Any tpflow frame~$f_i^q$ can suffer lower-priority blocking either due to the transmission of ($1$)~a lower-priority frame of the same preemption class or ($2$)~a frame of a lower preemption class. In the first case, term~($a$) captures the largest blocking time that can be caused by a frame of the same preemption class, since these frames are served in a non-preemptive manner by design. In the second case, if the blocking is caused by a frame of a lower preemption class, we have already shown in Lemma~\ref{lemma:lower-priority-tp-blocking} that this delay cannot exceed $\PB^{\mathcal{TP}}_i$ (i.e., term~($b$)). Therefore, a safe upper-bound on the blocking time suffered by any tpflow frame~$f_i^q$ (with $q \ge 1$) is given by the maximum between terms~($a$) and~($b$), and the theorem follows.
\end{proof}

\subsubsection{Lower-priority blocking for ``bpflows''}
Since bpflows belong to lowest preemption class by assumption, it follows that the maximum lower-priority blocking that any bpflow frame can experience is provided by the largest lower priority frame in the same class. This is given by the Equation~\ref{eqn:lower-priority-blocking-bpflow}.
\begin{equation}
    \label{eqn:lower-priority-blocking-bpflow}
    \LPB^{\mathcal{BP}}_i = \max_{j\: \in \: lp^{\mathcal{BP}}_{(i)}}\left\{C_j^+\right\}
\end{equation}

Now that we have discussed in details the computation of all lower-priority blocking terms, we can proceed with the computation of the same-priority blocking -- i.e., the delay due to frame(s) with the same priority as the flow under analysis.

\subsection{Same-priority blocking}
\label{subsec:same-priority blocking}
In the following subsections, we compute upper-bounds on the delay experienced by a frame due to the transmission of same-priority frame(s).

\subsubsection{Same-priority blocking for ``express flows''}
Every express frame $f_i^q$ can be blocked by all frames of the same priority that arrive before its arrival at time, say $a_i^q$, within the level-$i$ busy period. Also, all the previous $q-1$ instances of $f_i$ must be transmitted before $f_i^q$ is transmitted and hence, contribute to the same priority blocking term. Therefore, the maximum same-priority blocking $\SPB^{\mathcal{E}}_i$ that express frame $f_i^q$ can incur is given by Equation~\ref{eqn:same-priority-express}.
\begin{equation}
    \label{eqn:same-priority-express}
    \SPB^{\mathcal{E}}_i(q, a_i^q) =  \displaystyle\sum_{j\: \in\: sp(i)} \eta_j^+(a_i^q) \cdot C^+_j + (q-1) \cdot C_i^+
\end{equation}
In Equation~\ref{eqn:same-priority-express}, $sp(i)$ denotes the set of all flows with the same priority as~$f_i$. The first term computes the maximum delay due to the transmission of all frames with the same priority that arrive before $a_i^q$, while the second term computes the maximum delay incurred by~$f_i$ due to the transmission of all previous $q-1$ instances.
\subsubsection{Same-priority blocking for ``tpflow''}
\label{subsec:same-priority blocking-tp}
Similar to express frames, every tpflow frame $f_i^q$ can be blocked by all frames with the same priority that arrive before $a_i^q$ within the level-$i$ busy period as well as all the previous $q-1$ instances of~$f_i$. In addition, because $f_i^q$ is preemptable, it can incur additional delay even after the start of its transmission. It is guaranteed uninterrupted only during the transmission of its final non-preemptable fragment. In other words, the last fragment of $f_i^q$ must wait for all the preceding fragments of the instance to be transmitted. That is, the size of this last fragment is the minimum valid Ethernet frame size~\citep{Thiele2016Formal}. With the above-mentioned, the maximum same-priority blocking $\SPB^{tp}_i$ that $f_i^q$ can incur is given by Equation~\ref{eqn:same-priority-tpflow}.
\begin{equation}
    \label{eqn:same-priority-tpflow}
    \SPB^{\mathcal{TP}}_i(q, a_i^q) =\displaystyle\sum_{j\: \in\: sp(i)} \eta_j^+(a_i^q) \cdot C^+_j + (q-1) \cdot C_i^+ + \left(C_i^+ - \dfrac{84\: bytes}{rTX}\right)  
\end{equation}
In Equation~\ref{eqn:same-priority-tpflow}, the first term computes the maximum delay due to the transmission of all frames with the same priority as~$f_i$ that arrive before $a_i^q$, while the second term computes the delay incurred due to the transmission of all previous $q-1$ instances of $f_i$. Finally, the third term computes the maximum delay due to the transmission of all non-final fragments of $f_i^q$.
\subsubsection{Same-priority blocking of ``bpflows''}
The same priority blocking term for bpflows is identical to that of tpflows in Equation~\ref{eqn:same-priority-tpflow}. This is because the behavior of frames within these classes are identical in that they are transmitted in a non-preemptive manner; and they are served in a FIFO manner. This imply that a bpflow frame $f_i^q$ can be blocked by all frames with the same priority that arrive before its arrival time $a_i^q$ within the level-$i$ busy period; all previous $q-1$ instances of~$f_i$; and all its preceding fragments (i.e., the non-end ones) if it was preempted. For this class, Equation~\ref{eqn:same-priority-tpflow} also suffices, where $\mathcal{TP}$ in superscript is replaced with $\mathcal{BP}$ in order to reflect the corresponding frame class.

\subsection{Higher-priority Interference}
\label{subsec:higher-priority-interference}
Irrespective of its class, every frame~$f_i$ cannot commence its transmission in the presence of another frame of a higher priority~\citep{thiele2014improving, Thiele2016Formal}. This implies that all higher priority frames that arrive before the transmission of frame frame~$f_i^q$ will always impact its transmission. With the aforementioned, it follows that the higher priority interference term for the three classes of frames is given by Equation~\ref{eqn:higher-priority-blocking}. 
\begin{equation}
    \label{eqn:higher-priority-blocking}
    \HPI_i(\Delta t) = \displaystyle\sum_{j\: \in\: hp(i)} \eta_j^+(\Delta t)\cdot C^+_j
\end{equation}

\subsection{Preemption overheads}
\label{subsec:preemption-overead}
Each preemption operation involves some overhead upon its occurrence, which is equivalent to the time taken to transmit $24$~bytes of data~\citep{Thiele2016Formal}. This overhead is always added to the transmission time of the preempted frame. As such, since express flows are transmitted in a non-preemptive manner, then they do not incur any preemption overhead. Therefore, only tpflows and bpflows incur preemption overheads as they are preemptable. From an analytical standpoint, the approach adopted to compute the preemption overhead terms are identical for these two preemption classes.

Roughly speaking, the maximum preemption overheads that a preemptable frame $f_i^q$ can incur depends solely on the \textit{maximum number} of preemption events that can occur between its arrival time up until the transmission of the first bit of the last non-preemptable fragment. With this in mind, the maximum number of preemptions can occur in either of the following two cases: 
\begin{itemize}
    \item[($1$)] all preemptable frames transmitted between $a_i^q$ and the complete transmission of $f_i^q$ are preempted for the maximum number of times beyond which cutting a frame into further fragments would violate the minimum Ethernet frame size (see Equation~\ref{eqn:max-preemption}).
    \item[($2$)] all possible arrivals of higher priority frames belonging to a higher preemption class occur and each of these causes a preemption.
\end{itemize}
To assess the first case, we consider a preemptable flame~$f_i^q$ transmitted within the busy period of length, say $\Delta t$, then we calculate the maximum number of times $f_i^q$ and all other preemptable frames that are transmitted within the window of size $\Delta t$ can be preempted. We can distinguish between three different types of preemptable frames, namely: ($1$)~preemptable frames with a lower priority than~$f_i$; ($2$)~preemptable frames with the same priority as~$f_i$; and finally ($3$)~preemptable frames with a higher priority than~$f_i$. Below, we elaborate each of these three cases.

\subsubsection{Maximum number of preemptions incurred by a lower-priority preemptable frame}
This maximum number of preemptions occurs when a lower-priority preemptable frame, say~$f_j^k$, which is obstructing the transmission of $f_i^q$ gets preempted itself a maximum number of times. Frame~$f_j^k$ can either ($i$) belong to a lower preemption class than $f_i^q$ or ($ii$) share the same preemption class as~$f_i^q$. 

\noindent $\triangleright$ \textbf{Case~($i$).} If~$f_j^k$ belongs to a lower-preemption class, then it is preempted at most once by~$f_i^q$ or by any other frame belonging to a higher preemption class. By design, the preempted frame will not resume its transmission before all pending frames of higher preemption class (including $f_i^q$) have completed their transmission. \\
\noindent $\triangleright$ \textbf{Case~($ii$).} If~$f_j^k$ is in the same preemption class as $f_i^q$, then~$f_j^k$ can be preempted several times and $f_i^q$ can only start its transmission after the complete transmission of~$f_j^k$. By using Equation~\ref{eqn:max-preemption}, we derive the maximum number of preemptions $N_i^{\mathcal{P},\: lp}$ incurred a by a lower-priority preemptable frame in the same preemption class as~$f_i^q$ in Equation~\ref{eqn:max-preemption-lp-tpflow}.
\begin{equation}
    \label{eqn:max-preemption-lp-tpflow}
    N_i^{\mathcal{P},\: lp} = \max_{\{j \: \mid \: \operatorname{PC}_i\: = \: \operatorname{PC}_j\: \wedge\:  i \: > \: j\}}\left\{F_j^+\right\} 
\end{equation}
\subsubsection{Maximum number of preemptions incurred by same-priority preemptable frames}
This involves the preemptions incurred by frames with the same priority as $f_i^q$ that arrive before $a_i^q$ within the level-$i$ busy period as well as those suffered by $f_i^q$ up until its last non-preemptable fragment. By using Equation~\ref{eqn:max-preemption}, the maximum number of preemptions $N_i^{\mathcal{P},\: sp}(q, a_i^q)$ is computed in Equation~\ref{eqn:max-preemption-sp-tpflow}.
\begin{equation}
    \label{eqn:max-preemption-sp-tpflow}
        N_i^{\mathcal{P},\: sp}(q, a_i^q) = q \cdot F_i^+ - 1 +  \displaystyle\sum_{j\: \in\: sp(i)} \eta_j^+(a_i^q) \cdot F^+_j
\end{equation}
The first term of Equation~\ref{eqn:max-preemption-sp-tpflow} computes the maximum preemption incurred by the first $(q$ instances of~$f_i$ apart from the last fragment, while the second term computes the maximum preemption incurred by all other frames with the same priority as~$f_i$ that arrives before~$f_i^q$ within the busy-window.
\subsubsection{Maximum number of preemptions incurred by higher-priority preemptable frames}
This number involves the preemptions incurred by all frames with a higher priority than $f_i^q$ that are transmitted during~$\Delta t$, i.e., the transmission period of $f_i^q$. It is denoted by $N_i^{\mathcal{P},\: hp}(\Delta t)$ and occurs when all these frames get preempted for the maximum amount times, given by Equation~\ref{eqn:max-preemption-hp-tpflow}.
\begin{equation}
    \label{eqn:max-preemption-hp-tpflow}
     N_i^{\mathcal{P},\: hp}(\Delta t)  = \displaystyle\sum_{\{j\: \in\: hp(i)\: \wedge \: j \: \in\: \mathcal{P}\}} \eta_j^+(\Delta t)\cdot F^+_j
\end{equation}

Putting Equations~\ref{eqn:max-preemption-lp-tpflow},~\ref{eqn:max-preemption-sp-tpflow}, and~\ref{eqn:max-preemption-hp-tpflow} together, the maximum number of preemptions incurred by the preemptable frames transmitted during $\Delta t$ is given by Equation~\ref{eqn:sum-max-preemptions}.
\begin{equation}
    \label{eqn:sum-max-preemptions}
    N_i(q, a_i^q,\Delta t) = N_i^{\mathcal{P},\: lp} + N_i^{\mathcal{P},\: sp}(q, a_i^q) + N_i^{\mathcal{P},\: hp}(\Delta t)
\end{equation}

With this Equation~\ref{eqn:sum-max-preemptions}, we have everything we need to derive an upper-bound on the maximum preemption overhead suffered by any preemptable frame~$f_i^q$, as formalized by Theorem~\ref{theorem:preemption-overhead}.
\begin{theorem}[$\PO_i^{\mathcal{P}}(\Delta t,q,a_i^q)$]
\label{theorem:preemption-overhead}
For any preemptable flow~$f_i \in \mathcal{P}$, an upper-bound on the maximum preemption overhead incurred by frame~$f_i^q$ (with $q \ge 1$), arrived at time~$a_i^q$ within the busy-period~$\Delta t$, is given by Equation~\ref{eqn:preemption-overhead}.
\begin{equation}
    \label{eqn:preemption-overhead}
     \PO_i^{\mathcal{P}}(\Delta t,q,a_i^q) = \underbrace{\frac{24 \: bytes}{rTX} }_{(a)} \times 
  \min \bigg\{ \bigg(\underbrace{\sum_{j\: \in \: \{\mathcal{F}\: |\: \operatorname{PC}_j\:  < \: \operatorname{PC}_i\}} \eta^+_j(\Delta t)}_{(b)} \bigg) , \: \underbrace{\:N_i(q, a_i^q, \Delta t) }_{(c)}\bigg\}
\end{equation}
\end{theorem}
\begin{proof}
The maximum preemption overhead is reached in one of the following two cases: (Case~$1$)~All the preemptable frames incur the maximum possible number of preemptions; or (Case~$2$)~All arriving frames belonging to a higher preemption classes cause a preemption. For the first case, Equation~\ref{eqn:sum-max-preemptions}, which is captured in term~($c$) provide an upper-bound. For the situation described in Case~$2$, a computation of the maximum number of arrivals from frames in a higher preemption class is captured by term~($b$). Therefore, the actual number of preemptions cannot exceed the minimum of these two terms. Now, because each preemption operation generates an overhead corresponding to term ($a$), the theorem follows.
\end{proof}

\subsection{Worst-case queuing delay}
In Section~\ref{sec:analysis:approach}, we discussed the individual components of the worst-case queuing delay. For any frame~$f_i^q$ that arrives at time~$a_i^q$ within the busy period, we obtain an upper-bound $Q_i(q,a_i^q)$ on this factor by summing up all these terms, as formally stated in Equation~\ref{eqn:wcqd}. 

\begin{equation}
    \label{eqn:wcqd}
     Q_i(q,a_i^q) =  
         \begin{cases}
\LPB_i^{\mathcal{E}} + \SPB_i^{\mathcal{E}}(q,a_i^q) + \HPI_i(Q_i(q,a_i^q)) & \operatorname{if} f_i \: \in\: \mathcal{E}; \\ \\*
\LPB^{\mathcal{TP}}_i + \SPB^{\mathcal{TP}}_i(q, a_i^q) + \HPI_i(Q_i(q,a_i^q))+  \PO_i^{\mathcal{P}}(Q_i(q,a_i^q)) & \operatorname{if} f_i \: \in\: \mathcal{TP}; \\  \\*
\LPB^{\mathcal{BP}}_i + \SPB^{\mathcal{BP}}_i(q, a_i^q) + \HPI_i(Q_i(q,a_i^q))+  \PO_i^{\mathcal{P}}(Q_i(q,a_i^q)) & \operatorname{if} f_i \: \in\: \mathcal{BP}
\end{cases}
\end{equation}

Note that Equation~\ref{eqn:wcqd} defines a fixed-point iterative process since $Q_i(q,a_i^q)$ appears on both sides of the equation. As such, a valid solution for every frame~$f_i^q$ is obtained by starting the fixed-point algorithm with the base value $C_i^+$. The algorithm stops as soon as two consecutive values of $Q_i(q,a_i^q)$ are identical or the relative deadline associated to flow~$f_i$ is exceeded. In the latter case, the timing requirement of~$f_i$ is violated and there is no valid solution.

\subsection{Worst-case traversal time}
\label{subsec:Wctt}
For every frame~$f_i^q$ arriving at time $a_i^q$, the discussions conducted in the previous sections command that its worst-case traversal time~$(\WCTT_i(q, a_i^q))$ is obtained by combining Equations~\ref{eqn:busy-time}~and~\ref{eqn:response-time-q}, where $Q_i^+(q)$ (in Equation~\ref{eqn:busy-time}) and $\delta_i^-(q)$ (in Equation~\ref{eqn:response-time-q}) are substituted by $Q_i(q,a_i^q)$ and $a_i^q$, respectively. Formally, $\WCTT_i(q, a_i^q)$ is reported in Equation~\ref{eqn:WCTT-all}. 
\begin{equation}
    \label{eqn:WCTT-all}
    \WCTT_i(q, a_i^q) = \begin{cases}
 Q_i(q,a_i^q) + C^+_i  - a^q_i & \operatorname{if} f_i \: \in\: \mathcal{E};\\ \\*
 Q_i(q,a_i^q) + \dfrac{84 bytes}{rTX} -  a^q_i & \operatorname{if} f_i \: \in\: \mathcal{TP};\\ \\*
 Q_i(q,a_i^q) + \dfrac{84 bytes}{rTX} -  a^q_i & \operatorname{if} f_i \: \in\: \mathcal{BP} 
\end{cases}
\end{equation}
Finally, the worst-case traversal time for flow $f_i$ within the level-i busy period, denoted by $\WCTT_i^+$, is obtained by computing the maximum of all the $\WCTT_i(q, a_i^q)$, where $1\leq q \leq q_i^+$ and $q_i^+$ is the last frame of $f_i$ in the level-i busy period. Formally, this is expressed in Equation~\ref{eqn:WCTT-max}. 
\begin{equation}
    \label{eqn:WCTT-max}
        \WCTT_i^+ = \max_{1\leq q \leq q_i^+}\left\{\WCTT_i(q, a_i^q)\right\}
    \end{equation} 
This equation concludes the computation of $\WCTT_i^+$ for flow~$f_i$ within a switch node (i.e., the local analysis). Therefore, the overall traversal time for flow~$f_i$ (i.e., the global analysis) is obtained by summing up these values at all the individual switch nodes along its transmission path.
Here, the level-i busy period is a time interval $[\sigma, \mu]$ within which only frames belonging to~$hep(i)$ (except the first frame, which is generated from flow $f_j \in lp(i)$ with the longest non-preemptable fragment) are transmitted throughout $[\sigma, \mu]$, but no frame belonging to~$hep(i)$ is transmitted in $[\sigma - \epsilon, \sigma)$ or $(\mu, \mu + \epsilon]$ for any arbitrary small $\epsilon > 0$.\\
In order to perform the analysis, the scenario leading the longest level-i busy period for each flow $f_i$ was considered, i.e., the scenario where either ($1$)~a frame $f_j^k$ in $\operatorname{PC}_i < \operatorname{PC}_j$ with the longest non-preemptable fragment; or ($2$)~a frame $f_j^k$ in $\operatorname{PC}_i = \operatorname{PC}_j$ with the largest size and a lower priority than $f_i$, was released just before $f_i$; all the flows in $hep(i)$ release a frame at the same time as $f_i$ and finally, all future frames are released as soon as is legally permitted to do so.


==> sections/analysis/sections/conclusion.tex <==
In this chapter, we provided a formal timing guarantees for each flow under such a scheme by using a CPA based approach. Using a realistic automotive use-case, we assessed the performance improvements in terms of worst-case traversal time ($\WCTT$) over the $1$-level scheme. From our results, the multi-level preemption scheme shows an improvement up to $53.07\%$ in the $\WCTT$ guarantee for preemptable time-sensitive frames. Then, we demonstrated the tightness of the analysis with another automotive use-case from Renault. We concluded that a careful attention must be paid to the maximum size of each of these flows during the flow-to-preemption-class assignment at design time. Also, an interesting discussion was conducted on the performance improvement brought about by each extra preemption level in the frame transmission scheme and we showed that the trend was not linear on one hand; and each extra preemption level involves additional hardware implementation overheads, which may not be negligible. 

%In a near future, we seek to investigate: ($1$)~the optimal preemption-level scheme that will prove to be the perfect trade-off between the performance that each additional preemption level brings and the overhead of enabling this level; ($2$)~efficient flow priority assignment strategies in order to further improve the responsiveness of preemptable time-sensitive flows; and finally ($3$)~the interoperability of multi-level preemption with other TSN mechanisms.


==> sections/analysis/sections/cpa.tex <==
Before we present our proposed WCTT analysis, it is important to provide the reader with a brief background on the CPA approach for a smooth understanding of the rest of this paper. For a complete and detailed description of the fundamental concepts, we refer the interested reader to~\cite{henia2005system}. In this framework, a component is modeled as a resource~$\rho$, which provides some service to one or more tasks. Tasks' activations are abstracted by an event model, which defines an upper-bound (denoted by $\eta^+(\Delta t)$) and a lower-bound (denoted by $\eta^-(\Delta t)$) on the number of activations within any half-open time interval $[t, t+\Delta t)$. This framework also defines a distance function $\delta^+(q)$ (respectively, $\delta^-(q)$) which denotes an upper-bound (respectively, a lower-bound) on the maximum (respectively, minimum) time instant at which the $q^{\operatorname{th}}$ activation instance can occur~\citep{henia2005system, handbook2017cpa}. Figure~\ref{cpa-even-model} illustrates the event model of a task with a period and jitter of 50 time units. A jitter of 50 time units (and equal to the period) implies that two instances can occur simultaneously ($\delta^-(2) = 0$; $\eta^+(0) = 2$) or two periods apart ($\delta^+(2) = 500$; $\eta^-(500) = 0$).

\begin{figure}
  \centering
  \begin{tabular}[b]{c}
      \includegraphics[width=.39\linewidth, height =3in]{feupphdteses/sections/analysis/images/cpa-event-arrival-function} \\
    \small (a.) An event arrival function.
  \end{tabular} \qquad
  \begin{tabular}[b]{c}
      \includegraphics[width=.45\linewidth, height=2.95in]{feupphdteses/sections/analysis/images/cpa-distance-function} \\
    \small (b.) An event distance function
  \end{tabular}
  \caption{CPA event model for a task with a period and jitter of 50 time units.}
  \label{cpa-even-model}
\end{figure}


The service period of each task, say $\tau_i$, is bounded by two parameters: from above by $C_i^+$ and from below by $C_i^-$. These parameters respectively represent the longest and the shortest time it takes the resource, say $\rho$, to service an instance of $\tau_i$, in the absence of any blocking or interference. The worst-case response time (WCRT) of task $\tau_i$ is investigated within a so-called level-$i$ busy period. In summary, this is a time interval $[\sigma, \mu]$ within which only task instances belonging to~$hep(i)$ (except the first job, which is generated from task $\tau_j \in lp(i)$ with the longest $C_j^+$) are executed throughout $[\sigma, \mu]$, but no jobs belonging to~$hep(i)$ are executed in $[\sigma - \epsilon, \sigma)$ or $(\mu, \mu + \epsilon]$ for any arbitrary small $\epsilon > 0$.


Since the WCRT of $\tau_i$ may not occur at its first activation, CPA examines all the~$q$ activations of $\tau_i$ within the level-$i$ busy period. To this end, it defines a \textit{q-activation processing time} $B_i(q)$ which describes how long the resource $\rho$ is busy processing $q$ jobs of $\tau_i$. This is computed in Equation~\ref{eqn:busy-time}. 
\begin{equation}
    \label{eqn:busy-time}
        B_i(q) = Q^+_i(q) + C^+_i  
    \end{equation}

\noindent In Equation~\ref{eqn:busy-time}, note that $B_i(q)$ assumes a non-preemptive scheduling scheme. Here, $Q_i^+(q)$ is the time interval from the start of the level-i busy period to the beginning of service of the $q^{th}$ instance of~$\tau_i$. It is computed as in Equation~\ref{eqn:queueing-delay-cpa}. 
{\small
\begin{equation}
    \label{eqn:queueing-delay-cpa}
       Q_i^+(q) = \max_{j \: \in \: lp(i)} \left\{ C_j^{+} \right\}  + (q-1) \cdot C^+_i  + \displaystyle\sum_{k \in hp(i)} C^+_k \cdot \eta_k^+\left(Q_i(q)+ \epsilon\right)
    \end{equation}
}
\noindent In Equation~\ref{eqn:queueing-delay-cpa}, $lp(i)$ and $hp(i)$ denote the set of tasks with a lower and higher priority than $\tau_i$, respectively. The first term computes the maximum delay that can be experienced due to the presence of a lower priority task in the system; the second term estimates the delay experienced due to the processing of all preceding $q-1$ instances; and the third term computes all possible delays due to the service of higher priority tasks within $B_i(q)$.  It is worth mentioning that Equation~\ref{eqn:queueing-delay-cpa} is reminiscent of the Worst-Case Response Time estimation for the classical single-core fixed-priority tasks and it is also solved by using a fixed point algorithm, i.e., the solution is computed in an iterative manner and the algorithm stops as soon as two consecutive values of $Q_i^+(q)$ are equal or when one value exceeds the deadline. In the latter case, the set of flows is deemed unschedulable. After obtaining $Q_i^+(q)$, we can derive the maximum number of activations $q_i^+$ of $\tau_i$ within $B_i(q)$ by using Equation~\ref{eqn:maximum_activations}.
\begin{equation}
    \label{eqn:maximum_activations}
        q_i^+ =  \min \{ q \ge 1 \mid B_i(q) < \delta_i^-(q+1) \}
    \end{equation}
This equation computes the first $q_i$ instances of $\tau_i$ such that the completion time of instance $q_i$ is less than the earliest arrival time of instance $q_{i+1}$. The response time of the $q^{\operatorname{th}}$ instance of $\tau_i$ is given by computing the difference between the time instant when all the $q$ instances of $\tau_i$ have been processed and the arrival time of the instance $q$. Formally, this is given by Equation~\ref{eqn:response-time-q}.
\begin{equation}
    \label{eqn:response-time-q}
        R_i^+(q) = B_i(q) - \delta_i^-(q)
    \end{equation}
Finally, the WCRT $R_i^+$ of~$\tau_i$ is the maximum $R_i^+(q)$ over all $q_i^+$ activations of~$\tau_i$ within the busy window and is computed through Equation~\ref{eqn:response-time}. 
\begin{equation}
    \label{eqn:response-time}
        R_i^+ = \max_{1\leq q \leq q_i^+}\left\{R_i^+(q)\right\}
    \end{equation}

So far, we have discussed the worst-case delay at each resource node, also called the \textit{local analysis}. Specifically, a rigorous computation of the maximum possible blocking/interference that a task can suffer is carried out locally at every resource node. This means that the potential interference between any two tasks will be effectively captured when performing the local analysis at the shared resource node. But in many cases, real-time applications involve interacting tasks sharing different resources. To evaluate the WCRT of a task in this scenario, the CPA defines an \textit{event propagation} step in addition to the local analysis step. Here, the output of each resource along the execution path of a task serves as input for the next one and $R_i^+(q)$ at the last node is the WCRT of the task.
%which is a span of message transmissions with priorities greater than or equal to i. The busy interval ends when an instance transmits with priority less than i, or when the bus is idle.

The CPA approach has been applied to standard Ethernet~\citep{Rox2010, thiele2015improving}, AVB~\citep{Diemer2012}, and TSN~\citep{ Thiele2016BLS, Thiele2016Formal}. In these works, the output port of the switches are the \textit{resources} and flows are \textit{tasks}. The frames are \textit{jobs} or \textit{instances} of the tasks and the path of a flow is modeled as a chain of dependent tasks~\citep{Diemer2012}. Specifically, the resources render some \textit{service(s)} (transmission) to some task activations (frames) upon some event occurrence (frame arrivals) within a time window (a level-$i$ busy period). In this context, the service period of each frame is bounded by two parameters: from above by~$C^+$ and from below by~$C^-$. These parameters represent the longest and the shortest time to transmit the frame in absence of any interference. Obviously, these depend on the minimum and maximum possible payload $p^{-/+}$ of the flow to which the frame belongs to as well as the output link speed. Equation~\ref{sec:analysis:C+-} illustrates the relationship between these parameters\footnote{The minimum size of a frame is $84$~bytes w.r.t. the Standards specification.}.
\begin{equation}
\label{sec:analysis:C+-}
    C^{-/+} = \frac{\operatorname{42\: bytes} + \max\{\operatorname{42\: bytes}, \: p^{-/+}\}}{rTX}
\end{equation}
In this equation, $rTX$ represents the transmission speed on the port link and the constant terms (here,~$42$) represent the protocol overhead and minimum frame payload requirement as specified in the Standards~\cite{IEEE-Std-802.1Q-2018}. 
\begin{figure}[htb]
    \centering
    \includegraphics{feupphdteses/sections/analysis/images/End-to-end-delay-components-1}
    \caption{End-to-end delay components.}
    \label{fig:end-to-end-delay-components}
    \vspace{-0.1in}
\end{figure}
As shown in Figure~\ref{fig:end-to-end-delay-components}, the end-to-end delay that a frame experiences in a switch fabric consists of the following five components: ($1$)~the input delay at the switch input port; ($2$)~the processing delay; ($3$)~the queuing delay at the switch output port; ($4$)~the propagation delay; and finally ($5$)~the transmission delay~\citep{Finn2017}. As pointed out by Thiele and Ernst~\cite{Thiele2016Formal}, all these components are implementation dependent and usually in the order of a few clock cycles, except for the queuing delay, which is captured in Equation~\ref{eqn:queueing-delay-cpa} and whose components are illustrated in Figure~\ref{fig:queqing-delay-components}. 
\begin{figure}[htb]
    \centering
    \includegraphics[scale = 0.86]{feupphdteses/sections/analysis/images/cpa-delay-components-3}
    \caption{Queuing delay components.}
    \label{fig:queqing-delay-components}
    \vspace{-0.1in}
\end{figure}

In Figure~\ref{fig:queqing-delay-components}, frame $f_i^q$ arrives at time $a_i^q$ during the transmission of a lower preemption class frame, $\LP$ (green box). Before $a_i^q$, frame $\HP$ (red box) of the express class had arrived as well as two other frames $\SP$ (black boxes) with the same priority and preemption class as $f_i^q$. The preemption operation commands that a minimum number of bytes has been transmitted and a number of bytes is left so that the preempted fragment can meet the minimum size requirement of a valid Ethernet frame. This brings the highest possible blocking that a preempting frame can incur to the size of the largest non-preemptable fragment of a preemptable  frame, i.e., $143$~bytes of data~\citep{Thiele2016Formal} and explains the transmission process of~$\LP$ before it is preempted. Upon the preemption of $\LP$, $\HP$; all $\SP$ frames; and all newly arrived $\HP$ frames are transmitted, thus forcing $f_i^q$ to be served only afterwards.  

%Note that in the representation of the frame transmission process in Figure~\ref{fig:queqing-delay-components}, frames are labelled based on their contribution to the queuing delay, e.g., the segment of LP that is transmitted before $f_i^q$ is labelled as $\LPB$.

In addition to the queuing delay components captured in Equation~\ref{eqn:queueing-delay-cpa}, the preemption overhead is yet another term that should be taken into account. This is not the case in the general CPA model~\citep{handbook2017cpa}. The preemption overhead is a significant factor in the TSN frame transmission scheme. The total overhead induced by each preemption is $12$~bytes (i.e., $6$-byte preamble, $1$-byte start frame delimiter, $1$-byte frame count variable; and finally $4$-byte error check variable)~\citep{ojewale2018multi}. In addition, the \textit{Inter Frame Gap} (IFG) between two consecutive transmission has to be accounted for before the next frame/fragment is transmitted. According to the Standards, the size of each IFG equals the time it takes to transmit $12$~bytes of data. This brings the total overhead associated to each preemption to $24$~bytes. \cite{Thiele2016Formal} have also proven in that the maximum number of preemptions that a single frame can suffer is given by Equation~\ref{eqn:max-preemption}. Equation~\ref{eqn:max-preemption} provides an upper-bound on the number of times that an Ethernet frame can be preempted, due to the restrictions defined in the standards on the minimum valid frame size.
\begin{equation}
    \label{eqn:max-preemption}
    F^+_i = \Bigl\lfloor\dfrac{p_i^+ - 42\: bytes}{60\: bytes}\Bigr\rfloor
\end{equation}
In this equation, the constant terms (here,~$42$ and~$60$) are the minimum~payload requirements for the first and subsequent fragments of a preemptable frame in the Standards~\citep{IEEE-Std-802.1Q-2018}. For every flow~$f_i$, its worst-case traversal time is obtained by combining Equations~\ref{eqn:busy-time}~and~\ref{eqn:response-time-q}. We note that Equation~\ref{eqn:response-time-q} does not take into account the preemption overhead. This computation will be refined to integrate the cost in Section~\ref{subsec:Wctt}. Also, note that the CPA model allows arbitrary deadlines, i.e., there is no particular correlation between the deadline and the minimal inter-arrival time of each flow.



==> sections/analysis/sections/experiment.tex <==
In this section we perform the evaluation of the proposed approach. Specifically,  we consider two realistic use-cases from the automotive domain and evaluate the safety \& tightness of the proposed analysis.  
\subsection{Report on use-case 1}
\vspace{0.1cm}
\noindent $\triangleright$ {\bf Setup.} In this use-case, we consider a realistic network topology from the automotive domain, consisting of ten End Points~$\operatorname{EP}$s (a.k.a. Engine Control Units or ECUs) and seven full-duplex preemption enabled TSN switches $\SW_1, \SW_2, \ldots, \SW_7$ displayed as illustrated in Figure~\ref{fig:analysis:topology}. We considered seven flows -- $f_1, f_2, \ldots,  f_7$ -- where $f_1$ and $f_2$ are express; $f_3$ and $f_4$ are tpflows; and the remaining flows are bpflows. The name and make of the system are protected under an NDA. However, the specifications of the flows are provided in Table~\ref{tab:flows} and they are in the same range as those of the use-case presented by~\cite{alderisi2012towards}. We recall that flows are ordered according to their priorities, i.e., the smaller the subscript of a flow, the higher its priority. Three batches of analyses together with the associated simulations by using NeSTiNg~\citep{nesting_2019} to evaluate their tightness are conducted: ($a$)~All flows are transmitted in under the $1$-level preemption scheme (i.e., only express flows can preempt other flows); ($b$)~all flows are transmitted under the $2$-level preemption scheme (i.e., express frames can preempt all other frames; and tpflows can preempt bpflows); finally ($c$)~all flows are transmitted in a fully preemptive manner (i.e., any higher priority frame can preempt any lower priority frame).
\begin{figure}
\centering
\includegraphics[scale=1.4]{feupphdteses/sections/analysis/images/topology-multi-level-preemption-analysis}
\caption{Network topology}
\label{fig:analysis:topology}
\end{figure}

\begin{table}
  \centering
  \caption{Flow properties}
 
    \centering
    \begin{tabular}{ |p{0.5cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|} 
    \hline
    ID& Class& Src.& Dst.& Period ($\mu$s) & Deadline ($\mu$s)& Size (bytes)\\
     \hline
    1. & Express & EP 7 & EP3& 5000  & 150 & 200\\
   \hline
   
   2. &	Express & EP 6 & EP 1 & 10000 &	200	& 250\\
   \hline
  3. & Tpflow & EP 2 & EP 9 & 5000 &	500 & 300\\
  \hline
  4. & Tpflow &	EP 3 &	EP 8 & 5000 &	500 &	400 \\
  \hline
  5. & Bpflow & EP 4 & EP 10 & 1000 & 	- & 1300\\ 
  \hline
  6. & Bpflow &	EP 1 &	EP 8 & 1000 &	- & 1300\\
  \hline
  7. & Bpflow &	EP 9 & EP 5 & 1000 &	- &	1500\\
  \hline
\end{tabular}
  \label{tab:flows}
  %\includegraphics[scale=0.6]{images/use-case-parameters.PNG}
\end{table}

\vspace{0.1cm}
\noindent $\triangleright$ {\bf Results and discussion.}  Here, we report the results obtained from the experiments. We considered the safety and tightness of the proposed analysis. Also, we reported the behavior of the network with respect to ``each additional preemption level'' and the ``maximum  frame  size  in  each preemption class''. 

%In order to enable a fair comparison, we considered only scenarios in which all tested configurations allow all time sensitive flows to meet their deadlines.

\vspace{0.2cm}
\noindent $\triangleright \triangleleft$ \textbf{On the tightness of the proposed analysis}.  Fig.~\ref{fig:use-case-simulation-result-perf-comp} compares for each flow the maximum measured end-to-end delays -- $\mWCTT$ -- (see the yellow box plots) against the analytical $\WCTT$ bounds (see the red dots).
We can notice that all $\mWCTT$ fall below the corresponding $\WCTT$ when adopting the $1$-level preemption scheme (see Fig.~\ref{fig:use-case-simulation-result-1-level}), the $2$-level preemption scheme~(see Fig.~\ref{fig:use-case-simulation-result-2-level}), and finally, the fully preemptive scheme~(Fig.~\ref{fig:use-case-simulation-result-multi-level}). 
\begin{itemize}
    \item Under the $1$-level scheme, the observed gaps between the $\WCTT$ bounds and the $\mWCTT$ for express flows $f_1$ and $f_2$ are $1.6\%$ ($\WCTT: 120\mu$s,  $\mWCTT: 118\mu$s) and $16.25\%$ ($\WCTT: 144\mu$s,  $\mWCTT: 119.7\mu$s), respectively. This pessimism comes from the fact that $f_1$ and $f_2$ share the same path as~$f_7$. The gaps between $\WCTT$ and $\mWCTT$ for tpflows $f_3$ and $f_4$ are $30.92\%$ ($\WCTT: 328\mu$s,  $\mWCTT: 226.56\mu$s) and $43.05\%$ ($\WCTT: 520\mu$s,  $\mWCTT: 296.16\mu$s), respectively. This is due to the fact that tpflows share the same path as bpflows and can be blocked for long periods of time.
    \item Under the $2$-level scheme, both the $\WCTT$ and $\mWCTT$ for express flows remain the same. However, there is a significant improvement in the performance of tpflows in comparison to the $1$-level scheme. The maximum observed delay for $f_3$ and $f_4$ reduced by $21.17\%$ (from $226.56\mu$s to  $178.58118\mu$s) and $38.89\%$ (from $296.16\mu$s to $180.98\mu$s), respectively. Also, the gaps between $\WCTT$ and $\mWCTT$ for $f_3$ and $f_4$ reduced by $2.94\%$ ($\WCTT: 184\mu$s,  $\mWCTT: 178.58\mu$s) and $16.25\%$ ($\WCTT: 244\mu$s,  $\mWCTT: 180.98\mu$s), respectively.
    \item Under the fully-preemptive scheme, there is further improvement in performance of express flows and tpflows. Specifically, the $\mWCTT$ values of $f_1$ and $f_3$ reduced by $14.1\%$  (from $108\mu$s to  $101.3\mu$s) and $21.09\%$ (from $178.58\mu$s to  $140.9\mu$s), respectively, as compared to the $2$-level scheme. The gaps between $\WCTT$ and $\mWCTT$ for flows $f_1$, $f_2$, $f_3$, and $f_4$ under the fully-preemptive scheme are  $2.7\%$ ($\WCTT: 104\mu$s,  $\mWCTT: 101.3\mu$s), $17.77\%$ ($\WCTT: 148\mu$s,  $\mWCTT: 119.7\mu$s), $4.79\%$ ($\WCTT: 148\mu$s,  $\mWCTT: 140.9\mu$s), and $26.22\%$ ($\WCTT: 248\mu$s,  $\mWCTT: 180.98\mu$s), respectively. It is worth noticing the slight degradation in the performance of $f_2$ and $f_4$ ($1.67\%$ and $1.10\%$, respectively). This is due to the preemption overhead incurred by additional preemption operations. From this observation, it follows that there is a trade-off to find between the number of preemption levels allowed for the flow transmissions and the additional overheads that each new preemption level brings on the table. Note that we can define only up to six intermediate preemption levels since Ethernet offers a maximum of eight priority classes. We leave this pending question of the optimal number of preemption-levels for frame transmissions for future works. 
\end{itemize}
 
\begin{figure}
\centering
\begin{subfigure}{.8\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{feupphdteses/sections/analysis/images/new_1_level}
  \caption{1-level preemption scheme.}
  \label{fig:use-case-simulation-result-1-level}
\end{subfigure}%
\vspace*{1pt}
\begin{subfigure}{.8\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{feupphdteses/sections/analysis/images/new_2_level}
  \caption{2-level preemption scheme.}
  \label{fig:use-case-simulation-result-2-level}
\end{subfigure}
\vspace*{1pt}
\begin{subfigure}{.8\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{feupphdteses/sections/analysis/images/new_multi_level}
  \caption{fully-preemptive scheme.}
  \label{fig:use-case-simulation-result-multi-level}
\end{subfigure}
\caption{Observed end-to-end delay from simulation. Red dots represent WCTT bounds, black are outliers.}
\label{fig:use-case-simulation-result-perf-comp}
\end{figure}

\vspace{0.1cm}
\noindent $\triangleright \triangleleft$ \textbf{On the impact of each extra preemption level.} From Figure~\ref{fig:use-case-analysis-result}, we observe an improvement in the responsiveness of the tpflows when an extra preemption level is added to the frame transmission scheme. Specifically, this improvement reaches $43.9\%$ (from $328\mu$s to $184\mu$s) and $53.07\%$ (from $520\mu$s to $244\mu$s) for $f_3$ and $f_4$, respectively. The rationale behind this trend can be cast as follows. With the introduction of the extra preemption level, $f_3$ and $f_4$ become protected from any eventual long blocking time associated to the transmission of~$f_6$ and $f_5$ along their paths. Also, we note that the overhead induced by this extra preemption level is negligible: the $\WCTT$ $f_1$ and $f_2$ remains the same for both the $1$-level and $2$-level preemption schemes. The same condition roughly holds true for bplfows (i.e., flows~$f_5$, $f_6$, and $f_7$). Here, we note a cumulative performance degradation of $1.78\%$, which is negligible for the adopted use-case ( a degradation from $472\mu$s to $476\mu$s and $768\mu$s to $778\mu$s for $f_5$ and $f_6$, respectively). We also note that some $\mWCTT$ values for $f_5$ and $f_6$ (the black circles) fall outside the whiskers of the box plot. These outliers are the cases where an instance of a flow experiences an unusually high (or low) interference.

Still in Figure~\ref{fig:use-case-analysis-result}, we observe an average improvement of $9.6\%$ in the $\WCTT$ of tpflows when moving from a $2$-level preemption scheme to a fully preemptive approach. This suggests that the performance improvement is not linear despite the benefits brought about by each extra preemption level. On the downside, each preemption level involves extra hardware implementation overheads, which may turn out not to be negligible, unfortunately. This situation gives rise to an open question: What is the optimal trade-off in terms of preemption-level scheme to adopt for the flow transmission as the performance gain brought about by enabling each extra-preemption level is diminished by the hardware implementation overheads it brings? We are aware of this, but we leave the question out for future work as it deserves a thorough investigation. 

\begin{figure}
\centering
\includegraphics[width=\textwidth]{feupphdteses/sections/analysis/images/use-case-result-analysis-1}
\caption{WCTT for each flow under 1-level preemption, 2-level preemption and fully preemptive schemes.}
\label{fig:use-case-analysis-result}
\end{figure}

\vspace{0.1cm}
\noindent $\triangleright \triangleleft$ \textbf{On the impact of the frame sizes in each preemption class.} From the use-case setup, the maximum byte size of tpflows is reasonably small in comparison to that of the bpflows. We vary this parameter from $400$ to $1200$~bytes in order to investigate its effect on the $\WCTT$ for each tpflow. The results are reported in Figure~\ref{fig:use-case-analysis-result-perf-comp}.
\begin{figure}
\centering
\begin{subfigure}{.89\textwidth}
  \centering
  \includegraphics[width=\textwidth]{feupphdteses/sections/analysis/images/percentage-improvement-from-1-to-2}
  \caption{two-level preemption scheme.}
  \label{fig:use-case-analysis-result-perf-comp-1-to-2}
\end{subfigure}%
\newline
\begin{subfigure}{.89\textwidth}
  \centering
  \includegraphics[width=\textwidth]{feupphdteses/sections/analysis/images/percentage-improvement-from-1-to-multi-2}
  \caption{fully-preemptive scheme.}
  \label{fig:use-case-analysis-result-perf-comp-1-to-multi}
\end{subfigure}
\caption{Performance improvement w.r.t. maximum tpflow frame size.}
\label{fig:use-case-analysis-result-perf-comp}
\end{figure}

From Figure~\ref{fig:use-case-analysis-result-perf-comp-1-to-2}, we observe that the gains on the $\WCTT$ obtained from the multi-level preemption scheme over the $1$-level preemption approach diminishes with an increase in the maximum frame size. Specifically, the improvement drops from $43.9\%$ ($328\mu$s to $184\mu$s) to only $7.82\%$ ($614\mu$s to $566\mu$s) for~$f_3$ and from $53.07\%$ ($520\mu$s to $244\mu$s) to $32.3\%$ ($972\mu$s to $658\mu$s) for~$f_4$. This significant impact of the frame size on the performance of~$f_3$ can be explained by the increasing blocking time it suffers as the highest priority tpflow. We recall that frames in the same preemption class are transmitted in a non-preemptive manner. Consequently, careful attention must be paid to the maximum possible frame size of each tpflow during the flow-to-preemption-class mapping at design time. It is worth mentioning that the degradation is less severe when assuming a full preemptive scheme as illustrated in Figure~\ref{fig:use-case-analysis-result-perf-comp-1-to-multi}. Here, the performance gains over the $1$-level preemption scheme dropped from $54.87\%$ ($328\mu$s to $148\mu$s) to $33.55\%$ ($614\mu$s to $408\mu$s) for flow~$f_3$ and from $52.30\%$ ($520\mu$s to $248\mu$s) to $36.62\%$ ($972\mu$s to $616\mu$s) for flow~$f_4$. 


\subsection{Report on use-case 2.} To further evaluate the safety of the WCTT bounds, we consider another use-case scenario with a larger network and more flows provided by Renault and borrowed from~\cite{migge2018insights}. The adopted network topology is replicated in Figure~\ref{fig:renault-topology}.

$\triangleright$ {\bf Setup.} The network comprises $5$ full-duplex Ethernet switches and $14$ nodes: $4$ cameras (CAMs), $4$ displays (DSPs), $3$ control units (ECUs) and $3$ (functional) domain masters (DMs). The data transmission rate is $100$Mbit/s on all links. Assuming this setting, we consider a fully preemptive scheme, i.e., the preemption class of each flow is also its priority. The traffic specification consists of a total of $41$ flows as shown in table~\ref{tab:flow-specification}.
\begin{figure}
\centering
\includegraphics{feupphdteses/sections/analysis/images/renault}
\caption{Network topology}
\label{fig:renault-topology}
\end{figure}

\begin{table}
    \centering
    \begin{tabular}{ | m{5em} | m{6cm}| } 
        \hline
        Audio streams & -- 8 streams \newline  -- 128 and 256 byte frames \newline -- up to sub-10ms period and deadline \newline -- soft deadline constraints \\ 
        \hline
        Command and Control (C\&C) & -- 11 streams 256 to 1024 byte frames \newline -- up to sub-10ms periods and deadlines \newline -- deadline constraints (hard)\\ 
        \hline
        Video streams & -- 2 ADAS + 6 Vision streams \newline -- up to 30*1446 byte frame each 16ms (60FPS) or each 33ms (30FPS) \newline -- 10ms (ADAS) or 30ms deadline (Vision) \newline -- hard and soft deadline constraints  \\ 
        \hline
        Best-effort: file \& data tranfer, diagnostics&  -- 11 streams including TFTP traffic pattern \newline -- up to 0.2ms period \newline -- both throughput guarantees (up to 20Mbits per stream) and deadline constraints (soft) \\
        \hline
    \end{tabular}   
    \caption{Prototype flow specification with the characteristics and performance requirements for each traffic class.}
    \label{tab:flow-specification}
\end{table}

\vspace{0.15in}
\noindent $\triangleright$ {\bf Results and discussion.} Figure~\ref{fig:renault-results} presents the results obtained from the experiments. The numerical values are reported in Table~\ref{tab:renault-results}. From Figure~\ref{fig:renault-results}, it is observed that the $\mWCTT$ of all flows are less than the computed $\WCTT$ bounds. This also demonstrates the safety of the analysis presented in this work. The $\mWCTT$ values of Audio flows -- which are the highest priority flows -- are lower than the $\WCTT$ values by an average of $65.92$\%. The $\mWCTT$ values for Command and Control Traffic -- the highest priority traffic after Audio traffic -- are lower than the $\WCTT$ by an average of $42.84$\%. And finally, for the lower priority flows (Video and Best Effort flows), the $\mWCTT$ values are lower than the $\WCTT$ by an average of $36.53$\%. We noticed that the gap between the $\mWCTT$s and the $\WCTT$s are lowest for flows with the lowest priorities (Best Effort flows) and, generally speaking, the gap between $\mWCTT$ and $\WCTT$ values increases as the priority of flows increases. This is because lower priority flows are more likely to suffer the maximum possible inteferences as accounted for in the analysis. We plan to further investigate this phenomenon with the aim of reducing the pessimism in the $\WCTT$ values of higher priority flows and make the analysis as tight as possible.

\begin{figure}[htb]
\centering
\includegraphics[scale=0.6]{feupphdteses/sections/analysis/images/renault-use-case-results}
\caption{Observed end-to-end delays from simulation for the Renault use-case (in yellow box plots). The blue lines represent the WCTT bounds and the circles represent outlier values.}
\label{fig:renault-results}
\end{figure}

\begin{table}
\begin{tabular}{ |p{1cm}||p{1cm}|p{1cm}|p{1cm}|p{1.2cm}||p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|  }
 \hline
 \multicolumn{9}{|c|}{\textbf{mWCTT and WCTT for the Renault Automotive Use-Case}} \\
 \hline
      ID& Src. & Dest. & Size (bytes) & Priority &period ($\mu$s)& Deadline ($\mu$s)& mWCTT ($\mu$s)& WCTT ($\mu$s)\\
 \hline
  1&DM2&DSP1&210&1&5000&5000&72.5&310\\
 2&DM1&DSP1&200&1&5000&5000&95.8&310\\
 3&DM1&DM3&189&0&5000&5000&97.5&136\\
 4&DM2&DSP2&199&1&5000&5000&87.0&363\\
 5&ECU1&DSP2&179&0&5000&5000&77.5&163\\
 6&DM2&DSP2&159&0&5000&5000&75.8&177\\
 7&DM2&DSP2&225&0&5000&5000&115.4&362\\
 8&DM2&DSP1&138&0&5000&5000&59.5&177\\
 9&ECU3&DSP1&240&2&10000&10000&304.0&490\\
 10&ECU3&DM1&170&3&10000&10000&165.2&263\\
 11&ECU3&DM3&239&3&10000&10000&112.6&204\\
 12&ECU2&DSP2&200&2&10000&10000&322.0&499\\
 13&ECU1&DSP2&234&2&10000&10000&252.0&492\\
 14&ECU1&DSP2&214&3&10000&10000&247.0&589\\
 15&ECU1&DSP1&210&2&10000&10000&214.0&442\\
 16&ECU1&DM1&190&3&10000&10000&251.2&289\\
 17&ECU3&DM3&210&2&10000&10000&90.2&133\\
 18&ECU3&DSP1&242&3&10000&10000&167.5&630\\
 19&ECU1&DM1&250&2&10000&10000&121.8&215\\
 20&CAM4&DSP4&1446&5&10000&10000&723.2&1475\\
 21&CAM1&DSP1&1446&5&10000&10000&1304.9&1783\\
 22&CAM4&DSP4&1446&4&10000&10000&382.6&525\\
 23&CAM1&DSP3&1446&4&10000&10000&965.8&1217\\
 24&CAM2&DSP2&1446&4&10000&10000&505.9&1477\\
 25&CAM1&DSP2&1446&4&10000&10000&941.1&1597\\
 26&CAM4&DSP3&1446&5&10000&10000&1208.83&1355\\
 27&CAM4&DSP4&1446&5&10000&10000&1329.6&1475\\
 28&CAM1&DM3&1446&6&10000&10000&1529.7&2341\\
 29&ECU2&DM1&1446&7&10000&10000&1621.1&1939\\
 30&CAM1&DM2&1446&6&10000&10000&1500.6&1880\\
 31&CAM2&DM1&1446&7&10000&10000&1499.8&1518\\
 32&CAM2&DM2&1446&6&10000&10000&1220&1528\\
 33&CAM2&DM3&1446&7&10000&10000&1737.5&3757\\
 34&ECU2&DM2&1446&7&10000&10000&1076.2&1330\\
 35&CAM3&DM3&1446&6&10000&10000&1494.9&1867\\
 36&ECU3&DM1&1446&7&10000&10000&1742.4&1906\\
 37&CAM2&DM1&1446&7&10000&10000&1509.7&1518\\
 38&CAM4&DM1&1446&7&10000&10000&1863.7&2279\\
 39&CAM2&DM2&1446&7&10000&10000&1410.7&2826\\
 40&CAM2&DM3&1446&7&10000&10000&2005.6&3757\\
 41&CAM3&DM3&1446&7&10000&10000&1616.2&3157\\

 \hline
\end{tabular}
 \caption{Results: Renault use-case}
  \label{tab:renault-results}
 \end{table}
 
 

==> sections/analysis/sections/introduction.tex <==
One of the major requirements of distributed  real-time systems is ``\textit{real-time communication}'', i.e., the ability of data to move on the underlying network in a reliable and predictable manner. To date, an entire body of promising solutions have been proposed in literature, each targeting a set of domain-specific requirements. Few examples of well-established solutions include the \textit{Controller Area Network} (CAN) protocol~\cite{specification1991bosch}, the \textit{Local Interconnect Network} (LIN) protocol~\cite{specks2000lin}, the \textit{FlexRay} protocol~\cite{pop2008timing}, and TTEthernet~\cite{steiner2009ttethernet} that mainly focus on the automotive domain; the \textit{Avionics Full Duplex Switched Ethernet} (AFDX)~\cite{brajou2004airbus} that targets the avionic domain; and the so called field buses such as SERCUS III~\cite{schemm2004sercos}, EtherCAT~\cite{jansen2004real}, and PROFINET~\cite{feld2004profinet} that address the industrial domain. Most of these solutions now struggle to keep up with the growing bandwidth and performance demands of emerging applications in their respective domains~\cite{Thiele2016Formal}. On another front, with the convergence of Operation Technology (OT) and Information Technology (IT)~\cite{kamal2016and,Pop2018}, yet another challenge has settled on the table, justifying the need for new communication technologies that would facilitate the handling of heterogeneous traffic (real-time, non real-time, long and short frames) on the same network infrastructure. In this regard, among all the candidate solutions, Ethernet~\cite{IEEE802.1Q-2014} bursts forth as the leading and most promising replacement for all previous technologies. This is due to its ability to scale up to the increasingly stringent timing requirements and distance, as well as its high bandwidth capacity~\cite{Jia2013performance}. Unfortunately, the legacy Ethernet standards were originally designed targeting only non real-time applications and desirable features for real-time applications like ($1$)~frame preemption~\cite{IEEE802.3br-2016}; ($2$)~global time synchronization~\cite{IEEE802.1Qbv}; ($3$)~frame replication and elimination~\cite{Ieee2017802.1CB}; ($4$)~path control and reservation~\cite{Ieee802.1Qca}; and finally ($5$) network configuration~\cite{IEEE802QCC} among other features were missing. A tremendous amount of work has been achieved in this direction over the past few decades and several modifications and/or amendments have been made to the standards. Ethernet has successfully been enhanced with all the aforementioned features~\cite{Nasrallah2018}, thus leading to a set of \textit{updated standards}, referred to as \textit{Time-Sensitive Networking} (TSN)~\cite{IEEE} 

\vspace{0.2cm}

\noindent $\triangleright$ \textbf{IEEE 802.1Qbu.}
The IEEE~802.1Qbu~\cite{IEEEP802.1Qbu-2015} (now merged with the IEEE~802.1Q-2018 Standard~\cite{IEEE-Std-802.1Q-2018}) TSN sub-standard introduces a $1$-level frame preemption feature into the IEEE~802.1 networks. This allows to temporarily suspend the transmission of a frame prior to its completion for the speedy transmission of a higher priority frame. This standard is closely connected to the IEEE~802.3br~\cite{IEEE802.3br-2016} Standard, which allows urgent time-critical data frames to split non-critical frames in transit over a physical link into smaller fragments~\cite{bello2019perspective}. Specifically, depending on their priority levels and timing requirements, frames are mapped to two Media Access Control (MAC) Sublayer service interfaces namely, ($1$)~the ``\textit{Express MAC}'' (eMAC) and~($2$)~the ``\textit{Preemptable MAC}'' (pMAC). Frames mapped to the eMAC and pMAC interfaces are referred to as the ``express frames'' and ``preemptable frames'', respectively. These two classes are managed as follows: ($1$)~only express frames can preempt preemptable frames; and ($2$)~two frames belonging to the same class cannot preempt each other. Fig.~\ref{one-level-preemption} illustrates such a scenario at a given output node.
\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.72]{images/one-level-preemption}
    \caption{Illustration of the one-level preemption scheme.}
\label{one-level-preemption}
\vspace{-0.1in}
\end{figure}

In this figure, three frames ($f_1$, $f_2$ and $f_3$) are considered for transmission. Frames~$f_2$ and $f_3$ are eMAC frames (in red colored box), whereas $f_1$~is a pMAC frame (in green colored box). The downward arrows define the frame arrivals and upward arrows define the time instant at which the transmission of each frame is completed. Frame~$f_1$ arrives first (at time~$0$) and starts its transmission. However, upon the arrival of~$f_2$, $f_1$~is preempted and $f_2$ is transmitted. Now during the transmission of $f_2$, frame~$f_3$ arrives, but it cannot start its transmission because $f_2$, which is in the same service category, is being transmitted. The transmission of $f_3$ starts only after the transmission of $f_2$ is completed. Finally, as all the eMAC frames, which arrived after the preemption of $f_1$ have been transmitted, $f_1$~can resume its transmission.
As shown in the figure, preemption favors a prompt service of all eMAC frames, but this comes at the cost of some overheads, unfortunately. The overheads stem from the fact that fragments of split frames have to form valid Ethernet frames. As a matter of fact, pieces of information (e.g., the fragment count, an error correction code to detect whether all fragments have correctly been transmitted, etc.) must be added to the fragments of the preempted frame -- here, $f_1$ -- so that the network nodes can correctly transmit and receive all of them. In addition, these overheads are used to correctly reconstruct the original frame at each receiver node.The total overhead associated to the occurrence of each preemption is equivalent to the time taken to transmit $24$ bytes of data (i.e., $0.19 \mu s$ and $1.9 \mu s$, assuming a $1 Gb$ and $100 Mb$ speed Ethernet, respectively).
%Ojewale et al. provided an illustrative example of this mechanism (see~\cite{Ojewale2020Feasibility}, Figure 1)
Experimental studies show that this approach improves the performance of express frames~\cite{Thiele2016Formal, Jia2013performance}. Specifically, Thiele and Ernst~\cite{Thiele2016Formal} show that the performance of Standard Ethernet with frame preemption is comparable to that of IEEE 802.1Qbv~\cite{IEEE802.1Qbv}, thus making it an interesting alternative.
 \vspace{0.2cm}

\noindent $\triangleright$ \textbf{IEEE 802.1Qbv.}
The IEEE 802.1Qbv standard
defines a time-triggered gate control mechanism for TSN flows, using a Time-Aware Shaper (TAS). Here, each queue at a switch output port has a guaranteed transmission slot in a cyclic and pre-computed dispatch schedule called the Gate Control List~(GCL). A frame on a queue can be transmitted only when the gate of the queue is opened at the time period according to the GCL configuration. Note that each queue contains a unique class of frames, i.e., frames belonging to different traffic classes cannot share the same queue. The standard also specifies a so-called ``guard-band'' that ensured that the transmission of time-triggered flows is protected from any interference by other flows. The guard band is a time-period between the gate-close operation non-time-triggered queues and the commencement of transmission of time-triggered flows. The length of this guard band is equal to the time taken to transmit the largest possible non-time-sensitive frame on the network. While the guard band ensures that time-triggered traffic are protected from interference, it results in poor utilization of network bandwidth.
\vspace{0.2cm}

\noindent $\triangleright$ \textbf{Comparing IEEE 802.1Qbu and IEEE 802.1Qbv from a qualitative standpoint:} Thiele and Ernst~\cite{Thiele2016Formal} noted that a IEEE 802.1Qbu network is less complex to configure as only two basic steps are required: ($1$)~the assignment of priorities to flows; and ($2$)~the assignment of flows to preemption interfaces~\cite{park2019design}. Even though this process is non-trivial~\cite{park2019design}, it is bearable in comparison to the IEEE 802.1Qbv configuration. Here, TAS requires finding a suitable schedule for each flow at each switch output port and this problem has been shown to be NP-Hard~\cite{steiner2010evaluation}, unfortunately. On another front, IEEE 802.1Qbu solves an issue of IEEE 802.1Qbv. By combining frame preemption with TAS, optimal bandwidth utilisation is possible for non-scheduled traffic and this enables low-latency communication~\cite{bello2019perspective}. Nevertheless, the IEEE 802.1Qbv standard remains central to TSN. It defines up to 8 queues per port for forwarding traffic and frames are assigned to queues based on Quality of Service (QoS) priority. The TAS mechanism blocks all ports except one based on a predefined schedule in order to prevent delays during scheduled transmission. From an implementation standpoint, the performance of IEEE 802.1Qbu networks degrades in scenarios where the number of express frames is high~\cite{bello2019perspective}. This is due to the fact that frames of the same class are transmitted in non-preemptive manner. As a consequence, there are frames that cannot be classified as express, but have firm timing requirements. In order not to jeopardize the schedulability of these frames, and the schedulability of the entire system subsequently, these frames should not be blocked for prohibitively long time periods. The $1$-level preemption operation in the current version of the standards does not allow preemptable frames with firm timing requirements to leverage the basic benefits of enabling preemption, unfortunately. 

\vspace{0.2cm}
To circumvent the limitations of the $1$-level preemption scheme, a multi-level preemption scheme has been proposed~\cite{ojewale2018multi, Ojewale2020Feasibility}. This setup allows for more than two preemption classes and introduces a new class of flows called \textit{time-sensitive preemptable traffic}~(tpflows), i.e., flows with firm timing requirements. In this scheme, tpflow frames can be preempted by express frames and at the same time preempt lower priority frames to satisfy their timing requirements. Fig.~\ref{2-level-preemption-label-up} illustrates an example scenario that compares the improvement in the responsiveness of tpflows under a $1$-level and a $2$-level preemption setups.
\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.7]{images/2-level-preemption}
    \caption{Frame transmissions under $1$-level preemption and $2$-level preemption schemes.}
\label{2-level-preemption-label-up}
\vspace{-0.1in}
\end{figure}
In this figure, five frames ($f_1$, $f_2$, $f_3$, $f_4$, and $f_5$) are considered for transmission from a certain switch. All frames traverse in the same direction, so they compete for transmission from the output port. We assume three types of frames:~($1$)~frames $f_2$ and $f_4$ are express frames (in red colored boxes) with stringent timing constraints;~($2$)~frames $f_3$ and $f_5$ are preemptable frames (in black colored box) with firm timing constraints; and finally, ($3$)~$f_1$ is a preemptable frame with no timing constraint (in green colored box). In this example, it is assumed that frames with stringent and firm timing requirements must be transmitted before the arrival of the next one of the same type. We also assume that $f_3$ and $f_5$ have a higher priority than $f_1$. Frame $f_1$ arrives first (at time $0$) and starts its transmission, followed by frame $f_2$, and finally~$f_3$. 

%\vspace{0.1cm}
\noindent $\triangleright$ \textbf{In the $1$-level preemption paradigm:} upon the arrival of~$f_2$, $f_1$ is preempted since $f_2$ is an express frame. Then, upon the completion of this frame, $f_1$ resumes its transmission. This holds true despite the earlier arrival of~$f_3$, which has a higher priority than~$f_1$. This situation is due to the $1$-level preemption scheme as preemptable frames cannot preempt each other, thus exhibiting a \textit{priority inversion} problem. Consequently, the transmissions of~$f_3$ and~$f_5$ are delayed until the completion of $f_1$, thereby preventing $f_3$ from meeting its timing requirement. 

%\vspace{0.1cm}
\noindent $\triangleright$ \textbf{In the $2$-level preemption paradigm:} The aforementioned issue is circumvented. Here, frames~$f_3$ and $f_5$ received better services. Frame~$f_3$ is transmitted right after the completion of~$f_2$, and $f_5$ is transmitted right after the completion of~$f_4$. This allows~$f_3$ to meet its timing requirement, as well as reduces the completion times of both~$f_3$ and~$f_5$. 

\vspace{0.1cm}
\noindent Ojewale et al. already provided another example (see~\cite{Ojewale2020Feasibility}, Section VII) to promote the need for multi-level preemption which will not be replicated in this paper.

\vspace{0.1cm}
\par {\bf Contribution.} A worst-case traversal time (WCTT) analysis for TSN frames has been conducted in the literature by Thiele and Ernst~\cite{Thiele2016Formal} using Compositional Performance Analysis (CPA) framework~\cite{henia2005system}. However, the authors only considered the traditional $1$-level preemption scheme as defined in the standards. Also, Ojewale et~al.~\cite{ojewale2018multi, Ojewale2020Feasibility} propose the multi-level preemption scheme, but do not provide any formal timing guarantees for frames under such a scheme. In this paper, we build on top of these studies. We enrich the state of the art by developing a WCTT analysis of TSN frames, considering a multi-level preemption scheme. To the best of our knowledge, this is the first contribution in this direction. According to the TSN IEEE 802.1 Qbu standard, frame preemption can be implemented with or without the TSN shapers such as TAS and Credit-Based Shapers (CBS)~\cite{IEEE802.1BA}. In this work, we choose the latter scenario to focus purely on the evaluation of multi-level preemption without the added complexity of other protocol
mechanisms.

\vspace{0.1cm}
\par {\bf Paper organization.} The rest of the paper is structured as follows. The model of computation is presented in Section~\ref{sec:model} together with key notations used throughout the paper. Section~\ref{sec:cpa} provides a background on the CPA approach while Section~\ref{sec:analysis} presents the proposed analysis. Section~\ref{sec:experiment} contains experimental results from the evaluation of the proposed analysis, while Section~\ref{sec:related_work} discusses relevant related works. Finally, Section~\ref{sec:conclusion} concludes the paper and presents future research directions.



==> sections/analysis/sections/model.tex <==
% \noindent {\bf Network specification.} We assume an  Ethernet backbone network for a real-time distributed system. We model the network as a directed graph $G \equals (\mathcal{V}, \mathcal{L})$, where $\mathcal{V}$ is the set of all nodes and $\mathcal{L}$ is the set of all physical links in the network. We assume that every link is bi-directional; full-duplex; and operates at a single reference speed, say~$s > 0$. The tuple~$G$ is given with the interpretation that: ($1$)~$\mathcal{V} = \operatorname{EP} \cup \operatorname{SW}$, where~$\operatorname{EP} \equals \{\operatorname{EP}_1, \operatorname{EP}_2, \ldots \}$ represents the set of all end-points and~$\operatorname{SW} \equals \{\operatorname{SW}_1, \operatorname{SW}_2, \ldots\}$ the set of all switches. Each $\operatorname{EP}_k$ (with $k \ge 1$) has a single I/O port and can receive and send network traffic while $\operatorname{SW}$~consists only of forwarding nodes, each with a finite number of output ports, through which the traffic is routed. Each $\operatorname{SW}_{\ell}$ (with $\ell \ge 1$) is enabled with 802.1Qbu capability and decides, based on its internal routing table, to which output port a received frame will be forwarded.
% \vspace{0.1cm}

% \noindent {\bf Traffic specification.} We consider a network traffic consisting of a set $\mathcal{F} = \{f_1, f_2, ..., f_n\}$ of $n \ge 1$~flows partitioned into two traffic classes: the \textit{express traffic} (denoted by $\mathcal{E}$) and the \textit{preemptable traffic} (denoted by $\mathcal{P}$), i.e., $\mathcal{F} = \mathcal{E} \cupdot \mathcal{P}$. In other words, $\mathcal{E} \cup \mathcal{P} = \mathcal{F}$ and $\mathcal{E} \cap \mathcal{P} = \emptyset$. Each flow $f_i \in \mathcal{F}$ consists of a potentially infinite number of frames $f_i^k$ (with $k \ge 1$) and the smaller the subscript of a flow, the higher its priority. This means that flows with different priorities follow a total order. All frames generated by a flow inherit its priority. We assume that the preemptable traffic class is further partitioned into two disjoint sub-classes referred to as the \textit{time-sensitive preemptable traffic}~(tpflows), with firm timing requirements~(deadlines); and  \textit{best effort preemptable traffic}~(bpflows), with no timing requirements at all. We denote these two sub-classes as $\mathcal{TP}$ and $\mathcal{BP}$, respectively: $\mathcal{P} = \mathcal{TP} \cupdot \mathcal{BP}$. Frame $f_i^k$ is the $k^{\operatorname{th}}$ frame of $f_i$ and is characterized by its arrival time $a_i^k$ and its payload $p_i^k$. The size $p_i^k$ of flow $f_i$ is the sum of its payload and transmission overheads. Throughout this paper, we assume that the maximum size of any flow is limited to $1518$~bytes, i.e., the maximum Ethernet frame size as defined in the IEEE~802.3 Standard~\citep{IEEE802.3br-2016}. Every flow~$f_i$ is also assigned a unique preemption class $\operatorname{PC}_i$ that qualifies the set of flows with the same preemption properties as~$f_i$. For convenience, we assume that there are $m$ different preemption classes in the system ($1$~denotes the highest preemption class -- comprising only flows in $\mathcal{E}$, then $2$, $3$, and so on till $m > 1$, the lowest one -- comprising only flows in $\mathcal{BP}$). Note that $\operatorname{PC}_i \cap \operatorname{PC}_j = \emptyset$, $\forall i \neq j$ and the following rules are enforced.
% \begin{enumerate} 
% %\item[$R_1$--] Every $f_i \in \mathcal{E}$ can preempt all $f_j \in \mathcal{P}$;
% \item[$R_1$--] Every flow, say $f_i$, can preempt any other flow, say $f_j$, only if $\operatorname{PC}_i < \operatorname{PC}_j$, but flows in $\operatorname{PC}_j$ cannot preempt flows in $\operatorname{PC}_i$;
% \item[$R_2$--] Flows in the same preemption class cannot preempt each other and are transmitted with a strict priority order;

% \item[$R_3$--] Flows with the same priority are transmitted in a FIFO manner;

% \item[$R_4$--] Flows with the same priority always belong to the same preemption class but the converse is not true. In other words, flows with different priorities can be assigned to the same preemption class (see Figure~\ref{fig:preemption-class}).
% \end{enumerate}

% \begin{figure}
% \centering
% \includegraphics[scale=0.85]{feupphdteses/sections/analysis/images/preemption-class-model-1.PNG}
% \caption{System model: Preemption class vs. priority queues}
% \label{fig:preemption-class}
% \end{figure}

% 

==> sections/analysis/sections/related_work.tex <==
The Network Calculus~(NC)~\citep{reimann2013timing}; the  Trajectory Approach~(TA)~\citep{Tracjectory2006Martin}; and the Compositional Performance Analysis~(CPA)~\citep{henia2005system} have all been used as established techniques to provide timing guarantees for real-time Ethernet flows. In this section we report only the most significant contributions related to our topic. 

In NC, a so-called \textit{arrival curve} and \textit{service curve} are used to model the arrival of flows and the transmission bandwidth at a switch output port, respectively. To the best of our knowledge, only a hand-full of contributions using this approach are available in the literature on TSN related issues.\cite{zhao2018worst} provided a worst-case latency analysis for IEEE~802.1Qbv networks. To this end, they assumed that the Gate Control List~(GCL) and the priority assignment configurations are given. They validated the performance of their approach by using both synthetic and real-world use-cases in terms of scalability and effect of GCL overlapping characteristics on individual flows. The authors, in another work, also provided a latency analysis for AVB
traffic in TSN using NC~\citep{zhao2020latency}. However, their analyses only target non-preemptive TSN networks and lefts the preemptive case unanswered.

In TA,~\cite{Tracjectory2006Martin} investigated the highest number of frames that share the same trajectory as it is a potential source of delay for each of these flows. The adopted approach proceeds ``backwards'', i.e., from the receiver node to the source node. In another context, this approach as been used by~\cite{bauer2012trajectory} for the timing analysis of AFDX with strict priority, non-preemptive flows transmitted by following a FIFO scheduling strategy. In the work, the~TA has been further enhanced by exploring the basic idea according to which flows sharing a common link cannot arrive at the same time at a switch.~\cite{li2014trajectory} have proven the result to be optimistic and have corrected the flaw. Nonetheless, the analysis still considers only non-preemptive frame transmission. 

\cite{cao2016EligibleInterval, cao2016independent} introduced a so-called \textit{eligibility interval} approach for the timing analysis of Ethernet Audio Video Bridges~(AVB)~\citep{IEEE2011AVB} networks with Credit-Based Shapers~(CBS). In this approach, the worst-case performance of a flow is examined when a flow has some pending payload to transmit and a non-negative transmission credit. This approach was proven to be tight for AVB networks and subsequently extended for the timing guarantees of AVB flows in standard TSN~\citep{maxim2017delay}. Thangamuthu et al.~\cite{thangamuthu2015analysis} proposed a worst-case performance analysis for Switched Ethernet with Burst-Limiting Shaper~(BLS); Peristaltic Shaper~(PS); and Time-Aware Shaper~(TAS) for TSN, but concluded that only the TAS can schedule control traffic within the maximum delay imposed by the Standards. In a nutshell, PS imposes an organization on the reception and transmission of frames at each node by following well-defined time intervals. Here, every time window is divided into intervals (even and odd intervals) and all frames received within an interval are transmitted in the next interval only. BLS is an extension of CBS introduced by the AVB Standard~\citep{IEEE2011AVB}, wherein a transmission budget or ``credit'' is assigned to each traffic class to control its transmission rate and mitigate against burst traffic. Finally TAS defines a time-triggered gate control mechanism for TSN flows. Here, each flow class has a guaranteed transmission slot in a cyclic and pre-computed dispatch schedule.

CPA has been used extensively for the timing behavior of Ethernet flows~\citep{thiele2015improving, thiele2014improving}. It uses the so-called \textit{level-$i$ busy period} approach, activated by the so-called critical instant, to investigate the worst-case response time of each real-time flow~\citep{handbook2017cpa}. CPA was employed for the timing behavior of Switched Ethernet in~\citep{Rox2010} and for Ethernet AVB in~\citep{Diemer2012}. The analysis for Switched Ethernet was improved by~\cite{thiele2014improving} to tighten the worst-case response time bounds of each flows by up to $80\%$, then the same authors exploited the FIFO nature of Switched Ethernet transmission~\citep{thiele2015improving} to reduce the interference estimation in frame transmissions and achieved about $30\%$ latency improvement over the state-of-the-art CPA at the time. Still by using CPA,~\cite{Thiele2015Peristaltic} and~\cite{Thiele2016BLS} proposed the worst-case analysis for TSN with PS and BLS, respectively. Both contributions focused only the shapers, leaving frame preemption concerns beyond the scope of their work. On another front,~\cite{Thiele2016Formal} used CPA to provide worst-case guarantees for both Standard Ethernet and IEEE 802.1Qbv when frame preemption in enabled. Lo Bello et al. also provide a schedulability analysis for IEEE 802.1Qbv networks with preemption support~\citep{bello2020schedulability}. In these works, the authors address only the traditional $1$-level preemption scheme, as defined in the standards.
Recently, \cite{ojewale2018multi, Ojewale2020Feasibility} promoted the multi-level preemption approach for IEEE~802.1Qbu networks in order to circumvent the limitations of the $1$-level preemption scheme. The authors first investigated the feasibility and advantages of multi-level preemptions in time-sensitive Ethernet networks. Then, they focused on its feasibility and implementation requirements in details. Recently, \cite{knezic2020implementation} provided an improved implementation approach for the multi-level preemption scheme.  However, their works stop short of providing a formal analysis of the worst-case performance guarantees under the proposed scheme. We fill this gap in this thesis by providing the worst-case traversal time analysis of TSN frames under the multi-level preemption assumption, which is the first contribution in this direction to the best of our knowledge.

==> sections/background/background.tex <==
\chapter{Background}
\label{chap:background}
In this chapter, we introduce background concepts necessary for a smooth understanding of our contributions. In particular, we discuss the fundamentals of real-time communication, Ethernet technologies, TSN, and Frame Preemption in the context of DRES. In this regard, the rest of the chapter is organized as follows. First, we introduce real-time communication in Section~\ref{sec:background:real-time-com}. In Section~\ref{sec:background:real-time-protocols}, we describe a representative, but not exhaustive, selection of established real-time communication protocols from the literature. We then take a closer look at Ethernet and TSN, respectively, in Section~\ref{sec:background:Ethernet-details} and Section~\ref{sec:background:TSN}. Then, in Section~\ref{sec:background:preemption}, we discuss the TSN frame preemption feature as currently specified in the standards and recall its main limitations discussed in the previous chapter. Finally, in Section~\ref{sec:background:related_work}, we present a number of related works that are relevant to the challenges addressed in this dissertation.

\section{Real-time communication}
\label{sec:background:real-time-com}
The proper operation of DRES depends not only on the timely execution of computational tasks, but also on the timely communication between the embedded devices that make up the system~\citep{Malcom1992Advances} 
For traditional communication network applications such as electronic mail, file transfer, and remote desktop connections, the typical performance metrics of interest are: throughput, delay, and average messages/packets delivered~\citep{Aras1994Real}. For these types of applications, it is usually desirable to achieve low latency. Much of the complexity of network protocols arises from the need for lossless communication, and there are no specific timing constraints on messages. In contrast, DRES consists of multiple embedded real-time devices that must communicate within precise timing constraints. The distinguishing feature of real-time communication is that the value of the communication also depends on the time at which the messages are successfully delivered to the receiver~\citep{Aras1994Real, cottet2002scheduling}. Here, each message is assigned a so-called \textit{deadline} --the latest desired delivery time--and the value of the message is greatly diminished if it is delivered after its deadline. In some real-time applications, messages are even considered ''perishable'' and unusable if they are not delivered on time. In these applications, missing a deadline could lead to serious and/or catastrophic consequences, such as loss of life, injury to people, and/or financial loss. Figure~\ref{fig:autonomous-vehicle} illustrates a real-world use case with real-time communication, where an autonomous vehicle (the black car) crosses an intersection and detects an obstacle (the gray car in the red rectangle).

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.4]{feupphdteses/sections/feasibility/images/self-driving-car-obstacle avoidance.jpg}
    \caption{Obstacle detection in an autonomous vehicle. Source: Zendrive}
\label{fig:autonomous-vehicle}
\end{figure}

In this figure, the autonomous vehicle's detection sensor must not only correctly inform the braking system that an obstacle has been detected, but it must also transmit this information quickly enough for the braking system to make a decision in time to avoid a collision. If this information reaches the braking system only after a collision has occurred, it is useless. Therefore, real-time communication must be reliable and predictable, i.e., it must be ensured that the time required to relay the message does not exceed a predefined value that is less than or equal to the deadline. Other use cases include the Global Positioning System (GPS), multimedia systems, and surveillance systems, to name just a few examples.
\begin{tcolorbox}
    \centering
    In the dissertation, we focus on real-time communication in the context of DRES.
\end{tcolorbox} 

\section{Real-time communication protocols}
\label{sec:background:real-time-protocols}
Historically, real-time communication was implemented using point-to-point (P2P) connections between components (nodes) that need to communicate with each other~\citep{davis2007controller}. However, the number of connections (wires) required for a fully connected network increases very rapidly. In fact, the number of wires required for a fully connected P2P network with $n$ nodes is $\frac{n \times (n-1)}{2}$ -- that is, this number grows polynomially with the number of nodes. A fully connected network with only $5$ nodes requires up to $\frac{5 \times (5-1)}{2} = 10$ wires, as shown in Figure~\ref{fig:p2p}.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.9]{feupphdteses/sections/background/images/p2p-network}
    \caption{Illustration of a fully connected P2P network with $5$ nodes.}
\label{fig:p2p}
\end{figure}

With the ever-increasing number of interacting nodes in DRES, managing the number of wires becomes very difficult. To illustrate this assertion, suffice it to mention that an autonomous car today consists of over $100$ Electronic Control Units (ECUs). This would mean at least $4950$~wires to achieve a fully connected underlying network. To get around this hurdle, the so-called ``bus'' communication system was introduced~\citep{gustavson1984computer}. Unlike P2P communication networks, this is a shared communication path between multiple nodes. Here, a node must first be granted exclusive access to the shared communication path before it can send data. Once this access has been granted, the node can communicate. In one of the first access methods, namely master-slave, the sending node (called the ``master'') writes its message to the bus, and this is accessible to all other nodes (called the ``slaves''). The message contains an identifier, the addresses of the sender and receiver nodes, the data to be transmitted, and whether the communication event is a \textit{read} or a \textit{write}~\citep{gustavson1984computer}. The term ``read'' means that the master requests some information from the receiving node(s), while the term ``write'' means that the master shares some updates with the receiving node(s). After the message is received by the slaves, only the node(s) with the matching address(es) will process the message and perform the required actions. The other nodes will ignore and discard it.
Access to the shared communication path is controlled by the so-called Medium Access Control (MAC) protocol, which ensures that only one node can access the bus at a time. Note that this MAC varies from one bus implementation to another. 
Figure~\ref{fig:wire-to-bus} shows an example where the previous P2P network in Figure~\ref{fig:p2p} is converted to a bus-based network.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.9]{feupphdteses/sections/background/images/wire-to-bus}
    \caption{Bus communication with $5$ nodes}
\label{fig:wire-to-bus}
\end{figure}

In the remainder of this section, we briefly describe some of the most prominent shared medium real-time protocols in the literature.

\subsection{Fibre Distributed Data Interface (FDDI)}
FDDI is a shared network with a ring topology~\citep{cottet2002scheduling} in which the access control is performed using a so-called ``token''. The token is passed from one node to the next, in the order in which it is located in the physical ring network. A node can only transmit if it has the token. Conversely, if a node has nothing to transmit, it forwards the token immediately to the next node. However, to avoid the starvation of other nodes that would result from a node holding the token for an unbounded period of time, a parameter called Target Token Rotation Time (TTRT) is used. The TTRT specifies approximately the maximum time the token may take to traverse the entire ring. When a node receives the token, it measures the time the token took to circulate through the whole ring (called the Real Token Rotation Time) and subtracts this from the TTRT. This difference is called the Token Holding Time. If it is positive, the node is allowed to transmit during this time. If it is zero or negative the node must forward the token immediately. Consequently, the maximum time a node can hold the token and transmit is bounded, making token-based communication predictable. Figure~\ref{fig:fddi} shows a simplified architecture of an FDDI network with $5$~nodes.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.6]{feupphdteses/sections/background/images/fddi}
    \caption{Simplified architecture of an FDDI network with $5$ nodes.}
\label{fig:fddi}
\end{figure}

The \textit{token-bus} is a variant of FDDI in which the shared medium is a bus instead of a ring. Here, the logical successor of a node is not necessarily the same as its physical successor, which gives the MAC protocol additional flexibility.  

\subsection{Controller Area Network (CAN)}
CAN is also a bus-based communication technology and is often referred to as a ``CAN bus''. Its shared medium consists of a twisted pair of wires (``CAN high'' and ``CAN low'') to which all nodes are connected in parallel.  The extremities of the CAN bus must be connected to terminating resistors of $120\Omega$ (nominal) to reduce signal reflections~\citep{richards2002can}. Data transmission on a CAN bus is accomplished by a differential voltage signal between the CAN high and CAN low wires. When a device transmits logical 1, it applies a higher voltage to the CAN high wire and a lower voltage to the CAN low wire. Conversely, when a logical 0 is transmitted, it applies a lower voltage to the CAN high wire and a higher voltage to the CAN low wire. This creates a differential voltage between the two wires that is used to transmit the data. Other devices in the CAN network listen for this voltage difference and can decode the transmitted message. The transmission in differential voltage mode increases the resilience to electromagnetic interference. Figure~\ref{fig:can} shows a simplified architecture of a CAN network with $5$~nodes.

CAN uses a bit modulation called Non-Return-to-Zero that corresponds to keeping the voltage levels fixed during the whole bit time. The bus drivers of each node implement a so-called wire-AND function that grants the property of dominance. The logical 0 is called dominant while the logical 1 is called recessive. A single node transmitting a 0 forces the bus level to 0. Conversely, the bus level will be at 1 only when all nodes are transmitting 1~\citep{richards2002can}


\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.6]{feupphdteses/sections/background/images/can}
    \caption{Simplified architecture of a CAN network with $5$ nodes.}
\label{fig:can}
\end{figure}

Nodes access the CAN bus randomly and event-driven. If two nodes attempt to occupy the bus simultaneously, access is granted by non-destructive, bitwise arbitration, i.e., the node that wins the arbitration simply proceeds with the message without the message being destroyed or corrupted by another node. The identifier of a message (ID) is also its priority, and the lower the binary identifier of a message, the higher its priority. A node that wins the arbitration puts its data (called a ``signal'') on the bus, and all other nodes in the network have access to it. However, only the receiving node(s) receive(s) this message from the bus, while all other nodes simply ignore it. This protocol~\citep{specification1991bosch} was introduced by \href{https://www.bosch.com/}{Robert Bosch GmbH} in the early 1990s and was primarily intended for the automotive sector to meet speed and bandwidth requirements. 

Regarding the advantages and disadvantages of this protocol, it should be noted that CAN is very well-suited for applications with a large number of short messages. In addition, it is particularly well-suited when data is needed from more than one location due to the broadcast nature of the communication. However, it also has some serious limitations. First, the length of the CAN bus is limited. The maximum bus length at a bit rate of $10$~kbit/s is $1$~km, and the maximum length at $1$~Mbit/s is $40$~m. 
\begin{tcolorbox}
    The data rate during the arbitration phase cannot exceed 1 Mbit/s, even in more recent versions that allow higher speeds during the transmission of the payload of the message (e.g., CAN-FD). Due to its broadcast nature, the CAN protocol does not efficiently utilize the communication medium. Furthermore, there is no robust flow control mechanism other than priority arbitration.
\end{tcolorbox}


\subsection{Local Interconnect Network~(LIN)}
At the turn of the millennium, the LIN protocol emerged as a complementary technology to CAN~\citep{specks2000lin}, providing low-cost, low-speed connectivity for in-vehicle networks. LIN is a serial, broadcast, one-wire (as opposed to CAN's two-wire) interface and is typically implemented as a sub-bus of a CAN network. It allows automotive manufacturers to reduce costs by moving slow, non-safety-critical functions from a two-wire bus CAN to a single-wire. LIN is a master-slave network in which a master coordinates communication between up to 16 slave devices on the network.

\subsection{FlexRay}
FlexRay (``Flexible Ray'') is another bus-based communication protocol that also complements CAN in automotive networks~\citep{pop2008timing} by providing higher speed (up to $10$~Mbps) and more reliable communication on the sub-bus of a CAN network. FlexRay's higher speed means that its maximum bus length is significantly less than that of CAN. FlexRay is also significantly more expensive than CAN. It supports timed communication by performing cycle-based transmission. Specifically, each cycle is divided into two parts: the static segment and the dynamic segment. The static segment is divided into slices for individual communication types and provides stronger determinism than CAN, while the dynamic segment provides event-driven behavior.

\subsection{Ethernet}
The Ethernet communication protocol was developed by Robert Metcalfe at \href{https://www.parc.com/}{Xerox PARC} between 1973 and 1974~\citep{shoch1981introduction}. The name is based on the word ``ether'' -- an archaic word coined in the nineteenth century to describe the invisible medium through which light supposedly travels~\citep{huang1998ethernet}. Ethernet provides P2P communication via a simple passive medium (coaxial, twisted pair, or fiber optic cable) in which nodes communicate by sending messages to each other in the form of data packets. Each node is assigned a unique address and link-level communication is established using the addresses of the sender (source) and the receiver (destination). The receiver accepts only the packets addressed to it and ignores the rest. In 1980, the speed of Ethernet was already $10$~Mbit/s~\citep{shoch1981introduction}.
Similar to bus-based technologies, Ethernet was originally designed to use a common P2P medium for communication, creating a single collision domain. To avoid collisions, a fully distributed link access mechanism called \textit{Carrier Sense Multiple Access with Collision Detection} (CSMA/CD) is used~\citep{shoch1981introduction}. Specifically, a node can transmit its message only when the shared medium is not busy. Since all nodes are waiting for the medium to become free, it is possible for two or more nodes to detect the idle state at the same time and start transmitting. This eventually leads to a collision. In this case, the affected transmissions are aborted and the nodes wait a random amount of time before attempting to retransmit the messages. This process is repeated until the message is successfully transmitted, i.e., without collision. 
\begin{tcolorbox}
    The collision and retransmission of messages lead to low efficiency in bandwidth usage of Ethernet.
\end{tcolorbox}


\section{Ethernet for real-time communication}
\label{sec:background:Ethernet-details}
Although Ethernet predates CAN by nearly two decades and offers much more speed and bandwidth, many did not consider Ethernet as a solution for DRES until much later. This is because the older Ethernet standards were originally intended for non-real-time applications and have several limitations that make it challenging to use in DRES~\citep{Nasrallah2018}. As discussed in Section~\ref{sec:introduction:context}, one of these limitations is that it is unpredictable, i.e., there is no guarantee that data will be delivered within a predefined time period. Another limitation is its susceptibility to network congestion. Ethernet uses a shared medium for communication, which means that multiple devices can transmit data over the same network at the same time, which can cause collisions and delays that degrade network performance and make it difficult to transmit data in real-time.

Over the years, several changes have been made to these standards to address these shortcomings. For example, the IEEE 802.1p Task Group specified the so-called\textit{ Class of Service (CoS)} mechanism to speed up the transmission of some frames~\citep{IEEE802.1Q-2014}. In particular, this mechanism introduced the notion of \textit{priority} for Ethernet frames, where the CoS of a frame indicates its priority. With this mechanism, priorities can be assigned to FIFO queues and frames are stored in these queues based on their CoS classes. Eight CoS classes~\citep{IEEE802.1Q-2014} are defined, and frames are transmitted according to their CoS - the frames with the highest CoS first. Frames with the same CoS are stored in the same output queues and transmitted on a FIFO basis. 
\begin{tcolorbox}
    In the following sections, we introduce prominent protocols/features that have been introduced in the literature to mitigate the limitations of Ethernet for real-time communication.
\end{tcolorbox}

%With these and several other modifications, Ethernet has become the emerging communication technology for modern real-time networks. Its ability to meet the increasingly stringent speed and distance requirements, along with its high bandwidth capacity, made it an ideal replacement for earlier communication infrastructures. Over the years, several real-time Ethernet technologies have emerged, each offering real-time capabilities for different application areas. In the following, we present some of these technologies.


%In the following sections, we present prominent features that have been introduced in the literature to mitigate these limitations.

\subsection{Switched Ethernet}
The two problems, i.e., collision and retransmission of messages  (also referred to as ``frames''), were the main reasons for the introduction of Ethernet switches. Unlike classical Ethernet, where the medium is shared by the nodes, Switched Ethernet gives each node its own connection to a switch through its various ports. The switch then connects the node to one or more other switches and nodes in the network. With Switched Ethernet, collisions do not occur in the medium because of the dedicated connection between each node and the switch(es). However, collisions can still occur on a destination port if it receives frames from more than one port at a time. In a switch, each port has its own individual collision domain and resolves them individually. Figure~\ref{fig:switched-ethernet} shows a simplified architecture of a Switched Ethernet network with $5$~nodes.

 \begin{figure}[htb]
     \centering
     \includegraphics[scale=0.8]{feupphdteses/sections/background/images/switched_ethernet.pdf}
    \caption{A simplified architecture of a switched Ethernet network with $5$ nodes.}
 \label{fig:switched-ethernet}
 \end{figure} 

Each switch significantly mitigates the impact of the CSMA/CD arbitration mechanism on bandwidth utilization and makes the network less unpredictable. The internal architecture of a basic Ethernet switch is shown in Figure~\ref{fig:switch-architecture}, where the number of input and output ports are equal. 

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.8]{feupphdteses/sections/background/images/switched_Ethernet_port.PNG}
    \caption{Illustration of the internal Architecture of a basic Ethernet Switch}
\label{fig:switch-architecture}
\end{figure}

Frames enter the switch through the input ports and leave through the output ports. The Frames are first received in a buffer and, after complete and error-free reception, are sent to the switch fabric for forwarding. The switch fabric uses the destination address and the predefined transmission rules to determine the output ports to which the received Frames should be forwarded. The output ports are equipped with multiple FIFO queues that store frames waiting to be forwarded. In the remainder of this dissertation, the term ``Ethernet" will be used simply to refer to Switched Ethernet unless otherwise noted.

%\subsection{Real-time Ethernet}
%Other features like global time synchronisation, frame duplication and re-transmission among others, have also been added to Ethernet to make it more suitable for real-time applications~\cite{Nasrallah2018}. 

\subsection{EtherCAT}
EtherCAT, or ``\textit{Ethernet for Control Automation Technology}'', is a master-slave protocol developed by Berkhoff in 2003 and later standardized by the International Electronical Commission~\citep{iec200761158}. The protocol was originally developed with industrial control systems in mind. In a typical EtherCAT network, there is a single master node and multiple slave nodes. In contrast to Ethernet, where frames are sent from sender nodes to destination nodes, EtherCAT nodes communicate via so-called ``telegram'' messages. Specifically, telegrams are generated by the master nodes and sent through the network, passing through all slave nodes and being sent back to the master. The slave nodes read the data addressed to them as the telegram traverses the node, and process the data ``on the fly''. Note that these nodes can also insert data into the telegram as it passes through them. EtherCAT supports data rates of up to $1$~Gbit/s and can be used over both copper and fiber optic cables. It is developed and maintained by the \hyperlink{https://www.ethercat.org/default.htm}{EtherCAT Technology Group (ETG)}, a global organization that promotes the use of EtherCAT and other industrial Ethernet technologies. The ETG works closely with leading industrial automation companies and organizations to ensure that EtherCAT meets market needs and remains at the forefront of industrial Ethernet technology.

\subsection{PROFINET}
PROFINET, a portmanteau for Process Field Net, is a technical communication standard based on Ethernet~\citep{feld2004profinet}. It is part of the IEC 61158-2 standard~\citep{Winkel2016Standard} and is widely used in manufacturing and other industrial environments. PROFINET enables real-time communication and control of automation devices such as sensors, motors, and controllers. It supports ($1$)~a wide range of data rates, from $100$~Mbit/s to $1$~Gbit/s; and ($2$)~four real-time traffic classes, namely: \textit{ RT class UDP} (RT UDP), \textit{ RT class~$1$} (RT ~$1$), \textit{ RT class~$2$} (RT ~$2$), and \textit{ RT class~$3$} (RT ~$3$). RT ~$3$ has the highest priority, followed by RT ~$2$, then RT ~$1$, and finally RT UDP the lowest. In PROFINET, communication is cyclic and each cycle is divided into communication intervals. These intervals are reserved specifically for each of the classes. The nodes use a clock synchronization mechanism to ensure that the cycles are synchronized. All other traffic is blocked when a scheduled slot occurs. The protocol also supports a non-real-time class (NRT), which has a lower priority than the real-time classes and is transmitted largely based on standard Ethernet specifications.

%PROFINET requires specific hardware modifications and is not interoperable with other communication protocols.

\subsection{AFDX}
\label{sec:background:afdx}
\hyperlink{https://www.airbus.com/en}{Airbus} developed and trademarked what it calls \textit{Avionics Full-Duplex Switched Ethernet} (AFDX) in 2006 to improve the timing performance and reliability of standard Ethernet. As the name implies, AFDX targets real-time communication in avionics. Here, each node in the network is connected to a switch via a full-duplex link, meaning frames can move in opposite directions on a physical medium simultaneously. In this way, collisions can no longer occur on the physical medium, and CSMA/CD is no longer required. Full-duplex bidirectional transmission is achieved by using twisted pairs or fiber optic cables. While transmission links are collision-free, AFDX shifts the collision problem to the switching layer, where different frames compete for switching resources (e.g., input buffers, output queues, access to the transmission link, etc.). This can lead to congestion and frame loss at the switch's output ports if, at any given time, too many traffic arrives at a port than it can buffer or transmit. In addition, these congestion and frame losses negatively impact timing performance and reliability. To mitigate this, the protocol defines a virtual circuit - that is, a logical communication channel between a source node and one or more destination nodes. Each Virtual Link (VL) is associated with a so-called \textit{Bandwidth Allocation Gap} (BAG), which defines the minimum time interval between successive frames on the VL. To enforce the BAG, AFDX defines a so-called ``\textit{shaper}'' that limits the traffic rate at the source node to ensure deterministic communication behavior. The traffic resulting from this ``shaper'' became known as \textit{Rate-Constrained (RC)} traffic.

\subsection{TTEthernet}
\label{sec:background:ttethernet}
The concept of \textit{Time-Triggered Ethernet} first appeared in the work of~\cite{kopetz2005time} and TTEthernet is an industrial development that builds on this work~\citep{steiner2009ttethernet}. Here, messages are divided into three traffic classes: ($1$)~Time-Triggered~(TT) traffic; ($2$)~Rate-Constrained~(RC) traffic (as discussed in AFDX, see Section~\ref{sec:background:afdx}); and finally ($3$)~Best-Effort~(BE) traffic. As the name implies, the main communication mode in TTEthernet is the \textit{time-triggered} transmission. Specifically, TT traffic enjoys accelerated transmission and is transmitted based on a strict, pre-calculated offline schedule. When a time slot in the schedule is free of TT traffic, the available bandwidth is used for other traffic classes. In addition, TTEthernet requires a common time notion among the communicating nodes and thus network-wide clock synchronization. TTEthernet can provide deterministic behavior and timing guarantees for TT and RC traffic. However, the use of static offline schedules severely limits its configuration flexibility. Moreover, scheduling TT frames is equivalent to a bin-packing problem known as NP-hard~\citep{Nayak2017}.
\begin{tcolorbox}
    The time synchronization requirement is not necessary (nor applicable) for some real-time systems, especially in use-cases that require dynamic behavior and/or unsynchronized terminals.
\end{tcolorbox}


\subsection{Audio Video Bridging (AVB)}
\label{sec:background:avb}
In~$2005$ the IEEE formed the \textit{Audio Video Bridging} (AVB) Task Group to develop an Ethernet profile for the automotive industry~\citep{IEEE2011AVB}. The Task Group was particularly interested in supporting the transmission of time-sensitive media frames over automotive Ethernet networks. To accomplish this, AVB introduces three new standards: ($1$)~\textit{clock synchronization} (IEEE 802.1AS~\citep{IEEE802.1AS}); ($2$)~\textit{bandwidth reservation}~ (IEEE 802.1Qat~\citep{IEEE802.1Qat-2010}); and ($3$)~\textit{traffic shaping} (IEEE 802.1Qav~\citep{IEEE802.1Qav}). It defines two Stream Reservation classes: Class~$A$ and Class~$B$ (where Class~$A$ has a higher priority than Class~$B$) and only frames with real-time requirements are assigned to these classes. The transmission of frames is governed by the so-called \textit{credit-based shaper} (CBS) algorithm (explained in detail in Section~\ref{sec:background:cbs}), which guarantees fair access for time-sensitive frames in the network and ensures that frames are delivered with minimal delay.
\begin{tcolorbox}
    Although the AVB profile brings significant performance improvements to Ethernet, the standards can only guarantee a latency limit of $2$~ms or less over $7$~hops. Some emerging automotive applications  require as low as $500\mu$s -- $1$ms over several hops~\citep{IEEE802.1DG-2021}.
\end{tcolorbox}

\subsection{Time-Sensitive Networking (TSN)}
In~$2012$, the IEEE renamed the AVB Task Group the \textit{Time-Sensitive Networking} (TSN) Task Group to reflect the broadened scope of its work, which is to ``provide the specifications that enable time-synchronized, low-latency streaming services over IEEE 802 networks.''~\citep{IEEE}. In other words, the TSN Task Group is no longer focused only on the automotive domain but is expected to improve AVB standards and also extend the Ethernet Virtual Local Area Network (VLAN) protocol to meet the needs of time-sensitive applications in multiple domains. 

In response, the TSN Task Group published (and is still publishing) a set of standards to introduce features that enable Ethernet to meet the stringent timing, bandwidth, and Quality of Service (QoS) requirements for time-sensitive data in emerging DRES. These standards will be referred to hereafter as ``TSN standards'' or simply as ``TSN''. They deal with network transmission at the flow (also referred to as ``stream'') level. Each \textit{flow} is defined as an end-to-end unicast or multicast communication between two or more nodes. One node is referred to as the sender and the other(s) as the receiver(s). By this definition, each flow consists of a potentially infinite collection of frames transmitted from one node, e.g., $A$, to another node, e.g., $B$, separated by a minimum inter-arrival time between frames, also called \textit{period}.

\begin{tcolorbox}
TSN is designed to support low-latency flow transmission with high reliability and precise synchronization. This makes it ideal for applications where real-time data is critical, including DRES.
\end{tcolorbox}

\section{TSN features in details}
\label{sec:background:TSN}
TSN uses a combination of several features introduced in different standards to achieve real-time communication. In this section, we discuss these features in more detail. Recall that TSN standards are motivated by the shortcomings of traditional Ethernet for real-time communication, including: ($1$)~the lack of network-wide time synchronization; ($2$)~the lack of network resource reservation and enforcement mechanisms; ($3$)~the lack of flow/traffic control mechanisms; and ($4$)~the lack of appropriate flow integrity mechanisms. In the following subsections, we discuss TSN standardization efforts that address these shortcomings. For a structured approach to this discussion, we adopt a classification similar to ~\cite{Nasrallah2018}.
\vspace{0.2cm}

\subsection{Network-wide clock synchronization}
\label{sec:background:syncronisation}
The IEEE 802.1AS~\citep{IEEE802.1AS} standard uses a profile of the IEEE precision time protocol (PTP) 1588-200~\citep{IEEE1588-200} called generic PTP (gPTP)~\citep{teener2008overview} to synchronize clocks in a distributed network with a master-slave architecture. Specifically, it first uses what is called the \textit{Best Master Clock Algorithm} (BCMA) to select the so-called GrandMaster (GM) - i.e., the node in the network with the most accurate clock\footnote{The GM time source is International Atomic Time (TIA)~\citep{Nasrallah2018}}. Then a hierarchical spanning tree is created to communicate this time value across the network. In this process, each node serves as a master for all its child nodes. After receiving a clock value, each child node calculates its current time using a peer-path delay mechanism, i.e., an end-to-end communication delay between neighboring links with respect to the GM 

From this description, the direct conclusion is that the synchronization of the network clock depends heavily on the availability and correctness of GM. In other words, the network is not immune to the failure of GM. To mitigate this limitation, a revision of the IEEE 802.1AS standard~\citep{IEEE802.1AS-REV} has been introduced to improve \textit{fault tolerance}. The revision supports the presence of multiple timing references in the network. This would allow the network to switch to a different time domain if one GM fails. Another limitation of IEEE 802.1AS is the message transmission overhead associated with time synchronization. More centralized approaches have been proposed in the literature. However, such an approach would introduce a single point of failure into the network.

\begin{tcolorbox}
    We believe that further studies are needed to find a good compromise between distributed and centralized approaches to leverage the strengths of both.
\end{tcolorbox}


\subsection{Resource reservation}
The IEEE 802.1Qat~\citep{IEEE802.1Qat-2010} defines admission control and resource reservation mechanisms for full-duplex switched Ethernet networks. In this standard, the so-called ``\textit{Stream Reservation Protocol (SRP)}'' is introduced to ensure that both latency and bandwidth requirements can be met for each flow before it is admitted to the network. To this end, three other protocols (all defined in the IEEE 802.1Qat standard) are coordinated and used, namely: ($1$)~the Multiple MAC Registration Protocol~(MMRP); ($2$)~the Multiple Stream Registration Protocol~(MSRP); and finally~($3$)~the Multiple VLAN registration Protocol~(MVRP)~\citep{IEEE802.1Qat-2010, IEEE802.1Q-2014, Nasrallah2018}. As for the actual implementation of the SRP scheme, both resource requests and reservation requests of each flow are forwarded through the MMRP, while its VLAN membership in the network is registered with the MVRP. The MSRP performs the actual resource reservation throughout the network by communicating with all nodes on the path of the flow in a distributed manner. In short, the QoS requirement of each data flow is satisfied by: ($1$)~announcing the data flow in the network; ($2$)~registering the data flow path; ($3$)~calculating its worst-case turnaround time; ($4$)~establishing a communication domain between nodes where the reservation is enforced; and finally ($5$)~reserving bandwidth for the data flow~\citep{Nasrallah2018} 

Since the Multiple Registration Protocol (MRP) is decentralized, the database of traffic information at each node grows with the number of traffic flows. As a result, the traffic information to be exchanged between nodes becomes very large. To overcome this limitation, the IEEE TSN working group has developed a new protocol called \textit{Link-Local Reservation Protocol} (LLRP)~\citep{IEEE802.1CS-2019}. Unlike the MRP, this approach operates in a centralized manner. Such an approach reduces the communication overheads in resource management, but the configuration node may become a single point of failure. Consequently, this further emphasizes that the trade-off between centralized and distributed approaches remains an open problem that requires further research efforts.

\subsection{Flow integrity}
The IEEE 802.1CB~\citep{Ieee2017802.1CB} standard defines a mechanism for transmitting multiple copies of a frame. This is to ensure that a frame can be delivered even if errors such as link failures, bitflips, or congestion losses occur on one of its paths. In the specification of this standard, if multiple copies of a frame arrive at a node (regardless of whether it is an intermediate node or the destination node), only one copy is received and all others are discarded. To achieve a high level of reliability, it is desirable that each copy of a replicated frame traverse its own path from the sender node to the receiver node. However, achieving this is not trivial. There are recent research efforts in this direction \citep{ojewale2019routing, Singh2017}. Moreover, some user applications, such as ``lock'' -- `` unlock'' commands, sensor inputs, etc., require frames to be delivered in a specific order when replicas are present. In addition to 802.1CB, the IEEE 802.1Qca~\citep{Ieee802.1Qca} standard allows the path of each data flow to be calculated in advance. In this process, calculating the best routes for each data flow is not trivial, and therefore there are research efforts that address the selection of routing paths for TSN data flows.  

\begin{tcolorbox}
    Finally, the IEEE 802.1Qci~\citep{IEEE802.1Qci-2017} standard allows data flows to be aggregated, processed, filtered, and queued based on their unique identifiers~\citep{Nasrallah2018}. This is very useful for security purposes, as unidentified flows can be easily discarded.
\end{tcolorbox} 

\subsection{Flow control}
\label{sec:background:features}
TSN flow control mechanisms determine how frames belonging to a particular traffic class are handled at the output ports of TSN-enabled switches. These mechanisms include: ($1$)~Time-Aware Shaper~(TAS); ($2$)~Credit-Based Shaper~(CBS); ($3$)~Cyclic Queue Forwarding~(CQF); ($4$)~Asynchronous Traffic Shaper~(ATS); and finally the ($5$)~Frame Preemption~(FP). We describe these mechanisms in detail below.

\subsubsection{Time-Aware Shaper (TAS)}
\label{sec:background:tas}
To ensure low delay and low jitter for time-sensitive traffic, the IEEE 802.1Qbv~\citep{IEEE802.1Qbv} standard defines a \textit{timed gate control mechanism}, also known as a \textit{Time-Aware Shaper (TAS)}. TAS prescribes
\textit{independent time windows} by opening and closing the gate associated with each queue of a switch output port. Here, each queue has a guaranteed transmission slot in a cyclic and precomputed dispatch schedule called \textit{Gate Control List~(GCL)}. A frame in a queue can only be transmitted if the gate of the queue is opened at the time specified in the GCL configuration. Specifically, TAS follows the TDMA (Time Division Multiple Access) paradigm, which means that the transmission time is divided into time slots or ``windows''. The time-sensitive frames are transmitted in the so-called ``scheduled traffic window'' or ``protected window'' and the non-scheduled traffic is transmitted in the ``common slots'', i.e., slots for which no time-sensitive frame is scheduled. Each scheduled traffic window is preceded by a so-called ``guard band"' to prevent unscheduled traffic with a lower priority from blocking the transmission of scheduled traffic. The guard band is a period of time between the gate-close operation of non-time-sensitive queues and the start of the scheduled traffic window. The length of the guard band corresponds to the time required to transmit the largest possible non-time-sensitive frame in the network. Figure~\ref{fig:qbv} shows an example of frame transmission with TAS.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.6]{feupphdteses/sections/background/images/qbv-transmission}
    \caption{Illustration of frame transmission using TAS.}
\label{fig:qbv}
\end{figure}

In this figure, we consider two flows ($f_1$ and $f_2$) for transmission. We assume that $f_1$ is a scheduled time-sensitive flow, whereas $f_2$ is not time-sensitive. The frames of $f_1$ are always transmitted in a ``scheduled traffic window'' and those of $f_2$ in a ``common slot''. As can be noted, the second frame of~$f_2$ (arriving at time $t = 7$) cannot start its transmission immediately, although it arrives in a ``common slot''. The reason for this is the guard band that protects the transmission of the second frame of $f_1$ from any disruption. We recall that the transmission of a frame cannot begin during the guard band.

Among the drawbacks of this mechanism, it should be noted that while the guard band ensures that the transmission of time-sensitive traffic is protected from blockings, it results in poor use of network bandwidth \footnote{This is because a frame whose transmission time is greater than the guard band cannot begin its transmission during this period. We note that smaller frames can still be transmitted during the guard band.}. To ensure fully deterministic transmission of time-sensitive traffic, the time intervals for each flow along the path must be aligned. This alignment can only be achieved if all nodes have the same notion of time, i.e., if their clocks are synchronized. This synchronization mechanism was described in Section~\ref{sec:background:syncronisation}. In addition, the GCLs must be provided, the synthesis of which is also a very computationally intensive task. 
\begin{tcolorbox}
    The precomputed GCL is a very rigid approach that is unsuitable for dynamic changes in the network and traffic.
\end{tcolorbox}


%Another approach is to update the pre-computed GCLs. For both approaches, a centralized network configuration model is required \citep{Pruski2021Implementation}. Such a model is needed since the global view of the network is required for the GCLs synthesis.


\subsubsection{Credit-Based Shaper (CBS)}
\label{sec:background:cbs}
To provide bounded end-to-end delays, moderate the transmission bandwidth of AVB traffic classes, and protect the entire network from burst effects, the AVB Task Group introduces the \textit{Credit-Based Shaper (CBS)} -- specified in IEEE 802.1Qav~\citep{IEEE802.1Qav}. The purpose of this transmission scheme is to guarantee each of the so-called ``Stream Reservation (SR)'' classes an appropriate share of the link bandwidth, as mentioned in Section~\ref{sec:background:avb}. Unlike Strict Priority, CBS prevents the flows of high-priority classes from starving out those of lower-priority classes. For this purpose, a parameter \textit{credit} is defined for each class to regulate the frame transmission for each SR class at the output queues. The selection for head-of-queue frame transmission of an SR class is conditioned by the following: ($1$)~the value of the credit for the class is at least zero; and ($2$)~there are no other higher priority frames available for transmission~\citep{ZhaoLin2018AVB}. The variation of the credit is affected by ($i$)~the configuration parameter \textit{Sending Slope} (\emph{sendSlope}), which specifies the rate at which the credit is consumed; and ($ii$)~the parameter \textit{Idle Slope} (\textit{idleSlope}), which specifies the rate at which the credit is replenished. As defined in IEEE 802.1Qav~\citep{IEEE802.1Qav}, the idleSlope is a user-defined parameter that represents a fraction of the link speed, and the sendSlope is calculated as the difference between the link speed and the idleSlope. The credit of an SR class is reduced by the \textit{sendSlope} when a frame of the class is transmitted. This credit can be replenished in two scenarios: ($i$)~when a frame from the class is waiting to be transmitted and another interfering frame from another class is transmitted; and ($ii$)~when no frame from the class is in the queue. Non-real-time flows (i.e., best-effort flows) are transmitted when there is no waiting traffic from these classes or when the credits of both classes are negative. As already mentioned in Section~\ref{sec:background:avb}, CBS can only guarantee a latency limit of $2$~ms or less over $7$~hops. We recall that some emerging automotive applications require as low as $500\mu$s -- $1$ms over several hops~\citep{IEEE802.1DG-2021}. Figure~\ref{fig:cbs} shows an example of the CBS transmission process.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.8]{feupphdteses/sections/background/images/cbs-transmission}
    \caption{Illustration of frame transmission using CBS.}
\label{fig:cbs}
\end{figure}

In this figure, three flows ($f_1$, $f_2$, and $f_3$) are considered for transmission. We assume that $f_1$ and $f_2$ belong to Classes A, and B, respectively, and $f_3$ is a best efforts flow. The first frames of $f_1$ and $f_2$ arrive shortly after the first frame of $f_3$ start its transmission. Then the class credits of $f_1$ and $f_2$ which were initialized to $0$, start to increase according to their idleSlopes. As soon as the first frame $f_3$ completes its transmission, the first frame of $f_1$ starts its transmission and its class credit starts decreasing according to its sendSlope. Meanwhile, the class credit for $f_2$ continues to increase until the complete transmission of $f_1$, when its first frame begins transmission. During the transmission of the first frame of $f_2$, the class credit for $f_1$ starts increasing again until its second frame starts its transmission. 


An extension of CBS is the \textit{burst limiting shaper} (BLS)~\citep{Thiele2016BLS}. This shaper functions similarly to the CBS, but allows high-priority traffic to make a limited number of excess transmissions in the event of temporary congestion (burst).


%Under CBS, each AVB traffic class is assigned a transmission budget or ``credit'' to control its transmission rate. The transmission of a frame belonging to an AVB class then depends on the availability of the transmission credit of that class. The credit assigned to each class at design time is consumed as its frames are transferred. Once the credit is depleted, no new frames of the class can be transferred until the credit is replenished. This provides a window of opportunity to transfer frames that belong to other traffic classes. The replenishment of each budget is determined by the user depending on the desired QoS. 

\subsubsection{Cyclic Queue Forwarding (CQF)}
\label{sec:background:cqf}
The IEEE introduced the \textit{Cyclic Queue Forwarding (CQF)}~\citep{IEEE802.1Qci-2017}, which organizes the reception and transmission of frames at each node by following well-defined cyclic time intervals. Each time slot is divided into \textit{even} and \textit{odd} intervals. All frames received within one interval are not transmitted until the next interval. Here, any time-sensitive frame received in an even or odd cycle is scheduled for transmission at the next switch in the following cycle. The maximum delay for a time-sensitive frame cannot exceed two cycle times per hop. This makes the network very predictable, since the delay of a frame depends solely on the cycle time and the number of hops. Figure~\ref{fig:cqf} illustrates the frame transmission process with CQF.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.67]{feupphdteses/sections/background/images/cqf-transmission}
    \caption{Illustration of frame transmission using CQF}
\label{fig:cqf}
\end{figure}

In this figure, a time-sensitive frame $f_1$ arrives after a best-effort frame $f_2$ in the odd interval, but $f_1$ has been prioritized for transmission in the subsequent even interval. To ensure that the CQF behaves as desired, it is important that the scheduled cycle times for all frames are respected. This means that all transmitted frames must be received by the downstream switch during the expected cycle.
\begin{tcolorbox}
    Under CQF, careful consideration must be given to cycle times, the alignment of cycle times between switches in the network, and timing of first and last transmissions within a cycle must be carefully considered to meet timing requirements. 
\end{tcolorbox}

\subsubsection{Asynchronous Traffic Shaper (ATS)}
\label{sec:background:ats}
In addition to the TAS, CBS, and CQF transmission schemes, TSN also introduces \textit{Asynchronous Traffic Shaping}~(ATS)~\citep{Specht2016Urgency, IEEE802.1Qcr-2019} as a traffic control feature. ATS is intended to circumvent the need for a synchronized clock across the network, as is the case with TAS. It uses a queuing and buffering approach to control the flows. It achieves deterministic data transmission in two steps: ($1$)~ carefully queuing incoming frames to achieve frame isolation and prevent so-called ''\textit{head of line blocking}''; and ($2$)~dequeueing frames for transmission at a controlled rate to ensure that each flow has a fair chance of being transmitted without being discarded or delayed.

\begin{tcolorbox}
  ATS is based on an event-driven model, and transmission decisions are made at each node.
\end{tcolorbox}

\subsubsection{Frame Preemption}
Frame preemption was defined and introduced in the IEEE~802.3br~\citep{IEEE802.3br-2016} and IEEE~802.1Qbu standards~\citep{IEEE802.1Qbu}. These specify a $1$-level preemption scheme for Ethernet frames. We have already described the mechanism of this transmission scheme in detail in Section~\ref{sec::introduction:motivation}. Here, we briefly summarize this discussion. 

Briefly, two Medium Access Control (MAC) sublayer service interfaces are defined in the link layer: a ``preemptable MAC ~(pMAC) interface'' and an ``express MAC ~(eMAC) interface''. Frames assigned to the eMAC and pMAC service interfaces are referred to as ``\textit{express}'' and ``\textit{preemptable}''  frames, respectively. Each eMAC frame has a higher priority than any pMAC frame and can therefore preempt any of these frames to speed up its own transmission. Finally, frames of the same preemption class cannot preempt each other. The standards~\citep{IEEE802.1Qbu, IEEE802.3br-2016} describe not only the preemption operations, but also the hardware changes required at the switches to support the preemption, which occurs at the network MAC merge sublayer between the physical and MAC layers (see Figure~\ref{Image6}).

\begin{figure}[htb]
\centering
\includegraphics[scale=0.8]{feupphdteses/sections/feasibility/images/Image6}
\caption{The MAC merge sublayer managing service interfaces.}
\label{Image6}
\end{figure}

Frames on this sublayer are called Mframes~\citep{IEEE802.1Qbu}. Before each Mframe transmission, the sublayer checks whether the next switch/node supports preemption by performing a verification operation described in the standards~\citep{IEEE802.3br-2016}. Preemption is not enabled in the sender node until the verification operation confirms that it is supported by the receiver node. If it is, additional information describing the preemption properties is added to the Mframe headers. The sublayer is able to interrupt an interruptible Mframe that is being transmitted and can also prevent a new Mframe from starting transmission \citep{IEEE802.3br-2016}.

Among the advantages of frame preemption over the previously mentioned flow control mechanisms is that it allows more efficient use of available bandwidth, since the transmission of preemptable frames cannot compromise the timing requirements of express frames, and this is guaranteed without the use of a guard band.
\begin{tcolorbox}
  Frame Preemption is easy to configure and is particularly suitable for applications where time synchronization is not required (nor applicable), especially for use-cases that require dynamic behavior and/or unsynchronized endpoints, as is common with DRES.
\end{tcolorbox}


% Figure \ref{fig:outputport} shows the schematic diagram of a TSN output port with the flow control mechanisms mentioned above.
% \begin{figure}
%     %\includegraphics[scale=0.6]{feupphdteses/sections/background/images/tsnoutputport-2.PNG}
%     \includegraphics[scale=0.7]{feupphdteses/sections/background/images/tsnoutputport.pdf}
%     \caption {Schematic diagram of TSN frame forwarding at the egress port with flow control mechanisms.} 
%     \label{fig:outputport}
% \end{figure}

% In this figure, the gate control list for the TAS is shown in the table with entries $T_0, T_1,\ldots,T_N$. Each entry $T_i$ consists of a sequence of zeros and ones representing the gate event on the port's output queues (Q1, $\ldots$, Q8). An ``o'' indicates that the associated gate is open for transmission, while a ``c'' indicates that it is closed. For example, the first row in the table indicates that at time $T_0$ the port of Q1 is open for transmission and all others are closed. Similarly, at time $T_1$, the gate of Q1 is closed for transmission and the gates of all other queues (Q2 to Q8) are open. The last entry in the table states that the TAS schedule described in the table repeats cyclically. A frame in a queue can only be transmitted if its gate is open during the corresponding time period. Note that each queue contains a unique class of frames, i.e. frames belonging to different traffic classes cannot share the same queue. For AVB traffic classes (AVB1 and AVB2), the CBS is connected to the output port as described before to control the transmission of this traffic. The output port selects the frame to be transmitted based on the defined transmission selection algorithm (e.g., Strict Priority (ST) or Round-Robin (RR)). Finally, a flow that is already being transmitted can be interrupted by the so-called ``frame preemption'' function, which we discuss in the next section.

\section{A closer look at TSN frame preemption}
\label{sec:background:preemption}
In this section, we discuss the frame preemption feature in detail from four perspectives:~($1$)~the definition of the frame format that enables the preemption operations; ($2$)~the preemptive transmit process as defined in the standards; ($3$)~the preemptive receive process as defined in the standards; and finally~($4$)~the preemption overhead.

\subsection{Frame format specification}
It is important to preserve the Ethernet frame format when Mframes are preempted. To this end, the IEEE 802.3br standard defines Mframe formats in a preemption-enabled environment (see Figure~\ref{Image7a}). 
\begin{figure}[ht]
\centering
\includegraphics[scale=0.8, width=\columnwidth]{feupphdteses/sections/background/images/Image7-a}
\caption{Frame formats as specified in IEEE 802.3 Standards where the numbers are in bytes and represent the size of each field.}
\label{Image7a}
\end{figure}

As can be seen from this figure, the structure of an express frame (see~Figure~\ref{Image7a}b) differs from that of the corresponding standard Ethernet frame (see~Figure~\ref{Image7a}a) only by~one octet, called a ``\textit{Start Frame Delimiter}'' (SFD). This octet is replaced in the frame format by the ``\textit{Start Mframe Delimiter-Express}''~(SMD-E). In practice, however, SFD and SMD-E have the same value. Similarly, a preemptable frame that has not been preempted (see~Figure~\ref{Image7a}c) differs from a standard Ethernet frame only by a single octet, here the SFD is replaced by the ``\textit{Start Mframe Delimiter Start Fragment}'' (SMD-Sx). Now, assuming a frame that has been preempted, it is worth noticing that the first fragment remains almost the same as the original frame as shown in Figure~\ref{Image7b}. 

\begin{figure}
\centering
\includegraphics[scale=0.9, width=\columnwidth]{feupphdteses/sections/background/images/Image7-b}
\caption{Frame fragments formats as specified in IEEE 802.3br Standard where the numbers are in bytes and represent the size of each field.}
\label{Image7b}
\end{figure}

There are only two differences: ($1$)~the \textit{size}, which is smaller (because the original frame has been split into fragments); and ($2$)~the \textit{error checking code}~(FCS), which is replaced by a newly generated Mframe error checking code (MCRC) (see Figure~\ref{Image7b}b). All other fragment(s) consist of a frame header containing three components: ($i$)~a preamble; ($ii$)~a ''Start Mframe Delimiter for Continuation fragment'' (SMD-Cx); and ($iii$)~a so-called ``Frag Count'', which is used to monitor the correct order of incoming fragments and to detect missing fragments (see Figure~\ref{Image7b}c). All fragments are appended with the same MCRC, except for the last fragment, which ends with the FCS of the original preempted frame (see Figure~\ref{Image7b}d).

\subsection{Preemptive frame transmission}
The \textit{Transmit Processing} function is responsible for frame transmission at the MAC sublayer interface. The process begins with a verification procedure that checks whether the receiver node supports preemption. To do this, it sends a ``request frame'' to the receiver node to inquire whether it supports preemption. In return, the receiver node sends a response to confirm that it does or does not support preemption. This information is interpreted by the forwarding node based on the SMD value of the response frame. Transmission of a frame with preemption begins only after it is confirmed that both the sender and receiver nodes support preemption. Figure~\ref{std:frame-transmission} shows the detailed \textit{Transmit Processing} state diagram as defined in the IEEE 802.3br Standard. All labels, functions, and variables are as defined in~\cite{IEEE802.3br-2016}. The transmit process is triggered when a frame reaches the $\operatorname{INIT\_TX\_PROC}$ state.

\begin{figure}
\centering
\includegraphics[scale=0.9, width=\columnwidth]{feupphdteses/sections/background/images/transmit_process}
\caption{Preemptive frame transmission process as specified in IEEE 802.3br Standard.}
\label{std:frame-transmission}
\end{figure}

\subsubsection{On the transmission of express frames}
When an express frame reaches the Transmit Processing function, i.e., at $\operatorname{IDLE\_TX\_}$ $\operatorname{PROC}$, it is identified as ``express'' and then transits to the $\operatorname{EXPRESS\_TX }$ state, which is responsible for non-preemptive transmission. Upon completion, the function transitions to the $\operatorname{E\_TX\_COMPLETE}$ state, where it either returns to the idle state ($\operatorname{IDLE\_TX\_PROC }$) or resumes transmission of a pending preempted frame.

\subsubsection{On the transmission of preemptable frames} 
In contrast to the express frames transmission process, when a preemptable frame reaches the $\operatorname{IDLE\_TX\_PROC }$ state, the Transmit Processing function first checks whether the receiver node has preemption capabilities, and then returns to the $\operatorname{IDLE\_TX\_}$ $\operatorname{PROC}$ state (see connector ``C''). The function transitions to the $\operatorname{START\_PREAMBLE}$ state if the response is positive, which triggers the transmission in a preemptable manner. Note that the transmission can only be interrupted if an express frame arrives and the preemptable transmission has reached a feasible interrupt point. If a preemption occurs, an MCRC value is computed for the preemptable frame fragment ($\operatorname{TX\_MCRC}$) and the function transits to a waiting state ($\operatorname{RESUME\_WAIT}$). All pending express frames are then transmitted (see connector ``B'') and transmission of the preemptable resumes only after that. After the transfer is complete, or if preemption did not occur during the frame transmission, the function returns to the $\operatorname{IDLE\_TX\_PROC}$ state. For more detailed information about each state, see pages 48 to 52 of the IEEE 802.3br standard~(see~\citep{IEEE802.3br-2016}).

\subsection{Preemptive frame reception}
At the receiver node, a Medium Independent Interface (xMII) checks the SMD for each frame upon arrival, and the value of the SMD indicates whether the frame is an express or a preemptable frame~\citep{IEEE802.1Q-2014}. Express frames (i.e., frames containing SMD-E) are processed by an Express Filter, while preemptable frames are processed by a ``Receive processing'' construct. This specific Receive processing is responsible for ensuring that all fragments of a preempted frame are received completely and in the correct order. For this purpose, both the ``MCRC'' and the ``Frag Count'' values of each fragment are used. The frame transmission of any preempted frame is guaranteed to be complete because all fragments have the same MCRC value, but the last fragment embeds the FCS of the original frame. This means that the reception of a sequence of fragments belonging to a preempted frame is complete as soon as two consecutive fragments have a different error checking code at the receiver node. Figure~\ref{std:frame-reception} illustrates the \textit{Receive Processing} state diagram as defined in the IEEE 802.3br Standard (see~\citep{IEEE802.3br-2016}, pg. 51). Again, all labels, functions, and variables are defined as in~\citep{IEEE802.3br-2016} (see pgs. 45-48) and the reception process is triggered when a frame reaches $\operatorname{CHECK\_FOR\_START}$ state.

\subsubsection{On the reception of express frames}
When an express frame reaches the Receive Processing function, i.e., at the $\operatorname{CHECK\_FO}$ $\operatorname{R\_START}$ state, it is identified as ``express'' and then transits to the $\operatorname{EXPRESS}$ state, which is responsible for receiving it in a non-preemptive manner. Upon completion, the function transits to the $\operatorname{IDLE\_RX\_PROC}$ state.

\subsubsection{On the reception of preemptable frames}
Unlike the express frame reception process, the Receive Processing function enters the $\operatorname{CHECK\_FOR\_START}$ state when a preemptable frame reaches the $\operatorname{REPLACE\_SFD}$ state, in which the frame's SFD is replaced with a recomputed SMD value. After that, the function transitions to the $\operatorname{P\_RECEIVE\_DATA}$ state, which triggers reception in a preemptable manner. Note that this reception can only be interrupted if an express frame arrives and the preemptable transmission has reached a feasible preemption point. If a preemption occurs, reception is suspended and the function enters the $\operatorname{P\_WAIT\_FOR\_DV}$ $\operatorname{\_FALSE}$ state where it receives the preempting express frame(s). After these frames are fully received, the function transitions to the $\operatorname{P\_WAIT\_FOR}$ $\operatorname{\_RESUME}$ state, where it resumes receiving the preempted frame. Upon completion or if there was no preemption during frame reception, the function transitions back to the $\operatorname{IDLE\_RX\_PROC}$.

\begin{figure}
\centering
\includegraphics[scale=0.9, width=\columnwidth]{feupphdteses/sections/background/images/recieve_process}
\caption{Preemptive frame reception process as specified in IEEE 802.3 Standards.}
\label{std:frame-reception}
\end{figure}
\subsection{Preemption overhead}
The standards, in their current specifications, do not allow preemption to add any form of \textit{padding} to a fragment of a preempted frame. That is, the data portion of a fragment may not be augmented to meet the minimum Ethernet frame size requirement, which is $84$ bytes. To ensure this, the standards command that a preemptable frame must not be preempted until the following two conditions are met: ($1$)~the size of the fragment being transmitted is at least $84$ bytes; and ($2$)~the remaining fragment resulting from the occurrence of a preemption operation also meets the minimum frame size. Considering these two requirements, the longest non-preemptable Ethernet frame fragment is $143$~bytes long (see~\cite{Thiele2016Formal}, Lemma~$1$ for a detailed proof). This means that each express frame can be blocked for at most as long as it takes to transmit $143$~bytes of data on the link. This corresponds to blocking of $1.14\mu s$ and $11.44\mu s$, assuming an Ethernet with $1 Gb$ and $100 Mb$ speed, respectively. Recall that without preemption, the blockings were $12\mu s$ and $120\mu s$, assuming a $1 Gb$ and $100 Mb$ speed Ethernet, respectively. Roughly speaking, this translates to a reduction of $90.5 \%$, when preemption is enabled. On the other hand, the total overhead incurred by the occurrence of each preemption is $12$ bytes (i.e., $6$- byte preamble, $1$- byte SMD-Cx, $1$- byte Frag Count; and finally $4$- byte MCRC). In addition, the \textit{Inter Frame Gap} (IFG) between two consecutive transmissions must be accounted for before the next frame/fragment is transmitted. According to the standards, the size of each IFG is equal to the amount needed to transmit $12$ bytes of data. Thus, the total overhead associated with the occurrence of each preemption is $24$ bytes (i.e., $0.19 \mu s$ and $1.9 \mu s$, assuming Ethernet speeds of $1 Gb$ and $100 Mb$, respectively).

\subsection{Limitations of frame preemption}
As discussed in Section~\ref{sec::introduction:motivation}, a very noticeable limitation in the standards is the lack of configuration definitions that guarantee optimal/efficient performance in terms of frame responsiveness. Eight CoS classes are defined in the specification of Ethernet frames, but it is not clear which of them should be mapped to eMAC or pMAC frames in the TSN specification. It also follows from the discussion conducted in Section~\ref{sec:introduction:context} on the $1$-level preemption scheme that this scheme significantly improves the responsiveness of eMAC frames.~\cite{Thiele2016Formal} has experimentally shown that the $1$-level frame preemption scheme improves the performance of express frames. However, the performance of these frames is negatively affected when their number increases~\citep{bello2019perspective}. This tendency is due to the fact that frames of the same class are transmitted in a non-preemptive manner. As a result, frames may have stringent timing requirements but cannot be classified as express to preserve performance. Indeed, real-time traffic in embedded systems may have different timing requirements that do not fit into just one (express) preemption class~\citep{Gogolev2020Simpler}. In order not to jeopardize the schedulability of these frames, and subsequently the schedulability of the whole system, these frames should not be blocked for excessively long periods of time. The $1$-level preemption operation in the current version of the standards does not allow preemptable frames with stringent timing requirements to take advantage of the basic benefits of preemption.

In this dissertation, we proffer solutions to these shortcomings of the $1$-level preemption scheme by exploring and promoting the implementation of a \textit{multi-level preemption} scheme. With this new paradigm, all frames with stringent or firm timing requirements will get a significant improvement in their performance in terms of responsiveness. This, in turn, allows us to improve the QoS of the entire system and increase the workload that can be accommodated in a single communication network. On the other side of the realization of a multi-level preemption scheme, however, are a number of very difficult scientific problems. First, the feasibility of a multi-level preemption viz-a-viz the specification of the standards needs to be investigated. If it is found that a multi-level preemption scheme is feasible, a framework to model, analyze, optimize, and predict the temporal characteristics of such a scheme must be developed. Finally, the performance gains that the scheme brings must be measured and quantified. Our contributions, which we will present in the following chapters of this dissertation, address the above challenges. Before proceeding with the presentation of these contributions, we present related work in TSN frame preemption research in the next section.

%In this work, we focus on this class of frames, i.e., -- preemptable frames with firm timing constraints.

\section{Related Work}
\label{sec:background:related_work}
\input{feupphdteses/sections/background/related_work}

\section*{Chapter Summary}
\label{sec:background:summary}

In this chapter, we have given a detailed overview of real-time communication and the evolution of communication technologies. We introduced Ethernet and explained how various Ethernet-based technologies have been developed for real-time communications. Then we introduced TSN, the latest set of IEEE standards that add more real-time capabilities to Ethernet technologies. We then focused on a prominent TSN feature - Frame Preemption - and described its specifications in the standards. In particular, we examined the transmit and receive functions as they are currently defined in the standards and highlighted the limitations of the current specifications. Finally, we have looked at related research on frame preemption. 
\begin{tcolorbox}
    Now that all related concepts and technologies have been introduced, we will present the contributions of this dissertation in the following chapters.
\end{tcolorbox}


% \subsection{Network-wide Control and Management}
% \label{subsec:network-management}

% The performance that can be achieved with the TSN features discussed above depends strongly on how well the network is configured. In this section, we briefly discuss the network configuration and management mechanism
% used in TSN.

% \subsubsection{Initial Approach}

% Traditionally, in AVB, the network control was distributed. This means that the activities of the control plane, as required for CBS, were done locally by each switch. The Stream Reservation Protocol (SRP), specified in IEEE 802.1Qat~\citep{IEEE802.1Qat-2010}, deals with traffic advertisement and resource reservation on an end-to-end basis. 

% Briefly, the reservation procedure is as follows. When a switch receives for the first time the \emph{stream advertisement message}, it checks the available resources of each port. If there are ports that have available resources, the stream advertisement message is marked accordingly and forwarded. A port has available resources for a stream if (a) there is available bandwidth and (b) it is estimated that, by traversing this switch, the stream still meets its deadline. Bandwidth availability is rather intuitive, while the deadline check is more complex -- involving the estimation of the delay to reach and traverse this switch. This estimation uses the already allocated bandwidth and the idle slope.
% After a while, the switch receives the advertisement message back. This time it contains additional
% information returned by the end-stations interested in receiving the stream. Then the switch decides whether
% to accept and forward the stream.

% \subsubsection{TSN Novel Approach}

% With the improvements proposed through TSN features, some configurations should be synchronized across the network and the distributed configuration model is no longer enough. For example, with the original SRP, a switch was only allowed to decide whether to forward a stream or not, but there were no mechanisms to align the idle slopes across the network. Therefore, the IEEE 802.1Qcc~\citep{IEEE802QCC} amendment proposes enhancements for the SRP. One of the most important contributions of this amendment is the introduction of three network configuration models, namely, fully distributed, centralized network/ distributed user, and fully centralized models. For the fully distributed model, the reservation requests are carried out by User Network Information (UNI) messages. According to the specification \citep{IEEE802QCC}, the TSN features, such as frame preemption and TAS, can be configured only with the centralized network configuration models. 

% The centralized network/ distributed user model introduces the concept of Centralized Network Configuration (CNC). Here, end systems send UNI to the edge switches --- the switches that are directly connected to the end systems. The edge switches forward these UNIs to the CNC. Furthermore, CNC, using remote management, discovers network topology and switch capacities. Based on this general view of the network, the CNC  decides the resource allocation for each flow. Finally, the CNC, using again the remote management, conveys the updated resource allocation to the switches. 

% Finally, the fully centralized configuration model introduces the concept of Central User Configuration (CUC). There are application domains, such as automotive or industrial automation, where data production or consumption has to be synchronized with data transmission. For such cases,   the CUC is used for discovering the end systems and their traffic demands and capacities. Based on this, CUC generates the UNIs and sends them to the CNC. CNC determines now the configuration for switches and end systems and conveys the updated configuration to switches. Moreover, the CNC sends back to the CUC the configuration for end systems. Furthermore, it is the job of CUC to convey the configurations to the end systems.

%\section{Real-time systems}
% microprocessor technology is the engine room of the recent rise of digital technology. Nowadays, microprocessors are present in everyday gadgets ranging from mobile phones to home appliances, cars, manufacturing systems, and aircraft. Such devices/systems incorporating microprocessors to provide computation and control functions are often referred to as \textit{Embedded Systems}. A subset of embedded systems that must promptly react to state changes in the environment caused by human behavior, natural or artificial phenomenon, is referred to as \textit{real-time embedded systems} or simply as \textit{real-time systems}. In real-time systems, the timing requirements are the cardinal constraints~\cite{cottet2002scheduling}. Depending on the type of timing constraints, real-time systems are categorized as either \textit{Hard} of \textit{Soft}~\cite{Buttazzo2011}. For hard real-time systems, not satisfying timing constraints can lead to catastrophic consequences like personal injury, and loss of life or property. Conversely,  not satisfying timing constraints does not lead to serious consequences in soft real-time systems. 

==> sections/background/related_work.tex <==
Several works have studied the TSN frame preemption feature from different perspectives.  In the following subsections, we have grouped the discussion of related work with respect to the challenges that we address in this thesis. 

\subsection{Feasibility and implementation cost comparison}
\label{sec:related_work:feasibility}
\cite{kim2013preemptive} showed that preemptive switched Ethernet offers better performance than the standard IEEE 802.1Q/p protocol in terms of end-to-end transmission delays. This is especially true when real-time and non-real-time frames are transmitted over the same network.~\cite{Thiele2016Formal} also showed, still by simulation, that the end-to-end delays of express frames under preemptive Ethernet are very close to those of TAS, suggesting standard preemptive Ethernet as a promising alternative to TAS in scenarios where long CAM frames are not making use of the express class.

As for the hardware implementation, ~\cite{zhou2017analysis}
presented a \textit{VHSIC Hardware Description Language} (VHDL) design layout for the transmit and receive processes, as well as an FPGA-based hardware implementation of TSN sender and receiver nodes. By using a \textit{Field-Programmable Gate Array} (FPGA) based implementation,~\cite{hotta2015experimental} also provided a quantitative evaluation of the performance improvement associated with the preemption phase was also performed. The measurement results show that the maximum latency of express frames was significantly reduced (from $27.57 \mu s$ to $2.46 \mu s$ @$1$Gb/s). Other authors such as~\cite{Jia2013performance, simon2017ethernet} have also pointed out some challenges that could arise from preemption operations, such as starvation of low priority frames and buffer overflow (when there are more fragments of preempted frames to store than the buffer size of the switches/nodes). However, these authors have neither highlighted nor solved the problem of multi-level preemption.

There is a plethora of research comparing TSN traffic control approaches from a performance perspective. In this context, \cite{thangamuthu2015analysis} compares the performance of three TSN shapers, namely TAS, Burst Limiting Shaper and the Peristaltic Shaper (PS). In their work, the comparison metrics are delay and jitter. The authors conclude that TAS offers the best performance on both metrics. A similar work by~\cite{Thiele2015Peristaltic} compares TAS with PS and comes to a similar conclusion, i.e., TAS provides better end-to-end delay performance. However, they found that the performance of TAS deteriorates significantly when the end systems are not synchronized. 

Another work comparing TAS and frame preemption, by~\cite{Gogolev2020Simpler}, has shown through experiments that frame preemption is better for industrial networks with unsynchronized end systems. The authors point out that a serious limitation for frame preemption is the low Quality of Service (QoS) resolution, i.e., there are only two classes (eMAC and pMAC) specified for preemption in TSN. On another front, a work by~\cite{Nasrallah2019Performance} does a performance comparison between TAS and Asynchronous Traffic Shaping (ATS). The authors conclude that ATS compares favorably with TAS for sporadic (asynchronous) traffic. However, they find that the performance of Scheduled Traffic degrades under ATS as the best-efforts load increases. We note that none of the above work has compared these features from an implementation cost perspective.

%To mitigate the aforementioned limitation,~\cite{Ojewale2020Feasibility, Ojewale2021WorstCase} introduce the multi-level preemption paradigm. Here, the authors also compare TAS and frame preemption from a qualitative standpoint and promote the multi-level frame preemption feature as a viable alternative to TAS. Furthermore, ~\cite{knezic2020implementation} provided an enhanced implementation approach for the multi-level preemption feature, and the formal worst-case traversal time analysis of this approach was provided by~\cite{Ojewale2021WorstCase}.

However, there is not such a strong interest in comparing the performance of CBS with other shapers. There are works by~\cite{alderisi_etfa2013} and~\cite{lo-bello_etfa2014} that present simulation results for AVB-ST (Scheduled Traffic) in industrial automation and automotive applications, respectively. AVB-ST is a more rigorous approach than TAS, assuming that the scheduled traffic is strictly periodic and that precise offsets are provided for the scheduled frames. In these works, the baseline is considered to be pure CBS and the authors note that only by using AVB-ST is it possible to guarantee bounded delay and zero jitter for the scheduled traffic. A similar work by~\cite{meyer_etfa2013} highlights the importance of the quality of schedule tables. For example, with a non-dense table, the delay of AVB traffic increases but is still bounded and complies with the specification in~\cite{IEEE802.1BA}. When a compact schedule table is used, the delays of AVB traffic are still bounded, but no longer conform to the specification.

\subsection{Model and analysis}
\label{sec:related_work:analysis}
Most of the work in the literature on frame preemption in Ethernet have focused on the impact of preemption on end-to-end frame transmission delay. Simulations are usually used for this purpose (see, for example~\cite{Jia2013performance, kim2013preemptive, Thiele2016Formal, zhou2017analysis} for more details ). Most authors relying on this methodology acknowledge the effectiveness of frame preemption in Ethernet and have concluded that it allows system designers to drastically reduce the transmission delays of express frames while not significantly degrading the performance of preemptable frames. However, it is well known in the research community that simulation is neither a comprehensive nor a rigorous means of evaluating the performance of a system. This is because it does not guarantee that the case that causes the worst-case scenario will occur. Consequently, despite the extensive quantitative performance results obtained with this technique, more sophisticated approaches are needed to provide guarantees on the end-to-end delays of Ethernet frames. Network Calculus~(NC)~\citep{reimann2013timing}; Trajectory Approach~(TA)~\citep{Tracjectory2006Martin}; and Compositional Performance Analysis~(CPA)~\citep{henia2005system} have all been used as established techniques to provide timing guarantees for real-time Ethernet flows. %In this section, we report only the most significant contributions related to our topic. 

In NC, the so-called \textit{arrival curve} and \textit{service curve} are used to model the arrival of flows and the transmission bandwidth at a switch output port, respectively. To our knowledge, there are only a handful of papers in the TSN-related literature that use this approach. \cite{zhao2018worst} provided a worst-case latency analysis for IEEE ~802.1Qbv networks. For this purpose, they assumed that the Gate Control List~(GCL) and priority assignment configurations are given. They validated the performance of their approach against synthetic and real-world use cases in terms of scalability and the impact of GCL overlap features on individual flows. In another work, the authors also performed latency analysis for AVB traffic in TSN with NC~\citep{zhao2020latency}. However, their analyzes are only for non-preemptive TSN networks and leave the preemptive case unanswered.

In TA~\cite{Tracjectory2006Martin} examined the highest number of frames sharing the same trajectory, as this is a potential source of delay for each of these flows. The approach adopted proceeds ``backwards'', i.e., from the receiver node to the source node. In another context, this approach was used by~\cite{bauer2012trajectory} for timing analysis of AFDX with strict priority, non-preemptive flows transmitted according to a FIFO scheduling strategy. In the work,~ TA was further improved by investigating the basic idea that flows using a common link cannot arrive at a switch at the same time.~\cite{li2014trajectory} have proved the result to be optimistic and corrected the flaw. Nevertheless, the analysis still considers only non-preemptive frame transmission.

\cite{cao2016EligibleInterval, cao2016independent} introduced a so-called \textit{eligibility interval} approach for timing analysis of Ethernet Audio Video Bridges~(AVB)~\citep{IEEE2011AVB} Networks with Credit-Based Shapers~(CBS). This approach examines the worst-case performance of a flow when a flow has some pending payload to transmit and has a non-negative transmission credit. This approach has been shown to be tight for AVB networks and has subsequently been extended for timing guarantees of AVB flows in standard TSN~\citep{maxim2017delay}. Thangamuthu et al.~\cite{thangamuthu2015analysis} proposed a worst-case performance analysis for Switched Ethernet with Burst-Limiting Shaper~(BLS); Peristaltic Shaper~(PS); and Time-Aware Shaper~(TAS) for TSN, but concluded that only the TAS can schedule control traffic within the maximum delay imposed by the Standards.

CPA has been used extensively for the timing behavior of Ethernet flows~\citep{thiele2015improving, thiele2014improving}. It uses the so-called \textit{level-$i$ busy period} approach, activated by the so-called critical instant, to study the worst-case response time of each real-time flow~\citep{handbook2017cpa}. CPA was used for the timing behavior of Switched Ethernet in~\citep{Rox2010} and for Ethernet AVB in~\citep{Diemer2012}. The analysis for Switched Ethernet was improved by~\cite{thiele2014improving} to tighten the worst-case response time bounds of each flow by up to $80\%$, then the same authors exploited the FIFO nature of Switched Ethernet transmission~\citep{thiele2015improving} to reduce interference estimates in frame transmissions and achieved a latency improvement of about $30\%$ over the then-current state-of-the-art in CPA. Nevertheless, ~\cite{Thiele2015Peristaltic} and~\cite{Thiele2016BLS} proposed worst-case analysis for TSN using CPA with PS and BLS, respectively. Both contributions focused only on shapers, leaving frame preemption concerns beyond the scope of their work. On another front,~\cite{Thiele2016Formal} used CPA to provide worst-case guarantees for both Standard Ethernet and IEEE 802.1Qbv when frame preemption is enabled. Lo Bello et al. also provide a schedulability analysis for IEEE 802.1Qbv networks with preemption support~\citep{bello2020schedulability}. In these works, the authors only address the traditional $1$-level preemption scheme as defined in the standards.

Recently, \cite{knezic2020implementation} investigated the multi-level preemption from an implementation standpoint. However, their work falls short of providing a formal analysis of the worst-case performance guarantees. In this work, we fill this gap by providing a worst-case analysis of the traversal time of TSN frames under the multi-level preemption scheme, which to our knowledge is the first contribution in this direction.

\subsection{Network configuration} 
\label{sec:related_work:config}
An appropriate priority assignment policy plays a central role in the resulting performance of real-time systems~\citep{Davis2016Review}. For example, in CAN, the maximum reliable utilization was initially thought to be $35\%$ because message IDs (corresponding to message priorities) were assigned randomly or ad hoc~\citep{buttle2012real}.~\cite{Davis2016Review} later showed that Audley's Optimal Priority Assignment (AOPA) algorithm~\cite{audsley2001priority} can achieve reliable CAN utilization of over $80\%$. AOPA has become the reference scheme for priority assignment in many real-time systems and has been shown to be optimal when there are no priority inversions~\citep{Park2019Optimal}. ~\cite{davis2009robust} has introduced an improvement to AOPA -- the Robust Priority Assignment algorithm (RPA) --  which, in addition to being optimal, also maximizes the number of tolerable transmission errors in CAN. We note that both AOPA and RPA are not applicable to IEEE802.1 Qbu networks, as priority inversion may occur in these networks~\citep{Ojewale2020Feasibility}.

For systems where priority inversions may occur, Deadline Monotonic Priority Ordering (DMPO) and Deadline minus Execution time Monotonic Priority Ordering (D-CMPO) and the so-called ``DkC'' heuristic are commonly used, and it is well known that these heuristics dominate most other priority assignment heuristics in the literature in terms of schedulability~\citep{Davis2016Review, lee2021ml}. In particular, DMPO is the recommended priority assignment scheme in scenarios where preemption overheads are considered and/or fixed-priority scheduling with preemption thresholds. These two conditions also apply to IEEE802.1 Qbu networks, since each preemption introduces significant overhead, and thresholds are set for each preemption class~\citep{Ojewale2020Feasibility}. On the other hand, DMPO is not suitable for priority assignment in preemptive TSN because it provides a fully ordered priority list for the flowset, but Ethernet supports only up to eight priority levels. Consequently, this leads to another bin packing problem, which is known to be strongly NP-Complete.

In TSN, most of the work in the literature has focused on the configuration synthesis of time-triggered Ethernet networks, where flows are transmitted according to a pre-computed schedule. In this context, \cite{beji2014smt} has proposed a Satisfiability Modulo Theories (SMT) approach and~\cite{tamas2012synthesis} has proposed a heuristic for the communication synthesis of TTEthernet~\citep{steiner2009ttethernet}. On another front,~\cite{oliver2018ieee} and recently~\cite{reusch2020window} have proposed various frameworks for synthesizing the so-called Gate Control Lists for the IEEE 802.1 Qbv~\citep{IEEE802.1Qbv}. For event-triggered time-sensitive Ethernet networks,~\cite{specht2017synthesis} considered a TSN network with the Urgency Based Scheduler (UBS) and used an SMT approach to assign hard real-time flows to queues and priority levels to these queues on a per-hop basis. This work differs from ours in that it addresses the priority assignment for UBS only and assumes a non-preemptive frame transmission scheme.~\cite{gavriluct2020traffic} provided a method for assigning traffic classes to frames in TSN-based mixed criticality systems. However, none of these works addressed priority assignment and configuration synthesis of preemptive TSN networks.

Several works have applied Machine Learning (ML) techniques to various problems in the real-time domain~\citep{ae1990programmable, cardeira1994neural, cardeira1995preemptive, lee2021ml}. Most relevant to this work is the recent work of~\cite{lee2021ml}, in which the authors proposed a Priority Assignment Learning (PAL) framework for multi-core real-time systems. PAL was found to be more effective than existing approaches but suffers from severe scalability challenges as the number of tasks grows. There are other works in the literature that have applied ML techniques to TSN~\citep{mai2019hybrid, mai2019use, mai2021deep, navet2019using}.~\cite{mai2019use} and~\cite{navet2019using} employed ML techniques to search for feasible TSN configurations. We note that both works do not address the priority assignment problem as part of the configuration. The authors also presented a so-called ``hybrid'' approach that combines ML techniques with theoretical performance analysis to control the false prediction rate of ML models~\citep{mai2019hybrid}. In addition, Mai et al. recently presented a Generative Neural Network (GNN)-based technique for predicting a feasible TSN configuration~\citep{mai2021deep}. But the work stops short of defining any priority assignment scheme.

\cite{park2019design} showed that both the priority and preemption class assignment schemes used in a preemptive TSN network have a significant impact on the ability of frames to satisfy their timing constraints. In this regard, the authors proposed a framework to compute efficient priority assignments for flows and an efficient eMAC/pMAC queue boundary at each switch port. However, that work assumes a $1$-level preemption scheme, leaving open the question of an appropriate priority assignment policy, preemption levels, and flow-to-preemption-class assignment. These gaps are filled in this thesis.


%The contribution presented in this paper provides a priority assignment scheme for preemptive TSN. To the best of our knowledge, this is the first effort towards this direction.


%Park et al.~\cite{park2019design} proposed a framework to compute efficient priority assignments for flows and an efficient eMAC/pMAC queue boundary at each switch port. But, the work was conducted by assuming a $1$-level preemption scheme, thus leaving open the question of finding the appropriate preemption levels and a flow-to-preemption-class assignment. 




\subsection{Flow routing}
\label{sec:related_work:routing}
Routing time-sensitive flows is non- trivial~\citep{Nasrallah2018}. Routing optimization has been well studied in the literature and sophisticated techniques have been proposed~\citep{wang2000multicast, grammatikakis1998packet}. However, contributions on TSN routing schemes have started less than a decade ago. In this context, both the rapid spanning tree protocol and the shortest path bridging algorithms have been widely adopted in practice~\citep{Pop2016cyber}. On the other hand, the IEEE802.1 Qca standard~\citep{Ieee802.1Qca} specifies the Constrained Shortest Path First routing algorithm for TSN transmissions, but this algorithm does not prevent congestion situations and may increase contention in the network. ~\cite{arif2016load} proposed a methodology to evaluate the routes of a TSN end-to-end connection, but load balancing was not part of their objectives.

\cite{Nayak2017} investigated Integer Linear Programming (ILP) based algorithms for routing time sensitive flows in TSN networks with Time Aware Shapers. The proposed approach in their work differs from ours in that it does not consider the problems of congestion and load-balancing. Aiming at better load balancing for a TSN network,~\cite{Singh2017} has presented a meta-heuristics based algorithm capable of routing new traffic flows at runtime with minimal overhead. However, the proposed approach uses the shortest path algorithm (SPA) as the initial solution and does not consider all feasible routes. This limits the solution search space.~\cite{gavrilut2017fault} also took the same path and proposed heuristic methods for topology and routing synthesis. Their method attempts to achieve optimal utilization of switches and links and efficient routing of flows. However, they did not consider load-balancing. This thesis fills this gap: It addresses the problem of load balancing, disjoint routing for duplicate flows, and dynamic re-routing in congestion situations.

==> sections/conclusion/conclusion.tex <==
\chapter{Conclusions}
\label{chap:conclusion}
In this chapter, we summarize the findings and results of this thesis and outline possible future research directions. In particular, we summarize our contributions and draw some conclusions in Section~\ref{sec:conclusion:summary}. In Section~\ref{sec:thesis-validation} we examine the validity of the thesis statement, and finally, we outline the limitations of the work and possible areas for improvement in Section~\ref{sec:future-work}.

\section{Summary}
\label{sec:conclusion:summary}
To achieve low latency in the transmission of time-sensitive flows in Ethernet networks, the IEEE has introduced the IEEE ~802.1Qbu~standard, which specifies a $1$-level preemption scheme. Here, frames are divided into two different preemption classes --- namely, \textit{express frames} and \textit{preemptable frames} --- and a so-called preemptable frame can be interrupted before it is completed to allow fast transmission of \textit{express frames}; but any other preemptable frame cannot be transmitted until the already preempted frame is completed. While this approach improves the responsiveness of express frames, their performance is negatively affected as the number increases. In addition, there are a number of preemptable frames that cannot be promoted as express frames, but for which firm timing constraints apply. These frames may experience long blocking times because two frames belonging to the same preemption class cannot preempt each other. To overcome these limitations, we have proposed a multi-level preemption scheme in this work.

%, we have presented results on the feasibility, advantages and performance of a Multi-level preemption feature.

We first provided a detailed background and literature review on real-time communication in the context of Distributed Real-time Embedded Systems (DRES) in Chapter~\ref{chap:background}. Then, we examined the preemption mechanism in detail to determine the feasibility of a multi-level preemption scheme, and our analysis confirms its feasibility. In Chapter~\ref{chap:feasibility}, we detailed the changes required to achieve this goal and provided implementation recommendations to ensure frame integrity and interoperability. We then compared the hardware implementation costs of the multi-level preemption scheme with TAS and CBS. Then, a formal timing guarantee for each flow under such a scheme was given using a so-called \textit{Compositional Performance Analysis} in Chapter~\ref{chap:model-analysis-configuration}. In addition, we presented a configuration framework for determining the appropriate preemption level to enable, as well as a methodology for assigning flows to preemption classes for the preemption scheme. We extensively evaluated the performance of the proposed muti-level preemption scheme as well as the configuration framework in Chapter~\ref{chap:evaluation}. Finally, we studied traffic routing in the general context of TSN networks in Chapter~\ref{chap:routing}. Here, we propose two routing heuristics, called $\lbdrr$ and $\crdrr$, to solve the problem of congestion avoidance and congestion recovery, respectively.


\section{Thesis validation}
\label{sec:thesis-validation}
In Chapter~\ref{chap:introduction}, we stated the thesis supported by this dissertation as follows:
\begin{quote}
    \textit{We postulate that multi-level preemption when added to TSN can mitigate several shortcomings of this standard and unlock benefits in timeliness and resource utilization of DRES.}
\end{quote}

%We have demonstrated the validity of this claim on two fronts. First, we showed that the $1$-level preemption scheme as dictated by the current specification is indeed a limitation. From the motivation example in Chapter~\ref{chap:introduction}, to the results obtained in Chapters~\ref{chap:analysis} and~\ref{chap:configuration}, we showed that the $1$-level preemption scheme indeed causes a significant number of flows to miss their deadlines. Secondly, 

In this dissertation, we have shown that multi-level preemption leads to substantial improvements in performance. In particular, we have shown in Chapter~\ref{chap:evaluation} that multi-level preemption leads to an improvement of up to $53.07\%$ in $\WCTT$ guarantees for preemptable time-sensitive frames with firm timing constraints, and that the average number of schedulable flowsets increases with increasing preemption levels. In an extensive space exploration experiment, the schedulability ratio jumps from $45.5\%$ under the non-preemptive scheme to $85.8\%$ under the $1$-level preemption scheme, and the trend continues, albeit non-linearly, with each additional preemption level to peak at $98.1\%$ under a fully preemptive scheme. 
\begin{tcolorbox}
    From these observations, it follows that the constraints of the multi-level preemption mitigate the shortcomings of $1$-level preemption as defined in the standards and unlock benefits in terms of timeliness and resource utilization. Therefore, the thesis is validated.
\end{tcolorbox}


%may still cause a non-negligible number of flowsets (here $13\%$) to be unschedulable, despite the huge improvements it brings about over the non-preemptive scheme. This issue is circumvented by the multi-level preemption scheme. 



%\section{Conclusion}
%\label{sec:conclusion:conclusion}
%In this thesis, we highlighted a major limitation of the TSN frame preemption standard in that it supports just 1-level preemption. We then proposed a multi-level preemption scheme to alleviate this identified shortcoming. We established via formal analysis and extensive experiments that the proposed multi-level preemption scheme mitigates the shortcomings of the 1-level scheme and brings about significant performance improvement. 
It is important to note that each preemption level introduces additional hardware implementation overheads and that the framework presented in chapter~\ref{chap:model-analysis-configuration} is important to ensure that only the required preemption levels are enabled and hardware resources are conserved. 
\begin{tcolorbox}
    We also note that the improvement from additional preemptions is non-linear and drops off sharply after $4$ preemption levels. Interestingly, this ($4$) is also the point after which the implementation overheads of the multi-level preemption scheme overtake that of TAS, as shown by the results in Chapter~\ref{chap:feasibility}. 
\end{tcolorbox}

Recent studies have shown that the performance of standard Ethernet with Frame Preemption is comparable to that of widely studied time-aware shapers (TAS), which are more complex and expensive to implement. By addressing the key limitations of the $1$-level preemption scheme, this work provides a simpler and less expensive alternative communication solution.

\section{Limitations and future directions}
\label{sec:future-work}

In this section, we acknowledge the limitations of our work and suggest ways in which it could be improved and extended. We believe that this topic can be further explored and developed, and we encourage future research in this direction to accelerate the adoption of multi-level preemption systems in DRES. Below, we highlight the limitations and potential areas for improvement.

\subsection {Hardware implementation}
In this work, we have provided a detailed description of the required changes to the switch transmission and reception mechanisms to support multi-level preemption and the implication in terms of hardware overhead. However, due to resource constraints, we did not implement actual proof-of-concept switch hardware. Implementation costs were estimated using the resource utilization profile of the $1$-level preemption scheme, assuming that this utilization increases linearly with each additional level of preemption. This assumption is based on our proposed implementation approach, which requires an additional MAC merge sublayer for each additional level of preemption. We chose this approach because it ensures interoperability with other preemption schemes (non-preemptive and $1$- level) and does not require any change to the Ethernet frame format. We note that another approach has been proposed in the literature by~\cite{knezic2020implementation}. This approach promises an implementation with lower hardware overhead but requires modification of the standard Ethernet frame format, which may affect interoperability.
\begin{tcolorbox} The development of an actual proof-of-concept switch that supports multi-level preemption is an interesting direction for the future. In addition, studies on more efficient implementation approaches would greatly benefit multi-level preemption scheme.
\end{tcolorbox}


\subsection {Time-triggered and reservation-based models}
To analyze the timing properties of the multi-level preemption scheme, this work assumes only Ethernet with Strict Priority and Frame Preemption. We choose this model so that we can focus solely on evaluating multi-level preemption without the added complexity of other protocol mechanisms. 

\begin{tcolorbox}
    Further studies on the impact of multi-level preemption on time-triggered and reservation-based transmission schemes could be conducted to evaluate how these mechanisms can benefit from multi-level preemption. Another interesting research direction would be to compare the performance of strict priority and multi-level preemption with the time-triggered and reservation-based TSN traffic control mechanisms from WCTT and QoS perspectives.
\end{tcolorbox}


\subsection {Starvation}
In strict priority preemptive networks, lower priority flows are always at risk of starvation. We have not addressed this challenge in this dissertation. We believe that CBS is a promising candidate to protect frames of lower priority classes from starvation. Another promising concept that can be helpful in this regard is the so-called ``aging'' where the priority of a flow (or task) increases with respect to the amount of time that it has spent in the network (or system)~\citep{Buttazzo2011}. 
\begin{tcolorbox}
    We strongly believe that investigating novel methods to mitigate starvation in multi-level preemption schemes is a promising direction.
\end{tcolorbox}


%\subsection{Software defined preemption}
%TSN standards generally specify functions from a hardware implementation/configuration perspective. With the introduction of the pub/sub function in the Open Platform Communication Unified Architecture (OPC UA),~\citep{OPCUA}, work is beginning on the feasibility of implementing software-defined TSN functions in the OPC UA context~\citep{Julius2018Open, Gogolev2021End}. It would be interesting to investigate the frame preemption function in this context. In particular, it would be a worthwhile endeavor to investigate the feasibility of implementing TSN frame preemption (and also multi-level preemption) from the software-defined perspective.

%\subsection {Topology exploration}
%We believe that network topology has an impact on the number of transmission contention at switch output ports. Investigating the impact of different network topologies on the number of preemption levels and the overall performance of multi-level preemption schemes is also a promising direction.

%There is room for improvement in the configuration search space. Studies into how to further explore the search space for possible improvements of the priority assignment scheme would be of great benefit to the results presented in this thesis. Specifically, the effect of each of the selected flow characteristics on the outcome of the clustering algorithm could be explored.  Routing is fixed  and is always the same between any pair of nodes in this work. Thus, the impact of a static per-flow routing on schedulability and runtime for the multi-level preemption scheme could be considered. Last but not least, a comparison between an optimal priority assignment without preemption and a sub-optimal priority assignment with preemption would also be interesting to evaluate the trade-off between priority assignment and preemption.



==> sections/configuration/configuration.tex <==
\chapter{A Configuration Framework for Multi-level Preemption Schemes}
\label{chap:configuration}


%\section{Introduction}
\label{sec:configuration:intro}
\input{feupphdteses/sections/configuration/sections/introduction.tex}
%
\section{Definitions}
\label{sec:configuration:model}
\input{feupphdteses/sections/configuration/sections/model.tex}
%

%
\section{Proposed framework}
\label{sec:configuration:solution}
\input{feupphdteses/sections/configuration/sections/solution.tex}

%
\section{Evaluation}
\label{sec:configuration:experiment}
\input{feupphdteses/sections/configuration/sections/experiment.tex}

%
% \section{Related Work}
% \label{sec:configuration:related}
% \input{feupphdteses/sections/configuration/sections/related_work.tex}



\section{Chapter Summary}
\label{sec:configuration:conclusion}
\input{feupphdteses/sections/configuration/sections/conclusion.tex}
%



==> sections/configuration/sections/abstract.tex <==
To reduce the latency of time-sensitive flows in Ethernet networks, the IEEE TSN task Group introduced the IEEE~802.1Qbu~Standard, which specifies a $1$-level preemption scheme for IEEE~802.1 networks. Recently, a multi-level preemption approach has been proposed to address the limitations of the $1$-level preemption scheme. As is the case with most, if not all, real-time and/or time-sensitive preemptive systems, an appropriate priority assignment policy plays a central role in the resulting performance of both $1$-level and multi-level preemption schemes to avoid the over-provisioning and/or the sub-optimal use of hardware resources.  On another front, the multi-level preemption scheme raises new configuration challenges. Specifically, the \textit{right number} of preemption level(s) to enable, and the \textit{flow-to-preemption-class assignment} synthesis remain open problems. To the best of our knowledge, there is no prior work in the literature addressing these important challenges. In this work, we address these three challenges. We demonstrate the applicability of our proposed solution by using both synthetic and real life use-cases. \textcolor{blue}{ Our experimental results show that multi-level preemption improves the schedulability of flows by over $12\%$ compared to the $1$-level preemption scheme, and the proposed configuration framework improves the schedulability of flows by about $6\%$, compared to the dominant Deadline Monotonic Priority Ordering.}



==> sections/configuration/sections/conclusion.tex <==
In this chapter, we address the synthesis problem for multi-level frame preemption in TSN. Given a set of flows and the network topology, we present a framework to assign priorities to the flows, determine the appropriate preemption level to enable, and a flow-to-preemption-class assignment. We evaluate the performance of the proposed framework experimentally and our results show that the proposed scheme outperforms the DMPO scheme which is known to dominate most of the other priority assignment schemes in the literature. We also show that the proposed framework minimizes the number of preemption levels to guarantee schedulability. This is especially important as each additional preemption class comes along with significant hardware overheads that can increase the cost of switch manufacturing. In addition, our proposed framework demonstrates acceptable scalability for practical use-cases.


% As future work, studies into how to further explore the search space for possible improvements of the priority assignment scheme would be of great benefit to our proposed approach. Specifically, the effect of each of the selected flow characteristics on the outcome of the clustering algorithm could be explored. Another interesting research direction would be the comparison of the performance of multi-level preemption scheme against other TSN traffic control mechanisms from WCTT and QoS standpoints. Routing is fixed  and is always the same between any pair of nodes in this work. Thus, the impact of a static per flow routing on schedulability and runtime for the mutli-level preemption scheme could be considered. Last but not least, a comparison between an optimal priority assignment without preemption and a sub-optimal priority assignment with preemption would also be interesting to evaluate the trade-off between priority assignment and preemption.




==> sections/configuration/sections/experiment.tex <==
\subsection{Evaluation on a synthetic network.}
\noindent $\triangleright$ {\bf Setup.} We consider a quad-star topology consisting of six EPs and three TSN switches connected as shown in Figure~\ref{fig:configuration:synthetic-network}.
\begin{figure}[htb]
\centering
\includegraphics[scale=0.9]{feupphdteses/sections/configuration/images/synthetic_small_topology_priority_ass_c.PNG}
\caption{Synthetic network with quad-star topology.}
\label{fig:configuration:synthetic-network}
%\vspace{-0.1in}
\end{figure}
Link speeds are assumed constant and set to $100$MBits/s. In each batch of experiments, we randomly generated 1000 flowsets of equal sizes, i.e., each flowset has exactly the same number of flows as the others. We  varied the  sizes between $100$ and $250$ flows per flowset. Each generated flow is characterised by a source, destination, period, deadline, and size. The sources and destinations are chosen randomly among the EPs. The values of the periods and deadlines range from $500\mu s$ to $100000\mu s$. The values for the flow sizes range from $64$bytes to $1500$ bytes. We then assign priorities to the flows using our proposed approach. The priority assignment framework was implemented in Python 3.6, and the \texttt{scikit-learn}\footnote{https://scikit-learn.org/stable/modules/clustering.html} -- a free software machine learning library for the Python programming language -- was used for the k-means clustering. We benchmark our solution against DMPO because it is known to dominate most of the other priority assignment schemes in the literature~\citep{lee2021ml, Davis2016Review}. Furthermore, DMPO has been specifically recommended for fixed-priority preemptive systems with preemption thresholds~\citep{Davis2016Review}, which is a flow transmission model close to the one considered in this paper.  Since DMPO provides a fully ordered priority list for the flowset and Ethernet only supports up to eight priority levels, we perform a greedy bin packing of the ordered flows by assigning equal number of flows to each priority level. Also, as the exact number of priority levels that gives the best performance is not known under DMPO, we tried all possible numbers of priority levels $k$ (with $1 \leq k \leq 8$) and report the best performance. 

Our major evaluation metrics is the schedulability ratio, i.e, the percentage ($\%$) of flows that meet their timing requirement under the priority assignment scheme. To evaluate the schedulability of each scheme, we employ the worst-case traversal time (WCTT) analysis for preemptive TSN presented by~\cite{Ojewale2021WorstCase}. Here, the authors computed the WCTT of each flow by using a Compositional Performance Analysis (CPA) framework. For both our k-means approach and the DMPO, we ran the experiments several times each and then report the average observed schedulability performances. In the first batch of experiments, we assign priorities to the flows using DMPO and k-means, and evaluated the schedulability of flows by assuming a fully-preemptive scheme, i.e, a flow can preempt any other flow of lower priority than itself. In the second batch of experiments, we applied our preemption class assignment algorithm to determine the appropriate preemption level assignment for each flowset.

\noindent $\triangleright$ {\bf Results and discussion.}
Figure~\ref{fig:configuration:result-synthetic-network} shows the schedulability results under the k-means and DMPO schemes. From the Figure, k-means is able to schedule a higher number of flows than DMPO. Specifically, the average number of scedulable flowsets ranges from $999.5$ to $981$ for the k-means scheme, and from $998$ to $974$ for DMPO.
\begin{figure}[htb]
\centering
\includegraphics[scale=0.75]{feupphdteses/sections/configuration/images/synthetic_priority_assignment_result.png}
\caption{Schedulability: K-means vs. DMPO.}
\label{fig:configuration:result-synthetic-network}
\end{figure}
Figure~\ref{fig:configuration:runtime-synthetic-network} shows the average runtime per flowset for both k-means and DMPO. The reported execution times were obtained from a commodity hardware (Intel(R) Core(TM) i7-6500U CPU @ 2.50GHz, 16GB Memory). From Figure~\ref{fig:configuration:runtime-synthetic-network}, DMPO is much faster than the k-means algorithm. This is due to its complexity. At the core of DMPO is a sorting, with a complexity of $O(nlog(n))$ whereas k-means is known to have a complexity of $O(n^2)$~\citep{Pakhira2014Linear}. We note, however, that k-means is still reasonably fast for the priority assignment task with an average runtime of $1.6$s compared to DMPO's $0.79$s for flowsets with $250$ flows each.
\begin{figure}[htb]
\centering
\includegraphics[scale=0.75]{feupphdteses/sections/configuration/images/runtime-synthetic_cropped.png}
\caption{Runtime: K-means vs. DMPO.}
\label{fig:configuration:runtime-synthetic-network}
%\vspace{-0.1in}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[scale=0.75]{feupphdteses/sections/configuration/images/preemption_level_sched_bar_cropped.png}
\caption{Schedulability results w.r.t. increasing preemption levels }
\label{fig:configuration:preemption-level-schedulability}
%\vspace{-0.1in}
\end{figure}

Figure~\ref{fig:configuration:preemption-level-schedulability} shows the schedulability results for the preemption level assignment (Algorithm~\ref{alg:assignment-of-preemption-levels}). 
From the Figure, the average number of schedulable flowsets increases with increasing preemption levels. Specifically, the schedulability ratio jumps from $45.5\%$ under the non-preemptive scheme to $85.8\%$ under the $1$-level preemption scheme and the trend continues, in a non-linear manner though, with each additional preemption level to peak at $98.1\%$ under a fully preemptive scheme. From these observations, it follows that the limitations of the $1$-level preemption scheme may still cause a non-negligible number of flowsets (here $13\%$) to be unschedulable, despite the huge improvements it brings about over the non-preemptive scheme. This issue is circumvented by the multi-level preemption scheme. Note that the increase over the $4$-level preemption scheme is not significant and/or offers limited gain in this case. In addition, it is important to mention that each preemption level involves extra hardware implementation overheads and the framework presented in this paper is useful to evaluate the trade-off in terms of preemption-level scheme to adopt and the performance gain brought about by enabling each extra-preemption level.

Figure~\ref{fig:configuration:runtime-preemption-levels} shows the average runtime per flowset for each preemption level configuration. From the figure, it takes an average of $1.6$s to compute the preemption configuration and assess the schedulability of a flowset of $250$ flows, under a non-preemptive scheme. The execution time grows slowly as new preemption levels are added, and peaks at an average of $6.21$s per flowset for a fully preemptive scheme. This shows that despite the fact that the preemption level algorithm is a guided exhaustive search approach, its execution time is not prohibitive, and consequently, making the proposed scheme applicable in real-life scenarios.
\begin{figure}[htb]
\centering
\includegraphics[scale=0.75]{feupphdteses/sections/configuration/images/runtime-preemption-levels_cropped.png}
\caption{Average runtime w.r.t. increasing preemption levels}
\label{fig:configuration:runtime-preemption-levels}
%\vspace{-0.1in}
\end{figure}
\subsection{Evaluaton on real-life use-cases}
\noindent $\triangleright$ {\bf Setup.} SAE is the ``SAE automotive communication benchmark'' and Orion is the embedded communication network of the Orion Crew Exploration Vehicle (CEV). The network topologies of the SAE and Orion use-cases are depicted in Figures~\ref{fig:configuration:SAE}, and~\ref{fig:configuration:Orion}, respectively. In the figures, the EPs are represented with rectangles and the TSN switches are represented with hexagons. The flow parameters are provided by~\cite{gavriluct2020traffic}\footnote{The files for all test cases are available at https://bit.ly/2kpLrKj.}. Link speeds are assumed constant and set to $100$MBits/s. In the first batch of experiments, we assign priorities to the flows using the two priority assignment schemes, and evaluated the schedulability of flows by assuming a fully-preemptive scheme. In the second batch of experiments, we applied our preemption class assignment algorithm to determine the preemption level in which the number of schedulable flows is highest.
\begin{figure}
\centering
\includegraphics[scale=0.85]{feupphdteses/sections/configuration/images/SAE_cropped_c.pdf}
\caption{SAE automotive communication benchmark topology~\cite{gavriluct2020traffic}}
\label{fig:configuration:SAE}
%\vspace{-0.1in}
\end{figure}

\begin{figure}
\centering
\includegraphics[scale=0.75]{feupphdteses/sections/configuration/images/Orion_cropped_c.pdf}
\caption{Orion CEV network topology~\citep{zhao2017timing}.}
\label{fig:configuration:Orion}
%\vspace{-0.1in}
\end{figure}

\noindent $\triangleright$ {\bf Results and discussion.}
Table~\ref{tab:priority-experiment-results} shows the schedulability performance of the two priority assignment schemes evaluated. From the table, the k-means priority assignment scheme again outperforms DMPO in both use-cases. Precisely, k-means was able to schedule $97.46\%$ and $86.9\%$ compared to DMPO's $93.67\%$ and $80.4\%$, for the SAE and Orion networks, respectively. For the SAE benchmark network, the schedulability performance of the k-means algorithm matches the one reported by~\cite{gavriluct2020traffic} who employed a traffic-type assignment (TTA) approach to find a feasible schedule. To the best of our knowledge, this is the best reported performance in the literature.
\begin{table}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Name        & EPs & SWs & No. of flows & K-means Schedulability & DMPO Schedulability \\
\hline
SAE       &15& 7   & 79  &97.46 \% & 93.67\% \\
\hline
Orion CEV &31& 15  & 184 & 86.9\% & 80.4\%\\
\hline

\end{tabular} 
\caption{Experimental results from real-life use-cases}
\label{tab:priority-experiment-results}
\end{table}

Figure~\ref{fig:configuration:schedulability-use-cases} shows the behavior of the SAE and Oreon setups with increasing number of preemption levels. From the Figure, frame preemption clearly increases the number of schedulable flows for both SAE and Oreon. We also note that the number of scedulable flows continue to increase in the Oreon use-case until it peaks at $86.9\%$ under a $3$-level preemption scheme. On the other hand, the flows schedulability in the SAE use-case already peaked under $1$-level preemption. Observations like this can help system designers to decide the best number of preemption levels to enable for a system at design time, and ensure that just the needed preemption levels are implemented.
\begin{figure}
\centering
\includegraphics[scale=0.75]{feupphdteses/sections/configuration/images/schedulability_use_cases_cropped.png}
\caption{ \% of schedulable flows w.r.t. increasing preemption levels for SAE and Oreon.}
\label{fig:configuration:schedulability-use-cases}
%\vspace{-0.1in}
\end{figure}



==> sections/configuration/sections/introduction.tex <==
As is the case with most, if not all, real-time and/or time-sensitive preemptive systems, an appropriate \textit{priority-to-flow assignment} policy plays a central role in the resulting performance of both $1$-level and multi-level preemption schemes to avoid the over-provisioning and/or the sub-optimal use of hardware resources. In this scope, the so-called \textit{Audsley's Optimal Priority Assignment algorithm} (AOPA) has become the reference in many real-time systems\footnote{Here ``optimality'' refers to the capability of this algorithm to provide a priority-to-flow assignment that allows all flows to meet their timing requirements if such a scheme exists.} provided that there are no priority inversions~\citep{Park2019Optimal, davis2007controller}. This is not the case in preemptive TSN~\citep{ojewale2018multi, Ojewale2021WorstCase}. Indeed, Davis et al.~\citep{Davis2016Review} noted that AOPA is not applicable in fixed priority schemes with differed preemptions and/or preemption thresholds, and this is the case with preemptive TSN. Consequently, the so-called \textit{Deadline Monotonic Priority Ordering} (DMPO)~\citep{Davis2016Review} is often employed in practice and is known to dominate most of the other priority assignment heuristics in terms of schedulability~\citep{lee2021ml}. Nonetheless, DMPO is not suited for priority assignment in preemptive TSN neither, since it provides a fully ordered priority list for the flowset. Ethernet supports up to eight  priority levels only. With this limitation, a fully ordered priority list will lead to another bin packing problem, which is known to be strongly NP-Complete~\citep{lodi2002recent}. An efficient priority assignment scheme should not only provide the best possible priority order for flows but should also assign multiple flows into the same priority levels in the best possible manner.

Note that \textit{multi-level preemption scheme} brings about a whole new dimension to the configuration synthesis in addition to the priority assignment challenge. In fact, under a $1$-level preemption scheme, configuration decisions are somewhat simple and straightforward. They are limited to deciding whether each flow belongs to the express class or to the preemptable class. The picture darkens considerably when the multi-level preemption scheme is adopted. Here, the system designer must provide answers to two key questions: ($1$)~how to define the number of preemption levels to enable? and ($2$)~how to proceed with the flow-to-preemption-class mapping? In response to these concerns, it is worth noting that while Ethernet can support at most a seven-level preemption scheme\footnote{Ethernet features eight priorities level, and thus at most eight preemption classes. By assuming that a flow in a preemption class can preempt any other flow in another preemption class with a lower priority, it follows that Ethernet can support at most a seven-level preemption scheme.}, each additional preemption level comes with significant hardware overheads that can increase the cost of switch manufacturing~\citep{Pruski2021Implementation, Ojewale2020Feasibility}. To ensure an optimal use of hardware resources, the system designer must ensure that just the needed number of preemption levels are supported for the transmission of flows over the network. Figure~\ref{fig:configuration:config-samples} highlights the importance of the preemption level synthesis problem.  
\begin{figure}[!b]
\centering
\begin{subfigure}{.63\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{feupphdteses/sections/configuration/images/config_sample_1n}
  \caption{Flow $f_2$ misses its deadline with a $2$-level preemption scheme.}
  \label{fig:configuration:config-sample-1}
\end{subfigure}%
\vspace*{5pt}
\begin{subfigure}{.63\textwidth}
\centering
  \includegraphics[width=0.8\textwidth]{feupphdteses/sections/configuration/images/config_sample_2n}
    \caption{All flows meet their deadlines with a $3$-level preemption scheme.}
  \label{fig:configuration:config-sample-2}
\end{subfigure}
\vspace*{5pt}
\begin{subfigure}{.63\textwidth}
\centering
  \includegraphics[width=0.8\textwidth]{feupphdteses/sections/configuration/images/config_sample_3n}
    \caption{All flows meet their deadlines with a $2$-level preemption scheme.}
  \label{fig:configuration:config-sample-3}
\end{subfigure}
\caption{Motivation example for the multi-level preemption configuration.}
\label{fig:configuration:config-samples}
%\vspace{-0.2in}
\end{figure}
In Figure~\ref{fig:configuration:config-samples}, we consider the same four flows ($f_1$, $f_2$, $f_3$, $f_4$); and the flow priorities are set such that ``the smaller the index of a flow the higher its priority'', i.e., $f_1$ is assigned the highest priority and $f_4$ the lowest priority. An upward arrow represents the arrival time of a flow and a downward arrow represents the deadline. We assume four possible preemption classes: ($1$)~the \textit{highest preemption class}, wherein frames are represented by using ``red boxes''; ($2$)~the \textit{medium-higher preemption class}, wherein frames are represented by using ``yellow boxes''; ($3$)~the \textit{medium-lower preemption class}, wherein frames are represented by using ``black boxes''; and finally ($4$)~the \textit{lowest preemption class}, wherein frames are represented by using ``green boxes''. For this setting, there is no configuration under a non-preemptive nor a $1$-level preemption scheme that allows all flows to meet their timing constraints. By assuming the multi-level preemption scheme, we analyze three configuration scenarios.


In Figure~\ref{fig:configuration:config-sample-1}, flows are partitioned in three preemption classes and $f_2$ misses its deadline as it is unable to preempt~$f_3$ -- the two frames belong to the same preemption class. In Figure~\ref{fig:configuration:config-sample-2}, the situation improves for $f_2$ and it meets its deadline, nonetheless this is obtained at the cost of an additional preemption class. In Figure~\ref{fig:configuration:config-sample-3}, an appropriate configuration (again with three preemption classes) is used  and all frames meet their deadlines. From these observations, it follows that the performance of the multi-level preemption scheme strongly depends on the adopted configuration. 

\vspace{0.1cm}
\par {\bf Contribution.} In this chapter, we advance the state-of-the-art by addressing the aforementioned configuration questions. Given a set of flows and a TSN network, we first provide an offline priority assignment scheme for the flow set. Then, we provide an offline framework for determining the appropriate number of preemption levels on the one hand; and the flow-to-preemption-class assignment on the other hand. Put all together, the end goal of the proposed framework is twofold: ($1$)~to ensure that all flows meet their deadlines; and ($2$)~to ensure that hardware resources are utilized in an efficient manner. Note that frame preemption can be implemented with or without TSN shapers such as TAS and/or CBS (see~\cite{IEEE802.1Qbu}, page~$48$). We opt for an implementation without shapers so that we can focus solely on the evaluation of multi-level preemption without the added complexity of other protocol mechanisms.

\vspace{0.1cm}
\par {\bf Organization.} The rest of this chapter is organized as follows. Section~\ref{sec:configuration:model} presents some key definitions used throughout this chapter. Section~\ref{sec:configuration:solution} details our proposed framework. Experimental evaluations and performance assessment are presented in Section~\ref{sec:configuration:experiment}. Finally, Section~\ref{sec:configuration:conclusion} summarises the chapter. %Section~\ref{sec:configuration:related} discusses some related work.



==> sections/configuration/sections/model.tex <==
%\noindent $\triangleright$ {\bf Network specification.} We assume an  Ethernet backbone network for a real-time distributed system. We represent the network as a directed graph $G \equals (\mathcal{N}, \mathcal{L})$, where $\mathcal{N}$ is the set of all nodes and $\mathcal{L}$ is the set of all physical links in the network. We assume that every link is bi-directional; full-duplex; and operates at a single reference speed, say~$s > 0$. The tuple~$G$ is given with the interpretation that: ($1$)~$\mathcal{N} = \operatorname{EP} \cup \operatorname{SW}$, where~$\operatorname{EP} \equals \{\operatorname{EP}_1, \operatorname{EP}_2, \ldots \}$ represents the set of all end-points and~$\operatorname{SW} \equals \{\operatorname{SW}_1, \operatorname{SW}_2, \ldots\}$ is the set of all switches. Each $\operatorname{EP}_q$ (with $q \ge 1$) has a single output port and can receive and send network traffic while $\operatorname{SW}$~consists only of forwarding nodes, each with a finite number of output ports, through which the traffic is routed. Each $\operatorname{SW}_{\ell}$ (with $\ell \ge 1$) is enabled with multi-level preemption capability and decides, based on its internal routing table, to which output port a received frame will be forwarded. We also assume that each switch Input/Output port has $8$ priority queues and that each queue is assigned to flows of the corresponding priority level.

%\vspace{0.1cm}
%\noindent $\triangleright$ {\bf Traffic specification.} We consider $\mathcal{F} \equals \{f_1, f_2, ..., f_n\}$ a network traffic with $n \ge 1$~flows. Each flow $f_i \equals \langle src_i, dst_i, T_i, D_i, S_i, P_i, \operatorname{PC}_i \rangle$ consists of a potentially infinite number of instances (a.k.a. frames) and is characterized by: ($1$)~$src_i$, the source endpoint; ($2$)~$dst_i$, the destination endpoint; ($3$)~$T_i$, the minimum inter-arrival time between two consecutive frames of $f_i$, i.e., by assuming that the first frame of~$f_i$ is released at~$src_i$ at time~ $a_{i,1} \ge 0$, then $a_{i,\lambda + 1} - a_{i,\lambda} \ge T_i$ for all $\lambda \ge 1$, where $a_{i,\lambda}$ is the release time of the $\lambda^{\operatorname{th}}$ frame; ($4$)~$D_i$, the relative deadline, i.e., $d_{i,\lambda} \equals a_{i,\lambda} + D_i$ is the latest time instant by which the $\lambda^{\operatorname{th}}$ frame of $f_i$ must reach $dst_i$; ($5$)~$S_i$, the size of $f_i$ (in bytes); ($6$)~$P_i$ (with $0 \leq P_i \leq 7$), the priority; and finally ($7$)~$\operatorname{PC}_i$ the preemption class. For the sake of convenience, we assume that $0$ is the highest priority and $7$ is the lowest\footnote{The specification in the standards suggests the opposite. However, we opted to keep both the frame priority and preemption class in the same format (ascending order starting from $0$) to improve readability.}. For preemption classes, we assume in the same vein that the smaller the value, the higher the preemption class. Flows with the same priority always belong to the same preemption class but the converse is not true. In other words, flows with the same preemption class may have different priorities (see Figure~\ref{fig:configuration:preemption-class}). Finally, the priority and the preemption class parameters lie at the core of the configuration problem addressed in this chapter and are determined in Section~\ref{sec:configuration:solution}. 

% \begin{figure}[htb]
% \centering
% \includegraphics[scale=0.7]{feupphdteses/sections/configuration/images/queue-preemption-class-config}
% \caption{Preemption classes; priority queues and Configuration.}
% \label{fig:configuration:preemption-class}
% \vspace{-0.1in}
% \end{figure}

% %\vspace{0.1cm}
% \noindent $\triangleright$ {\bf Flow configuration.} For a flow set $\mathcal{F}$, we denote by $\mathcal{C}^m \equals \{ \mathcal{C}_1^m, \mathcal{C}_2^m, \mathcal{C}_3^m, \ldots \}$ the set of all possible flow configurations, assuming an $m$-level preemption scheme\footnote{An $m$-level preemption scheme implies $m+1$ preemption classes.} (with $ 0 \leq m \leq 7$). Each configuration $\mathcal{C}_x^m$ (with $x \ge 1$) is an \textit{integer list} that defines the preemption class of each priority level. Concretely, $\mathcal{C}_x^m  \equals [c_{x,0}^m, c_{x,1}^m, \ldots, c_{x,p-1}^m]$, where $p$ is the number of different priorities in $\mathcal{F}$ and $c_{x,\sigma}^m$ (with $ 0 \leq \sigma \leq p-1$) is the preemption class of all flows $f_i \in \mathcal{F}$ with priority $P_i = \sigma$. In other words, a preemption configuration is a non-decreasing and surjective function. Figure~\ref{fig:configuration:preemption-class} illustrates an example of flow configuration $\mathcal{C}_x^3$ for a $3$-level preemption scheme (i.e., with $4$ preemption classes). Here, we assume that $x=1$ in order to refer to the ``first configuration'' out of the set of all possible configurations $\mathcal{C}^3$. Flows with priorities $0$ and~$1$ are assigned to the preemption class~$0$, i.e, $c_{1,0}^3 = 0$ and $c_{1,1}^3 = 0$; flows with priority $2$ are assigned to the preemption class~$1$; flows with priorities $3$, $4$ and~$5$ are assigned to the preemption class~$2$; and finally, flows with priorities $6$ and~$7$ are assigned to the preemption class~$3$. Therefore, the resulting  configuration is $\mathcal{C}_1^3 = [0,0,1,2,2,2,3,3]$. Note that we assume a network-wide configuration, i.e., $\mathcal{C}_1^3$ applies to all switches. Furthermore, for any $m$-level preemption scheme the following rules are enforced.

% \begin{enumerate}
%     \item [$R_1$--] Every flow $f_i$ can be assigned to one and only one preemption class;
%     \item [$R_2$--] To reduce priority inversion, any flow, say $f_j$, with a lower priority than another flow, say $f_i$, cannot be assigned to a higher preemption class than that of $f_i$;
%     \item[$R_3$--] To conserve hardware resources, every preemption class must have at least one flow assigned to it. 

% \end{enumerate}

In addition to the system model in chapter~\ref{chap:model}, we introduce the following definitions for any flow set $\mathcal{F}$ and network $\mathcal{G}$.

\begin{definition}[Valid configuration]
\label{def:valid-config}
Any configuration will be stamped as ``valid'' if upon the flow-to-preemption-class assignment, it conforms to Rules $R_1$, $R_2$ and $R_3$.
\end{definition}

\begin{definition}[Solution]
\label{def:solution}
Any valid configuration will be considered a ``solution'' if all flows $f_i \in \mathcal{F}$ meet their deadlines.
\end{definition}

Rule~$R_2$ from Section~\ref{sec:model:configuration} implies that $\mathcal{C}_x^m$ (with $x \ge 1$) is always sorted in an ascending order, i.e., $c_{x,\sigma}^m \le c_{x,\ell}^m$ for all $0 \le \sigma \le \ell \le p-1$. Rule~$R_3$ implies that each integer from $0$ to $m$ must appear \textit{at least once} in each valid configuration. Consequently, the task of generating all valid configurations $\mathcal{C}^m$ can be mapped to the problem of generating all ordered multisets~\citep{blizard1989multiset} of cardinality $p$ with elements taken from the set $\{0, \ldots, m\}$, where $p$ is the number of unique flow priorities in $\mathcal{F}$.  
In the following section, we first provide a priority assignment scheme in Section~\ref{subsec:configuration:priority-assignment}, and then a preemption class assignment scheme in Section~\ref{subsec:configuration:preemption-class-assignment}

%\begin{definition}[Optimal solution]
%\label{def:optimal-solution}
%A solution is said to be ``optimal'' if it utilizes the minimum number of preemption levels.  %and where flows are assigned to the lowest possible preemption class
%\end{definition}



==> sections/configuration/sections/priority_assignment.tex <==
In this section, we present the priority assignment scheme for TSN flows based on the traditional \textit{k-means clustering algorithm}~\citep{hastie2009elements}. This is a popular unsupervised Machine Learning (ML) algorithm that partitions items in an unlabeled list into $k$ different clusters (with $k \ge 1$). Specifically, it computes $k$ focal points called ``centroids'' within the data space in an  iterative manner. Clusters are formed around the centroids by assigning each item to the closest centroid to it. Finally, the location of each centroid is updated to the center of all data points assigned to it after each iteration. In the context of this work, the ``items'' to be assigned are TSN flows and the $k$ clusters are the flow priorities. We recall that Ethernet supports eight (8) priority levels, thus $k \leq 8$. The k-means algorithm performs clustering based on some selected characteristics of the items, referred to as ``features''.  These features capture the domain-specific knowledge of the real-life objects/concepts that the items represent. In this scope, the features need to be defined and sometimes transformed into a format that the k-means algorithm can process. The process of defining and preparing features for ML algorithms is called ``feature engineering''. In the following section, we summarize the feature engineering for our TSN priority assignment problem.

\subsubsection{Feature engineering}
\label{sec:configuration:solution:feature-engin}
For the priority assignment problem, five of the seven flow parameters defined in the system model (see Section~\ref{sec:model:traffic}) are considered for the clustering process, since the other parameters are yet to be determined (i.e., the priority and the preemption class). In other words, the tuple $\langle  {src}_i, {dst}_i, T_i, D_i, S_i \rangle$ is considered for each flow $f_i \in \mathcal{F}$. On another front, ${src}_i$ and ${dst}_i$ are used to determine the path length $\operatorname{PL}_i$ of flow $f_i$, i.e., the number of links traversed by $f_i$ from ${src}_i$ to ${dst}_i$. Therefore, the number of features employed for the clustering problem can be reduced to the tuple $\langle \operatorname{PL}_i, T_i, D_i, S_i \rangle$. 

Note that these selected features are not on the same unit scale. As a matter of fact, flow periods and deadlines can range from a few microseconds to hundreds of thousands of microseconds. At the other end of the table, flow sizes can only take values from $64$ bytes to $1500$ bytes (i.e., the minimum and maximum valid Ethernet frame sizes, respectively). Finally, the range of ${PL}_i$ depends largely on the network topology. In such a scenario, features with large values might dominate those with lower values, thereby impacting the actual performance of the k-means algorithm negatively. To ensure that this is not the case and make sure that each feature has an impact on the learning process, a process called ``normalisation'' is usually carried out on the selected feature set~\citep{hastie2009elements}. In this work, this normalization process is carried out on each of the features as follows. Regarding the flow length, all values are modified to obtain features in the interval $[-1, 0]$. To this end, we divide all flow lengths by the negative value of the longest flow path. Similarly, both $T_i$ and $D_i$ are normalized by dividing all values by the largest values of $T_i$ and $D_i$, respectively, to obtain features in the interval $[0, 1]$. Finally, the values of $S_i$ are normalized with the maximum frame size in the flowset to obtain features in the interval $[0, 1]$. The rationale behind the normalization of flow paths with the negative value of the longest flow path is to make flows with shorter paths have higher feature values. This is further explained in the following section. %Note that with the normalization process, flows with longer paths, smaller periods, deadline, and sizes are assigned smaller feature values.

\subsubsection{Clustering and priority assignment}
\label{sec:configuration:solution:clustering}

In this section, we describe our strategy for assigning the priorities to flows through partitioning the $n$ flows in $\mathcal{F}$ into $k$ clusters (with $1 \leq k \leq 8$) by using the k-means algorithm. The overall objective is to assign priorities to flows in a manner that allows as many as possible flows to be schedulable, i.e., meet their deadlines.  Figure~\ref{fig:configuration:k-means-flowcart} presents the adopted flowchart. From the figure, the process begins with the feature engineering processes described in Section~\ref{sec:configuration:solution:feature-engin}. After this step, two important questions need to be addressed: 
\begin{enumerate}
    \item[$Q_1$:] How to determine the value of $k$? In other words, how to determine the number of clusters (priorities) in which the flows should be divided into? 
    \item[$Q_2$:] How to determine the relative order among the clusters during the priority assignment process?
\end{enumerate}

\begin{figure}[htb]
\centering
\includegraphics[scale=0.5]{feupphdteses/sections/configuration/images/k-means-priority-assignment.png}
\caption{Flowchart: k-means priority assignment algorithm.}
\label{fig:configuration:k-means-flowcart}
%\vspace{-0.1in}
\end{figure}

\textbf{About $Q_1$}. Since we do not know which value of $k$ will yield the maximum number of schedulable flows, we initialize $k$ to $1$ and iterate through all possible values ($1 \leq k \leq 8$).\\


\textbf{About $Q_2$}. At each iteration, we perform k-means clustering on the normalized features and obtain the centroid of each of the $k$ clusters. Each centroid is a vector of the means of the features of items in the cluster. Afterwards, we compute the mean of each centroid. Recall that from the normalization process, flows with longer paths, smaller periods, deadlines, and sizes are assigned smaller feature values. As such, the smaller the final value of the centroid of a given cluster, the longer the path and the smaller the period; deadline and size of each of its members in general. In practice, flows with longer paths are more at risk of missing their deadlines as they may experience delays on the links they traverse. Also, flows with shorter periods and deadlines are usually assigned higher priorities in fixed priority scheduling theory because they are more at risk of missing their deadlines (think about Rate Monotonic and Deadline Monotonic policies). Finally, the sizes of non time-critical flows are typically larger than those of the time-critical ones (see~\cite{LOBELLO2020153, Ojewale2021WorstCase} for examples inspired by real-life use-cases from the automotive domain). With the aforementioned observations, we opted for assigning priorities to the clusters in ascending order of their centroid means. Specifically, \textit{the lower the centroid mean, the higher the priority}. In this work, we assume that all features have equal importance in the priority assignment process. Obviously, other feature engineering approaches can be adopted, where specific characteristics of the network are exploited. For example, the path length may be given a higher weight in a line topology network. We also note that the schedulability tests in the priority assignment process (see Figure~\ref{fig:configuration:k-means-flowcart}) depend necessarily on the preemption level assignment, which has not been defined at this point. To resolve this dependency, the schedulability is evaluated by assuming a fully-preemptive scheme, i.e, every flow can preempt any other flow with a lower priority.

==> sections/configuration/sections/problem-description.tex <==
We recall that the configuration synthesis consist of two components: ($1$)~determining the optimal preemption level for the flowset  and ($2$)~the assignment of queues to preemption classes. With regards, to the first component, the Ethernet networks can only support up to 8 priority levels. This implies that the search space for the optimal preemption level for a flowset is within the range $0 \leq p \leq 7$, where $0$ represents a non-preemptive scheme and $7$ represent a fully preemptive scheme. If the number of unique flow priorities in the network is less than $8$, then the search interval for the optimal preemption level will be within the range $0 \leq p \leq n-1$, where $n$ is the number of unique flow priorities in the network. 

With regards to the second aspect of the synthesis, the search space for a feasible solution within a preemption level $m$ includes all valid configurations~$\mathcal{C}_x^m \in \mathcal{C}^m$. We recall that each $c_{x,k}^m \in \mathcal{C}_x^m$ represent the preemption class to which flows of priority $k$ is assigned. Rule~$R_2$ in Section~\ref{sec:configuration:model} implies that $\mathcal{C}_x^m$ is always ordered. Also, Rule~$R_3$ implies that for a given preemption level $m$, the $\mathcal{C}_x^m$ will always contain all integers from $0$ to $m$. With the aforementioned, the problem of generating all possible configurations for the flowset $\mathcal{F}$ with preemption level $m$ can be mapped to the problem of generating all ordered multisets~\cite{blizard1989multiset} of cardinality $n$ with elements taken from the set $\{0, \ldots, m\}$, where $n$ is the number of unique flow priorities in $\mathcal{F}$. Rule~$R_3$ also implies that each element of the set $\{0, \ldots, m\}$ must appear atleast once, in the multisets. 
In the following section, we describe our proposed solution to the synthesis problem.




==> sections/configuration/sections/related_work.tex <==
An appropriate priority assignment policy plays a central role in the resulting performance of real-time systems~\citep{Davis2016Review}. For example, in the Controller Area Network (CAN)~\citep{specification1991bosch}, the maximum reliable utilization level was intially believed to be at 35\% due to the legacy practice of assigning message IDs (which corresponds to messages priorities) in a random or an ad-hoc manner~\citep{buttle2012real}. Davis et al.~\cite{Davis2016Review} later showed that a reliable CAN utilization over 80\% can be achieved using Audley's Optimal Priority Assignment (AOPA) algorithm~\cite{audsley2001priority}. AOPA has become the reference priority assignment scheme in many real-time systems and has been proved to be optimal when there are no priority inversions~\cite{Park2019Optimal}. ~\cite{davis2009robust} introduced an improvement of the AOPA -- the Robust Priority Assignment algorithm (RPA) --  which, in addition to being optimal, maximizes the number of tolerable transmission errors in CAN. We note that both AOPA and RPA are not applicable to IEEE802.1 Qbu networks because priority inversion can occur in these networks~\citep{Ojewale2020Feasibility}.

For systems where priority inversions can occur, the Deadline Monotonic Priority Order and Deadline minus Execution time Monotonic Priority Order (D-CMPO), and the so-called ``DkC'' heuristics are  often employed and these heursitics are known to dominate most of the other priority assignment heuristics in the literature in terms of schedulability~\citep{Davis2016Review, lee2021ml}. Specifically, DMPO is the recommended priority assignment scheme in scenarios where preemption overheads are taken into account and/or fixed-priority scheduling with preemption thresholds. These two conditions also apply to the IEEE802.1 Qbu networks as each preemption results in significant overhead and thresholds are set for each preemption class~\citep{Ojewale2020Feasibility}. On another front, DMPO is not suited for priority assignment in preemptive TSN because it provides a fully ordered priority list for the flowset but Ethernet only supports up to eight  priority levels. This will consequently lead to another bin packing problem which is known to be strongly NP-Complete.

For TSN, most work in the literature focused on the configuration synthesis of time-triggered Ethernet networks where flows are transmitted by following a pre-computed schedule. In this regard,~\cite{beji2014smt} proposed a Satisfiability Modulo Theories (SMT) approach and Tamas-Selicean et al.~\cite{tamas2012synthesis} proposed a heuristics for the communication synthesis of TTEthernet~\citep{steiner2009ttethernet}. On another front,~\cite{oliver2018ieee} and recently~\cite{reusch2020window} proposed different frameworks for the synthesis of the so-called Gate Control Lists for the TSN IEEE802.1 Qbv~\citep{IEEE802.1Qbv}. For event-triggered time-sensitive Ethernet networks,~\cite{specht2017synthesis} considered a TSN network with the Urgency Based Scheduler (UBS) and used an SMT approach to assign hard real-time data flows to queues and priority levels to these queues on a per hop basis. This work differs from our work in that it addresses the priority assignment for UBS only and the work assumes a non-preemptive frame transmission scheme.~\cite{gavriluct2020traffic} provided a method to assign traffic classes to frames in TSN-based mixed-criticality systems. However, none of these works addressed the priority assignment and configuration synthesis of preemptive TSN networks.

Several works have applied ML techniques to different problems in the real-time domain~\citep{ae1990programmable, cardeira1994neural, cardeira1995preemptive, lee2021ml}. Among these, the most relevant to this work is the recent work of~\cite{lee2021ml} where the authors proposed a Priority Assignment Learning (PAL) framework for multi-core real-time systems. PAL was found to be more effective than existing approaches but suffers severe scalability challenges as the number of tasks grows. There are other works in the literature that have applied ML techniques to Ethernet TSN~\citep{mai2019hybrid, mai2019use, mai2021deep, navet2019using}. Mai et. al.~\cite{mai2019use} and Navet et al.~\cite{navet2019using} employed ML techniques to search for feasible TSN configurations. We note that both works do not address the priority assignment problem as part of the configuration. The authors also presented a so-called ``hybrid'' approach that combines ML techniques with theoretical performance analysis to control the false prediction rate of the ML models~\citep{mai2019hybrid}. Furthermore, Mai et al. recently provided a Generative Neural Networks (GNN)-based technique to predict a feasible TSN configuration~\citep{mai2021deep}. But the work stops short of defining any priority assignment scheme.

\cite{park2019design} showed that both the priority and the preemption class assignment schemes employed in a preemptive TSN network have a significant impact on the ability of the frames to satisfy their timing constraints. In this regards, proposed a framework to compute efficient priority assignments for flows and an efficient eMAC/pMAC queue boundary at each switch port. But, the work was conducted by assuming a $1$-level preemption scheme, thus leaving open the question of finding the appropriate priority assignment policy, preemption levels, and a flow-to-preemption-class assignment. These gaps are closed in this contribution. 


%The contribution presented in this paper provides a priority assignment scheme for preemptive TSN. To the best of our knowledge, this is the first effort towards this direction.


%Park et al.~\cite{park2019design} proposed a framework to compute efficient priority assignments for flows and an efficient eMAC/pMAC queue boundary at each switch port. But, the work was conducted by assuming a $1$-level preemption scheme, thus leaving open the question of finding the appropriate preemption levels and a flow-to-preemption-class assignment. 




==> sections/configuration/sections/solution.tex <==
\subsection{Priority assignment}
\label{subsec:configuration:priority-assignment}
\input{feupphdteses/sections/configuration/sections/priority_assignment.tex}

\subsection{Preemption class assignment}
\label{subsec:configuration:preemption-class-assignment}

\subsubsection{Synopsis.}
Our preemption class assignment solution builds on the priority assignment scheme. It begins from a non-preemptive setup and proceeds by using a guided exhaustive search approach described as follows. At each step, we introduce an additional preemption level and test all possible flow-to-preemption-class configurations to check if all timing requirements are met. Our algorithm terminates as soon as a solution is found. Otherwise, another preemption level is added to the flow transmission scheme and a new test is carried out. Note that we are interested in determining the schedulability of a flow set only, and not on whether there are multiple solutions for a given flow set. This process is performed in an iterative manner up until a valid configuration is found at a given preemption level; or the maximum number of preemption levels (i.e., $7$) is exceeded. In the latter case, a valid configuration could not be found and the flow set is deemed ``unschedulable''. Below, we provide the step-by-step details of our proposed solution, which consists of two algorithms, namely ($1$)~the \textit{flow-to-preemption-class assignment}; and ($2$)~the \textit{valid configuration search}.
\vspace{0.1cm}

\subsubsection{Flow-to-preemption-class assignment.}
\label{subsec:configuration:assignment-of-preemption-levels}
Algorithm~\ref{alg:assignment-of-preemption-levels} presents the pseudo-code for this step. Two arguments are required as inputs, namely: ($1$)~the network topology $G$; and ($2$)~the flow set~$\mathcal{F}$. In the description, notation ``$\operatorname{P.Len}$'' refers to the length of list~$P$ and ``$[y]*\eta$'' refers to a list of length $\eta$ filled up with ``$y$'', e.g., $[0]*3 = [0,0,0]$. The algorithm proceeds as follows.

First, the set $\operatorname{P}$ of all unique flow priorities in $\mathcal{F}$ is stored in variable P (see line~\ref{alg:ass-begin-init}). Thereafter, a systematic search is carried out through all preemption levels $m$ (with $1 \leq m \leq \operatorname{P.Len} - 1$) for a solution (see lines~\ref{alg:ass-begin-loop-level} to~\ref{alg:ass-end-loop-level}). At each preemption level $m$, after the initialization phase (see lines~\ref{alg:search-init} to~\ref{alg:search-end-right-part-init}), a recursive function $\operatorname{VALID\_CONFIGS}()$ is invoked (see line~\ref{alg:search-valid-conf-call}). This function returns the set of all valid configurations for preemption level~$m$, i.e., $\mathcal{C}^m$. Then, a search through this set is conducted to find a solution (see lines~\ref{alg:ass-begin-conf-check} to~\ref{alg:ass-end-conf-check}). If a solution is found, then Algorithm~\ref{alg:assignment-of-preemption-levels} terminates with this solution (see line~\ref{alg:ass-return-present-conf}), otherwise $m$ is incremented and the process is repeated for the next preemption level, $(m+1)$. In case all iterations are exhausted and no solution is found, then a $\operatorname{NULL}$ value is returned (see line~\ref{alg:ass-return-fail}), which implies that the flow set is not schedulable. We note that for the schedulability test (see line~\ref{alg:ass-check-sched}), we employ the worst-case traversal time (WCTT) analysis for multi-level preemption schemes presented by Ojewale et al.~\cite{Ojewale2021WorstCase}. Here, the authors computed the WCTT of each flow by using a Compositional Performance Analysis (CPA) framework.  

\begin{algorithm}[tb]
\SetAlgoLined
\KwData{Network topology $G$; Flow set $\mathcal{F}$.}
\KwResult{A valid flow-to-preemption-class configuration.}
$\operatorname{P} \gets [Set\: of\: all\: unique\: flow \: priorities\: in \: \mathcal{F}]$\label{alg:ass-begin-init}

    \For{$m = \operatorname{0}\:  to \: \operatorname{P.Len} - 1$}{\label{alg:ass-begin-loop-level}
            %$\operatorname{preemption\_level} = i$
            $\mathcal{C}^m \gets \emptyset$\label{alg:search-init}\\
            
            $\operatorname{leftPart} \gets []$\label{alg:search-left-part-init}\\
        $\operatorname{rightPart} \gets [m]* \operatorname{P.Len}$\label{alg:search-init-all-flows-to-i} 
        
        \For{$j = 0\:  to \: m$}{
             $\operatorname{rightPart}[j] = j$\label{alg:search-init-highest-priorities-init}
         }\label{alg:search-end-right-part-init}
            $\mathcal{C}^m = \operatorname{VALID\_CONFIGS}(\mathcal{C}^m, \operatorname{leftPart},\:  \operatorname{rightPart})$\label{alg:search-valid-conf-call} 
            
            \ForEach{$\mathcal{C}_x^m \in \mathcal{C}^m$}{\label{alg:ass-begin-conf-check}
                %$\mathcal{F}_{temp} = \mathcal{F}$\\
                \ForEach{$f_i \in \mathcal{F}$}{
                    $\operatorname{PC}_i = c_{x,P_i}^m $ %f_i.priority
                }\label{als:ass-update-config}
                 
                 \If{$\operatorname{SCHEDULABLE}                 (\mathcal{F})$}{\label{alg:ass-check-sched}
                    \Return $\operatorname{\mathcal{C}_{x}^m}$\label{alg:ass-return-present-conf}
                }
            }\label{alg:ass-end-conf-check}  
    }\label{alg:ass-end-loop-level}

\Return{$\operatorname{NULL}$}\label{alg:ass-return-fail}
\caption{ASSIGN\_PREEMPTION\_CLASS($G$,$\mathcal{F}$)}
\label{alg:assignment-of-preemption-levels}
\end{algorithm}

\subsubsection{Valid configuration search.}
\label{subsec:configuration:valid-configs}
Algorithm~\ref{alg:valid-config} presents the pseudo-code. $\operatorname{ VALID\_CONFIGS}$() is a recursive function that computes the set of all valid configurations for a preemption level~$m$. It takes $3$ inputs: ($1$)~an initialization of the set $\mathcal{C}^m$ (which is usually an empty set at the start); ($2$)~a $\operatorname{leftPart}$ list (which is also usually empty at the start); and finally ($3$)~a $\operatorname{rightPart}$ which is a configuration initialization for the preemption level $m$. The notations in Algorithm~\ref{alg:valid-config} have the same meanings as those of Algorithm~\ref{alg:assignment-of-preemption-levels}. Additionally, the notation $\operatorname{ListA} + \operatorname{ListB}$ implies a concatenation operation of two lists. In summary, $\operatorname{VALID\_CONFIGS}$ solves the multisets generation problem described in Section~\ref{sec:configuration:model}.
Since the algorithm is recursive, the first step is to test for the base case (see lines~\ref{alg:valid-conf-begin-base-case} to~\ref{alg:valid-conf-end-base-case}). This is when the items in the $\operatorname{rightPart}$ are either all the same or all unique. In this case, the algorithm terminates and returns a merged (and sorted) list of $\operatorname{leftPart}$ and $\operatorname{rightPart}$. If the base condition is not met, then the recursive step (see lines~\ref{alg:valid-conf-length-diff} to~\ref{alg:valid-conf-end-recursive-case}) is executed. 


\begin{algorithm}[tb]
\SetAlgoLined
\KwData{Set of generated configurations $\mathcal{C}^m$;\: a left partition; and an initial configuration for preemption level $m$}
\KwResult{Set of generated configurations $\mathcal{C}^m$}

%$\operatorname{configurations}.append \newline(\operatorname{All\: ordered \: combinations\: of \: init\_config\_list})$
$ \operatorname{rightPartSet} =  sorted(set(\operatorname{rightPart}))$\label{alg:valid-conf-init}

    \If{$\operatorname{rightPart.Len} == \operatorname{rightPartSet.Len}\: \newline  OR \:  \operatorname{rightPartSet.Len ==1}$}{\label{alg:valid-conf-begin-base-case}
    
        $\mathcal{C}^m.add(sorted(\operatorname{leftPart+rightPart}))$ 
        
        \Return {$\mathcal{C}^m$}
}\label{alg:valid-conf-end-base-case}
    $\operatorname{diff} = \operatorname{rightPart.Len} - \operatorname{rightPartSet.Len}$\label{alg:valid-conf-length-diff}\\
    $\operatorname{diff}+=1$\\	
    $\operatorname{currentLeft} = \operatorname{rightPartSet.getFirstElem}$\label{alg:valid-conf-begin-new-left}\\
    $\operatorname{rightPartSet.removeFirstElem}$\label{alg:valid-conf-end-new-left}\\
    \For{$x = 1\:  to \: diff$}{\label{alg:valid-conf-begin-recursice-case} 		
        $\operatorname{tempLeft} = [\operatorname{currentLeft}]*x$\\
        
        $\operatorname{newLeftPart} = \operatorname{leftPart} + \operatorname{tempLeft}$	\\	
        $\operatorname{rightSize} = \operatorname{rightPart.Len} - x$	\\	
        $\operatorname{newRightPart} = list(\operatorname{rightPartSet})$	\\
        
       \If{$\operatorname{rightSize} > \operatorname{newRightPart.Len}$}{
       
            $\operatorname{lenDiff} = \operatorname{rightSize}-\operatorname{rightPartSet.Len}$	\\		
           $\operatorname{newRightPart} = [\operatorname{rightPartSet.getFirstElem}]*\operatorname{lenDiff}~+ list(\operatorname{rightPartSet})$\\
}		
        $\mathcal{C}^m = \operatorname{VALID\_CONFIGS}(\mathcal{C}^m, newLeftPart,\newline newRightPart)$\label{alg:valid-conf-recursive-call}
}\label{alg:valid-conf-end-recursive-case}
    \Return {$\mathcal{C}^m$}\label{alg:valid-config-return}
\caption{VALID\_CONFIGS($\mathcal{C}^m$, leftPart, rightPart)}
\label{alg:valid-config}
\end{algorithm}

\subsubsection{Computational Complexity} We recall that the problem of searching for all valid configurations (Algorithm~\ref{alg:valid-config}) was mapped to the multi-set problem which is known to have exponential complexity. \cite{stanley2011enumerative} already showed that the number of multisets of cardinality $k$ to be taken from $m$-element set is given by:
\[
     \frac{(k+m-1)!}{k!(m-1)!} %\binom{k+m-1}{m} =
\] 
We recall that every element of $\{ 1,2, \ldots, m\}$ must appear at least once in each multiset (see Section~\ref{sec:configuration:model}). This constraint reduces the number of elements order to be decided from $k$ to $k-m$. By replacing $k$ with $k-m$, the total number of valid configurations $|\mathcal{C}^m|$ for preemption level $m$ with $k$ unique priorities, is given by Equation~\ref{eqn:complexity}. 

\begin{equation}
    \label{eqn:complexity}
    |\mathcal{C}^m| =  \frac{(k-1)!}{(k-m)!(m-1)!}
\end{equation}
Algorithm~\ref{alg:assignment-of-preemption-levels} invokes function $\operatorname{VALID\_CONFIGS}()$ continuously until a solution is found or the maximum number of preemption levels is exceeded. Consequently, the maximum number of valid configurations to be tested is given by Equation~\ref{eqn:complexity-sum}.

\begin{equation}
    \label{eqn:complexity-sum}
    \sum_{m=1}^{P.Len -1} |\mathcal{C}^m|
\end{equation}
%\textcolor{red}{Putting Equations~\ref{eqn:complexity} and~\ref{eqn:complexity-sum} together, the computational complexity of the preemption class assignment solution is $\mathcal{O}(2^n)$ where \textit{n} is the number of unique priorities in $\mathcal{F}$. We note that while the complexity of this solution is exponential, the value of $n$ cannot exceed $8$, thus, making the complexity of this approach reasonable and bounded.}
Now that we have provided the specifics of our proposed framework for  determining the priority assignment and a valid configuration for a given flow set, we can proceed with demonstrating its applicability and evaluate its performance in the next section. To this end purpose, we consider two different settings:~($1$)~a synthetic use-case; and ($2$)~two real-life use-cases from the literature -- SAE~\citep{gavriluct2020traffic} and Orion~\citep{zhao2017timing}.



==> sections/evaluation/analysis-experiments.tex <==
In this section, we evaluate the safety and tightness of the proposed WCTT analysis. In Section~\ref{sec:evaluation-wctt-synthetic}, we consider a synthetic network modeled after a realistic automotive network, and in Section~\ref{sec:evaluation-wctt-renault}, we consider a Renault use case.

\subsection{Report on a synthetic workload}
\label{sec:evaluation-wctt-synthetic}

\noindent $\triangleright$ {\bf Setup.} We consider a synthetic network that is adapted from realistic network topology from an automotive use case, consisting of ten End Points~$\operatorname{EP}$s (ECUs in this case) and seven full-duplex preemption-enabled TSN switches $\SW_1, \SW_2, \ldots, \SW_7$ displayed as illustrated in Figure~\ref{fig:analysis:topology}. 

\begin{figure}[htb]
\centering
\includegraphics[scale=0.95]{feupphdteses/sections/analysis/images/topology-multi-level-preemption-analysis}
\caption{Network topology}
\label{fig:analysis:topology}
\end{figure}

We have considered seven flows -- $f_1, f_2, \ldots,f_7$ -- where $f_1$ and $f_2$ are express; $f_3$ and $f_4$ are tpflows; and the remaining flows are bpflows. The name and make of the system are protected by a non-disclosure agreement. However, the specifications of the flows are given in Table~\ref{tab:flows} and are the same range as that presented by~\cite {alderisi2012towards}. We recall that the flows are ordered by their priorities, i.e., the smaller the index of a flow, the higher its priority. Three batches of analyzes are performed along with their associated simulations using NeSTiNg~\citep{nesting_2019}, to evaluate their tightness:

\begin{enumerate} 
    \item [($a$)] All flows are transmitted under the $1$-level preemption scheme (i.e., only express flows can preempt other flows). 

    \item[($b$)] All flows are transmitted under the $2$-level preemption scheme (i.e., express frames can preempt all other frames; and tpflows can preempt bpflows).

    \item[($c$)] All flows are transmitted in a fully preemptive manner (i.e., any higher priority frame can preempt any lower priority frame).
\end{enumerate}

\begin{table}
  \centering
  \caption{Flow properties}
 
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
ID & Class   & Source & Destination & Period ($\mu$ s) & Deadline ($\mu$ s) & Size (bytes) \\ \hline
1  & express & EP 7   & EP 3        & $5000$           & $150$              & $200$        \\ \hline
2  & express & EP 6   & EP 1        & $10000$          & $200$              & $250$        \\ \hline
3  & tpflow  & EP 2   & EP 9        & $5000$           & $500$              & $300$        \\ \hline
4  & tpflow  & EP 3   & EP 8        & $5000$           & $500$              & $400$        \\ \hline
5  & bpflow  & EP 4   & EP 10       & $1000$           & -                  & $1300$       \\ \hline
6  & bpflow  & EP 1   & EP 8        & $1000$           & -                  & $1300$       \\ \hline
7  & bpflow  & EP 9   & EP 5        & $1000$           & -                  & $1500$       \\ \hline
\end{tabular}
  \label{tab:flows}
  %\includegraphics[scale=0.6]{images/use-case-parameters.PNG}
\end{table}

\vspace{0.1cm}
\noindent $\triangleright$ {\bf Results and discussion.}  Here we report the results we obtained in the experiments. We have tested the safety and tightness of the proposed analysis. We also report the behavior of the network with respect to ``each additional preemption level'' and the ``maximum frame size in each preemption class''. 

%In order to enable a fair comparison, we considered only scenarios in which all tested configurations allow all time-sensitive flows to meet their deadlines.

\vspace{0.2cm}
\noindent $\triangleright \triangleleft$ \textbf{On the tightness of the proposed analysis}.  Table~\ref{tab:result-wctt-synthetic} compares the maximum measured end-to-end delays -- $\mWCTT$ --  with the analytical $\WCTT$ bounds. 

\begin{table}[htb]
\resizebox{\textwidth}{!}{\begin{tabular}{|c|cc|cc|cc|}
\hline
\textbf{Flows} & \multicolumn{2}{c|}{\textbf{$1$-level preemption}}                      & \multicolumn{2}{c|}{\textbf{$2$-level preemption}}                                   & \multicolumn{2}{c|}{\textbf{Fully preemptive}}                          \\ \hline
               & \multicolumn{1}{c|}{\textbf{WCTT ($\mu s$)}} & \textbf{mWCTT ($\mu s$)} & \multicolumn{1}{c|}{\textbf{WCTT ($\mu s$)}} & \textbf{mWCTT ($\mu s$)} & \multicolumn{1}{c|}{\textbf{WCTT ($\mu s$)}} & \textbf{mWCTT ($\mu s$)} \\ \hline
\textbf{$f_1$} & \multicolumn{1}{c|}{$120.00$}                   & $118.00$                    & \multicolumn{1}{c|}{$120.00$}                                & $118.00$                    & \multicolumn{1}{c|}{$104.00$}                   & $101.30$                  \\ \hline
\textbf{$f_2$} & \multicolumn{1}{c|}{$144.00$}                   & $119.70$                  & \multicolumn{1}{c|}{$144.00$}                                & $119.70$                  & \multicolumn{1}{c|}{$148.00$}                   & $119.70$                  \\ \hline
\textbf{$f_3$} & \multicolumn{1}{c|}{$328.00$}                   & $226.56$                 & \multicolumn{1}{c|}{$184.00$}                                & $178.58$                 & \multicolumn{1}{c|}{$148.00$}                   & $140.90$                  \\ \hline
\textbf{$f_4$} & \multicolumn{1}{c|}{$520.00$}                   & $296.16$                 & \multicolumn{1}{c|}{$244.00$}                                & $180.98$                 & \multicolumn{1}{c|}{$248.00$}                   & $180.98$                 \\ \hline
\textbf{$f_5$} & \multicolumn{1}{c|}{$472.00$}                   & $322.20$                  & \multicolumn{1}{c|}{$476.00$}                                & $398.00$                    & \multicolumn{1}{c|}{$384.00$}                   & $384.00$                    \\ \hline
\textbf{$f_6$} & \multicolumn{1}{c|}{$768.00$}                   & $711.00$                    & \multicolumn{1}{c|}{$778.00$}                                & $714.00$                    & \multicolumn{1}{c|}{$780.00$}                   & $716.00$                    \\ \hline
\textbf{$f_7$} & \multicolumn{1}{c|}{$560.00$}                   & $494.95$                 & \multicolumn{1}{c|}{$560.00$}                                & $494.50$                  & \multicolumn{1}{c|}{$560.00$}                   & $495.00$                    \\ \hline
\end{tabular}}
\caption{Results from the synthetic workload: WCTT vs. mWCTT}
\label{tab:result-wctt-synthetic}
\end{table}

Figures~\ref{fig:use-case-simulation-result-1-level}, \ref{fig:use-case-simulation-result-2-level}, and \ref{fig:use-case-simulation-result-multi-level} show the gaps between the measured end-to-end delays and the analytical WCTT values. We can see that all measured end-to-end delays (see the yellow box plots) fall below the corresponding $\WCTT$ (see the red dots) when using the $1$-level preemption scheme (see Figure~\ref{fig:use-case-simulation-result-1-level}), the $2$-level preemption scheme~(see Figure~\ref{fig:use-case-simulation-result-2-level}), and finally the fully preemptive scheme~(see Figure~\ref{fig:use-case-simulation-result-multi-level}).

\begin{figure}[htb]
  \centering
   \includegraphics[scale=0.7]{feupphdteses/sections/analysis/images/new_1_level.png}
  \caption{1-level preemption scheme: Observed end-to-end delay from simulation. Red dots represent WCTT bounds, black are outliers. }
  \label{fig:use-case-simulation-result-1-level}
\end{figure}

\begin{figure}[htb]
  \centering
  \includegraphics[scale=0.7]{feupphdteses/sections/analysis/images/new_2_level.png}
  \caption{2-level preemption scheme: Observed end-to-end delay from simulation. Red dots represent WCTT bounds, black are outliers.}
  \label{fig:use-case-simulation-result-2-level}
\end{figure}

\begin{figure}[htb]
  \centering
  \includegraphics[scale=0.7]{feupphdteses/sections/analysis/images/new_multi_level.png}
  \caption{Fully-preemptive scheme: Observed end-to-end delay from simulation. Red dots represent WCTT bounds, black are outliers.}
  \label{fig:use-case-simulation-result-multi-level}
\end{figure}

\begin{itemize}
    \item Under the $1$-level scheme, the observed gaps between the $\WCTT$ bounds and the $\mWCTT$ for the $f_1$ and $f_2$ express flows are $1.6\%$ ($\WCTT: 120\mu$s, $\mWCTT: 118\mu$s) and $16.25\%$ ($\WCTT: 144\mu$s, $\mWCTT: 119.7\mu$s), respectively. This pessimism stems from the fact that $f_1$ and $f_2$ share the same path as~$f_7$. The gaps between $\WCTT$ and $\mWCTT$ for tpflows $f_3$ and $f_4$ are $30.92\%$ ($\WCTT: 328\mu$s, $\mWCTT: 226.56\mu$s) and $43.05\%$ ($\WCTT: 520\mu$s, $\mWCTT: 296.16\mu$s), respectively. This is due to the fact that tpflows use the same path as bpflows and can be blocked for long periods of time.
   \item Under the $2$-level scheme, both the $\WCTT$ and the $\mWCTT$ remain the same for express flows. However, compared to the $1$-level scheme, there is a significant improvement in the performance of tpflows. The maximum observed delay for $f_3$ and $f_4$ decreased by $21.17\%$ (from $226.56\mu$s to $178.58118\mu$s) and $38.89\%$ (from $296.16\mu$s to $180.98\mu$s), respectively. The $\WCTT$ and $\mWCTT$ gaps for $f_3$ and $f_4$ also decreased by $2.94\%$ ($\WCTT: 184\mu$s, $\mWCTT: 178.58\mu$s) and $16.25\%$ ($\WCTT: 244\mu$s, $\mWCTT: 180.98\mu$s), respectively.
   
    \item Under the fully preemptive scheme, there is further improvement in the performance of express flows and tpflows. In particular, the $\mWCTT$ values of $f_1$ and $f_3$ decreased by $14.1\%$ (from $118\mu$s to $101.3\mu$s) and $21.09\%$ (from $178.58\mu$s to $140.9\mu$s), respectively, compared to the $2$-level scheme. The gaps between $\WCTT$ and $\mWCTT$ for flows $f_1$, $f_2$, $f_3$, and $f_4$ under the fully-preemptive scheme are $2.7\%$ ($\WCTT: 104\mu$s, $\mWCTT: 101.3\mu$s), $17.77\%$ ($\WCTT: 148\mu$s, $\mWCTT: 119.7\mu$s), $4.79\%$ ($\WCTT: 148\mu$s, $\mWCTT: 140.9\mu$s), and $26.22\%$ ($\WCTT: 248\mu$s, $\mWCTT: 180.98\mu$s), respectively. Of note is the slight degradation in the performance of $f_2$ and $f_4$ ($1.67\%$ and $1.10\%$, respectively). This is due to the overhead incurred by the additional preemption operations. From this observation, it follows that a tradeoff must be made between the number of preemption levels allowed for the flow transmissions and the additional overhead introduced by each new preemption level. Note that we can only define up to six intermediate levels of preemption since Ethernet offers a maximum of eight priority classes. %We leave the question of the optimal number of preemption levels for frame transmissions for future work.
\end{itemize}
 
\vspace{0.1cm}
\noindent $\triangleright \triangleleft$ \textbf{On the impact of each additional preemption level.} In Figure~\ref{fig:use-case-analysis-result}, we observe an improvement in the responsiveness of tpflows when an additional preemption level is added to the frame transmission scheme. 

\begin{figure}[htb]
\centering
\includegraphics[scale=0.6]{feupphdteses/sections/analysis/images/use-case-result-analysis-1}
\caption{WCTT for each flow under 1-level preemption, 2-level preemption, and fully preemptive schemes.}
\label{fig:use-case-analysis-result}
\end{figure}

Specifically, this improvement reaches $43.9\%$ (from $328\mu$s to $184\mu$s) and $53.07\%$ (from $520\mu$s to $244\mu$s) for $f_3$ and $f_4$, respectively. The reasons for this trend can be explained as follows. The introduction of the additional preemption level protects $f_3$ and $f_4$ from possible long blocking periods associated with the transmission of~$f_6$ and $f_5$ on their paths. We also note that the overhead introduced by this additional preemption level is negligible: the $\WCTT$ $f_1$ and $f_2$ remain the same for both the $1$-level and $2$-level preemption schemes. The same condition holds approximately for bplfows (i.e., flows~$f_5$, $f_6$, and $f_7$). Here we find a cumulative performance degradation of $1.78\%$, which is negligible for the adopted use case (a degradation from $472\mu$s to $476\mu$s and $768\mu$s to $778\mu$s for $f_5$ and $f_6$, respectively). We also note that some $\mWCTT$ values for $f_5$ and $f_6$ (the black circles) fall outside the whiskers of the box plot. These outliers are the cases where an instance of a flow experiences an unusually high (or low) interference.

Still in Figure~\ref{fig:use-case-analysis-result}, we see an average improvement of $9.6\%$ in the $\WCTT$ of tpflows when we switch from a $2$-level preemption scheme to a fully preemptive approach. This suggests that the performance improvement is not linear, despite the benefits that each additional preemption level brings. On the downside, each preemption level introduces additional hardware implementation overheads that may prove to be non-negligible. This situation raises an open question: What is the optimal tradeoff in terms of the preemption-level scheme to be chosen for flow transmission, given that the performance gain achieved by enabling each additional preemption level is diminished by the associated hardware implementation cost? 
\begin{tcolorbox}
    This question underscores the importance of the configuration framework presented in Chapter~\ref{chap:model-analysis-configuration}, which ensures that only the required preemption levels are activated.  
\end{tcolorbox}


\vspace{0.1cm}
\noindent $\triangleright \triangleleft$ \textbf{On the impact of the frame sizes in each preemption class.} From the use-case setup, the maximum byte size of tpflows is reasonably small in comparison to that of the bpflows. We vary this parameter from $400$ to $1200$~bytes in order to investigate its effect on the $\WCTT$ for each tpflow. The results are reported in Figures~\ref{fig:use-case-analysis-result-perf-comp-1-to-2} and \ref{fig:use-case-analysis-result-perf-comp-1-to-multi}.

\begin{figure}[htb]
  \centering
  \includegraphics[scale=0.8]{feupphdteses/sections/analysis/images/percentage-improvement-from-1-to-2}
  \caption{$2$-level preemption scheme: Performance improvement w.r.t. maximum tpflow frame size.}
  \label{fig:use-case-analysis-result-perf-comp-1-to-2}
\end{figure}%

\begin{figure}[htb]
  \centering
  \includegraphics[scale=0.8]{feupphdteses/sections/analysis/images/percentage-improvement-from-1-to-multi-2}
  \caption{Fully-preemptive scheme: Performance improvement w.r.t. maximum tpflow frame size.}
  \label{fig:use-case-analysis-result-perf-comp-1-to-multi}
\end{figure}


In Figure~\ref{fig:use-case-analysis-result-perf-comp-1-to-2}, we see that the gain in $\WCTT$ obtained by the multi-level preemption scheme over the $1$-level preemption approach decreases with an increase in the maximum frame size. Specifically, the improvement decreases from $43.9\%$ ($328\mu$s to $184\mu$s) to only $7.82\%$ ($614\mu$s to $566\mu$s) for~$f_3$ and from $53.07\%$ ($520\mu$s to $244\mu$s) to $32.3\%$ ($972\mu$s to $658\mu$s) for~$f_4$. This significant impact of frame size on the performance of~$f_3$ can be explained by the increasing blocking time it suffers as the highest priority tpflow. We recall that frames of the same preemption class are transmitted non-preemptively. Therefore, when assigning flows to preemption classes at design time, careful attention must be paid to the maximum possible frame size of each preemption class. It is worth noting that the degradation is less severe when a fully preemptive scheme is adopted, as shown in Figure~\ref{fig:use-case-analysis-result-perf-comp-1-to-multi}. Here, the performance gain over the $1$-level preemption scheme decreased from $54.87\%$ ($328\mu$s to $148\mu$s) to $33.55\%$ ($614\mu$s to $408\mu$s) for flow~$f_3$ and from $52.30\%$ ($520\mu$s to $248\mu$s) to $36.62\%$ ($972\mu$s to $616\mu$s) for flow~$f_4$.

\subsection{Report on a Renault automotive network.} 
\label{sec:evaluation-wctt-renault}

To further evaluate the safety of WCTT bounds, we consider another use-case scenario with a larger network and more flows, provided by Renault and borrowed from~\cite{migge2018insights}. The assumed network topology is shown in Figure~\ref{fig:renault-topology}.

\vspace{0.1in}
\noindent $\triangleright$ {\bf Setup.} The network includes $5$ full-duplex Ethernet switches and $14$ nodes: $4$ cameras (CAMs), $4$ displays (DSPs), $3$ control units (ECUs), and $3$ (functional) domain masters (DMs). The data transmission rate is $100$Mbit/s on all links. Under this assumption, we consider a fully preemptive scheme, i.e., the preemption class of each flow is also its priority. The traffic specification consists of a total of $41$ flows, as shown in Table~\ref{tab:flow-specification}.
\begin{figure}
\centering
\includegraphics[scale=0.9]{feupphdteses/sections/analysis/images/renault}
\caption{Network topology}
\label{fig:renault-topology}
\end{figure}

\begin{table}
    \centering
    \begin{tabular}{ | m{5em} | m{6cm}| } 
        \hline
        Audio streams & -- 8 streams \newline  -- 128 and 256 byte frames \newline -- up to sub-10ms period and deadline \newline -- soft deadline constraints \\ 
        \hline
        Command and Control (C\&C) & -- 11 streams 256 to 1024 byte frames \newline -- up to sub-10ms periods and deadlines \newline -- deadline constraints (hard)\\ 
        \hline
        Video streams & -- 2 ADAS + 6 Vision streams \newline -- up to 30*1446 byte frame each 16ms (60FPS) or each 33ms (30FPS) \newline -- 10ms (ADAS) or 30ms deadline (Vision) \newline -- hard and soft deadline constraints  \\ 
        \hline
        Best-effort: file \& data transfer, diagnostics&  -- 11 streams including TFTP traffic pattern \newline -- up to 0.2ms period \newline -- both throughput guarantees (up to 20Mbits per stream) and deadline constraints (soft) \\
        \hline
    \end{tabular}   
    \caption{Prototype flow specification with the characteristics and performance requirements for each traffic class.}
    \label{tab:flow-specification}
\end{table}

\vspace{0.15in}
\noindent $\triangleright$ {\bf Results and discussion.} Figure~\ref{fig:renault-results} presents the results obtained from the experiments.

\begin{figure}[htb]
\centering
\includegraphics[scale=0.57]{feupphdteses/sections/analysis/images/renault-use-case-results}
\caption{Observed end-to-end delays from simulation for the Renault use-case (in yellow box plots). The blue lines represent the WCTT bounds and the circles represent outlier values.}
\label{fig:renault-results}
\end{figure}

The numerical values are listed in Table~\ref{tab:renault-results}. From Figure~\ref{fig:renault-results} it can be seen that the $\mWCTT$ of all flows are smaller than the computed $\WCTT$ bounds. This also gives further confidence on the safety of the analysis presented in this work. The $\mWCTT$ values of Audio flows -- which are the flows with the highest priority - are on average $65.92$\% lower than the $\WCTT$ values. The $\mWCTT$ values for Command and Control Traffic -- the highest priority traffic after Audio traffic -- are on average $42.84$\% lower than the $\WCTT$ values. Finally, the $\mWCTT$ values for the lower priority flows (Video and Best Effort flows) are on average $36.53$\% lower than the $\WCTT$ values. 
\begin{tcolorbox}
    We found that the distance between the $\mWCTT$ values and the $\WCTT$ values is smallest for the lowest priority flows (Best Effort flows), and that the gap between the $\mWCTT$ and the $\WCTT$ values generally increases as the priority of flows increases. The reason for this is that lower-priority flows are more likely to be exposed to the maximum possible interference, as considered in the analysis.
\end{tcolorbox}
 

%We plan to further investigate this phenomenon with the aim of reducing the pessimism in the $\WCTT$ values of higher priority flows and making the analysis as tight as possible.


\begin{table}
\begin{tabular}{ |p{1cm}||p{1cm}|p{1cm}|p{1cm}|p{1.2cm}||p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|  }
 \hline
 \multicolumn{9}{|c|}{\textbf{mWCTT and WCTT for the Renault Automotive Use-Case}} \\
 \hline
      ID& Src. & Dest. & Size (bytes) & Priority &period ($\mu$s)& Deadline ($\mu$s)& mWCTT ($\mu$s)& WCTT ($\mu$s)\\
 \hline
  1&DM2&DSP1&210&1&5000&5000&72.5&310\\
 2&DM1&DSP1&200&1&5000&5000&95.8&310\\
 3&DM1&DM3&189&0&5000&5000&97.5&136\\
 4&DM2&DSP2&199&1&5000&5000&87.0&363\\
 5&ECU1&DSP2&179&0&5000&5000&77.5&163\\
 6&DM2&DSP2&159&0&5000&5000&75.8&177\\
 7&DM2&DSP2&225&0&5000&5000&115.4&362\\
 8&DM2&DSP1&138&0&5000&5000&59.5&177\\
 9&ECU3&DSP1&240&2&10000&10000&304.0&490\\
 10&ECU3&DM1&170&3&10000&10000&165.2&263\\
 11&ECU3&DM3&239&3&10000&10000&112.6&204\\
 12&ECU2&DSP2&200&2&10000&10000&322.0&499\\
 13&ECU1&DSP2&234&2&10000&10000&252.0&492\\
 14&ECU1&DSP2&214&3&10000&10000&247.0&589\\
 15&ECU1&DSP1&210&2&10000&10000&214.0&442\\
 16&ECU1&DM1&190&3&10000&10000&251.2&289\\
 17&ECU3&DM3&210&2&10000&10000&90.2&133\\
 18&ECU3&DSP1&242&3&10000&10000&167.5&630\\
 19&ECU1&DM1&250&2&10000&10000&121.8&215\\
 20&CAM4&DSP4&1446&5&10000&10000&723.2&1475\\
 21&CAM1&DSP1&1446&5&10000&10000&1304.9&1783\\
 22&CAM4&DSP4&1446&4&10000&10000&382.6&525\\
 23&CAM1&DSP3&1446&4&10000&10000&965.8&1217\\
 24&CAM2&DSP2&1446&4&10000&10000&505.9&1477\\
 25&CAM1&DSP2&1446&4&10000&10000&941.1&1597\\
 26&CAM4&DSP3&1446&5&10000&10000&1208.83&1355\\
 27&CAM4&DSP4&1446&5&10000&10000&1329.6&1475\\
 28&CAM1&DM3&1446&6&10000&10000&1529.7&2341\\
 29&ECU2&DM1&1446&7&10000&10000&1621.1&1939\\
 30&CAM1&DM2&1446&6&10000&10000&1500.6&1880\\
 31&CAM2&DM1&1446&7&10000&10000&1499.8&1518\\
 32&CAM2&DM2&1446&6&10000&10000&1220&1528\\
 33&CAM2&DM3&1446&7&10000&10000&1737.5&3757\\
 34&ECU2&DM2&1446&7&10000&10000&1076.2&1330\\
 35&CAM3&DM3&1446&6&10000&10000&1494.9&1867\\
 36&ECU3&DM1&1446&7&10000&10000&1742.4&1906\\
 37&CAM2&DM1&1446&7&10000&10000&1509.7&1518\\
 38&CAM4&DM1&1446&7&10000&10000&1863.7&2279\\
 39&CAM2&DM2&1446&7&10000&10000&1410.7&2826\\
 40&CAM2&DM3&1446&7&10000&10000&2005.6&3757\\
 41&CAM3&DM3&1446&7&10000&10000&1616.2&3157\\
 \hline
\end{tabular}
  \caption{Results: Renault use-case}
  \label{tab:renault-results}
  \vspace{-3.9pt}
 \end{table}

==> sections/evaluation/configuration-experiment.tex <==
In this section, we evaluate the performance of the priority assignment algorithm and demonstrate the applicability of the preemption class assignment framework. In Section~\ref{sec:evaluation-config-synthetic} we consider a synthetic network and a synthetic workload, and in Section~\ref{sec:evaluation-config-use-cases} we consider two real-world use cases: the SAE automotive benchmark and the Orion Crew Exploration Vehicle (CEV).

\subsection{Evaluation on a synthetic workload.}
\label{sec:evaluation-config-synthetic}
\noindent $\triangleright$ {\bf Setup.} We consider a quad-star topology consisting of six EPs and three TSN switches connected as shown in Figure~\ref{fig:configuration:synthetic-network}.
\begin{figure}[htb]
\centering
\includegraphics[scale=0.9]{feupphdteses/sections/configuration/images/synthetic_small_topology_priority_ass_c}
\caption{Synthetic network with quad-star topology.}
\label{fig:configuration:synthetic-network}
%\vspace{-0.1in}
\end{figure}
The link speeds are assumed to be constant and fixed at $100$MBits/s. In each batch of experiments, we randomly generated 1000 flowsets of equal size, i.e., each flowset has exactly the same number of flows as the others. We varied the sizes between $100$ and $250$ flows per flowset. Each generated flow is characterized by a source, destination, period, deadline, and size. The sources and destinations are randomly selected among the EPs. The values for the periods and deadlines range from $500\mu s$ to $100000\mu s$. The values for the flow sizes range from $64$ bytes to $1500$ bytes. We then assign priorities to the flows using our proposed approach. The priority assignment framework was implemented in Python 3.6, and \href{https://scikit-learn.org/stable/modules/clustering.html}{\texttt{scikit-learn}} -- a free machine learning software library for the Python programming language -- was used for k-means clustering. We compare our solution to DMPO because it is known to outperform most other priority assignment schemes in the literature~\citep{lee2021ml, Davis2016Review}. In addition, DMPO has been specifically recommended for preemptive schemes with fixed priority and preemption thresholds~\citep{Davis2016Review}, a model very similar to the one considered in this work. Since DMPO provides a fully ordered priority list for the flowset and Ethernet only supports up to eight priority levels, we perform greedy bin packing of the ordered flows by assigning the same number of flows to each priority level. Since the exact number of priority levels that gives the best performance with DMPO is not known, we tried all possible numbers of priority levels $k$ (with $1 \leq k \leq 8$) and report the best performance.
\begin{tcolorbox}
    Our main evaluation metric is the schedulability ratio, i.e., the percentage ($\%$) of flows that meet their timing requirement under the priority assignment scheme.
\end{tcolorbox}


To evaluate the schedulability of each scheme, we use the worst-case traversal time (WCTT) analysis presented in Chapter~\ref{chap:model-analysis-configuration}. For both our k-means approach and DMPO, we ran each of the experiments multiple times and then report the average observed performance on schedulability. In the first set of experiments, we assign priorities to the flows using DMPO and k-means, and evaluate the schedulability of the flows under the assumption of a fully preemptive scheme, i.e., a flow can preempt any other flow with a lower priority than itself. In the second set of experiments, we applied our preemption class assignment algorithm to determine the appropriate preemption level for each flowset.

\vspace{0.1in}
\noindent $\triangleright$ {\bf Results and discussion.}
Figure~\ref{fig:configuration:result-synthetic-network} shows the schedulability results under the k-means and DMPO schemes. 

\begin{figure}[htb]
\centering
\includegraphics[scale=0.8]{feupphdteses/sections/configuration/images/synthetic_priority_assignment_result.png}
\caption{Schedulability: K-means vs. DMPO.}
\label{fig:configuration:result-synthetic-network}
\end{figure}

From the figure, it can be seen that k-means is able to schedule a higher number of flows than DMPO. Specifically, the average number of schedulable flowsets ranges from $999.5$ to $981$ for the k-means scheme and from $998$ to $974$ for DMPO.
Figure~\ref{fig:configuration:runtime-synthetic-network} shows the average runtime per flowset for both k-means and DMPO.

\begin{figure}[htb]
\centering
\includegraphics[scale=0.8]{feupphdteses/sections/configuration/images/runtime-synthetic_cropped.png}
\caption{Runtime: K-means vs. DMPO.}
\label{fig:configuration:runtime-synthetic-network}
%\vspace{-0.1in}
\end{figure}

The reported execution times were obtained from a commodity hardware (Intel(R) Core(TM) i7-6500U CPU @ 2.50GHz, 16GB memory). From Figure~\ref{fig:configuration:runtime-synthetic-network} it can be seen that DMPO is much faster than the k-means algorithm. This is due to its complexity.
\begin{tcolorbox}
    The core of DMPO is a sort with complexity $O(nlog(n))$, while k-means is known to have complexity $O(n^2)$~\citep{Pakhira2014Linear}. However, we note that k-means is still quite fast for the priority assignment task with an average runtime of $1.6$s compared to DMPO's $0.79$s for flowsets of $250$ flows each.
\end{tcolorbox}
 

\begin{figure}[htb]
\centering
\includegraphics[scale=0.75]{feupphdteses/sections/configuration/images/preemption_level_sched_bar_cropped.png}
\caption{Schedulability results w.r.t. increasing preemption levels }
\label{fig:configuration:preemption-level-schedulability}
%\vspace{-0.1in}
\end{figure}

 Figure~\ref{fig:configuration:preemption-level-schedulability} shows the schedulability results for the preemption level assignment (Algorithm~\ref{alg:assignment-of-preemption-levels}). The figure shows that the average number of schedulable flowsets increases as the preemption level increases. Specifically, the schedulability ratio jumps from $45.5\%$ under the non-preemptive scheme to $85.8\%$ under the $1$-level preemption scheme, and the trend continues, albeit non-linearly, with each successive preemption level to peak at $98.1\%$ under a fully preemptive scheme. It follows from these observations that the limitations of the $1$-level preemption scheme can result in a non-negligible number of flowsets ($13\%$ in this case) being unschedulable, despite the enormous improvements it brings over the non-preemptive scheme. This problem is circumvented by the multi-level preemption scheme. Note that the improvement over the $4$-level preemption scheme is not significant and/or provides limited benefit in this case. In addition, it is important to recall that each preemption level introduces additional hardware implementation overhead. 
\begin{tcolorbox}
    The configuration framework is useful to evaluate the trade-off between the preemption level scheme to be used and the performance gain from enabling each additional preemption level.
\end{tcolorbox}

Figure~\ref{fig:configuration:runtime-preemption-levels} shows the average runtime per flowset for each preemption level configuration.

\begin{figure}[htb]
\centering
\includegraphics[scale=0.75]{feupphdteses/sections/configuration/images/runtime-preemption-levels_cropped.png}
\caption{Average runtime w.r.t. increasing preemption levels}
\label{fig:configuration:runtime-preemption-levels}
%\vspace{-0.1in}
\end{figure}
From the figure, computing the preemption configuration and evaluating the schedulability of a flowset with $250$ flows under a non-preemptive scheme takes $1.6$s on average. The execution time increases slowly as new preemption levels are added, reaching a peak of $6.21$s on average per flowset under a fully preemptive scheme. This shows that despite the fact that the preemption level algorithm is a guided exhaustive search approach, its execution time is not prohibitive, making the proposed scheme applicable in real-world scenarios.

\subsection{Evaluation on real-life use-cases}
\label{sec:evaluation-config-use-cases}

\noindent $\triangleright$ {\bf Setup.} SAE is the ``SAE automotive communication benchmark'' and Orion is the embedded communication network of the Orion Crew Exploration Vehicle (CEV). The network topologies for the SAE and Orion use cases are shown in Figures~\ref{fig:configuration:SAE} and ~\ref{fig:configuration:Orion}, respectively.

\begin{figure}[htb]
\centering
\includegraphics[scale=0.85]{feupphdteses/sections/configuration/images/SAE_cropped_c.pdf}
\caption{SAE automotive communication benchmark topology~\cite{gavriluct2020traffic}}
\label{fig:configuration:SAE}
%\vspace{-0.1in}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[scale=0.72]{feupphdteses/sections/configuration/images/Orion_cropped_c.pdf}
\caption{Orion CEV network topology~\citep{zhao2017timing}.}
\label{fig:configuration:Orion}
%\vspace{-0.1in}
\end{figure}

In the figures, EPs are represented by rectangles and TSN switches by hexagons. The flow parameters are given by~\cite{gavriluct2020traffic}\footnote{The files for all test cases are available at https://bit.ly/2kpLrKj.}. The link speeds are assumed to be constant and fixed at $100$MBits/s. In the first set of experiments, we assign priorities to the flows using the two priority assignment schemes (k-means and DMPO) and evaluate the schedulability of the flows by assuming a fully preemptive scheme. In the second set of experiments, we applied our preemption class assignment algorithm to determine the preemption level where the number of schedulable flows is the highest.

\vspace{0.1in}
\noindent $\triangleright$ {\bf Results and discussion.}
Table~\ref{tab:priority-experiment-results} shows the schedulability performance of the two priority assignment schemes evaluated. 

\begin{table}[htb]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Name}        & \textbf{EPs }& \textbf{SWs} & \textbf{No. of flows} & \textbf{K-means}& \textbf{DMPO} \\
\hline
SAE       &15& 7   & 79  &97.46 \% & 93.67\% \\
\hline
Orion CEV &31& 15  & 184 & 86.9\% & 80.4\%\\
\hline

\end{tabular} 
\caption{Experimental results from real-life use-cases}
\label{tab:priority-experiment-results}
\end{table}

The table shows that the k-means priority assignment scheme again outperforms DMPO in both use cases. More specifically, k-means was able to schedule $97.46\%$ and $86.9\%$ compared to DMPO's $93.67\%$ and $80.4\%$ for the SAE and Orion networks, respectively. For the SAE benchmark network, the performance of the k-means algorithm in terms of schedulability matches that reported by~\cite{gavriluct2020traffic}, which used a traffic type assignment (TTA) approach to find a feasible schedule. As far as we know, this is the best performance reported in the literature. Figure~\ref{fig:configuration:schedulability-use-cases} shows the behavior of the SAE and Orion setups as the number of preemption levels increases.

\begin{figure}[htb]
\centering
\includegraphics[scale=0.8]{feupphdteses/sections/configuration/images/schedulability_use_cases_cropped.png}
\caption{ \% of schedulable flows w.r.t. increasing preemption levels for SAE and Orion.}
\label{fig:configuration:schedulability-use-cases}
%\vspace{-0.1in}
\end{figure}
From the figure, we see that frame preemption significantly increases the number of schedulable flows for both SAE and Orion. We also note that the number of schedulable flows continues to increase in the Orion use case until it reaches a peak value of $86.9\%$ for a $3$-level preemption scheme. On the other hand, the schedulability of flows in the SAE use case peaks at a $1$-level preemption.
\begin{tcolorbox} 
Observations like these can help system designers to decide the best number of preemption levels to enable for a system at design time and ensure that only the needed preemption levels are implemented.
\end{tcolorbox}





==> sections/evaluation/evaluation.tex <==
\chapter{Evaluation}
\label{chap:evaluation}

In the previous chapter, we proposed a WCTT analysis and configuration framework for the multi-level preemption scheme. In this chapter, we report the results of their evaluations from a quantitative perspective, using synthetic and real-world use cases. In particular, in Section~\ref{sec:analysis:experiment}, we evaluate the safety and tightness of the computed WCTT upper bounds and how they evolve under a multi-level preemption scheme compared to the non-preemptive and $1$-level preemption schemes. We also evaluate the impact of each additional preemption level on the transmission of flows and assess the impact of the frame sizes in each preemption class. In Section~\ref{sec:configuration:experiment}, we evaluate the effectiveness of the priority and preemption class assignment schemes. For this purpose, our main evaluation metric is the schedulability ratio, i.e., the percentage ($\%$) of flows that meet their timing requirements. 

\section{WCTT evaluation}
\label{sec:analysis:experiment}
\input{feupphdteses/sections/evaluation/analysis-experiments.tex}

\section{Configuration framework evaluation}
\label{sec:configuration:experiment}
\input{feupphdteses/sections/evaluation/configuration-experiment.tex}

\section*{Chapter Summary}
\label{sec:evaluation:summary}

In this chapter, we experimentally evaluated the safety of the WCTT bounds and the performance of the proposed framework. Using a realistic automotive use case, we evaluated the performance improvements in terms of worst-case traversal time ($\WCTT$) over the $1$-level scheme. Our results show that the multi-level preemption scheme has an improvement of up to $53.07\%$ in the $\WCTT$ guarantee for preemptable time-sensitive frames. We then demonstrated the safety of the analysis using another use case from Renault. We concluded that the maximum size of each of these flows must be carefully considered when assigning flows to preemption classes at design time. We also discussed the performance improvement achieved by each additional preemption level in the frame transmission scheme. We have shown that, on the one hand, the trend is not linear and, on the other hand, each additional preemption level introduces additional hardware implementation costs that may not be negligible. Our results show that the proposed upper bounds are safe and that the WCTT values of time-sensitive preemptable flows are much lower for a multi-level preemption scheme than for a $1$-level preemption scheme.
\begin{tcolorbox}
    Our results show that the proposed priority-assignment scheme outperforms the DMPO scheme, which is known to dominate most other priority-assignment schemes in the literature. We also show that the proposed framework minimizes the number of preemption levels to ensure schedulability.
\end{tcolorbox}
\noindent This is particularly important since each additional preemption level is associated with significant hardware overheads that can increase the cost of manufacturing switches. Furthermore, our proposed framework demonstrates acceptable scalability for practical use cases. In the next chapter, we consolidate the observed performance improvements by providing routing heuristics to further improve the responsiveness and reliability of frame transmission in TSN.

==> sections/feasibility/feasibility.tex <==
\chapter{From 1-level to Multi-level Preemption}
\label{chap:feasibility}

% \begin{center}
% 	\fbox{\bf
% 		\centering
% 		\begin{minipage}{\linewidth}
% 			\centering
% 			The outcome of the work that has been presented in this chapter titled ``Multi-level preemption in {TSN}: feasibility and requirements analysis'' was accepted at the $23^{rd}$ IEEE International Symposium on Real-Time Distributed Computing\footnote{https://isorc.github.io/2020/}, 
% 			(ISORC'20) held at Nashville, USA.   
% 	\end{minipage}}
% \end{center}


In this chapter, we critically examine the feasibility, overheads, and changes required to enable multi-level preemption in TSN. To investigate the possibility of additional preemption levels, we assume a special case where three frame classes and two preemption levels are considered. In Section~\ref{sec:operational-feasibility}, we explore the dynamics of the $1$-level preemption scheme as defined in the standards to assess the feasibility of enabling more than one level of preemption and propose modifications and implementation recommendations to enable multi-level preemption. We do this at both the frame transmission level (see Section~\ref{sec::feasibility:transmission}) and the reception level (see Section~\ref{sec::feasibility:reception}). We also discuss interoperability (see Section~\ref{sec:feasibility:interoperability}) and frame buffering (see Section~\ref{sec:feasibility:buffering}) in the multi-level preemption scheme. Finally, in Section~\ref{sec:feasibility:implementation-cost}, we quantify the implementation cost of multi-level preemption in terms of hardware overheads and compare this cost with that of other TSN flow control mechanisms. In particular, we discuss the hardware development and comparison metrics (see Section~\ref{sec:implementation:hw-background}), the comparison methodology and context (see Section~\ref{sec:implementation:methodology}), and the evaluation results (see Section~\ref{sec:implementation:complexities}).

\section{Feasibility of Multi-level Preemption}
\label{sec:operational-feasibility}

To achieve multi-level preemption in TSN, it is necessary that the switch nodes are able to identify more than two classes of frames. That is, each switch node in which preemption is enabled should be able to distinguish frames that belong to a different class than the traditional eMAC and pMAC classes. To achieve this goal, we need to extend the definition set of the SMD octet used to determine whether a frame is preemptable or not at the MAC merge sublayer. In this way, it would be possible to further partition the set of preemptable frames. In their current specifications, the standards define $11$ different SMD values~\citep{IEEE802.3br-2016}. These values not only allow the distinction between eMAC and pMAC frames, but also describe the verification frames (i.e., the frames that are sent to determine whether the next node supports preemption). In addition, the current specification of preemption in the standards does not allow frames belonging to the same class to preempt each other~\citep{IEEE802.3br-2016}. To maintain this convention, and especially for interoperability reasons (discussed later in this document), it is important to define an additional MAC Merge sublayer interface to support each additional level of preemption, as shown in Figure~\ref{additional-mac}.

\begin{figure}[htb]
\centering
\includegraphics[scale=0.8]{feupphdteses/sections/feasibility/images/additional-mac}
\caption{Modified MAC merge sublayer with an additional preemptable service interface named \textit{time-sensitive preemptable MAC} (tpMAC). Added features are represented in red color}
\label{additional-mac}
\end{figure}

In this figure, an additional preemptable service interface called \textit{time-sensitive preemptable MAC } (tpMAC) is introduced between the eMAC and pMAC interfaces to handle the so-called \textit{time-sensitive preemptable frames} -- a subset of preemptable frames with firm timing constraints. This ensures that frames of any class can be assigned to a unique MAC merge sublayer interface. In addition, both the \textit{Transmit Processing} and \textit{Receive Processing} functions would need to be modified before multi-level preemption could be enabled. We have described these two processes in detail in Section~\ref{sec:background:preemption}. Therefore, in the following sections, we will focus only on the proposed changes to support multi-level preemption.


\subsection{Frame transmission under a multi-level preemption scheme}
\label{sec::feasibility:transmission}

For frame transmission under a multi-level preemption scheme, we need the SMD values for the verification process. Recall that the current SMD values are defined to inform the sender whether or not the receiver supports frame preemption. However, in the case of multi-level preemption, the receiver requires new SMD values that represent the number of preemption levels that the receiver node supports. Figure~\ref{transmission} illustrates a \textit{Transmit Processing} state diagram to support an additional preemption level that extends the basic $1$-level preemption scheme presented in Figure~\ref{std:frame-transmission}.

\begin{figure}
\centering
\includegraphics[scale=0.72]{feupphdteses/sections/feasibility/images/transmission-11.pdf}
\caption{Modified Transmit Processing state diagram for two-level preemption. Added features are represented in red color}
\label{transmission}
\end{figure}

In this figure, all new proposed transitions and/or modules are marked with red dashed lines. Below is a description of how they work. All labels, functions, and variables are as defined in the standard~(see pgs. 45--48).

\vspace{0.15in}
\noindent $\triangleright$ {\bf On the proposed modifications for enabling an additional level of preemption}.
Adding an additional level of preemption does not require any change to the transmission process of express frames, since we are concerned with the transmission of preemptable frames with firm timing requirements. New states must be added for such frames. In Figure~\ref{transmission}, we define two preemptable MAC merge sublayer interfaces, denoted $p_1$ and $p_2$ (corresponding to tpMAC and pMAC in Figure~\ref{additional-mac}, respectively), and enforce the following rules.

\begin{itemize} 
\item Any $p_1$ frame can preempt any $p_2$ frame, but the converse is not true. 

\item Upon preemption, any $p_2$ frame can continue its transmission only if all pending express and $p_1$ frames/fragments have completed their transmission.

\end{itemize}
With this new preemption level, we must not only check if the receiver node has preemption capabilities, but also check its preemption level ($0$, $1$ or $2$). When a preemptable frame reaches the state $\operatorname{IDLE \_TX \_PROC}$, then the function ($i$)~transitions to the state $\operatorname{START \_PREAMBLE}$ if it is a $p_1$ frame; or ($ii$)~transition to the newly defined state $\operatorname{START \_PREAM}$ $\operatorname{BLE\_2}$ if it is a $p_2$ frame.

\begin{tcolorbox}
In this context, each $p_1$ frame is transmitted in a similar manner to a pMAC frame in the present specification, while each $p_2$ frame is transmitted in such a way that it can be preempted by both express and $p_1$frames. If preempted, the $p_2$ frame is not resumed and sent to completion until all pending express and $p_1$ frames/fragments have been completed.
\end{tcolorbox}

\subsection{Frame reception under a multi-level preemption scheme}
\label{sec::feasibility:reception}

Similar to transmission, adding an additional level of preemption does not require any change to the reception process of express frames. This is because we are only concerned by the reception of preemptable frames with firm timing requirements. For such a frame, new states must be added. The changes are shown in Figure~\ref{reception} with red dotted lines.

\begin{figure}
\centering
%\includegraphics[width=\columnwidth]{images/reception.pdf}
\includegraphics[scale=0.72]{feupphdteses/sections/feasibility/images/reception.pdf}
\caption{Modified Receive Processing state diagram for two-level preemption. Added features are represented in red color}
\label{reception}
\end{figure}

In this figure, we also define two preemptable MAC Merge Sublayer interfaces, denoted $p_1$ and $p_2$, and enforce the following rules.
\begin{itemize} 
\item Any $p_1$ frame can preempt any $p_2$ frame, but the converse is not true.

 \item Upon preemption, any $p_2$ frame can resume its reception only when the reception of all pending express and $p_1$ frames/fragments is complete.
\end{itemize}
With this new preemption level, the receiver node not only confirms that it has preemption capabilities, but also its preemption level ($0$, $1$, or $2$). When a preemptable frame reaches the $\operatorname{CHECK \_FOR \_START}$ state, the function ($i$) transitions to the~$\operatorname{P\_RECEIVE}$ $\operatorname{\_DATA}$ state if it is a $p_1$ frame; or ($ii$) to the newly defined $\operatorname{P2\_RECEIVE \_DATA}$ state if it is a $p_2$ frame.
\begin{tcolorbox}
    In this context, each $p_1$ frame is received in a similar manner to a pMAC frame in the present standard specification, while each $p_2$ frame is received in such a way that it can be preempted by both express and $p_1$ frames. When a preemption occurs, reception of the $p_2$ frame can only continue when reception of all pending express and $p_1$ frames/fragments is complete.
\end{tcolorbox}



At this point, we have described the changes required to enable multi-level preemption. In addition to these changes, there are other important operational factors, i.e., \textit{interoperability} and \textit{frame buffering}, that need to be reconsidered before a full roll-out of nodes with multi-level preemption. We address these issues in the following subsections.

\subsection{Interoperability}
\label{sec:feasibility:interoperability}
In practice, nodes with more than one level of preemption will coexist with other nodes that support only one level of preemption or no preemption at all. This coexistence can be ensured through the verification process in the Transmit Process function mentioned earlier. After a forwarding node sends a verification request to verify that the receiving node supports preemption, the response should include not only that information but also the level of preemption that the node supports. Similar to the $1$-level preemption scheme, multi-level preemption is only enabled if the receiver node supports multi-level preemption.
\begin{tcolorbox}
    If $k$-level preemption (with $k \in \mathbb{N}$) is supported, the forwarding node will transmit the frames in a $k$-level preemptive manner.
\end{tcolorbox}


\subsection{Frame buffering}
\label{sec:feasibility:buffering}
Multi-level preemption requires careful attention to how input buffers are used when receiving incoming frames. We recall that the reception of a sequence of fragments belonging to a preempted frame is completed as soon as two consecutive fragments have a different error-checking code at the receiver node. Once this mismatch occurs, the receiver node assembles the contents of its buffer as a single frame. In the case of multi-level preemption, the mismatch may also result from the reception of a preemptable frame of a higher preemption class. In this case, there are two sets of preemptable frame fragments at the receiver node's input port.

\begin{tcolorbox} We recommend that frames of different preemption classes be received in different input buffers. This would guarantee the integrity of each frame during preemption operations.
\end{tcolorbox}
 

%\section{Introduction}
\label{sec:implementation:intro}
\input{feupphdteses/sections/implementation/sections/introduction}

%
%\section{The TSN Switch Model}
\label{sec:implementation:background}
\input{feupphdteses/sections/implementation/sections/background}
%
%
\input{feupphdteses/sections/implementation/sections/implementation-complexity}



\section*{Chapter Summary}
In this chapter, we examine the transmission and reception functions as currently defined in the standards, and point out necessary changes to allow for an additional level of preemption. We then provide recommendations for interoperability and frame buffering. We also compare the implementation costs of frame preemption with those of TAS and CBS, based on FPGA resource utilization for each of the features. Based on our results, we find that TAS has the highest initial resource utilization among the three features, thereby making it the most expensive to implement. This is even more true when the cost of time synchronization is included. For Frame Preemption, the cost is significantly higher than that of CBS but much lower than that of TAS. When multi-level preemption is implemented according to our specifications, the cost increases linearly. Up to four levels of preemption, they are lower than those of TAS, after which they overtake TAS. We note that this projection does not include the additional overhead of time synchronization software required by TAS. CBS is the cheapest to implement, although it is not able to meet the stringent timing requirements of emerging applications.



==> sections/feasibility/sections/abstract.tex <==
Ethernet is increasingly being considered as the solution to high bandwidth requirements of timing critical applications that make their way in cars, planes or smart factories to mention a few examples. Until recently, Ethernet frames used to be transmitted exclusively in a non-preemptive manner. That is, once a frame starts transmitting on a switch output port, its transmission cannot be interrupted by any other frame until completion. This constraint may cause time critical frames to be blocked for long periods of time because of the transmission of non-critical frames. The IEEE 802.3br standard addressed this issue by introducing a one-level Ethernet frame preemption paradigm, where frames are categorised into two classes depending on their priority levels: the express frames and the preemptable frames. Express frames can preempt preemptable frames and two frames belonging to the same class cannot preempt each other. While this approach partially solves the problem for express frames, some preemptable frames can still suffer long blocking, irrespective of their priority level. In this work, we address this problem by proposing a multi-level preemption paradigm for Ethernet frame transmission where preemptable frames can preempt each other. The feasibility, implementation requirements and timing analysis of the proposed approach are presented in details. 

%

==> sections/feasibility/sections/acknowledgment.tex <==
This work was partially supported by National Funds through FCT (Portuguese Foundation for Science and Technology) and co-financed by ERDF (European Regional Development Fund) under the Portugal2020 Program, within the CISTER Research Unit (CEC/04234).

==> sections/feasibility/sections/benefits.tex <==
% \noindent $\triangleright$ {\bf Benefits}.
The following are the benefits that we envision With the implementation of multi-level preemption:
\begin{enumerate}
    \item The priority inversion problem caused by one-level preemption will be solved.
    \item All frames with a stringent or firm timing requirements will get a clear improvement of their average performance in terms of responsiveness.
    \item Improved schedulability for all time-sensitive flows in preemptive TSN networks. 
\end{enumerate}

% 
% \noindent $\triangleright$ {\bf Costs} The implementation costs of enabling multi-level preemption has been detailed in section~\ref{sec:operational-feasibility}.

==> sections/feasibility/sections/conclusion.tex <==
At this stage of this work, we examined the feasibility of multi-level preemption in Ethernet networks and provided a set of recommendations. Now, we seek to develop a formal worst case transmission delay analysis of frames assuming multi-level preemption and conduct experiments to demonstrate its effectiveness in time sensitive Ethernet networks. An improvement is expected for medium priority frames with affordable preemption overhead in terms of buffer size and SMD definitions.

%A more stable behaviour of express frames is also expected under TSN as having more than one preemption level ensures better QoS for AV traffic.


==> sections/feasibility/sections/experiment.tex <==
As a proof of concept for multi-level preemption, we adopt the same topology and flow characteristics in ~\cite{Thiele2016Formal}. This is to enable comparison with the state of the art. Figure ~\ref{fig:topology} shows the quad star topology of eight nodes and four switches. The nodes and switches are connected by links with different speeds. Table ~\ref{tab:flows} presents the description of the flows for the experiment. There are three traffic classes: (1) control data traffic (CDT), (2) general control traffic (GCT), and finally (3) camera traffic (CAM). CDT traffic corresponds to latency critical traffic (corresponds to the red frames in figure ~\ref{image1}) and has the highest priority. GCT also have latency requirements but with much less critical constraints (corresponds to the black frames in figure ~\ref{image1} and is our main focus of improvement) and CAM traffic are large frames with more relaxed latency constraints (corresponds to the green frames in figure ~\ref{image1}). Unlike ~\cite{Thiele2016Formal} which assumes two level preemption however, we assume three levels of preemption. Here, CDT can preempt both GCT and CAM traffic. GCT can also preempt CAM traffic. Table ~\ref{tab:flows} also describes the minimum and maximum payloads and periods for each traffic class. In addition, the table describes how traffic is transmitted either to a single destination (unicast), multiple destination (multicast) or all destinations (broadcast). The notation n(d) for multicast transmission implies that there are n multicast streams to d destinations. 

\begin{figure}
\centering
\includegraphics[scale=0.6]{feupphdteses/sections/chapter-2/images/topology.png}
\caption{Netowrk topology from ~\cite{Thiele2016Formal}}
\label{fig:topology}
\end{figure}

\begin{table}
    \centering
    \begin{tabular}{|p{2cm}||p{1.2cm}|p{2cm}|p{1.5cm}|}
         \hline
            & CDT & GCT &CAM  \\ 
        \hline
        Unicast & 8 &18 & 3\\
        Multicast & 2(2) & 11(2), 4(3)1(4) & 1(2)\\
        Broadcast &  0 &   6 &  0 \\ 
        \hline
        Payload (bytes) & [14, 144] & [1, 250] & [875, 1400]  \\ 
        \hline
        Average (bytes) & 70 & 50 & 1231  \\ 
        \hline
        Period & 5ms & [10ms, 1s] & [100us, 1ms]  \\ 
        \hline
        Average  & 5ms & 230ms & 440us  \\ 
        \hline
    \end{tabular}
    \label{tab:flows}
    \caption{The network flow properties}
\end{table}





==> sections/feasibility/sections/feasibility.tex <==

To achieve multi-level preemption, it is important, firstly, that the switch nodes can identify more than two classes of frames (eMAC and pMAC frames). At the MAC merge sublayer where preemption occurs, identification of the preemptive transmission class of a frame is done using the frame header (SMD). The standards currently define 11 values for the SMD \cite{IEEE802.3br-2016}. These values describe frame headers for verification (frames sent to determine if the next node supports preemption), express and preemptable frames. By adding additional definitions to distinguish different levels of the preemptable frame class, it would be possible to assign preemptable frames into different MAC merge sublayer (see Fig.~\ref{Image6}) interfaces based on their priorities specified by the new SMD values. 

Also, the current frame preemption specification does not allow frames of the same MAC merge sublayer interface to preempt each other \cite{IEEE802.3br-2016}. To keep this convention, and especially for the sake of interoperability (which will be discussed later), it is required to define an additional MAC Merge sublayer interfaces to support each additional preemption level. This ensures that frames of each preemption priority class can be assigned to a unique sub layer with clearly defined preemption priority levels.
% An approach to this would have been to allow frames from the same interface to preempt each other. We consider this approach less desirable because it does not conform to the way preemption is implemented in the standards. In the IEE802.3br ~\cite{IEEE802.3br-2016}, preemption occurs at the pMAC when an interrupt is generated by the eMAC interface (a higher priority interface). Allowing the same interface to interrupt itself would affect interoperability.
The Transmit Processing function, which receives frames from the MAC sublayer interfaces, would also need to be extended to support multi-level preemption. The current verification procedure in the function (only) checks if preemption is supported  by the next node. To achieve this, the Transmit Processing function of the forwarding node sends a request frame to the receiving node to inquire if it supports preemption. The receiving node, in return, sends a response. This response is interpreted (based on the SMD value of the response frame) by the forwarding node to determine if preemption is supported by the receiving node or otherwise. Newly defined SMD values for the response packet, when added to the standard definitions, can be used to inform the forwarding node, of not just whether the receiving node supports preemption or not, but also the level of preemption it supports. Preemptive frame transmission can then begin after this verification process. A Transmit Processing state diagram to support 2-level preemption, which is an extension of the Transmit Processing state diagram in \cite{IEEE802.3br-2016} (see pg. 50) is shown in Fig.~\ref{transmission}. All labels, functions and variables are as defined in \cite{IEEE802.3br-2016} (see pg. 45-48). As shown in the state diagram, from the idle state (when the node is not transmitting any frame), the frame can transmit verification frames and express frames in the same manner as specified in ~\cite{IEEE802.3br-2016} -  the frames are transmitted in a non-preemptive manner and the process returns to the idle state. For preemptable frame, however, there is a slight modification in the process. The frames are characterised, based on their SMD into level 1 (p1) or level 2 (p2) preemptable frames and are assigned to different MAC sublayer interfaces for transmission. Here we define p1 and p2 interfaces as variants of the p interface defined already in the standard. We assume that the p1 interface can preempt the p2 interface. The frame transmission of p1 and p2 interfaces are similar to those of the p interface as defined in the standards except in that; (a) p1 can preempt p2’s transmission,(b) after the transmission of p1, it does not return to a state that checks if there are p2 frame fragments to be transmitted, before transitioning into the idle state, and (c) p2 can correctly resume the transmission of its fragments after preemption by a sequence of express or p1 frames/fragments.   

\begin{figure*}
\centering
%\includegraphics[width=\columnwidth]{images/transmission-1.pdf}

\includegraphics[scale=0.7]{feupphdteses/sections/chapter-2/images/transmission-1.pdf}
\caption{Modified Transmit Processing state diagram for two-level preemption. Added features are represented in dotted lines}
\label{transmission}
\vspace{-0.2in}
\end{figure*}

At the receiving node,  preemptive reception commences when the receiving node has received the verification request and has confirmed that it supports preemption. The xMII, which currently separates express frames from preemptable frames would also need a slight modification to recognise other preemption levels. With new SMD values defined, the xMII can be easily configured to separate frames into respective preemption levels. This paves way for preemptive frame reception at the node. Also, a Receive Processing state diagram to support 2-level preemption and ensure correct reception of all frames is shown in Fig.~\ref{transmission}. It is an extension of the Receive Processing state diagram in \cite{IEEE802.3br-2016} (see pg. 51). All labels, functions and variables are as defined in \cite{IEEE802.3br-2016} (see pg. 45-48). 

From the figure, the Receive Processing  construct starts from the idle state. When a frame is received, the header of the frame is checked to determine the frame type. Verification and express frames are received in a non-preemptive manner like in ~\cite{IEEE802.3br-2016}. If the header inspection detects a preemptable frame, it transits to the “REPLACE\_SMD” state where the frame SFD is replaced with SMD values that correspond to its preemption priority levels. Level 1 (p1) and level 2 (p2) preemptable frames are received via different interfaces. The reception of an express frame can preempt the reception of either of the two preemptable frame classes. Also, p1 frames can preempt the reception of p2 frames and p2 frames can correctly resume their reception after having being preempted by express or p1 frames

\begin{figure*}
\centering
%\includegraphics[width=\columnwidth]{images/RECEPTION-1.pdf}
\includegraphics[scale=0.7]{feupphdteses/sections/chapter-2/images/RECEPTION-1.pdf}
\caption{Modified Receive Processing state diagram for two-level preemption. Added features are represented in dotted lines}
\label{reception}
\vspace{-0.2in}
\end{figure*}

Ethernet frame preemption standards do not specify the buffer mechanism to store received frames of both express and preemptable frames. In the case of multi-level preemption, however, careful attention must be paid to how the input buffers are used to receive incoming frame. As already mentioned in chapter \ref{chap:Chapter4}, a preemptable frame is considered to be completely received when there is a mismatch in the MCRC of the preemptable fragments. The receiving node transmit the content of its buffer as a single frame once this mismatch occurs. In the case of multi-level preemption, however, the mismatch may occur due the reception of a higher priority preemptable frame. In this case, there will be two set of preemptable frame fragments at the input port of the receiving node. We recommend that frames of different priority levels should be received in different input buffers. This guarantees the integrity of each frame during preemption operations. 

Switches that support multi-level preemption can also inter-operate with switches that support one-level preemption and those that do not support preemption at all. This is achieved by the verification process mentioned earlier in the Transmit Process function. After a forwarding node sends a request to verify if the receiving node supports preemption, the reply from the receiving node indicates whether or not the node supports preemption and also what level of preemption the node supports. As is the case with nodes that support 1-level preemption, preemption capability is only enabled if the next node supports preemption. Otherwise, preemption is disabled and the node forwards the frame in a non-preemptive manner. Similarly, multi-level preemption, is only enabled if the receiving node also supports multi-level preemption. If the receiving node only supports 1-level preemption, the forwarding node  will then transmit frames in a 1-level preemptive manner. 








%We note some initial observations on the feasibility of multi-level frame preemption from the implementation requirements and the traffic behaviour viewpoints.
%\subsection{Requirements for Multi-Level Preemption Support}
%If an Mframe containing SMD-Sx (signalling the start of the transmission of a new preemptable frame) arrives at a node and Receive processing has not completed the reception of  a previous preempted frame, Receive processing ensures that the MAC detects a ``FrameCheckError'' in the partially received frame (see~\cite{IEEE802.1Q-2014}, page~44). This mechanism implies that the node can detect the start of another preemptable frame, which is important to support multi-level preemption. Although the start of another preemptable frame would be flagged as an error, the IEEE 802.3br standard states that other techniques may be employed to respond to an incomplete frame transmission as long as the MAC behaves as though a FrameCheckError occurred. This submission opens the door to multi-level preemption specification, while still conforming to the standard. To this end, we recommend the specification of a mechanism to ensure the transmission of a frame in a higher preemption class without jeopardizing the integrity of the preempted frame. This operation should be performed such that the receiver node/switch correctly resumes the reception of the preempted frame later on.

%The standards do not describe any mechanism to reassemble more than one frame in a buffer. We recommend the specification of such a mechanism to enable multi-level preemption as the buffer must be able to correctly reassemble and transmit a second frame, while already containing fragments of a first frame. In addition, the xMII that separates express frames from preemptable frames can be configured to distinguish between different priority levels for preemptable frames. As such, no additional frame filtering mechanism would be required for multi-level preemption.

%We believe that the current preemptable frames format in the standards~\cite{IEEE802.3br-2016} is sufficient to handle multi-level preemption. To this end, we recommend that new values be defined for the one octet SMD contained in the header (See Fig.~\ref{Image7}) to support more preemption levels. The standard currently defines eleven values for this octet. Additional values can be defined to check the level of preemption supported by the next node and to indicate the frame preemption levels.

%\subsection{Interoperability}
%We believe that a switch node supporting multi-level preemption can interoperate with those supporting only one-level or no preemption at all. With the new recommended SMD values, the MAC merge sublayer will be able to verify if the next node supports preemption and if this is the case, how many levels are supported. If just one level of preemption is supported, then all preemptable frames are transmitted on a single pMAC interface and multi-level preemption is disabled. In this case, all non-express frames are treated as preemptable frames and will not preempt each other. In the case preemption is not supported at all, frames are transmitted as already specified in the {IEEE}~802.1Q standards. 

%\subsection{Timing Behavior of Medium Priority Frames}
%We observed that the end-to-end transmission delays of express frames remain the same in both one-level and multi-level preemption conditions. However, it was also observed that mpFrames can be blocked for long periods by preempted bpFrames under one-level preemption where they both share the pMAC interface. % By allowing a second level of preemption that enables mpFrames to preempt bpFrames, there is a significant improvement in the end-to-end transmission delays of mpFrames.  An illustration of this observation is presented in Fig.~\ref{image4} where mpFrames preempt bpFrames and are transmitted more promptly to achieve better response times compared to one-level preemption.  This observation can be extended to provide a better QoS for non-express scheduled traffic, depending on the application.
%
%\begin{figure}
%\centering
%\includegraphics[width=\columnwidth]{Image4.png}
%
%\caption{Frame transmission under Multi-level preemption compared to 1-level preemption.}
%\label{image4}
%\vspace{-0.2in}
%\end{figure}
%
%
%In TSN, one-level preemption poses the same challenge as in standard Ethernet in that AV traffic can be blocked by a large lower priority frame. As shown in Fig.~\ref{fig_first_case}, when a lower priority frame is the last preempted frame before the protected window, then the preempted frame has to resume first; even in the presence of AV traffic and positive Credits for transmission. Failure to transmit a preempted lower priority frame leave the system at the risk of a non-preemptive transmission of AV traffic with a reduced guard band. This can cause interference with the protected traffic and disrupt the whole transmission flow. The situation is illustrated in Fig.~\ref{fig_second_case} where AV frames are transmitted instead of resuming a preempted lower priority frame thus leading to an AV frame interfering with a protected window as a second preemption cannot take place. Allowing multi-level preemption solves this problem.
%\begin{figure}[!ht]
%\centering
%\subfloat{\includegraphics[scale=0.6]{Image2.png}
%%\caption{}
%\label{fig_first_case}}
%\hfil
%\subfloat{\includegraphics[scale=0.6]{Image3.png}
%\label{fig_second_case}}
%\caption{a: Lower priority frame blocking AV frames due to 1-level preemption. b: AV traffic interfering with Protected window because it cannot be preempted}
%%\label{fig_tsn}
%\vspace{-0.2in}
%\end{figure}


==> sections/feasibility/sections/introduction.tex <==
 In this chapter, we critically examine the operational feasibility and required modifications to allow multi-level preemption. Specifically, we investigate dynamics of one-level preemption as currently specified in the standards to evaluate the possibilities of allowing more than one level of preemption . We use three levels of priorities and 2~levels of preemption to investigate the feasibility of multi-level preemption in Ethernet. Finally, we propose some required modifications and implementation recommendations for enabling multi-level preemption. 
 

==> sections/feasibility/sections/problem_statement.tex <==
We consider a network traffic consisting of $n$~streams $s_1, s_2, \ldots, s_n$  partitioned into traffic classes: \textit{express traffic}, \textit{ preemptable traffic}. Express traffic frames have very strict timing requirements. Frames from this traffic class are reffered to as \textit{express frames}. Preemptable traffic frames are divided into two sub-classes: \textbf{Medium Priority Preemptable traffic} (mpFrames) which although have stringent timing constraints, but are not as strict as those of express traffic frames and the \textbf{Best Effort Preemptable traffic} (bpframes) with no timing constaints at all. A Stream $s_i$, with $i \in [1,n]$, consists of a potentially infinite number of frames $s_i^j$ ($j \ge 1$) with an inter-arrival time of at least $T_i$ units between two consecutive frames. Frame $s_i^j$ is characterised by its arrival time $a_i^j$ and its size $c_i^j$.  We assume that each stream is assigned a unique fixed priority and all frames generated from this stream inherit its priority. We also assume that any express frame has a higher priority than all preemptable frames and the following constraints are enforced:
\begin{enumerate}
\item[$\triangleright$]  Any express frame can preempt all preemptable frames,
\item [$\triangleright$] Any mpFrame has higher priority than all bpFrames and therefore, can preempt these,
\item[$\triangleright$]  Frames from the same class cannot preempt each other.
\end{enumerate}

%\begin{figure}
%\centering
%\includegraphics[scale=0.7, width=\columnwidth]{Image8.png}
%
%\caption{A receiving node that supports multi-level preemption.}
%\label{Image8}
%\vspace{-0.2in}
%\end{figure}
With the above assumptions and constraints, we investigate the feasibility of using multi-level preemption to limit the blocking of non-express traffic with strict timing constraints (mpFrames) by less important frames(bpFrames) in Ethernet networks. 
%With the above assumptions and constraints, frame transmission simulation is then carried out under an ethernet frame transmission scheme with multi-level preemption that ensure that medium priority frames are not blocked by lower priority frames. A benchmark simulation that assumes just one-level preemption is also carried out. The objective is to compare the delay experienced by frames of each traffic class under the two conditions. The simulation experiment will be carried out for both Standard Ethernet and TSN networks and a formal Compositional Performance Analysis to estimate the worst-case transmission Time of frames will be presented.

==> sections/implementation/implementation.tex <==
%\usepackage[inline]{trackchanges}
%\addeditor{APR}
%\addeditor{VGA}
%\addeditor{MAO}

\section{Implementation Cost}
\label{chap:Implementation}

% \begin{center}
% 	\fbox{\bf
% 		\centering
% 		\begin{minipage}{\linewidth}
% 			\centering
% 			The outcome of the work that has been presented in this chapter titled ``Implementation Cost Comparison of TSN Traffic Control Mechanisms'' was accepted at the $26^{th}$ {{IEEE International Conference}} on {{Emerging Technologies}} and {{Factory Automation}} \footnote{https://2021.ieee-etfa.org/}, 
% 			(ETFA'21) held at Vasteras, Sweden.   
% 	\end{minipage}}
% \end{center}

In the previous chapters, we have extensively discussed the feasibility of multi-level preemption. In this Chapter, we provide a
comparison of the implementation
cost of the Multi-level preemption scheme to other TSN traffic control mechanisms. This comparison can help system designers in choosing which of the mechanism(s) to deploy for their applications. The rest of the chapter is organized as follows. First, we provide the motivation for the implementation cost comparison in Section~\ref{sec:implementation:intro}. Section~\ref{sec:implementation:background} provides context by describing the relevant TSN switch components and the traffic control features that were adopted for this comparison.
Section~\ref{sec:implementation:hw-background} provides an introduction to hardware implementations, metrics and
methodology used.
Section~\ref{sec:implementation:complexities} presents the results and
Section~\ref{sec:implementation:related_work} outlines related work.
Finally, Section~\ref{sec:implementation:conclusion} concludes this Chapter.  


%\section{Introduction}
\label{sec:implementation:intro}
\input{feupphdteses/sections/implementation/sections/introduction}

%
%\section{The TSN Switch Model}
\label{sec:implementation:background}
\input{feupphdteses/sections/implementation/sections/background}
%
%
\input{feupphdteses/sections/implementation/sections/implementation-complexity}


%\clearpage
\section{Related work}
\label{sec:implementation:related_work}
\input{feupphdteses/sections/implementation/sections/related-work}

%
\section{Chapter summary and conclusion}
\label{sec:implementation:conclusion}
\input{feupphdteses/sections/implementation/sections/conclusion.tex}







==> sections/implementation/sections/abstract.tex <==
The IEEE Time-Sensitive Networking (TSN) Task Group specifies a set of
standards that enables real-time communication with predictable and bounded
delays over the Ethernet. Specifically, TSN introduces a new set of so-called
\emph{shapers}, which regulate traffic arrival and transmission in the networks.
Prominent among those are the IEEE 802.1 Qbv Time Aware Shaper (TAS) and
IEEE 802.1Qav Credit-Based Shaper (CBS).
Another traffic control mechanism is the IEEE 802.1Qbu Frame
Preemption. Most works in the literature have focused on the quantitative
performance comparison between these mechanisms. However, the discussion on how
they compare in terms of implementation cost has received less attention.
In this paper, we provide a comprehensive
comparison of the implementation
cost of the aforementioned TSN traffic control mechanisms.
This comparison can help system designers in choosing which of the mechanism(s)
to deploy for their applications.

%Such a discussion would guide system designers

==> sections/implementation/sections/acknowledgment.tex <==
This work is partially supported by Comcores ApS and Innovationsfonden Denmark through grants 8053-00031B and 9066-00048B; and also by National Funds through FCT/MCTES (Portuguese Foundation for Science and Technology), within the CISTER Research Unit (UIDB/04234/2020).


==> sections/implementation/sections/background.tex <==

% \subsection{TSN Switch}
% A TSN network consists of nodes, which are either end systems and switches. An end system can be any device that sends and/or receives data over the network, such as an ECU,  Camera, Radar, or Lidar. Switches are intermediate nodes between end systems, and they usually do not generate traffic. Any two nodes are connected by a full-duplex link, that is characterized by \textit{speed} -- the maximum rate at which it can transmit data.
% \label{switch-model} 

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{feupphdteses/sections/implementation/Images/tsn-switch.pdf}
%     \caption{Example block diagram of a TSN switching system}
%     \label{fig:tsn-switch}
%     \vspace{-0.1in}
% \end{figure}

% An Ethernet switch that supports one
% or more TSN features is referred to as a \textit{TSN switch}. Again, in this chapter,
% we consider three TSN features: ($1$)~Frame Preemption($2$)~the Time-Aware Shaper (TAS) and
% ($3$).~the Credit-Based Shaper (CBS).

% In the block diagram presented in Fig.~\ref{fig:tsn-switch}, the frames flow through the TSN MAC (supporting frame preemption),
% are processed in the ingress processing block, then moved to the egress processing block via the switch fabric. After that, they are queued at the output and await servicing. This is where the TSN shapers provide control data to the queue management system. When selected for transmission, they exit through the egress processing path of the TSN MAC. In addition to being a well-designed piece of hardware, a TSN switch has to be configured appropriately to meet the traffic requirements. This configuration process falls under the responsibility of Control and Management (C\&M) planes. The exact description of C\&M planes can be found in~\citep{rfc7426}. According to this document, the control plane ``instructs network devices (...) how to process and forward packets''; while the management plane ``monitors, configures and maintains'' ports of the network node. The data plane contains all functions responsible for handling the traffic directly. In Fig.~\ref{fig:tsn-switch}, the ingress and egress processing blocks extract header information, which is then used by the lookup engine to make forwarding decisions. The TAS and CBS blocks exchange the control information with the queue management block, 
% influencing when the frames are dequeued. This can be directly mapped to the transmission selection function of the forwarding process from~\cite{IEEE-Std-802.1Q-2018}. Correct operational parameters must be set apriori to ensure consistent shaping across the network. Since the shaping functions do not depend on the transmitted data itself, they can be classified as belonging to C\&M planes.

%\subsection{TSN traffic}
%Data traffic in networks can be usually divided into flows, where a flow is a sequence of frames sent from a source end-system to one or more destination end-systems, through a set of TSN switches. Generally, flows can be further classified as either \emph{periodic} or  \emph{aperiodic}~\citep{buttazzo2011}. In TSN networks, the emphasis is placed on periodic flows, for which \emph{flow-instances} (a single frame or a small burst) are produced recurrently at the source, and are separated by a predefined time interval (\emph{period}). Flows in TSN networks must also meet timing constraints. The most common one of those is the \emph{deadline}, which imposes a maximum \emph{end-to-end delay} for all frames belonging to a flow. Another common requirement is the \emph{end-to-end delay variation}, commonly referred to as \emph{jitter}. A multitude of flows can exist in a network, but treating each of them differently would require fine classification resolution, and therefore high (and expensive) processing capabilities in each network node. Consequently, in TSN, the flows with similar QoS and timeliness requirements are grouped in traffic classes. In IEEE 802.1Q, there exist up to eight traffic classes. Each of the aforementioned flows must be mapped to a traffic class. At each switch, flows are further mapped to Internal Priority Values (IPV), and then to actual egress queues.




==> sections/implementation/sections/conclusion.tex <==
In this chapter, we compare the implementation cost  of frame preemption with that of TAS and CBS. The aim of this comparison is to guide system designers on the choice of the TSN feature to adopt, provided that the temporal performance requirements are met. The cost comparison is based on FPGA resource utilization for each of the features. From our results, we observe that TAS has the highest starting resource utilization among the three features, thereby making it the most expensive to implement. It is even more so, if costs of achieving time synchronization are included.
The CBS is the cheapest to implement. For frame preemption, while the cost is significantly higher than that of CBS, it is very much lower than that of TAS. If multi-level preemption is implemented according to the recommendations of Chapter~\ref{chap:feasibility}, the cost grows linearly. It is less than TAS for up to four levels of preemption, after which it overtakes TAS. We note that this projection does not include the additional overhead of time synchronization software, which is required by TAS.

%For future work, comparison of the implementation cost of more TSN flow control features can be considered. Here, the features such as ATS and Cyclic queuing and forwarding are the prime candidates. Additionally, the overhead of integrating these features together is also worth investigating.
% \add[APR]{
%Finally, extending the comparison for different FPGA vendors and device families would make the results more generalizable.



==> sections/implementation/sections/implementation-complexity.tex <==
\subsection{Hardware development and comparison metrics}
\label{sec:implementation:hw-background}

To compare the cost of a hardware implementation of TAS, CBS, and Frame Preemption, we use resource utilization reports for hardware modules executing the flow control features. These modules are implemented in Xilinx FPGA devices. The reports are obtained during the digital design process (described in Section~\ref{sec:hwdev}) and include the number of basic hardware blocks (described in Section~\ref{sec:xil-res}) required for the implementation of each feature.
%Section~\ref{sec:implementation:methodology} then describes the comparison methodology, and finally, Section~\ref{sec:implementation:complexities} presents the results.

\subsubsection{Digital design process}
\label{sec:hwdev}

The TSN modules are implemented as Register Transfer Level (RTL) Silicon Intellectual Property (IP) Cores. The source code of these IP cores, written in a Hardware Description Language (HDL), is then processed by Computer-Aided Design (CAD) tools \citep{brown2014} to:
\begin{enumerate} \item express the design with logic gates (\textit{logic synthesis}), \item map the obtained logic circuit to components specific to a particular implementation technology, and then place and route them on either a silicon wafer or a subtype of Programmable Logic Devices (PLDs) \textit{(physical design)}.
\end{enumerate}
 
One of the outputs of the \textit{physical design} is the \textit{size} of the implemented module. For Application Specific Integrated Circuits (ASICs), the physical design maps the logic circuitry to cell libraries, and the end result for size is simply an area on a wafer. 
\begin{tcolorbox}
    In FPGAs, which are a subtype of PLDs, the devices already have a fixed number of resources that the circuit is mapped to. The size is then expressed as the number and type of resources used.
\end{tcolorbox}


\subsubsection{Xilinx FPGAs}
\label{sec:xil-res}

At a high level, a basic FPGA device consists of Logic Blocks, Programmable  Interconnect, and I/O pins \citep{brown2014}.
In Xilinx devices, the key resources used to implement sequential and combinational circuits are Configurable Logic Blocks (CLBs). These blocks contain Look-Up Tables (LUTs) ( an n-input truth table) for combinatorial logic and memory elements for sequential logic (CLB registers). The CLBs also contain dedicated carry logic for arithmetic operations (CARRY8) and Multiplexers (FnMUX) to maximize resource utilization within a block. For more information on FPGA resources as well as modern FPGA architecture, we refer the interested reader to~\citep{xilinx-ug574, xilinx-ds890}.
In addition to CLBs, some FPGA devices contain specialized blocks and hard IPs (non-programmable modules that perform a specific function, such as transceivers). These specialized blocks include:
\begin{itemize}
 \item Block Random Access Memories (BRAM), which contain arrays of Static RAM (SRAM) cells and sometimes FIFO logic, \item Digital Signal Processing (DSP) blocks, which are used to perform more complex arithmetic operations, 
\item Clock tiles, which contain primitives for clock generation and buffering.
\end{itemize}
\begin{tcolorbox}
   All of our synthesis runs were performed for the Xilinx Zynq UltraScale+ family device \texttt{xczu9cg-ffvb1156-1-e}, as this device is used in the popular ZCU102 boards. 
\end{tcolorbox}

\subsection{Comparison methodology and context}
\label{sec:implementation:methodology}

To accurately contextualize the costs added by each TSN feature, we have chosen an absolute baseline to be the whole \texttt{xczu9cg-ffvb1156-1-e} device. We note that a basic switching system without TSN features could also be used for this purpose. However, since the size of a switching system can vary significantly across different architectures and configurations, the entire FPGA device is a better reference point.
We also compare the TSN features with each other. This comparison is enabled by a weakly coupled and modular design. In such a design, the queuing and buffer systems are common for TAS and CBS. Therefore, the memories and logic in them can be excluded from the comparison. In contrast, the comparison of Frame Preemption and TSN Shaper presents an additional challenge. The TSN MAC must have some buffer capacity at the receiver nodes to correctly reassemble the frame fragments. The size of these buffers depends on the maximum frame size, but we assume that it is minimal compared to the buffers in the switch output buffers (queues). Therefore, the buffers in the TSN MAC are also excluded from the comparison.


The results obtained have the disadvantage that they only approximate the NRE cost by capturing the final \textit{size} of the product. They do not capture the RE costs associated with testing each chip. This approximation is made possible by the assumption that the larger the device, the longer and more difficult the development. This assumption is at odds with the fact that the optimization phase of development aims to reduce area/resources. When a significant amount of development effort is put into this phase, the result is a \textit{smaller} device. Nevertheless, it can be assumed that the degree of optimization is similar within an organization, so we can use the resource utilization reports for our comparison.

\subsection{Evaluation results}
\label{sec:implementation:complexities}
In this section, we describe the implementations of CBS, TAS, and ( multi-level ) preemption and provide the associated resource utilization numbers are given. Specifically, we first describe the implementation of CBS and TAS (see Section~\ref{sec:feasibility:cbsTasImplementation}) and discuss their resource utilization (see Section~\ref{sec:feasibility:cbsTasUtilization}). We then describe the implementation and resource utilization of multi-level preemption (see Section~\ref{sec:feasibility:preemptionImplementation}). The implementations themselves are proprietary and are therefore only presented at a high level of abstraction.

\subsubsection{CBS \& TAS Implementations}
\label{sec:feasibility:cbsTasImplementation}

A functional block diagram of TAS and CBS is presented in Figure~\ref{fig:shapers}. 

\begin{figure}[htb]
    \centering
\includegraphics{feupphdteses/sections/implementation/Images/shapers.pdf}
    \caption{TAS and CBS block diagram}
    \label{fig:shapers}
\end{figure}

In this figure, the \textit{configuration register bank} (separate for TAS and CBS) contains all the necessary run-time configurable registers and interface implementations so that both TAS and CBS modules can be managed by external software. The \textit{CBS controller} implements the CBS algorithm and performs credit bookkeeping based on the current configuration and transmission status provided by the queuing system. CBS provides the \textit{transmission allowed} flag for each supported priority, which is then used by the queuing system to select frames for transmission. For credit management, CBS needs information about the current \textit{queue state} and \textit{transmission status.} 


TAS provides the \textit{gate state} and \textit{gate guard} control signals to the queue management system. The \textit{gate guard} control signal enables the use of fixed guard bands (as defined in Annex Q of IEEE 802.1Q~\citep{IEEE-Std-802.1Q-2018} and in Section~\ref{sec:background:tas}). This implementation of the guarding feature calculates how long the gate remains open, which is necessary to prevent transmission window overrun errors.
 
In addition, TAS contains a memory holding Gate Control Lists (GCL).
By default, this memory is mapped to BRAMS. However, we can accurately estimate its size in bits based on the number of supported priorities and the number of supported entries. This estimate is shown in Equation~\ref{eq:tas-mem}, where $M$ is the memory size in bits, $n$ is the number of supported GCL entries, $\mathrm{ TI }_\mathrm{width}$ is the bit size of the time interval entry, and $N_\mathrm{IPVs}$ is the number of supported priorities~\citep{Pruski2021Implementation}.

\begin{equation}
M = 2 \times n \times (\mathrm{ TI }_\mathrm{width} + N_\mathrm{IPVs})
\label{eq:tas-mem}
\end{equation}

Finally, TAS requires a synchronized Time of Day (ToD) to be available in the system. This is illustrated by the \textit{tod provider} entity in Figure~\ref{fig:shapers}. The overhead (in terms of resource usage) of this subsystem is included in our results for TAS and labeled as Time-Stamping Unit (TSU).

\subsubsection{Resource utilization for TAS and CBS}
\label{sec:feasibility:cbsTasUtilization}

For the TSN shapers, we performed synthesis runs for $1$, $2$, $4$, and $8$ supported priorities (N\_IPVs). The corresponding counts for LUTs, Registers, CARRY8, and F7 Muxes are shown in Figure~\ref{fig:shapers-res-all}.

\begin{figure}[htb]
\centering \includegraphics{feupphdteses/sections/implementation/Images/shapers-res-all.pdf} 
\caption{CBS and TAS CLBs} \label{fig:shapers-res-all}
\end{figure}

As can be seen, LUTs, Registers, and CARRY8 adders scale linearly with the number of supported priorities. This is explained by the fact that both the credit-keeping modules in CBS and the guarding modules in TAS are instantiated per priority. When TAS and CBS are used together, they affect each other in terms of resource utilization. However, we did not observe any significant additional overhead in such a scenario.

Table~\ref{tab:tas-over-cbs} provides the percentage of total resources available on \texttt{xczu9cg-ffvb1156\\-1-e} used by TAS IP (in rows marked \textit{\%TOT}), and also the overhead of TAS over CBS (how much more resources it uses, rows marked \textit{/CBS}). As expected, the TAS is significantly larger, with overhead being as high as $15$ times larger in the case of only one supported priority. A significant portion of this can be attributed to the TSU (as seen in Figure~\ref{fig:qbu-res-all}), together with the previously explained guarding feature (not visualized). What is worth noticing, is that the LUT utilization of TAS is around 2\%. With an instance of TAS required per egress port, it makes scaling it with port numbers especially expensive. Since F7 MUXes only start being used in CBS with 8 priorities, and their utilization numbers are very low, they are omitted from Table~\ref{tab:tas-over-cbs}.

 \begin{table}
\centering
\caption{TAS IP resource utilization and overhead over CBS}
\label{tab:tas-over-cbs}
\begin{tabular}{@{}llrrr@{}}
\toprule
N\_IPVs            & Type  & CLB LUTs & CLB Registers & CARRY8 \\
\midrule
\multirow{2}{*}{1} & \%TOT & 1.8\%    & 0.8\%         & 0.6\%  \\
                   & /CBS  & 1512\%   & 1500\%        & 2122\% \\
\midrule
\multirow{2}{*}{2} & \%TOT & 1.9\%    & 0.8\%         & 0.6\%  \\
                   & /CBS  & 1187\%   & 1116\%        & 1366\% \\
\midrule
\multirow{2}{*}{4} & \%TOT & 2\%      & 0.9\%         & 0.7\%  \\
                   & /CBS  & 913\%    & 763\%         & 863\%  \\
\midrule
\multirow{2}{*}{8} & \%TOT & 2.4\%    & 1\%           & 0.8\%  \\
                   & /CBS  & 663\%    & 500\%         & 567\%  \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Frame Preemption implementation}
\label{sec:feasibility:preemptionImplementation}
% \begin{figure}
%     \centering
%     \includegraphics{feupphdteses/sections/implementation/Images/qbu-combined.pdf}
%     \caption{(Multi-level) Frame Preemption block diagram}
%     \label{fig:qbu}
% \end{figure}
%This is shown in Figure~\ref{fig:qbu} where the \textit{supporting logic} encompasses everything necessary for the integration of the modules.

% A simplified block diagram of multi-level frame preemption system is shown in Figure~\ref{fig:qbu}. A single-level frame preemption is fully encompassed by \textit{TSN MAC} module. As mentioned in Section~\ref{sec:background:preemption}, it consists of eMAC, pMAC, and MMS.

Recall that our proposed implementation approach of multi-level preemption is to introduce new pMAC interfaces on the MAC Merge Sublayer (MMS). However, we note that due to resource constraints (hardware availability and IP restrictions), we could only implement $1$-level preemption feature on hardware and the hardware utilization results were extrapolated based on the predicted behavior of our implementation approach.
\begin{tcolorbox} We project that our approach causes a doubling of resources for the $2$-level, a tripling for the $3$-level, and so on.
\end{tcolorbox}

\begin{figure}[htb] \centering \includegraphics{feupphdteses/sections/implementation/Images/qbu-res-all.pdf} \caption{Resource utilization for TSN MAC } \label{fig:qbu-res-all}
\end{figure}

In Figure~\ref{fig:qbu-res-all}, stacked bar charts are used to visualize the resource utilization of the major submodules of the TSN MAC. Table~\ref{tab:qbu-overhead} shows the percentage of total resources available on the target device in \textit{\% TOT } rows. Since the increase in utilization is linear, only the resource utilizations for levels zero, one, and two are shown. In addition, in rows marked \textit{\% OH } list the implementation overhead compared to the non-preemption MAC (row $0$). The values are exclusive of supporting~logic. The MMS implements more complex preemption operations, which explains why its size is more than twice that of the simple MAC. With three traffic classes, a $2$-level preemption scheme would be preferable to TAS if it can meet the performance requirements. However, if more traffic classes need to be supported, the choice is not so clear. 

\begin{tcolorbox}
    If multi-level preemption is implemented according to our specifications, the cost grows linearly. It is less than TAS for up to four levels of preemption, after which it overtakes TAS.
\end{tcolorbox}

However, with a linear increase to eight classes, multi-level preemption would be significantly more expensive than TAS. This does not take into account the additional software required for time synchronization in TAS (TSU).

% \note[VGA]{Again my observation about percents greater than 100!}
\begin{table}
\centering
\caption{Frame preemption resource utilization and overhead}
\label{tab:qbu-overhead}
\begin{tabular}{@{}llrrrr@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}Pre.\\ levels\end{tabular} & Type & CLB LUTs & CLB Registers & CARRY8 & F7 Muxes \\
\midrule
0                  & \%TOT & 0.16\%   & 0.06\%   & 0.01\%    & 0.00\%   \\
\midrule
\multirow{2}{*}{1} & \%TOT & 0.66\%   & 0.28\%   & 0.15\%    & 0.01\%   \\
                   & \%OH    & 411.21\% & 467.37\% & 2550.00\% & 450.00\% \\
\midrule
\multirow{2}{*}{2} & \%TOT & 1.15\%   & 0.51\%   & 0.29\%    & 0.01\%   \\
                   & \%OH    & 723.11\% & 835.03\% & 5000.00\% & 800.00\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics{feupphdteses/sections/implementation/Images/qbu-comp.pdf}
    \caption{Resource increase caused by adding preemption levels.}
    \label{fig:qbu-multi-lvl}
\end{figure}


==> sections/implementation/sections/introduction.tex <==
\section{Implementation cost}
\label{sec:feasibility:implementation-cost}
As part of the feasibility analysis of multi-level preemption, we quantify the hardware implementation costs of the scheme and compare them to those of two other widely studied TSN traffic control mechanisms, namely TAS and CBS (see their detailed descriptions in Sections~\ref{sec:background:tas} and \ref{sec:background:cbs}). Most studies in the literature that compared these mechanisms did so mainly from a performance perspective~\citep{Gogolev2020Simpler, Thiele2016Formal, Hellmanns2020Performance, Nasrallah2019Performance} and focused on the worst-case delay and jitter guarantees of frames. However, a detailed discussion of how these mechanisms compare implementation costs were still lacking. System designers are interested in both achieving acceptable performance and reducing hardware costs by choosing simpler and less complex solutions. As long as the performance requirements are met, businesses will opt for the cheapest solution. Comparing implementation costs would help system designers decide which feature(s) to use for their applications. If the cost of implementing multi-level preemption is significantly lower than the other traffic control mechanisms, this is another compelling reason to adopt it.

When estimating switch manufacturing costs, device manufacturers use the term \textit{non-recurring engineering (NRE)} for one-time costs and \textit{recurring engineering (RE)} for costs that are repeated for each device (e.g., testing)~\citep{Pruski2021Implementation}. In our context, NRE costs are the most appropriate metric because they have the most to do with the hardware components of the switch. To compare NRE costs, a survey of well-known vendors on the development costs of the TSN features would be ideal. However, due to the sensitive nature of this information, vendors are unwilling to disclose it. Instead, we focus on metrics that are easier to obtain, such as the FPGA resource utilization profile from our collaborators at \href{https://www.comcores.com/contact/}{Comcores ApS}, which is described in more detail in Section~\ref{sec:implementation:hw-background}.

\begin{tcolorbox}
    Our comparison is based on the assumption that more resources used means a more costly implementation.
\end{tcolorbox}




==> sections/implementation/sections/qualitative-comparion.tex <==
\note[VGA]{Here are only ideas, but I don't see what this section should add. Here will come metrics that have to be compared on the next section?}

\subsection{Real-time performance} 
latency and jitter improvements for real-time traffic;
\subsection{Bandwidth utilization}
evaluates bandwidth consumed and/or wasted by the protocols;
\subsection{Mutual isolation} can the shaper handle heterogeneous traffic types
without mutual interference;
\subsection{Granularity of QoS control}
diversity and parametrization of allowed QoS policies;
\subsection{Traffic management}
supported logical management architectures and how it affects resource
management efficiency; (queueing/buffer requirements; internal priority/service
class assignments, centralised or distributed management etc)

\subsection{Flexibility}
applications should be able to create and modify reservations promptly, in order
to adapt to environment or production changes;


==> sections/implementation/sections/related-work.tex <==
There is a plethora of research that compares the TSN traffic control
approaches from a performance standpoint.
On this front,~\cite{thangamuthu2015analysis} compare the
performance of three TSN shapers, namely, TAS, burst limiting shaper and the Peristaltic Shaper (PS). In this work, the comparison metrics are delay and jitter. The authors conclude that TAS provides the best performance for both metrics. A similar work by~\cite{Thiele2015Peristaltic} compares
TAS with PS, reaching a similar conclusion, i.e., TAS provides better
end-to-end delay performance. They noted, however, that the performance of TAS degrades significantly when end systems are not synchronized.~\cite{Thiele2016Formal} also compare the performance of TAS and frame preemption and conclude that the two approaches achieve very similar end-to-end delays. The authors go further to suggest, that standard Ethernet with frame preemption is a viable alternative to TAS. 

Another work comparing TAS and frame preemption, by~\cite{Gogolev2020Simpler}, demonstrated via experiments that frame preemption is more suitable for industrial networks with unsynchronized end systems. The authors point out that a serious limitation for frame preemption is the low Quality of Service  (QoS) resolution , i.e., there are only two classes (eMAC and pMAC) specified for preemption in TSN. To mitigate the aforementioned limitation,~\cite{Ojewale2020Feasibility, Ojewale2021WorstCase} introduce the multi-level preemption paradigm. Here, the authors also compare TAS and frame preemption from a qualitative standpoint and promote the multi-level frame preemption feature as a viable alternative to TAS. Furthermore, ~\cite{knezic2020implementation} provided an enhanced implementation approach for the multi-level preemption feature and the formal worst-case traversal time analysis of this approach was provided by~\cite{Ojewale2021WorstCase}. On another front, a work by~\cite{Nasrallah2019Performance} conducts a performance comparison of TAS and Asynchronous Traffic Shaping (ATS). The authors surmise that ATS performs well compared to TAS for sporadic (asynchronous) traffic. They noted, however, that the performance of Scheduled Traffic degrades with increasing Best-Efforts load under ATS. We note that none of the aforementioned works have compared these features from an implementation complexity perspective.

There is not such intense interest though in comparing the performance of CBS with other shapers. There are the works of~\cite{alderisi_etfa2013} and~\cite{lo-bello_etfa2014} that present simulation results for AVB-ST (Scheduled Traffic) in industrial automation and automotive areas, respectively. AVB-ST is a stern approach of TAS, assuming that the scheduled traffic is strictly periodic and that precise offsets are provided for the scheduled frames. In these works, the baseline is considered the pure CBS, and the authors observe that only by using AVB-ST the bounded delay and zero jitter for the scheduled traffic is ensured. A similar work, by~\cite{meyer_etfa2013}, highlights the importance of quality of schedule tables. For example, for a non-dense table, the delay of AVB traffic increases but is still bounded and compliant with the specification in~\cite{IEEE802.1BA}. On the other hand, when using a compact schedule table, the delays of AVB traffic are still bounded, but not compliant anymore with the specification.  

On the hardware implementation front,~\cite{zhou2017analysis}
present a VHDL design layout for the transmission and reception processes as well as an FPGA-based hardware implementation of TSN sender and receiver nodes.~\cite{hotta2015experimental} present another FPGA implementation of an Ethernet switch supporting frame preemption.
% Knezic et al.~\cite{knezic2020} present a method with a potential to decrease the implementation
% resources of multi-level preemption.
%\note[VGA]{For me is not clear how these articles about hardware implementation correlate with our work!}


==> sections/introduction/introduction.tex <==
\chapter{Introduction}
\label{chap:introduction}
The rise of digital technology has changed people's lives in many ways. Technology components such as sensors, actuators, communication, and computing infrastructures have created an intertwined ecosystem. From traditional systems such as manufacturing, avionics and automotive to emerging systems such as service robots and autonomous systems, digital technology is now at the heart of virtually all human endeavors. Microprocessor technology is driving this new phenomenon. It is becoming ever smaller in miniaturization, yet ever more sophisticated and powerful. Today, microprocessors can be found in everyday devices, from cell phones to home appliances to production systems and aircraft. Such devices/systems that contain microprocessors to provide computation and control functions are often referred to as \textit{embedded systems}. In some application scenarios, such as automotive and industrial automation, an embedded system consists of multiple hardware and software components that must communicate over a network medium. This class of embedded systems is referred to as \textit{distributed embedded systems}. The subset of distributed embedded systems that requires not only functional correctness - i.e., functions must provide logically correct outputs - but also temporal correctness - i.e., these outputs must be available within a specified time interval - is called \textit{Distributed Real-time Embedded Systems (DRES)}. In this work, we focus on the \textit{communication} aspects of DRES. In this kind of systems, different components communicate over a wired or wireless medium, depending on the specific constraints of the target application domain. While wireless communication offers more flexibility and mobility, wired communication is usually preferred because it offers high reliability and is less susceptible to signal loss and interference. 

\begin{tcolorbox}
In this dissertation, some key contributions to real-time wired communication in DRES are presented.
\end{tcolorbox}

The remainder of this chapter is organized as follows. First, we explain the motivation for this research and identify the research gap that we aim to fill in Section~\ref{sec::introduction:motivation}. Then, we present the thesis and the corresponding research question in~\ref{sec:introduction:thesis_statement}. The research methodology is elicited in Section~\ref{sec:introduction:methodology}, which is followed by a summary of the main contributions in Section~\ref{sec:introduction:contribution}. Finally, Section~\ref{sec:introduction:significance} explains the significance of the contributions, and Section~\ref{sec:introduction:thesis_structure} describes the structure of the remainder of the dissertation.

\section{Research Context}
\label{sec:introduction:context}
One of the key requirements of DRES is \textit{real-time communication}, i.e., the ability of data to move reliably and predictably through the underlying network. To date, a variety of solutions have been proposed in the literature, each targeting a set of domain-specific requirements. Some examples of established solutions include the \textit{Controller Area Network} (CAN) protocol~\citep{specification1991bosch}, the \textit{Local Interconnect Network} (LIN) protocol~\citep{specks2000lin}, the \textit{FlexRay} protocol~\citep{pop2008timing}, and TTEthernet~\citep{steiner2009ttethernet}, which focus mainly on the automotive sector; \textit{Avionics Full Duplex Switched Ethernet} (AFDX)~\citep{brajou2004airbus}, which targets the avionics sector; and protocols such as SERCUS III ~\citep{schemm2004sercos}, EtherCAT~\citep{jansen2004real} and PROFINET~\citep{feld2004profinet}, which are aimed at the industrial domain. As a matter of fact, most of these solutions are now struggling to keep up with the growing bandwidth and performance requirements of emerging applications in their respective domains~\citep{Thiele2016Formal}. Another development is the convergence of Operations Technology (i.e., the hardware and software systems used to control and monitor industrial processes) and Information Technology (i.e., the systems and tools used to manage, store, and process data), which presents a new challenge and requires new communication technologies to handle different types of traffic (real-time, non-real-time, long and short frames) on the same network infrastructure.

Ethernet~\cite{shoch1981introduction} has emerged as a leading and promising replacement for all previous technologies, capable of meeting increasingly stringent time and distance requirements and providing high bandwidth capacity~\citep{Thiele2016Formal, Jia2013performance}. In this protocol, data is transmitted over the network using a digital packet called a ''frame'' (see Figure~\ref{Ethernet-frame} for the structure of a basic Ethernet frame). The first field is the ''preamble'' -- $7$~bytes -- which consists of alternating 1s and 0s and is used to synchronize the sender and receiver. This field is followed by what is called the ``Start Frame Delimiter'' -- $1$~byte --, which indicates the start of the frame; then come the ''Media Access Control'' (MAC) destination and source addresses\footnote{The MAC address is a unique identifier assigned to each device on a network} -- $6$~bytes each --, which identify the devices sending and receiving the data. These two fields are followed by what is called the ''Ethertype'' -- $2$~bytes --, which specifies the type of data being transmitted (e.g., Internet Protocol (IP), Address Resolution Protocol (ARP), etc.). This field is followed by the ''Data'' field -- $46$ to $1500$~bytes --, which contains the actual data that will be transmitted. Finally, the last field is the ''frame check sequence'' -- $4$~bytes -- which is used to detect errors during transmission. This is a mathematical calculation that is performed on the frame to ensure that it was transmitted and received correctly.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.6]{feupphdteses/sections/introduction/images/ethernet-frame-format.pdf}
    \caption{Ethernet frame format as defined by the IEEE.}
\label{Ethernet-frame}
\end{figure}

The original Ethernet standards were intended only for non-real-time applications and have several limitations that complicate their use in DRES. In their specification, a frame must not interrupt the transmission of other frames, regardless of its timing constraints. In other words, the frames are transmitted non-preemptively as illustrated in Figure~\ref{non-preemptive}.
\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.7]{feupphdteses/sections/introduction/images/non-preemptive-transmission.pdf}
    \caption{Illustration of the Ethernet non-preemptive transmission scheme.}
\label{non-preemptive}
\end{figure}

In this figure, three frames ($f_1$, $f_2$, and $f_3$) are considered for transmission in a First-In-First-Out (FIFO) order. The up arrows define the frame arrivals and the down arrows define the time instant by which the transmission of each frame must be completed. Frame~$f_1$ arrives first (at time~$0$) and starts its transmission. During the transmission of $f_1$, frames~$f_2$ and $f_3$ arrive, but cannot begin their transmission despite their stringent timing constraint because $f_1$ is being transmitted. Both frames are given a window of three time units for their transmission. Consequently, they do not meet their timing requirements, i.e., they miss their deadlines. In addition to the potentially large delay incurred by frames due to the non-preemptive transmission scheme, another major limitation of Ethernet when it comes to real-time applications is its unpredictable nature in the sense that it does not guarantee the delivery of data within a predefined time period. This can be particularly challenging in automotive and industrial automation, where real-time control is critical. Furthermore, Ethernet is susceptible to network congestion because it uses a shared medium for communication. This means that multiple devices can transmit data simultaneously, which in turn can cause collisions and delays that degrade network performance and make it difficult to transmit data in a timely manner.

A lot has been done by standardization bodies, academia, and industry experts in the last two decades to address these limitations and several changes and/or additions have been made to the Ethernet standards to include features for real-time communication~\citep{Nasrallah2018}. The latest set of \textit{updated standards} in this direction is referred to as \textit{Time-Sensitive Networking} (TSN)~\citep{IEEE}. In this set, the IEEE ~802.1Qbu~\citep{IEEE802.1Qbu} TSN sub-standard (now merged with the IEEE ~802.1Q-2018 standard~\citep{IEEE-Std-802.1Q-2018}) introduces a \textit{$1$-level frame preemption} scheme to the IEEE~802.1 networks. In contrast to the original Ethernet specification, this scheme allows the transmission of a frame to be temporarily suspended prior to its completion in order to expedite the transmission of a more urgent frame. This standard is closely related to the IEEE ~802.3br~\citep{IEEE802.3br-2016} standard, which allows urgent time-critical frames to split non-critical frames transmitted over a physical link into smaller fragments~\citep{bello2019perspective}. In particular, frames are mapped to two MAC sublayer service interfaces depending on their priority and timing requirements, namely ($1$)~the ``\textit{Express MAC}'' (eMAC) and~($2$)~the ``\textit{Preemptable MAC}'' (pMAC). Frames that map to the eMAC and pMAC interfaces are referred to as ``express frames'' and ``preemptable frames'', respectively. These two classes are managed as follows: ($i$)~only express frames can preemptable frames; and ($ii$)~two frames belonging to the same class cannot preempt each other. Figure~\ref{one-level-preemption} illustrates such a scenario.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.7]{feupphdteses/sections/introduction/images/frame-preemption-ilustration}
    \caption{Illustration of the $1$-level preemption scheme.}
\label{one-level-preemption}
\end{figure}

In this figure, three frames ($f_1$, $f_2$, and $f_3$) are considered, and the priorities of the frames are set so that ``the smaller the index of a frame, the higher its priority'', i.e., $f_1$ gets the highest priority and $f_3$ the lowest. As in the previous example, an up arrow represents the arrival time of a frame and a down arrow represents the deadline. We assume that frames are transmitted according to a $1$-level preemption scheme and are divided into two preemption classes: ($1$)~the \textit{highest preemption class (express)}, in which frames are represented by ``red boxes''; and ($2$)~the \textit{lowest preemption class (preemptable)}, in which frames are represented by ``green boxes''. The light gray boxes represent the costs associated with the occurrence of a preemption. As can be seen, preemption favors prompt service of all express frames, but this comes at the cost of some overhead. The extra cost comes from the fact that fragments of split frames must form valid Ethernet frames. Namely, information such as the number of fragments (Fragment Count), an error correction code (CRC) to determine if all fragments were transmitted correctly, etc. must be added to the fragments of the preempted frame - here $f_1$ - so that the network nodes can send and receive them all correctly. The total overhead associated with the occurrence of each preemption is equivalent to the time required to transmit $24$ bytes of data (i.e., $0.19 \mu s$ and $1.9 \mu s$, assuming an Ethernet with $1$~Gb and $100$~Mb speeds, respectively). Experimental studies show that this approach improves the performance of express frames~\citep{Thiele2016Formal, Jia2013performance}. In particular, Thiele and Ernst~\citep{Thiele2016Formal} show that the performance of standard Ethernet with frame preemption in terms of worst-case delay guarantees is comparable to that of the so-called ``Time-Aware Shaper'' -- a time-triggered gate control mechanism defined in the IEEE 802.1Qbv standard~\citep{IEEE802.1Qbv} for TSN frame transmission, making it an interesting alternative.
% \vspace{0.2cm}

%  \noindent $\triangleright$ \textbf{IEEE 802.1Qbv.}
% The IEEE 802.1Qbv standard
% defines a time-triggered gate control mechanism for TSN flows, using a Time-Aware Shaper (TAS). Here, each queue at a switch output port has a guaranteed transmission slot in a cyclic and pre-computed dispatch schedule called the Gate Control List~(GCL). A frame on a queue can be transmitted only when the gate of the queue is opened at the time period according to the GCL configuration. Note that each queue contains a unique class of frames, i.e., frames belonging to different traffic classes cannot share the same queue. The standard also specifies a so-called ``guard-band'' that ensured that the transmission of time-triggered flows is protected from any interference by other flows. The guard band is a time-period between the gate-close operation non-time-triggered queues and the commencement of transmission of time-triggered flows. The length of this guard band is equal to the time taken to transmit the largest possible non-time-sensitive frame on the network. While the guard band ensures that time-triggered traffic are protected from interference, it results in poor utilization of network bandwidth.
% \vspace{0.2cm}

% \noindent $\triangleright$ \textbf{Comparing IEEE 802.1Qbu and IEEE 802.1Qbv from a qualitative standpoint:} Thiele and Ernst~\citep{Thiele2016Formal} noted that an IEEE 802.1Qbu network is less complex to configure as only two basic steps are required: ($1$)~the assignment of priorities to flows; and ($2$)~the assignment of flows to preemption interfaces~\citep{park2019design}. Even though this process is non-trivial~\citep{park2019design}, it is bearable in comparison to the IEEE 802.1Qbv configuration. Here, TAS requires finding a suitable schedule for each flow at each switch output port and this problem has been shown to be NP-Hard~\citep{steiner2010evaluation}. On another front, IEEE 802.1Qbu solves an issue of IEEE 802.1Qbv. By combining frame preemption with TAS, optimal bandwidth utilization is possible for non-scheduled traffic and this enables low-latency communication~\citep{bello2019perspective}. Nevertheless, the IEEE 802.1Qbv standard remains central to TSN. It defines up to 8 queues per port for forwarding traffic and frames are assigned to queues based on Quality of Service (QoS) priority. The TAS mechanism blocks all ports except one based on a predefined schedule in order to prevent delays during scheduled transmission. From an implementation standpoint, the performance of IEEE 802.1Qbu networks degrades in scenarios where the number of express frames is high~\citep{bello2019perspective}. This is due to the fact that frames of the same class are transmitted in a non-preemptive manner. As a consequence, there are frames that cannot be classified as express but have firm timing requirements. In order not to jeopardize the schedulability of these frames, and the schedulability of the entire system subsequently, these frames should not be blocked for prohibitively long time periods. The $1$-level preemption operation in the current version of the standards does not allow preemptable frames with firm timing requirements to leverage the basic benefits of enabling preemption. 
\section{Motivation}
\label{sec::introduction:motivation}
\cite{bello2019perspective, Gogolev2020Simpler, ASHJAEI2021novel} pointed out some limitations of the $1$-level preemption scheme as specified in the standards. Most importantly, \cite{bello2019perspective} and~\cite{Gogolev2020Simpler} noted that this scheme is prone to performance degradation when the number of express frames is high. In this manuscript, we consider the scheme from a different perspective and point out that:

\begin{tcolorbox}
The $1$-level preemption scheme greatly improves the responsiveness of express frames but exhibits some serious limitations and poor performance when it comes to transmitting \textit{preemptable frames with firm timing requirements}. 
\end{tcolorbox}

\noindent There are frames that cannot be classified as express frames, but have firm timing requirements. These frames should not be blocked for an excessive amount of time by lower priority frames, so as not to jeopardize the schedulability of these frames and thus the schedulability of the entire system. The current specification of the $1$-level preemption scheme does not allow these frames to take advantage of the basic benefits of preemption. Recall that the TSN standards mandate that frames belonging to the same class cannot preempt each other. Figure~\ref{fig:intro:1-level-preemption} illustrates such a scenario.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.8]{feupphdteses/sections/introduction/images/motivation-1-level-pre-n2}
    \caption{Limitation of the 1-level preemption scheme with $f_3$ as ``preemptable''.}
\label{fig:intro:1-level-preemption}
\end{figure}

In this figure, four frames ($f_1$, $f_2$, $f_3$, $f_4$) are considered and the priorities are set such that ``the smaller the index of a frame, the higher its priority'', i.e. $f_1$ gets the highest priority and $f_4$ the lowest. Express frames are represented by ``red boxes'' and preemptable frames by ``green boxes''. The light gray box represents the cost associated with the occurrence of a preemption. We are interested in the fate of frame~$f_3$, which has a firm deadline of $9$ time units after its release at time~$t=1$. In this scenario, frame~$f_4$ arrives first and begins its transmission. At time~$t=1$, frame~$f_3$ (with a higher priority than~$f_4$), arrives but cannot preempt $f_4$ because both belong to the same preemption class. At time ~$t=2$, $f_2$ (which is express) arrives and preempts the transmission of ~$f_4$. At time~$t=3$, $f_1$ (which has a higher priority than~$f_2$) arrives but cannot preempt $f_2$ since both belong to the same preemption class. After the express frames are completed, $f_4$ resumes its transmission despite $f_3$ being ready and pending. This is due to the actual specification of the $1$-level preemption scheme and illustrates a priority inversion. Finally, due to this long blocking, $f_3$ eventually misses its deadline.

Intuitively, to circumvent this hurdle, one might want to move $f_3$ to the express class, since its timing requirement cannot be satisfied in the preemptable class. Figure~\ref{fig:intro:1-level-preemption-2} illustrates such a scenario.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.8]{feupphdteses/sections/introduction/images/motivation-1-level-pre-n3}
    \caption{Limitation of the 1-level preemption scheme with $f_3$ as ``express''.}
\label{fig:intro:1-level-preemption-2}
\end{figure}

In this scenario, frame~$f_3$ (which is now express) arrives and preempts the transmission of~$f_4$. At time~$t=2$, frame~$f_2$ arrives (with a higher priority than~$f_3$), but cannot preempt $f_3$ since both belong to the same preemption class. At time~$t=3$, $f_1$ (with a higher priority than~$f_2$) arrives and begins its transmission immediately after $f_3$. After the completion of $f_1$, $f_2$ starts its transmission. Consequently, $f_2$ misses its deadline due to the blocking by $f_3$ and the transmission of $f_1$. 

The above challenges encourage us to think about relaxing the $1$-level preemption constraint. Using a hypothetical \textit{$2$-level preemption scheme}, we re-examine the scenarios shown in Figures~\ref{fig:intro:1-level-preemption} and~\ref{fig:intro:1-level-preemption-2} and show the result in Figure~\ref{fig:intro:2-level-preemption}. 

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.8]{feupphdteses/sections/introduction/images/motivation-mutli-level-pre-n2}
    \caption{Frame transmissions under a 2-level preemption scheme.}
\label{fig:intro:2-level-preemption}
\end{figure}

In this figure, we now assume three possible preemption classes: ($1$)~the \textit{highest preemption class}, in which frames are represented by ``red boxes''; ($2$)~the \textit{middle preemption class}, in which frames are represented by ``yellow boxes''; and finally ($3$)~the \textit{lowest preemption class}, in which frames are represented by ``green boxes''. We assume that frames in a higher preemption class can preempt any frame in a lower preemption class and that frames in the same preemption class cannot preempt each other, similar to standards. As we can see from the figure, frame $f_3$ is better served because it is transmitted immediately after $f_2$ and $f_1$ are completed. This results in no priority inversion, and all frames are able to meet their timing requirements.

From this example, it is clear that preemptable frames with firm timing requirements (in the yellow-colored box) suffer from poor responsiveness under the $1$-level preemption paradigm, but the situation already improves under a $2$-level preemption paradigm. Since this type of frame is not uncommon in real-time applications, this provides a clear motivation to investigate not only a $2$-level, but a \textit{multi-level preemption scheme} in TSN to get the maximum benefit from this approach. Another notable limitation in the standards is the lack of configuration definitions to ensure optimal/efficient performance in terms of frame responsiveness. Eight Classes of Service (CoS) are defined in the specification of Ethernet frames~\citep{IEEE802.1Q-2014}, but it is not clear which of them should be mapped to Express or Preemptable frames in the TSN specification. Last but not least, the TSN standards do not specify efficient routing techniques to optimize network performance.
\vspace{0.5cm}


\section{Thesis statement and research questions}
\label{sec:introduction:thesis_statement}
In this work, we propose solutions to the shortcomings of the $1$-level preemption scheme specified in the TSN standards. In this framework, the thesis statement is as follows:

\vspace{0.2cm}
\noindent \fbox{\begin{tcolorbox}
\textit{We postulate that multi-level preemption, when added to TSN, can mitigate several shortcomings of the frame preemption standard and unlock timeliness and resource utilization benefits of DRES.}
\end{tcolorbox}}
\vspace{0.2cm}

Based on this thesis, we investigate and promote the implementation of a \textbf{Multi-level Preemption Scheme}. With this new paradigm, we envision that all frames with strict and/or firm timing requirements receive a significant improvement in their performance in terms of responsiveness. This, in turn, allows us to improve both the Quality of Service~(QoS) and the reliability of the overall system, and to increase the workload that can be accommodated in the underlying communication network. However, achieving this goal involves a number of challenging scientific problems, which are formulated in three research questions presented below.
\begin{enumerate}
    \item[$(\operatorname{RQ}_1)$.] \textbf{Research Question~1:} At this stage, we are interested in investigating the operational feasibility of multi-level preemption within the specifications of the TSN standards. In particular, we are investigating how the scheme can be achieved with the least changes to the standard specifications while maintaining interoperability with other existing Ethernet/TSN transmission schemes. We are also interested in how the resource utilization overhead of the multi-level preemption scheme can be minimized and how this overhead compares to other TSN traffic control mechanisms from a qualitative perspective. Formally, the first research question is as follows.

\vspace{0.2cm}
\begin{tcolorbox}
    How feasible is a multi-level preemption scheme in TSN with the current specifications in the standards and what are the requirements for its efficient implementation?
\end{tcolorbox} 
\vspace{0.2cm}

    \item[$(\operatorname{RQ}_2)$.] \textbf{Research Question~2:} Compliance with timing requirements is essential for any real-time communication medium. Therefore, formal timing analyzes must be performed to provide safe timing guarantees when a new feature and/or scheme is proposed. These analyzes not only provide real-time guarantees but also allow evaluation of the newly proposed feature and/or scheme from a quantitative perspective. The need to perform such analyzes for the proposed multi-level preemption scheme leads us to the second research question, which is formulated as follows.

\vspace{0.2cm}
\begin{tcolorbox}
     How does multi-level preemption affect the temporal behavior of time-critical data flows if we want to provide real-time guarantees?
\end{tcolorbox}
\vspace{0.2cm}

\item[$(\operatorname{RQ}_3)$.] \textbf{Research Question~3:} The performance of any real-time transmission scheme depends heavily on the configuration chosen, and the multi-level preemption is no exception. Therefore, determining the appropriate configuration framework to achieve the best possible performance is a task that deserves our utmost attention. This fact leads us to the final research question, which is formulated as follows.

\vspace{0.2cm}
\begin{tcolorbox}
    How can a TSN network with a multi-level preemption scheme be configured to achieve efficient and/or optimal performance?
\end{tcolorbox}
    
\end{enumerate}

\section{Research methodology}
\label{sec:introduction:methodology}
To validate the thesis, a deductive research methodology was used. In this method, a hypothesis is first developed based on the state-of-the-art. Then, a strategy is established to test the hypothesis using a series of observations to determine if it is supported by the data. The key characteristic of this approach is that the conclusion is necessarily true if the original principles or ideas are true. In the context of our research, the thesis is the main hypothesis. We arrive at this thesis after a thorough review of the Frame Preemption specification in the TSN standards and all related work in the literature on the subject. We identify three main research questions, namely $\operatorname{RQ}_1$, $\operatorname{RQ}_2$, and $\operatorname{RQ}_3$, whose answers would allow us to confirm or reject the thesis.

$\operatorname{RQ}_1$ is a qualitative assessment that involves a comprehensive analysis and comparison of different implementation profiles. In this framework, the qualitative evaluation criteria are ($1$)~feasibility; ($2$)~resource utilization; ($3$)~ease of configuration; and finally ($4$)~flexibility of a TSN network with multi-level preemption. Specifically, we conduct a comprehensive study of TSN standards, along with various other materials, including several presentations and review documents from the IEEE TSN Task Group~\citep{IEEE}. In addition, collaboration with industry partners at \href{https://www.comcores.com/}{Comcores ApS, Lyngby, Denmark} is initiated to obtain data on the resource utilization profiles of various TSN traffic control mechanisms. All this information  is extensively analyzed and relevant conclusions and recommendations are derived.

In contrast to $\operatorname{RQ}_1$, $\operatorname{RQ}_2$ and $\operatorname{RQ}_3$ are quantitative assessments. To answer these, we explore relevant scientific theories and tools. In addition, extensive discussions with thesis advisors and, in some cases, collaborators from the real-time communication research community were conducted. The first goal of these discussions is to develop a model that effectively captures the characteristics of a TSN network with multi-level preemption. Once this model is successfully developed, we identify the key metrics to be used in evaluating the proposed scheme. We then systematically and consistently conduct experiments to compare the new scheme to existing ones in the literature. The results of these experiments are analyzed in depth to draw unbiased conclusions about the effectiveness of the multi-level preemption scheme.

\section{Overview of the contributions}
\label{sec:introduction:contribution}

In this section, we summarize the main findings of our research in relation to the research questions outlined in Section~\ref{sec:introduction:thesis_statement} and explain how our work contributes to the existing body of knowledge in the field of real-time communication. To this end, the section is organized under three headings, namely: ($1$)~\textit{feasibility and implementation cost}; ($2$)~\textit{model and analysis}; and finally, ($3$)~\textit{configuration and evaluation}.

\subsection{Feasibility and implementation cost}
This contribution addresses $\operatorname{RQ}_1$. It examines the preemption mechanism in detail to determine the feasibility of a multi-level preemption scheme, and our analysis confirms its feasibility. First, we examine the Ethernet frame format to determine how different preemption classes can be encoded without radical changes to the standard specifications. We then examine the frame transmission and reception processes to understand how additional frame preemption classes would fit into the existing definitions. Special care was taken to avoid deadlock situations or transmission errors. We explain the changes required to achieve this goal and provide implementation recommendations to ensure frame integrity and interoperability. In this context, we also compare the hardware implementation costs of the multi-level preemption scheme with the time-triggered (TAS) and credit-based shaper (CBS) approaches. Here, the results show that the implementation cost of frame preemption, while significantly higher than that of CBS, is very much lower than that of the prevailing TAS. In particular, the results show significantly lower resource consumption for up to four preemption levels compared to TAS. Note that in this comparison we do not consider the additional overheads of the time synchronization software required by TAS. The above contributions are presented in the following publications:

\begin{itemize}
    \item \textbf{M. A. Ojewale}, P. Meumeu Yomsi and B. Nikolić, \textit{Multi-Level Preemption in TSN: Feasibility and Requirements Analysis}, IEEE 23rd International Symposium on Real-Time Distributed Computing (ISORC), 2020, pp. 47-55,\url{https://doi.org/10.1109/ISORC49007.2020.00017}.
    
    \item A. Pruski, \textbf{M. A. Ojewale}, V. Gavrilut, P. Meumeu Yomsi, M. S. Berger and L. Almeida, \textit{Implementation Cost Comparison of TSN Traffic Control Mechanisms}, 26th IEEE International Conference on Emerging Technologies and Factory Automation (ETFA), 2021, pp. 01-08, \url{https://doi.org/10.1109/ETFA45728.2021.9613463}.
\end{itemize}

\subsection{Model and analysis}
This contribution answers $\operatorname{RQ}_2$. It provides formal worst-case upper bounds on the delays experienced by each frame under the multi-level preemption scheme, using the so-called \textit{Compositional Performance Analysis} (CPA) approach. For this purpose, four delay components are identified and summed, namely ($1$)~the delay due to the transmission of a lower priority frame; ($2$)~the delay due to the transmission of frames of the same priority; ($3$)~the delay due to the transmission of higher priority frames; and finally ($4$)~the delay due to the preemption overhead. Formal proofs are presented to establish numerical upper bounds for each of these components. We evaluate the safety of these upper bounds by comparing the numbers obtained with those from extensive simulations using NeSTiNg~\citep{nesting_2019}, a simulation model for~TSN built on the OMNeT++ framework~\citep{OMNeT}. We also evaluate the performance improvements over the $1$-level preemption scheme using a realistic automotive use case. Our results show that the multi-level preemption scheme provides up to $53.07\%$ improvement in terms of worst-case traversal time (WCTT) reduction for preemptable time-critical frames. The above contributions are presented in the following publications:

\begin{itemize}
    \item \textbf{M. A. Ojewale}, P. Meumeu Yomsi, G. Nelissen, \textit{On Multi-level Preemption in Ethernet}, Work-in-Progress (WiP) Session, 30th Euromicro Conference on Real-Time Systems (ECRTS), pp. 16-18, 2018.
        
    \item \textbf{ M. A. Ojewale}, P. Meumeu Yomsi, B. Nikolić, \textit{Worst-case traversal time analysis of TSN with multi-level preemption}, Journal of Systems Architecture (JSA), Volume 116, 2021, 102079, ISSN 1383-7621, \url{https://doi.org/10.1016/j.sysarc.2021.102079}.


\end{itemize}

\subsection{Configuration and evaluation}

This contribution answers $\operatorname{RQ}_3$. It addresses the synthesis problem for multi-level frame preemption in TSN. Specifically, given a set of flows and network topology,we present a framework to ($1$)~assign priorities to flows; ($2$)~determine the appropriate level of preemption to enable; and finally ($3$)~assign flows to preemption classes. We experimentally evaluate the performance of the proposed framework and our results show that the proposed scheme outperforms Deadline Monotonic Priority Ordering, which is known to dominate most other priority assignment schemes in the literature. Our approach ensures that only the required number of preemption levels are enabled since each additional preemption level is associated with significant hardware overheads that can increase switch manufacturing costs.

We also examine $\operatorname{RQ}_3$ from the perspective of flow routing. Indeed, among others. \cite{Nayak2017}, \cite{Singh2017}, and~\cite{gavrilut2017fault} highlighted the importance of routing in achieving low latency, predictability, and reduced architectural cost. In this work, we follow the same path and focus on the routing problem of TSN flows, since an inappropriate routing strategy can increase the number of transmission operations, resulting in additional delays. Moreover, the blocking time of flows in the network may increase if too many flows try to traverse the same path at the same time. We believe that a strategy that minimizes the number of transmission operations and the blocking time of each flow would help circumvent and/or mitigate these situations. Specifically, we proposed two routing heuristics, the algorithm \textit{Load-Balanced, Dynamic, and Replication-aware Routing} ($\lbdrr$) and the algorithm \textit{Congestion Recovering, Dynamic and Replication-aware Routing} ($\crdrr$), to address the load-balancing and congestion issues in TSN. We evaluated the performance of the proposed schemes compared to the popular \textit{Shortest Path} (SPA) and \textit{Weighted Equal Cost Multi-Path} (wt-ECMP) routing algorithms and found an improvement of more than $70\%$ and $20\%$, respectively. These improvements are observed in terms of the maximum load transmitted on an edge. Moreover, the proposed heuristics show high scalability in terms of increasing the number of flows. The above contributions are captured in the following publications:

\begin{itemize}
    \item \textbf{M. A. Ojewale}, P. Meumeu Yomsi, and L. Almeida, \textit{A Configuration Framework for Multi-level Preemption Schemes in Time Sensitive Networking}, 30th International Conference on Real-Time Networks and Systems (RTNS 2022). Association for Computing Machinery, New York, NY, USA, 219–229. \url{https://doi.org/10.1145/ 3534879.3534891}.

    
    \item \textbf{M. A. Ojewale} and P. Meumeu Yomsi, \textit{Routing heuristics for load-balanced transmission in TSN-based networks}, SIGBED Rev. 16, 4 (December 2019), 20–25. \url{https://doi.org/10.1145/3378408.3378411}.
    
\end{itemize}
 
\section{Significance of the contributions}
\label{sec:introduction:significance}
The results presented in this dissertation have significant implications for the field of real-time communication. A recent survey of communication solutions in the industry shows that Ethernet is leading the race in several DRES domains~\citep{Akesson2020AnES}. In addition, studies have shown that the performance of standard Ethernet with frame preemption is comparable to that of the widely studied Time Aware Shaper (TAS), which is more complex and expensive to implement~\citep{Thiele2016Formal, bello2019perspective, Gogolev2020Simpler}. Frame preemption is not only easier to implement and configure, but also allows more efficient use of network bandwidth, requires fewer hardware resources to implement, and is more flexible than TAS ~\citep{Pruski2021Implementation, Gogolev2020Simpler}. However, several studies have pointed out that the major limitation of the current frame preemption specification in the standards is that it only allows one level of preemption~\citep{bello2019perspective, Gogolev2020Simpler, ASHJAEI2021novel}. 

\begin{tcolorbox}
    By addressing the main limitations of TSN frame preemption specifications, this work promotes standard Ethernet with multi-level frame preemption as a simpler and cheaper alternative communication solution that could lead to a paradigm shift in the development of future DRES.
\end{tcolorbox}

 

\section{Dissertation structure}
\label{sec:introduction:thesis_structure}
The rest of this document is structured as follows.
\begin{itemize}
	\item Chapter~\ref{chap:background} introduces background concepts necessary for a smooth understanding of our contributions. First, real-time communication is introduced, and then an inexhaustive but representative set of protocols developed for real-time communication is discussed. Then Ethernet and TSN are examined in detail. Then the TSN frame preemption feature is discussed in detail and some of its limitations are mentioned. Finally, some related work relevant to this thesis is presented.
 
	\item Chapter~\ref{chap:feasibility} details the findings on the feasibility and implementation costs of multi-level preemption in TSN. It contains a detailed analysis of how the processes for transmitting and receiving frames can be modified to support multi-level preemption. It also includes the requirements analysis results and some recommendations for implementation. In addition, the chapter quantifies the hardware implementation cost for multi-level preemption on an FPGA platform and compares it to the implementation cost of other TSN traffic control mechanisms.

    \item Chapter~\ref{chap:model-analysis-configuration} discusses the framework chosen for modeling and analysis in this thesis. This includes the network, traffic, and configuration models and assumptions, as well as an explanation of the CPA framework. The chapter also covers a detailed WCTT analysis of traffic flows under a multi-level preemption scheme using the CPA approach and presents the configuration framework for this scheme.

	\item Chapter~\ref{chap:evaluation} contains the extensive quantitative evaluations of both the WCTT analysis and the configuration framework presented in the previous chapter. Using synthetic and real-world use cases, we comprehensively evaluate the performance of the multi-level preemption scheme.
	
	\item Chapter~\ref{chap:routing} presents routing heuristics to improve the responsiveness and reliability of frame transmission in TSN. In particular, two routing heuristics, referred to as $\lbdrr$ and $\crdrr$, have been proposed to solve the congestion avoidance and congestion recovery problems, respectively.
	
	\item Chapter~\ref{chap:conclusion} contains a summary of the results of the thesis, the validation of the thesis, and the relevant conclusions. Finally, this chapter discusses the limitations of the thesis and some directions for future work.
\end{itemize} 

==> sections/model-analysis-config/analysis.tex <==
% \chapter{Worst-Case Traversal Time Analysis}
% \label{chap:analysis}
% \begin{center}
% 	\fbox{\bf
% 		\centering
% 		\begin{minipage}{\linewidth}
% 			\centering
% 			The outcome of the work that has been presented in this chapter titled ``Worst-case traversal time analysis of TSN with multi-level preemption'' was accepted in the {Journal of Systems Architecture} ({JSA}), Vol. 116, 2021. \footnote{https://doi.org/10.1016/j.sysarc.2021.102079}.   
% 	\end{minipage}}
% \end{center} In Chapter~\ref{chap:feasibility} and~\ref{chap:Implementation}, we have extensively discussed the feasibility of multi-level preemption and provided implementation recommendations.

In this section, we present results on the worst-case traversal time (WCTT) of frames under the assumption of multi-level preemption. To this end, we extend the worst-case performance analysis for $1$-level preemption presented by~\cite{Thiele2016Formal}, where the authors used the Compositional Performance Analysis (CPA) framework to analyze the delay experienced by each frame in a switched Ethernet network. We recall that CPA is useful for analyzing large and complex systems because it allows decomposing the performance of a system into the performance of its individual components, which allows for identifying bottlenecks and optimizing the overall performance of the system. First, we give a brief background on CPA in Section~\ref{sec:analysis:cpa} and then present the analysis in Section~\ref{sec:analysis:approach}

%
% \section{Model of computation}
% \label{sec:analysis:model}
% \input{feupphdteses/sections/analysis/sections/model.tex}
%
\subsection{A brief background on CPA}
\label{sec:analysis:cpa}
Before presenting our proposed WCTT analysis, it is important to give the reader a brief background on the CPA approach so that they can easily understand the rest of this chapter. For a complete and detailed description of the basic concepts, we refer the interested reader to~\citep{henia2005system}. In this framework, a component is modeled as a resource~$\rho$ that provides a service to one or more tasks. Task activations are abstracted by an event model that defines an upper-bound (denoted by $\eta^+(\Delta t)$) and a lower-bound (denoted by $\eta^-(\Delta t)$) on the number of activations within a half-open time interval $[t, t+\Delta t)$. This framework also defines a distance function $\delta^+(q)$ (resp. $\delta^-(q)$), which gives an upper (resp. lower) bound on the maximum (resp. minimum) time at which the activation instance $q^{\operatorname{th}}$ can occur~\citep{henia2005system, handbook2017cpa}. Figure~\ref{cpa-even-model} illustrates the event model of a task with a period and jitter of 50-time units. A jitter of 50 time units (and equal to the period) means that two instances can occur simultaneously ($\delta^-(2) = 0$; $\eta^+(0) = 2$) or two periods apart ($\delta^+(2) = 100$; $\eta^-(100) = 0$).

\begin{figure}
  \centering
  \begin{tabular}[b]{c}
      \includegraphics[width=.40\linewidth, height =3in]{feupphdteses/sections/analysis/images/cpa-event-arrival-function} \\
    \small (a.) An event arrival function.
  \end{tabular} \qquad
  \begin{tabular}[b]{c}
      \includegraphics[width=.45\linewidth, height=3.1in]{feupphdteses/sections/analysis/images/cpa-distance-function} \\
    \small (b.) An event distance function
  \end{tabular}
  \caption{CPA event model for a task with a period and jitter of 50 time units.}
  \label{cpa-even-model}
\end{figure}

The service period of each task, say $\tau_i$, is bounded by two parameters: from above by $C_i^+$ and from below by $C_i^-$. These parameters represent the longest and shortest time, respectively, that the resource, say $\rho$, takes to service an instance of $\tau_i$ without blocking or interference. The worst-case response time (WCRT) of the task $\tau_i$ is examined within what is called a \textit{level-$i$ busy period}. In summary, this is a time interval $[\sigma, \mu]$ in which only task instances belonging to~$hep(i)$ (except the first job generated from task $\tau_j \in lp(i)$ with the longest $C_j^+$), executed throughout $[\sigma, \mu]$, but no jobs belonging to~$hep(i)$ are executed in $[\sigma - \epsilon, \sigma)$ or $(\mu, \mu + \epsilon]$ for any arbitrary small $\epsilon > 0$.

Since the WCRT of $\tau_i$ may not occur on its first activation, the CPA examines all~$q$ activations of $\tau_i$ within the level-$i$ busy period. To this end, it defines an \textit{q-activation processing time} $B_i(q)$, which describes how long the resource $\rho$ is busy processing $q$ jobs of $\tau_i$. This is computed in Equation~\ref{eqn:busy-time}.

\begin{equation}
    \label{eqn:busy-time}
        B_i(q) = Q^+_i(q) + C^+_i  
    \end{equation}

\noindent Note in Equation~\ref{eqn:busy-time} that $B_i(q)$ assumes a non-preemptive scheduling scheme. Here $Q_i^+(q)$ is the time interval between the start of the level-i busy period and the start of service of the $q^{th}$ instance of~$\tau_i$. It is calculated as in Equation~\ref{eqn:queueing-delay-cpa}.

\begin{equation}
    \label{eqn:queueing-delay-cpa}
       Q_i^+(q) = \max_{j \: \in \: lp(i)} \left\{ C_j^{+} \right\}  + (q-1) \cdot C^+_i  + \displaystyle\sum_{k \in hp(i)} C^+_k \cdot \eta_k^+\left(Q_i(q)+ \epsilon\right)
    \end{equation}

\noindent In Equation~\ref{eqn:queueing-delay-cpa}, $lp(i)$ and $hp(i)$ denote the set of tasks with a lower and higher priority than $\tau_i$, respectively. The first term computes the maximum delay that can be caused by the presence of a lower-priority task in the system; the second term estimates the delay caused by processing all previous $q-1$ instances, and the third term computes all possible delays caused by serving higher priority tasks within $B_i(q)$. It is worth noting that Equation~\ref{eqn:queueing-delay-cpa} is reminiscent of the Worst-Case Response Time estimation for the classical single-core fixed-priority tasks and is also solved using a fixed-point algorithm, i.e., the solution is computed iteratively and the algorithm stops as soon as two consecutive values of $Q_i^+(q)$ are equal or when a value exceeds the deadline. In the latter case, the set of tasks is deemed unschedulable. Having obtained $Q_i^+(q)$, we can derive the maximum number of activations $q_i^+$ of $\tau_i$ within $B_i(q)$ using Equation~\ref{eqn:maximum_activations}.

\begin{equation}
    \label{eqn:maximum_activations}
        q_i^+ =  \min \{ q \ge 1 \mid B_i(q) < \delta_i^-(q+1) \}
    \end{equation}
    
This equation computes the first $q_i$ instances of $\tau_i$ such that the completion time of instance $q_i$ is less than the earliest arrival time of instance $q_{i+1}$. The response time of the $q^{\operatorname{th}}$ instance of $\tau_i$ is given by the difference between the time when all $q$ instances of $\tau_i$ are processed and the arrival time of instance $q$. Formally, this is given by Equation~\ref{eqn:response-time-q}.

\begin{equation} 
\label{eqn:response-time-q} 
R_i^+(q) = B_i(q) - \delta_i^-(q) 
\end{equation}

Finally, the WCRT $R_i^+$ of~$\tau_i$ is the maximum $R_i^+(q)$ over all $q_i^+$ activations of~$\tau_i$ within the busy window and is calculated by Equation~\ref{eqn:response-time}. 

\begin{equation}
    \label{eqn:response-time}
        R_i^+ = \max_{1\leq q \leq q_i^+}\left\{R_i^+(q)\right\}
    \end{equation}

So far, we have discussed the worst-case delay at each resource node, also referred to as \textit{local analysis}. Specifically, at each resource node, a rigorous computation is performed on the maximum possible blocking/interference that a task can suffer. This means that the potential interference between any two tasks is effectively captured when performing local analysis at the shared resource node. However, in many cases, real-time applications involve interacting tasks that share different resources. To evaluate the WCRT of a task in this scenario, the CPA defines an \textit{event propagation} step in addition to the local analysis step. Here, the output of each resource along the execution path of a task serves as the input to the next, and $R_i^+(q)$ at the last node is the WCRT of the task.


The CPA approach has been applied to standard Ethernet~\citep{Rox2010, thiele2015improving}, AVB~\citep{Diemer2012}, and TSN~\citep{ Thiele2016BLS, Thiele2016Formal}. In these works, the output ports of the switches are \textit{resources} and flows are \textit{tasks}. The frames are \textit{jobs} or \textit{instances} of the tasks and the path of a flow is modeled as a chain of dependent tasks~\citep{Diemer2012}. Specifically, resources render some \textit{service(s)} (transmission) to some task activations (frames) upon the occurrence of an event (arrival of frames) within a time window (a level-$i$ busy period). In this context, the service period of each frame is bounded by two parameters: from above by~$C^+$ and from below by~$C^-$. These parameters represent the longest and the shortest time for the frame to transmit in the absence of any interference. They depend, of course, on the minimum and maximum possible payload $p^{-/+}$ of the flow to which the frame belongs and on the speed of the output link. Equation~\ref{sec:analysis:C+-} illustrates the relationship between these parameters\footnote{The minimum size of a frame is $84$~bytes according to the specification of the Standard}.
\begin{equation}
\label{sec:analysis:C+-}
    C^{-/+} = \frac{\operatorname{42\: bytes} + \max\{\operatorname{42\: bytes}, \: p^{-/+}\}}{rTX}
\end{equation}

In this equation, $rTX$ represents the transmission speed on the port link and the constant terms (here,~$42$) represent the protocol overhead and minimum frame payload requirement as specified in the Standards~\citep{IEEE-Std-802.1Q-2018}.

\begin{figure}[htb]
    \centering 
    \includegraphics[scale=0.7]{feupphdteses/sections/analysis/images/End-to-end-delay-components-1} 
    \caption{End-to-end delay components.} 
    \label{fig:end-to-end-delay-components}
\end{figure}

As shown in Figure~\ref{fig:end-to-end-delay-components}, the end-to-end delay experienced by a frame in a switch fabric is composed of the following five components: ($1$)~the input delay at the switch input port; ($2$)~the processing delay; ($3$)~the queuing delay at the switch output port; ($4$)~the propagation delay; and finally ($5$)~the transmission delay~\citep{Finn2017}. As pointed out by~\cite{Thiele2016Formal}, all of these components are implementation-dependent and are generally on the order of a few clock cycles, with the exception of the queueing delay, which is captured in Equation~\ref{eqn:queueing-delay-cpa} and whose components are shown in Figure~\ref{fig:queqing-delay-components}.

\begin{figure}[htb]
    \centering
    \includegraphics[scale = 0.75]{feupphdteses/sections/analysis/images/cpa-delay-components-3}
    \caption{Queuing delay components.}
    \label{fig:queqing-delay-components}
    \vspace{-0.1in}
\end{figure}

In Figure~\ref{fig:queqing-delay-components}, frame $f_i^q$ arrives at time $a_i^q$ during the transmission of a frame of the lower preemption class (green box). Before $a_i^q$, the express class frame (first red box) and two other frames (first two yellow boxes) with the same priority and preemption class as $f_i^q$ had arrived. The preemption operation commands that a minimum number of bytes have been transmitted and a number of bytes remain for the preempted fragment to satisfy the minimum size of a valid Ethernet frame. This brings the highest possible blocking that a preempting frame can experience to the size of the largest non-preemptable fragment of a preemptable frame, i.e., $143$~bytes of data~\citep{Thiele2016Formal} and explains the transmission process of the lower priority frame before it is preempted. After the lower priority frame is preempted, the express frame, all pending frames of the same priority, and all newly arrived express frames are transmitted, thus forcing $f_i^q$ to be served only afterward.

In addition to the queueing delay components captured in Equation~\ref{eqn:queueing-delay-cpa}, preemption overhead is another term that should be considered. This is not the case in the general CPA model~\citep{handbook2017cpa}. Preemption overhead is an important factor in the TSN frame transmission scheme. The total overhead incurred by each preemption is $12$~bytes (i.e., $6$-byte preamble, $1$-byte start frame delimiter, $1$-byte frame count variable; and finally $4$-byte error check variable)~\citep{ojewale2018multi}. In addition, the \textit{Inter Frame Gap} (IFG) between two consecutive transmissions must be considered before the next frame/fragment is transmitted. According to the standards, the size of each IFG is equal to the time required to transmit $12$~bytes of data. Thus, the total overhead associated with each preemption amounts to $24$~bytes. \cite{Thiele2016Formal} have also proved that the maximum number of preemptions that a single frame can suffer is given by Equation~\ref{eqn:max-preemption}.

\begin{equation} \label{eqn:max-preemption} F^+_i = \Bigl\lfloor\dfrac{p_i^+ - 42\: bytes}{60\: bytes}\Bigr\rfloor
\end{equation}

Equation~\ref{eqn:max-preemption} provides an upper bound on the number of times an Ethernet frame can be preempted based on the minimum valid frame size constraints defined in the standards. In this equation, the constant terms (here~$42$ and~$60$) are the minimum~payload requirements for the first and subsequent fragments of a preemptable frame in the standards~\citep{IEEE-Std-802.1Q-2018}. For each flow~$f_i$, its worst-case traversal time is obtained by combining the Equations~\ref{eqn:busy-time}~and~\ref{eqn:response-time-q}.

\begin{tcolorbox} We note that Equation~\ref{eqn:response-time-q} does not account for preemption overhead. This computation is refined to include the cost in Section~\ref{subsec:Wctt}. Note also that the CPA model allows for arbitrary deadlines, i.e., there is no particular correlation between the deadline and the minimum inter-arrival time of each flow.
\end{tcolorbox}

\subsection{Proposed analysis}
\label{sec:analysis:approach}
In the multi-level preemption scheme, each frame can belong to only one of the following three categories: ($1$)~can preempt other frames and is not preemptable, i.e., it cannot be preempted by any other frame because it belongs to the highest preemption class (e.g., express traffic); ($2$)~can preempt other frames and can also be preempted; and finally, ($3$)~cannot preempt other frames and can be preempted by any frame in the categories~($1$) and ($2$). We refer to the categories ($1$), ($2$), and ($3$) as ``express flows'', ``preemptable flows with firm timing requirements'' (tpflows), and ``best effort flows'' (bpflows), respectively. With this nomenclature in mind, we have all we need to discuss the components of the end-to-end delay of a frame, say~$f_i^q$, arriving at time $a_i^q$. Briefly, there are four components, namely:
\begin{tcolorbox}
\begin{enumerate} \item the \textit{lower priority blocking} -- i.e., the delay due to frames with a lower priority than~$f_i$; \item the \textit{same-priority blocking} -- i.e., the delay due to frames with the same priority as $f_i$; \item the \textit{higher priority interference} -- i.e., the delay associated with frame(s) with a higher priority than~$f_i$;~and finally, \item the \textit{preemption overheads}, i.e., the delay due to preemption overheads.
\end{enumerate}
\end{tcolorbox}
 

\subsubsection{Lower-priority blocking}
\label{subsec:Lower-priority blocking}
In this section, we derive an upper bound on the lower-priority blocking experienced by a frame in each flow class.
\vspace{0.1in}

\noindent $\triangleright$ {\bf Lower-priority blocking for ``express flows''.}
Each express frame can experience the maximum lower-priority blocking in two scenarios: ($i$)~if it is blocked by the largest lower-priority express frame since frames in the same preemption class are served non-preemptively; or ($ii$)~if it is blocked by the largest non-preemptable fragment of a preemptable frame. Recall that any preemptable frame less than or equal to $143$~bytes is non-preemptable. Lemma~\ref{lemma:lower-priority-express-blocking} provides an upper bound for blocking due to scenario~($ii$).

\begin{lemma}[$\PB^{\mathcal{E}}_i$]
\label{lemma:lower-priority-express-blocking}
For any express flow~$f_i \in \mathcal{E}$, the maximum blocking of a frame~$f_i^q$ (with $q \ge 1$) caused by a preemptable frame is given by Equation~\ref{eqn:lower-priority-blocking-lemma}.

\begin{equation} 
\label{eqn:lower-priority-blocking-lemma} 
\PB^{\mathcal{E}}_i = \min \Bigg\{ \underbrace{\max_{j\: \in \: \mathcal{P}} \left\{C_j^+\right\}}_{(a)},\: \underbrace{\dfrac{143\: bytes}{rTX}}_{(b)} \Bigg\} 
\end{equation}
\end{lemma}

 \begin{proof}
If all preemptable frames are shorter than $143~bytes$, then the maximum blocking time for any express frame is caused by the largest of these frames. This is captured by term~($a$). On the other hand, the longest non-preemptable fragment of any preemptable frame is $143$~bytes long~\citep{Thiele2016Formal}. This implies a maximum blocking time of $\frac{143\: bytes}{rTX}$ (where $rTX$ is the link speed). This is captured by term ($b$). Therefore, a tight upper bound on the blocking time caused by a preemptable frame to any express frame~$f_i^q$ (with $q \ge 1$) is given by the minimum between terms~($a$) and~($b$), and the lemma follows.
\end{proof}
 
From Lemma~\ref{lemma:lower-priority-express-blocking}, Theorem~\ref{theorem:Lower-priority-blocking-express} provides a tight upper bound on the lower-priority blocking incurred by any express frame.
 
 \begin{theorem}[$\LPB^{\mathcal{E}}_i$]
 \label{theorem:Lower-priority-blocking-express}
 
For any express flow~$f_i \in \mathcal{E}$, if $lp^{\mathcal{E}}(i)$ represents the set of express frames with a lower priority than that of $f_i$, then a tight upper bound on lower-priority blocking for each frame~$f_i^q$ (with $q \ge 1$) is given by Equation~\ref{eqn:lower-priority-blocking-express}.

\begin{equation}
\label{eqn:lower-priority-blocking-express} \LPB^{\mathcal{E}}_i = \max \Bigg\{ \underbrace{\max_{j\: \in \: lp^{\mathcal{E}}(i)}\left\{C_j^+\right\}}_{(a)}, \: \underbrace{ \PB^{\mathcal{E}}_i }_{(b)} \Bigg\}
\end{equation}
 \end{theorem}
 \begin{proof}
 
Each express frame~$f_i^q$ can suffer lower-priority blocking due either to the transmission of ($1$)~a lower-priority express frame or ($2$)~preemptable frame. In the first case, term~($a$) captures the largest blocking time, since frames of the same preemption class are served non-preemptively. On the other hand, if the blocking is caused by a preemptable frame, then Lemma~\ref{lemma:lower-priority-express-blocking} provides an upper bound for lower-priority blocking, i.e., $\PB^{\mathcal{E}}_i$ (term~($b$)). Therefore, a tight upper bound on the blocking time of any express frame~$f_i^q$ (with $q \ge 1$) is given by the maximum between terms~($a$) and~($b$), and the theorem follows.
\end{proof}

\begin{tcolorbox}
    Note that Equations~\ref{eqn:lower-priority-blocking-lemma} and~\ref{eqn:lower-priority-blocking-express} are similar to Equations~5 and~7 in~\citep{Thiele2016Formal}. We explicitly address this behavior in the analysis for the sake of completeness.
\end{tcolorbox}

\noindent $\triangleright$ {\bf Lower-priority blocking for ``tpflows''.}
\label{subsec:Lower-priority blocking-tp}
Any flow can preempt all flows in a lower preemption class by design, but the converse is not true. A tpflow is not an exception to this rule. This means that any tpflow frame~$f_i^q$ can be blocked at most by ($i$)~the largest non-preemptable fragment of any preemptable frame in a lower preemption class or ($ii$)~a lower-priority frame of the same preemption class as $f_i$, since frames of the same class are serviced in a non-preemptable way. Lemma~\ref{lemma:lower-priority-tp-blocking} computes an upper bound on the blocking time incurred by a tpflow frame due to frames in lower preemption classes.

\begin{lemma}[$\PB^{\mathcal{TP}}_i$]
\label{lemma:lower-priority-tp-blocking}
For each flow~$f_i \in \mathcal{ TP }$, the maximum blocking time of each frame~$f_i^q$ (with $q \ge 1$) caused by a frame of a lower preemption class is given by Equation~\ref{eqn:lower-priority-tp-blocking-lemma}.

\begin{equation}
    \label{eqn:lower-priority-tp-blocking-lemma}
    \PB^{\mathcal{TP}}_i =  \: \min \Bigg\{ \underbrace{ \max_{j\: \in \: \{lp(i)\: \mid \:  \operatorname{PC}_j \:  > \: \operatorname{PC}_i\}} \left\{C_j^+\right\}}_{(a)},
\underbrace{\dfrac{143\: bytes}{rTX}}_{(b)} \Bigg\}
\end{equation}
\end{lemma}
 \begin{proof}
The proof of Lemma~\ref{lemma:lower-priority-tp-blocking} is similar to that of Lemma~\ref{lemma:lower-priority-express-blocking}. Given a frame~$f_i^q$, if all frames in a lower preemption class are shorter than $143~bytes$, then the maximum blocking incurred by $f_i^q$ is caused by the largest of these frames. This is captured by term~($a$). Otherwise, the longest non-preemptable fragment of any preemptable frame is $143$~bytes long~\citep{Thiele2016Formal} and this implies a maximum blocking time of $\frac{143\: bytes}{rTX}$ (where $rTX$ is the link speed). This is captured by term ($b$). Therefore, a tight upper bound on the blocking time caused by a preemptable frame of a preemption class lower than~$f_i^q$ is given by the minimum between terms~($a$) and~($b$), and the lemma follows.
\end{proof}

From Lemma~\ref{lemma:lower-priority-tp-blocking}, Theorem~\ref{theorem:Lower-priority blocking-tp} derives a tight upper bound on the lower-priority blocking that occurs on any tpflow frame.
\begin{theorem}[$\LPB^{\mathcal{TP}}_i$]
\label{theorem:Lower-priority blocking-tp}
For any tpflow flow~$f_i \in \mathcal{ TP }$, the maximum lower-priority blocking of any frame~$f_i^q$ (with $q \ge 1$) is given by Equation~\ref{eqn:lower-priority-tpflow}.
\begin{equation}
    \label{eqn:lower-priority-tpflow}
\LPB^{\mathcal{TP}}_i =\max \Bigg\{ \underbrace{\max_{ j\: \in \: \{lp(i)\: \mid \: \operatorname{PC}_i\: = \: \operatorname{PC}_j\}}\left\{C_j^+\right\} }_{(a)}, \:  \underbrace{\PB^{\mathcal{TP}}_i}_{(b)} \Bigg\}
\end{equation}
 \end{theorem}
 
\begin{proof}
Each tpflow frame~$f_i^q$ can be blocked either due to the transmission of ($1$)~frame with lower priority of the same preemption class or ($2$)~a frame with a lower preemption class. In the first case, term~($a$) captures the largest blocking time that can be caused by a frame of the same preemption class, since these frames are served in a non-preemptive manner by design. In the second case, when the blocking is caused by a frame of a lower preemption class, we have already shown in Lemma~\ref{lemma:lower-priority-tp-blocking} that this delay cannot exceed $\PB^{\mathcal{TP}}_i$ (i.e., term~($b$)). Therefore, a safe upper bound on the blocking time suffered by any tpflow frame~$f_i^q$ (with $q \ge 1$) is given by the maximum between terms~($a$) and~($b$), and the theorem follows.
\end{proof}

\noindent $\triangleright$ {\bf Lower-priority blocking for ``bpflows''.}
Since bpflows by assumption belong to the lowest preemption class, it follows that the maximum lower-priority blocking that a bpflow frame can experience is given by the largest lower-priority frame in the same class. This is given by the Equation~\ref{eqn:lower-priority-blocking-bpflow}.
\begin{equation}
    \label{eqn:lower-priority-blocking-bpflow}
    \LPB^{\mathcal{BP}}_i = \max_{j\: \in \: lp^{\mathcal{BP}}_{(i)}}\left\{C_j^+\right\}
\end{equation}

Now that we have discussed in detail the computation of all lower-priority blocking terms, we can proceed with the computation of the same-priority blocking -- i.e., the delay due to frame(s) with the same priority as the flow under analysis.

\subsubsection{Same-priority blocking}
\label{subsec:same-priority blocking}
In the following subsections, we compute upper bounds on the delay that a frame experiences when frames of the same priority are transmitted.
\vspace{0.1in}

\noindent $\triangleright$ {\bf Same-priority blocking for ``express flows''.}
Each express frame $f_i^q$ can be blocked by all frames of the same priority that arrive before it at the time, say $a_i^q$, within the level $i$ busy period. Moreover, all previous $q-1$ instances of $f_i$ must be transmitted before $f_i^q$ is transmitted, and therefore contribute to the same priority blocking term. Therefore, the maximum same-priority blocking $\SPB^{\mathcal{E}}_i$ that express frame $f_i^q$ can experience is given by Equation~\ref{eqn:same-priority-express}.
\begin{equation}
    \label{eqn:same-priority-express}
    \SPB^{\mathcal{E}}_i(q, a_i^q) =  \displaystyle\sum_{j\: \in\: sp(i)} \eta_j^+(a_i^q) \cdot C^+_j + (q-1) \cdot C_i^+
\end{equation}
In Equation~\ref{eqn:same-priority-express}, $sp(i)$ denotes the set of all flows with the same priority as~$f_i$. The first term computes the maximum delay due to the transmission of all frames with the same priority that arrive before $a_i^q$, while the second term computes the maximum delay that~$f_i$ incurs due to the transmission of all previous $q-1$ instances.
\vspace{0.1in}

\noindent $\triangleright$ {\bf Same-priority blocking for ``tpflow''.}
\label{subsec:same-priority blocking-tp}
Similar to express frames, each tpflow frame $f_i^q$ can be blocked by all frames with the same priority that arrive before $a_i^q$ within the level-$i$ busy period, as well as by all previous $q-1$ instances of~$f_i$. Moreover, since $f_i^q$ is preemptable, there may be an additional delay even after its transmission begins. Only during the transmission of its last fragment, which is not preemptable, is it guaranteed not to be interrupted. In other words, the last fragment of $f_i^q$ must wait until all previous fragments of the instance have been transmitted. The size of this last fragment is equal to the minimum valid Ethernet frame size~\citep{Thiele2016Formal}. With the above, the maximum same-priority blocking $\SPB^{\mathcal{TP}}_i$ that $f_i^q$ can suffer is given by Equation~\ref{eqn:same-priority-tpflow}.

\begin{equation}
    \label{eqn:same-priority-tpflow}
    \SPB^{\mathcal{TP}}_i(q, a_i^q) =\displaystyle\sum_{j\: \in\: sp(i)} \eta_j^+(a_i^q) \cdot C^+_j + (q-1) \cdot C_i^+ + \left(C_i^+ - \dfrac{84\: bytes}{rTX}\right)  
\end{equation}
In Equation~\ref{eqn:same-priority-tpflow}, the first term computes the maximum delay due to the transmission of all frames with the same priority as~$f_i$ that arrive before $a_i^q$, while the second term computes the delay due to the transmission of all previous $q-1$ instances of $f_i$. Finally, the third term computes the maximum delay due to the transmission of all non-final fragments of~$f_i^q$.
\vspace{0.1in}

\noindent $\triangleright$ {\bf Same-priority blocking of ``bpflows''.}
The notion of same-priority blocking for bpflows is identical to that of tpflows in Equation~\ref{eqn:same-priority-tpflow}. The reason for this is that the behavior of frames within these classes is identical since they are transmitted non-preemptively and in a FIFO manner. This means that a bpflow frame $f_i^q$ can be blocked by all frames with the same priority that arrive before its arrival time $a_i^q$ within the level-$i$ busy period; all previous $q-1$ instances of~$f_i$; and by all preceding fragments (i.e., the non-terminal fragments) if it has been preempted. For this class, Equation~\ref{eqn:same-priority-tpflow} also suffices, with the $\mathcal{TP}$ superscript replaced by $\mathcal{BP}$ to reflect the corresponding frame class.

\subsubsection{Higher-priority Interference}
\label{subsec:higher-priority-interference}
Regardless of its class, any frame~$f_i$ cannot start its transmission if another frame with higher priority~\citep{thiele2014improving} is present. This means that any frames of higher priority that arrive before the frame~$f_i^q$ is transmitted will always interfere with its transmission. It follows that the higher-priority interference term for the three classes of frames is given by Equation~\ref{eqn:higher-priority-blocking}.
\begin{equation}
    \label{eqn:higher-priority-blocking}
    \HPI_i(\Delta t) = \displaystyle\sum_{j\: \in\: hp(i)} \eta_j^+(\Delta t)\cdot C^+_j
\end{equation}

\subsubsection{Preemption overheads}
\label{subsec:preemption-overead}
Each preemption operation has some overhead associated with it, equal to the time it takes to transmit $24$~bytes of data. This overhead is always added to the transmission time of the preempted frame. Since express frames are transmitted in a non-preemptive manner, they do not incur preemption overhead. Therefore, only tpflows and bpflows incur preemption overheads since they are preemptable. From an analytical point of view, the approach to compute the preemption overhead terms is identical for these two preemption classes.

Roughly speaking, the maximum preemption overheads that a preemptable frame $f_i^q$ can incur depends only on the \textit{maximum number} of preemption events that can occur between its arrival time until the transmission of the first bit of the last non-preemptable fragment. In this sense, the maximum number of preemption events can occur in either of the following two cases: 

\begin{itemize} 

\item[($1$)] all preemptable frames transmitted between $a_i^q$ and the complete transmission of $f_i^q$ are preempted for the maximum number of times beyond which cutting a frame into more fragments would violate the minimum Ethernet frame size (see Equation~\ref{eqn:max-preemption}).

\item[($2$)] all possible arrivals of higher priority frames belonging to a higher preemption class occur and each of them causes a preemption.
\end{itemize}

To evaluate the first case, we consider a preemptable frame~$f_i^q$ transmitted within the busy period of length, say $\Delta t$. Then we compute the maximum number of times that $f_i^q$ and all other preemptable frames transmitted within the window of size $\Delta t$ can be preempted. We can distinguish between three different types of preemptable frames, namely: ($1$)~preemptable frames with a lower priority than~$f_i$; ($2$)~preemptable frames with the same priority as~$f_i$; and finally ($3$)~preemptable frames with a higher priority than~$f_i$. We discuss each of these three cases below.
\vspace{0.1in}

\noindent $\triangleright$ {\bf Maximum number of preemptions incurred by a lower-priority preemptable frame.}
This maximum number of preemptions occurs when a preemptable frame with lower priority, e.g.~$f_j^k$, which is obstructing the transmission of $f_i^q$ gets preempted a maximum number of times. Frame~$f_j^k$ can either ($i$) belong to a lower preemption class than $f_i^q$ or ($ii$) have the same preemption class as~$f_i^q$.\\ 

\textbf{Case~($i$).} If~$f_j^k$ belongs to a lower preemption class, then it will be preempted at most once by~$f_i^q$ or by another frame belonging to a higher class. By design, the preempted frame will not resume its transmission until all pending frames of a higher preemption class (including $f_i^q$) have completed their transmission. \\

\textbf{Case~($ii$).} If~$f_j^k$ is in the same preemption class as $f_i^q$, then~$f_j^k$ can be preempted multiple times and $f_i^q$ can begin its transmission only after~$f_j^k$ has completed its transmission. Using Equation~\ref{eqn:max-preemption}, we derive the maximum number of preemptions $N_i^{\mathcal{P},\: lp}$ incurred by a preemptable frame with lower priority in the same preemption class as~$f_i^q$ in Equation~\ref{eqn:max-preemption-lp-tpflow}.

\begin{equation}
    \label{eqn:max-preemption-lp-tpflow}
    N_i^{\mathcal{P},\: lp} = \max_{\{j \: \mid \: \operatorname{PC}_i\: = \: \operatorname{PC}_j\: \wedge\:  i \: > \: j\}}\left\{F_j^+\right\} 
\end{equation}
\vspace{0.1in}

\noindent $\triangleright$ {\bf Maximum number of preemptions incurred by same-priority preemptable frames.}
This number includes the preemptions incurred by frames with the same priority as $f_i^q$ that arrive before $a_i^q$ within the level-$i$ busy period as well as the preemptions suffered by $f_i^q$ up to its last non-preemptable fragment. Using Equation~\ref{eqn:max-preemption}, the maximum number of preemptions $N_i^{\mathcal{P},\: sp}(q, a_i^q)$ is computed in Equation~\ref{eqn:max-preemption-sp-tpflow}.
\begin{equation}
    \label{eqn:max-preemption-sp-tpflow}
        N_i^{\mathcal{P},\: sp}(q, a_i^q) = q \cdot F_i^+ - 1 +  \displaystyle\sum_{j\: \in\: sp(i)} \eta_j^+(a_i^q) \cdot F^+_j
\end{equation}
The first term of Equation~\ref{eqn:max-preemption-sp-tpflow} computes the maximum preemption incurred by the first $q$ instances of~$f_i$ apart from the last fragment, while the second term computes the maximum preemption incurred by all other frames with the same priority as~$f_i$ arriving before~$f_i^q$ within the busy-window.
\vspace{0.1in}

\noindent $\triangleright$ {\bf Maximum number of preemptions incurred by higher-priority preemptable frames.}
This number includes the preemptions incurred by all frames with a higher priority than $f_i^q$ transmitted during~$\Delta t$, i.e., the transmission period of $f_i^q$. It is denoted by $N_i^{\mathcal{P},\: hp}(\Delta t)$ and occurs when all these frames are preempted as many times as possible, which is given by Equation~\ref{eqn:max-preemption-hp-tpflow}.
\begin{equation}
    \label{eqn:max-preemption-hp-tpflow}
     N_i^{\mathcal{P},\: hp}(\Delta t)  = \displaystyle\sum_{\{j\: \in\: hp(i)\: \wedge \: j \: \in\: \mathcal{P}\}} \eta_j^+(\Delta t)\cdot F^+_j
\end{equation}

Putting Equations~\ref{eqn:max-preemption-lp-tpflow},~\ref{eqn:max-preemption-sp-tpflow}, and~\ref{eqn:max-preemption-hp-tpflow} together, the maximum number of preemptions incurred by the preemptable frames transmitted during $\Delta t$ is obtained from Equation~\ref{eqn:sum-max-preemptions}.
\begin{equation}
    \label{eqn:sum-max-preemptions}
    N_i(q, a_i^q,\Delta t) = N_i^{\mathcal{P},\: lp} + N_i^{\mathcal{P},\: sp}(q, a_i^q) + N_i^{\mathcal{P},\: hp}(\Delta t)
\end{equation}

With this Equation~\ref{eqn:sum-max-preemptions} we have everything we need to derive an upper bound for the maximum preemption overhead of any preemptable frame~$f_i^q$, as formalized in the Theorem~\ref{theorem:preemption-overhead} below.

\begin{theorem}[$\PO_i^{\mathcal{P}}(\Delta t,q,a_i^q)$]
\label{theorem:preemption-overhead}
For any preemptable flow~$f_i \in \mathcal{P}$, an upper bound on the maximum preemption overhead incurred by frame~$f_i^q$ (with $q \ge 1$) arriving at time~$a_i^q$ within the busy-period~$\Delta t$, is given by Equation~\ref{eqn:preemption-overhead}.
\begin{equation}
    \label{eqn:preemption-overhead}
     \PO_i^{\mathcal{P}}(\Delta t,q,a_i^q) = \underbrace{\frac{24 \: bytes}{rTX} }_{(a)} \times 
  \min \bigg\{ \bigg(\underbrace{\sum_{j\: \in \: \{\mathcal{F}\: |\: \operatorname{PC}_j\:  < \: \operatorname{PC}_i\}} \eta^+_j(\Delta t)}_{(b)} \bigg) , \: \underbrace{\:N_i(q, a_i^q, \Delta t) }_{(c)}\bigg\}
\end{equation}
\end{theorem}
\begin{proof}
The maximum preemption overhead is reached in one of two cases: ( Case~$1$)~All preemptable frames incur the maximum possible number of preemptions; or ( Case~$2$)~All incoming frames belonging to a higher preemption classes cause a preemption. For the first case, Equation~\ref{eqn:sum-max-preemptions} contained in term~($c$) provides an upper bound. For the situation described in Case~$2$, a computation of the maximum number of arrivals of frames in a higher preemption class is captured by term~($b$). Therefore, the actual number of preemptions cannot be greater than the minimum of these two terms. Now, since each preemption operation generates an overhead equal to term ($a$), the theorem follows.
\end{proof}

\subsubsection{Worst-case queuing delay}
So far, we have discussed the individual components of the worst-case queuing delay. For each frame~$f_i^q$ arriving at time~$a_i^q$ within the busy period, we obtain an upper bound $Q_i(q,a_i^q)$ for this factor by summing all these terms, as formally stated in Equation~\ref{eqn:wcqd}.

\begin{equation}
    \label{eqn:wcqd}
     Q_i(q,a_i^q) =  
         \begin{cases}
\LPB_i^{\mathcal{E}} + \SPB_i^{\mathcal{E}}(q,a_i^q) + \HPI_i(Q_i(q,a_i^q)) & \operatorname{if} f_i \: \in\: \mathcal{E}; \\ \\*
\LPB^{\mathcal{TP}}_i + \SPB^{\mathcal{TP}}_i(q, a_i^q) + \HPI_i(Q_i(q,a_i^q))+  \PO_i^{\mathcal{P}}(Q_i(q,a_i^q)) & \operatorname{if} f_i \: \in\: \mathcal{TP}; \\  \\*
\LPB^{\mathcal{BP}}_i + \SPB^{\mathcal{BP}}_i(q, a_i^q) + \HPI_i(Q_i(q,a_i^q))+  \PO_i^{\mathcal{P}}(Q_i(q,a_i^q)) & \operatorname{if} f_i \: \in\: \mathcal{BP}
\end{cases}
\end{equation}

Note that Equation~\ref{eqn:wcqd} defines an iterative fixed-point process, since $Q_i(q,a_i^q)$ appears on both sides of the equation. Therefore, a valid solution for each frame~$f_i^q$ is obtained by starting the fixed point algorithm with the base value $C_i^+$. The algorithm stops as soon as two consecutive values of $Q_i(q,a_i^q)$ are identical or the relative deadline associated with the flow~$f_i$ is exceeded. In the latter case, the timing requirement of~$f_i$ is violated and there is no valid solution.

\subsubsection{Worst-case traversal time}
\label{subsec:Wctt}

For each frame~$f_i^q$ arriving at time $a_i^q$, it follows from the discussions in the previous sections that its worst-case traversal time~$(\WCTT_i(q, a_i^q))$ is given by the combination of the Equations~\ref{eqn:busy-time}~and~\ref{eqn:response-time-q}, where $Q_i^+(q)$ (in Equation~\ref{eqn:busy-time}) and $\delta_i^-(q)$ (in Equation~\ref{eqn:response-time-q}) are replaced by $Q_i(q,a_i^q)$ and $a_i^q$, respectively. Formally, $\WCTT_i(q, a_i^q)$ is given in Equation~\ref{eqn:WCTT-all}.

\begin{equation}
    \label{eqn:WCTT-all}
    \WCTT_i(q, a_i^q) = \begin{cases}
 Q_i(q,a_i^q) + C^+_i  - a^q_i & \operatorname{if} f_i \: \in\: \mathcal{E};\\ \\*
 Q_i(q,a_i^q) + \dfrac{84 bytes}{rTX} -  a^q_i & \operatorname{if} f_i \: \in\: \mathcal{TP};\\ \\*
 Q_i(q,a_i^q) + \dfrac{84 bytes}{rTX} -  a^q_i & \operatorname{if} f_i \: \in\: \mathcal{BP} 
\end{cases}
\end{equation}

Finally, the worst-case traversal time for the flow $f_i$ within the level-i busy period, denoted by $\WCTT_i^+$, is obtained by computing the maximum of all $\WCTT_i(q, a_i^q)$, where $1\leq q \leq q_i^+$ and $q_i^+$ is the last frame of $f_i$ in the level-i busy period. Formally, this is expressed in Equation~\ref{eqn:WCTT-max}.

\begin{equation}
    \label{eqn:WCTT-max}
        \WCTT_i^+ = \max_{1\leq q \leq q_i^+}\left\{\WCTT_i(q, a_i^q)\right\}
    \end{equation} 
    
This equation completes the computation of $\WCTT_i^+$ for the flow~$f_i$ within a switch node (i.e., the local analysis). Therefore, the overall traversal time for flow~$f_i$ (i.e., the global analysis) is obtained by adding these values at all individual switch nodes along its transmission path.
Here, the level-i busy period is a time interval $[\sigma, \mu]$ in which only frames belonging to~$hep(i)$ (except for the first frame generated by the flow $f_j \in lp(i)$ with the longest non-preemptable fragment) are transmitted throughout $[\sigma, \mu]$, but no frame belonging to~$hep(i)$ is transmitted in $[\sigma - \epsilon, \sigma)$ or $(\mu, \mu + \epsilon]$ for any arbitrary small $\epsilon > 0$.\\
\begin{tcolorbox}
    To perform the analysis, we considered the scenario that results in the longest level-i busy period for each flow $f_i$ was considered, i.e., the scenario in which either ($1$)~a frame $f_j^k$ in $\operatorname{PC}_i < \operatorname{ PC }_j$ with the longest non-preemptable fragment; or ($2$)~a frame $f_j^k$ in $\operatorname{PC}_i = \operatorname{ PC }_j$ with the largest size and a lower priority than $f_i$, was released just before $f_i$; all flows in $hep(i)$ release a frame at the same time as $f_i$ and finally all future frames are released as soon as legally permissible.
\end{tcolorbox}




==> sections/model-analysis-config/configuration.tex <==
As with most, if not all, real-time and/or time-critical preemptive systems, an appropriate \textit{priority-to-flow assignment} policy plays a central role in the resulting performance of both $1$-level and multi-level preemption schemes to avoid over-provisioning and/or suboptimal use of hardware resources. In this scope, the so-called \textit{Audsley's Optimal Priority Assignment algorithm} (AOPA) has become the reference in many real-time systems, provided there are no priority inversions~\citep{Park2019Optimal, davis2007controller}. Here, ``optimality'' refers to the ability of this algorithm to provide a priority-to-flow assignment that allows all flows to meet their timing requirements when such a scheme exists. \cite{Davis2016Review} noted that AOPA is not applicable in fixed priority schemes with differed preemptions and/or preemption thresholds, and this is the case with preemptive TSN. Therefore, the so-called \textit{Deadline Monotonic Priority Ordering} (DMPO)~\citep{Davis2016Review} is often used in practice and is known to dominate most other priority assignment heuristics in terms of schedulability~\citep{lee2021ml}. Nevertheless, DMPO is also not suitable for priority assignment in preemptive TSN, as it provides a fully ordered priority list for the flowset. Ethernet only supports up to eight priority levels. With this limitation, a fully ordered priority list leads to another bin packing problem, which is known to be strongly NP-Complete~\citep{lodi2002recent}. An efficient priority assignment scheme should not only provide the best possible priority ordering for flows but also assign multiple flows to the same priority levels in the best possible way.

Note that \textit{multi-level preemption scheme} brings a whole new dimension of configuration synthesis in addition to the challenge of priority assignment. In a $1$-level preemption scheme, the configuration decisions are in fact quite simple and straightforward. They are limited to deciding whether each flow belongs to the express class or the preemptable class. The picture darkens considerably when multi-level preemption is adopted. In this case, the system designer must answer two important questions:
\begin{tcolorbox}
    \begin{enumerate}
    \item How should the number of preemption levels to be activated be determined?

    \item How should the mapping between flow and preemption class be made?     
\end{enumerate}
\end{tcolorbox}


In response to these concerns, it is worth noting that Ethernet can support at most a seven-level preemption scheme\footnote{Ethernet has eight priority levels and thus at most eight preemption classes. Assuming that a flow in one preemption class can preempt any other flow in another preemption class with a lower priority, it follows that Ethernet can support at most a seven-level preemption scheme.}. As reported in Chapter~\ref{chap:feasibility}, each additional preemption level adds significant hardware overheads that can increase the switch manufacturing cost. To ensure optimal use of hardware resources, the system designer must ensure that only the required number of preemption levels are supported for transmitting flows over the network. Figures~\ref{fig:configuration:config-sample-1}, \ref{fig:configuration:config-sample-2}, and \ref{fig:configuration:config-sample-3} illustrate the importance of the preemption level synthesis problem.

\begin{figure}[htb]
  \centering
  \includegraphics[scale=0.8]{feupphdteses/sections/configuration/images/config_sample_1n}
  \caption{Flow $f_2$ misses its deadline with a $2$-level preemption scheme.}
  \label{fig:configuration:config-sample-1}
\end{figure}%

\begin{figure}[htb]
\centering
  \includegraphics[scale=0.8]{feupphdteses/sections/configuration/images/config_sample_2n}
    \caption{All flows meet their deadlines with a $3$-level preemption scheme.}
  \label{fig:configuration:config-sample-2}
\end{figure}

\begin{figure}[htb]
\centering
  \includegraphics[scale=0.8]{feupphdteses/sections/configuration/images/config_sample_3n}
    \caption{All flows meet their deadlines with a $2$-level preemption scheme.}
  \label{fig:configuration:config-sample-3}
\end{figure}

%\caption{Motivation example for the multi-level preemption configuration.}

In these figures, we consider the same four flows ($f_1$, $f_2$, $f_3$, $f_4$). We assume four possible preemption classes: ($1$)~the \textit{highest preemption class}, in which frames are represented by ``red boxes''; ($2$)~the \textit{middle-high preemption class}, in which frames are represented by ``yellow boxes''; ($3$)~the \textit{middle-low preemption class}, where frames are represented by ``black boxes''; and finally ($4$)~the \textit{lowest preemption class}, where frames are represented by ``green boxes''. For this setting, there is no configuration under either a non-preemptive or a $1$-level preemption scheme that allows all flows to meet their timing constraints. Assuming the multi-level preemption scheme, we analyze three configuration scenarios.

In Figure~\ref{fig:configuration:config-sample-1}, flows are divided into three preemption classes and $f_2$ misses its deadline because it is unable to preempt~$f_3$ -- the two frames belong to the same preemption class. In Figure~\ref{fig:configuration:config-sample-2}, the situation improves for $f_2$ and it meets its deadline, but at the cost of an additional preemption class. In Figure~\ref{fig:configuration:config-sample-3}, an appropriate configuration (again with three preemption classes) is used and all frames meet their deadlines. From these observations, it follows that the performance of the multi-level preemption system is highly dependent on the configuration chosen.
\begin{tcolorbox} 
In this section, we advance the state of the art by addressing the above configuration issues. Given a set of flows and a TSN network, we first provide an offline priority assignment scheme for the flow set. Then, we provide an offline framework for determining the appropriate number of preemption levels on the one hand and the flow- to-preemption-class assignment on the other. Taken together, the proposed scheme has two goals: ($1$) to ensure that all flows meet their deadlines, and ($2$) to ensure that hardware resources are used efficiently.
\end{tcolorbox}

\subsection{Definitions}
\label{sec:model-analysis-config:definitions}
In addition to the system model in Section~\ref{sec:model-analysis-config:model}, we introduce the following definitions for any flow set $\mathcal{F}$ and network $\mathcal{G}$.

\begin{definition}[Valid configuration]
\label{def:valid-config}
Any configuration will be stamped as ``valid'' if, upon the flow-to-preemption-class assignment, it conforms to Rules $R_1$, $R_2$ and $R_3$.
\end{definition}

\begin{definition}[Solution]
\label{def:solution}
Any valid configuration will be considered a ``solution'' if all flows $f_i \in \mathcal{F}$ meet their deadlines.
\end{definition}

Rule~$R_2$ from Section~\ref{sec:model:configuration} implies that $\mathcal{C}_x^m$ (with $x \ge 1$) is always sorted in ascending order, i.e. $c_{x,\sigma}^m \le c_{x,\ell}^m$ for all $0 \le \sigma \le \ell \le p-1$. Rule~$R_3$ implies that every integer from $0$ to $m$ must occur \textit{at least once} in every valid configuration. 

\begin{tcolorbox}
    Consequently, the task of generating all valid configurations $\mathcal{C}^m$ can be mapped to the problem of generating all ordered multisets~\citep{blizard1989multiset} of cardinality $p$ with elements from the set $\{0, \ldots, m\}$, where $p$ is the number of unique flow priorities in $\mathcal{F}$.
\end{tcolorbox}


%

%
\subsection{Proposed framework}
\label{sec:model-analysis-config:solution}
In this section, we first provide a priority assignment scheme in Section~\ref{subsec:model-analysis-config:priority-assignment}, and then a preemption class assignment scheme in Section~\ref{subsec:model-analysis-config:preemption-class-assignment}

\subsubsection{Priority assignment}
\label{subsec:model-analysis-config:priority-assignment}
In this section, we present the priority assignment scheme for TSN flows based on the traditional \textit{k-means clustering algorithm}~\citep{hastie2009elements}. This is a popular unsupervised Machine Learning (ML) algorithm that is scalable and robust to noise and outliers in the data. Briefly, the algorithm works as follows. It partitions the elements of an unlabeled list into $k$ distinct clusters (with $k \ge 1$). Specifically, $k$ foci, called ``centroids," are iteratively computed within the data space. Clusters are formed around the centroids by assigning each element to the centroid closest to it. Finally, the position of each centroid is updated after each iteration to the midpoint of all data points assigned to it.
\begin{tcolorbox}
    In the context of this work, the ``elements'' to be assigned are flows and the $k$ clusters are the priorities.
\end{tcolorbox}
We recall that Ethernet supports eight (8) priority levels, so $k \leq 8$. The k-means algorithm performs clustering based on some selected characteristics of the elements, called ``features''. These features capture the domain-specific knowledge about the real-world objects/concepts that the items represent. In this framework, the features need to be defined and sometimes transformed into a format that the k-means algorithm can process. The process of defining and preparing features for ML algorithms is called ``feature engineering''. In the following section, we summarize the feature engineering for our TSN priority assignment problem.
\vspace{0.1in}

\noindent $\triangleright$ {\bf Feature engineering.}
%\label{sec:configuration:solution:feature-engin}
For the priority assignment problem, five of the seven flow parameters defined in the system model (see Section~\ref{sec:model:traffic}) are considered for the clustering process since the other parameters still need to be determined (i.e., priority and preemption class). In other words, the tuple $\langle {src}_i, {dst}_i, T_i, D_i, S_i \rangle$ is considered for each flow $f_i \in \mathcal{F}$. On the other hand, ${src}_i$ and ${dst}_i$ are used to determine the path length $\operatorname{PL}_i$ of the flow $f_i$, i.e., the number of links that $f_i$ traverses from ${src}_i$ to ${dst}_i$. Therefore, the number of features used for the clustering problem can be reduced to the tuple $\langle \operatorname{PL}_i, T_i, D_i, S_i \rangle$.

Note that these selected features are not on the same unit scale. In fact, the flow periods and deadlines can range from a few microseconds to hundreds of thousands of microseconds. At the other end of the table, the flow sizes can only take values between $64$ bytes and $1500$ bytes (i.e., the minimum and maximum valid Ethernet frame sizes, respectively). Finally, the range of ${ PL }_i$ largely depends on the network topology. In such a scenario, features with large values could dominate those with lower values, negatively affecting the actual performance of the k-means algorithm. To ensure that this is not the case, and to ensure that each feature has an impact on the learning process, a process called ``normalization'' is usually performed on the selected feature set~\citep{hastie2009elements}. In this work, this normalization process is performed for each of the features as follows. With respect to the flow length, all values are changed to obtain features in the interval $[-1, 0]$. For this purpose, we divide all flow lengths by the negative value of the longest flow path. Similarly, both $T_i$ and $D_i$ are normalized by dividing all values by the largest values of $T_i$ and $D_i$, respectively, to obtain features in the interval $[0, 1]$. Finally, the values of $S_i$ are normalized by the maximum frame size in the flowset to obtain features in the interval $[0, 1]$. The reason for normalizing the flow paths with the negative value of the longest flow path is that flows with shorter paths have higher feature values. This is explained in more detail in the following section. Note that with the normalization process, flows with longer paths, smaller periods, deadlines, and sizes are assigned smaller feature values.
\vspace{0.1in}

\noindent $\triangleright$ {\bf Clustering and priority assignment.}
%\label{sec:configuration:solution:clustering}
Here we describe our strategy for assigning priorities to flows by partitioning the $n$ flows in $\mathcal{F}$ into $k$ clusters (with $1 \leq k \leq 8$) using the k-means algorithm. The overall goal is to assign priorities to flows in such a way that as many flows as possible can be scheduled, i.e., meet their deadlines. Figure~\ref{fig:configuration:k-means-flowcart} shows the assumed flowchart.

\begin{figure}[htb]
\centering
\includegraphics[scale=0.9]{feupphdteses/sections/configuration/images/k-means-priority-assignment}
\caption{Flowchart: k-means priority assignment algorithm.}
\label{fig:configuration:k-means-flowcart}
%\vspace{-0.1in}
\end{figure}

From the figure, it is clear that the process begins with the feature engineering process described above. After this step, two important questions need to be clarified. 
\begin{tcolorbox} 
\begin{enumerate} 
\item[$Q_1$:] How does one determine the value of $k$? In other words, how do you determine the number of clusters (priorities) into which to divide the flows?
\item[$Q_2$:] How does one determine the relative order between clusters during the priority assignment process?
\end{enumerate}
\end{tcolorbox}

\textbf{About $Q_1$}. Since we do not know which value of $k$ gives the maximum number of schedulable flows, we initialize $k$ to $1$ and iterate through all possible values ($1 \leq k \leq 8$).

\textbf{About $Q_2$}. At each iteration, we perform k-means clustering with the normalized features and obtain the centroid of each of the $k$ clusters. Each centroid is a vector of the mean values of the features of the elements in the cluster. We then compute the mean of each centroid. Recall that because of the normalization process, flows with longer paths, smaller periods, deadlines, and sizes are assigned smaller feature values. Thus, the smaller the final value of the centroid of a given cluster, the longer the path and, in general, the smaller the period; deadline, and size of each of its members. In practice, flows with longer paths are at greater risk of not meeting their deadlines because of delays that may occur on the links they traverse. In addition, flows with shorter periods and deadlines are typically given higher priorities in fixed priority scheduling theory because they are at greater risk of missing their deadlines (think about Rate Monotonic and Deadline Monotonic policies). Finally, the sizes of non-time-critical flows are usually larger than the time-critical ones (see~\cite{LOBELLO2020153, Ojewale2021WorstCase} for examples inspired by real-world automotive use-cases).
\begin{tcolorbox}
 Based on the above observations, we chose to assign priorities to the clusters in ascending order of their centroid means. More specifically, \textit{the lower the centroid mean, the higher the priority}.
\end{tcolorbox}
In this work, we assume that all features have the same importance in the priority assignment process. Of course, other approaches to feature engineering can be used where specific properties of the network are exploited. For example, path length can be given a higher weight in a network with line topology. We also note that the schedulability tests in the priority assignment process (see Figure~\ref{fig:configuration:k-means-flowcart}) necessarily depend on the assignment of the preemption level, which is not defined at this point. To resolve this dependency, schedulability is evaluated assuming a fully preemptive scheme, i.e., any flow can preempt any other flow with a lower priority.

\subsubsection{Preemption class assignment}
\label{subsec:model-analysis-config:preemption-class-assignment}

\noindent $\triangleright$ {\bf Synopsis.}
Our solution for preemption class assignment builds on the priority assignment scheme. It starts with a non-preemptive scheme and uses a guided exhaustive search approach described as follows. At each step, we introduce an additional preemption level and test all possible configurations of flow-to-preemption-class to verify that all timing requirements are met. Our algorithm terminates once a solution is found. Otherwise, another preemption level is added to the flow transmission scheme and a new test is performed. Note that we are only interested in determining the schedulability of a flow set and not whether there are multiple solutions for a given flow set. This process is iterated until a valid configuration is found for a given preemption level or the maximum number of preemption levels (i.e., $7$) is exceeded. In the latter case, no valid configuration could be found and the flow set is classified as ``unschedulable". In the following, we provide the step-by-step details of our proposed solution, which consists of two algorithms, namely ($1$)~the \textit{flow-to-preemption-class assignment}; and ($2$)~the \textit{valid configuration search}.
\vspace{0.1in}

\noindent $\triangleright$ {\bf Flow-to-preemption-class assignment.}
\label{subsec:configuration:assignment-of-preemption-levels}
Algorithm~\ref{alg:assignment-of-preemption-levels} shows the pseudocode for this step. Two arguments are required as inputs, namely: ($1$)~the network topology $G$; and ($2$)~the flow set~$\mathcal{F}$. In the description, the notation ``$\operatorname{P.Len}$'' refers to the length of the list~$P$ and ``$[y]*\eta$'' refers to a list of length $\eta$ filled up with ``$y$'', e.g., $ [0]*3 = [0,0,0]$. The algorithm proceeds as follows.

First, the set of all unique flow priorities in $\mathcal{F}$ is stored in the variable $\operatorname{P}$ (see line~\ref{alg:ass-begin-init}). Then, a systematic search through all preemption levels $m$ (with $1 \leq m \leq \operatorname{P.Len} - 1$) is performed for a solution (see lines~\ref{alg:ass-begin-loop-level} to~\ref{alg:ass-end-loop-level}). At each preemption level $m$, after the initialization phase (see lines~\ref{alg:search-init} to~\ref{alg:search-end-right-part-init}), a recursive function $\operatorname{ VALID \_CONFIGS}()$ is called (see line~\ref{alg:search-valid-conf-call}). This function returns the set of all valid configurations for the preemption level~$m$, i.e. $\mathcal{C}^m$. It then searches this set to find a solution (see lines~\ref{alg:ass-begin-conf-check} to~\ref{alg:ass-end-conf-check}). If a solution is found, Algorithm~\ref{alg:assignment-of-preemption-levels} terminates with that solution (see line~\ref{alg:ass-return-present-conf}), otherwise $m$ is incremented and the process is repeated for the next preemption level $(m+1)$. If all iterations are exhausted and no solution is found, a $\operatorname{NULL}$ value is returned (see line~\ref{alg:ass-return-fail}), indicating that the flow set is ``unschedulable''. We note that for the schedulability test (see line~\ref{alg:ass-check-sched}) we use the worst-case traversal time (WCTT) analysis presented in Section~\ref{sec:model-analysis-config:analysis}.

\begin{algorithm}[tb]
\SetAlgoLined
\KwData{Network topology $G$; Flow set $\mathcal{F}$.}
\KwResult{A valid flow-to-preemption-class configuration.}
$\operatorname{P} \gets [Set\: of\: all\: unique\: flow \: priorities\: in \: \mathcal{F}]$\label{alg:ass-begin-init}

    \For{$m = \operatorname{0}\:  to \: \operatorname{P.Len} - 1$}{\label{alg:ass-begin-loop-level}
            %$\operatorname{preemption\_level} = i$
            $\mathcal{C}^m \gets \emptyset$\label{alg:search-init}\\
            
            $\operatorname{leftPart} \gets []$\label{alg:search-left-part-init}\\
        $\operatorname{rightPart} \gets [m]* \operatorname{P.Len}$\label{alg:search-init-all-flows-to-i} 
        
        \For{$j = 0\:  to \: m$}{
             $\operatorname{rightPart}[j] = j$\label{alg:search-init-highest-priorities-init}
         }\label{alg:search-end-right-part-init}
            $\mathcal{C}^m = \operatorname{VALID\_CONFIGS}(\mathcal{C}^m, \operatorname{leftPart},\:  \operatorname{rightPart})$\label{alg:search-valid-conf-call} 
            
            \ForEach{$\mathcal{C}_x^m \in \mathcal{C}^m$}{\label{alg:ass-begin-conf-check}
                %$\mathcal{F}_{temp} = \mathcal{F}$\\
                \ForEach{$f_i \in \mathcal{F}$}{
                    $\operatorname{PC}_i = c_{x,P_i}^m $ %f_i.priority
                }\label{als:ass-update-config}
                 
                 \If{$\operatorname{SCHEDULABLE}                 (\mathcal{F})$}{\label{alg:ass-check-sched}
                    \Return $\operatorname{\mathcal{C}_{x}^m}$\label{alg:ass-return-present-conf}
                }
            }\label{alg:ass-end-conf-check}  
    }\label{alg:ass-end-loop-level}

\Return{$\operatorname{NULL}$}\label{alg:ass-return-fail}
\caption{ASSIGN\_PREEMPTION\_CLASS($G$,$\mathcal{F}$)}
\label{alg:assignment-of-preemption-levels}
\end{algorithm}
\vspace{0.1in}

\noindent $\triangleright$ {\bf Valid configuration search.}
%\label{subsec:configuration:valid-configs}
Algorithm~\ref{alg:valid-config} presents the pseudocode. The recursive function $\operatorname{ VALID \_CONFIGS}$() computes the set of all valid configurations for a preemption level~$m$. It takes $3$ inputs: ($1$)~an initialization of the set $\mathcal{C}^m$ (which is usually an empty set at the beginning); ($2$)~a list $\operatorname{leftPart}$ (which is also usually empty at the beginning); and finally ($3$)~a $\operatorname{rightPart}$, which is a configuration initialization for the preemption level $m$. The notations in Algorithm~\ref{alg:valid-config} have the same meaning as those of Algorithm~\ref{alg:assignment-of-preemption-levels}. In addition, the notation $\operatorname{ListA} + \operatorname{ListB}$ implies a concatenation operation of two lists. In summary, $\operatorname{ VALID \_CONFIGS}$ solves the multiset generation problem described in Section~\ref{sec:model-analysis-config:definitions}.
Since the algorithm is recursive, the first step is to test for the base case (see lines~\ref{alg:valid-conf-begin-base-case} to~\ref{alg:valid-conf-end-base-case}). This is the case when the elements in $\operatorname{rightPart}$ are either all the same or all unique. In this case, the algorithm terminates and returns a merged (and sorted) list of $\operatorname{leftPart}$ and $\operatorname{rightPart}$. If the base condition is not satisfied, the recursive step (see lines~\ref{alg:valid-conf-length-diff} to~\ref{alg:valid-conf-end-recursive-case}) is executed.


\begin{algorithm}[tb]
\SetAlgoLined
\KwData{Set of generated configurations $\mathcal{C}^m$;\: a left partition; and an initial configuration for preemption level $m$}
\KwResult{Set of generated configurations $\mathcal{C}^m$}

%$\operatorname{configurations}.append \newline(\operatorname{All\: ordered \: combinations\: of \: init\_config\_list})$
$ \operatorname{rightPartSet} =  sorted(set(\operatorname{rightPart}))$\label{alg:valid-conf-init}

    \If{$\operatorname{rightPart.Len} == \operatorname{rightPartSet.Len}\: \newline  OR \:  \operatorname{rightPartSet.Len ==1}$}{\label{alg:valid-conf-begin-base-case}
    
        $\mathcal{C}^m.add(sorted(\operatorname{leftPart+rightPart}))$ 
        
        \Return {$\mathcal{C}^m$}
}\label{alg:valid-conf-end-base-case}
    $\operatorname{diff} = \operatorname{rightPart.Len} - \operatorname{rightPartSet.Len}$\label{alg:valid-conf-length-diff}\\
    $\operatorname{diff}+=1$\\	
    $\operatorname{currentLeft} = \operatorname{rightPartSet.getFirstElem}$\label{alg:valid-conf-begin-new-left}\\
    $\operatorname{rightPartSet.removeFirstElem}$\label{alg:valid-conf-end-new-left}\\
    \For{$x = 1\:  to \: diff$}{\label{alg:valid-conf-begin-recursice-case} 		
        $\operatorname{tempLeft} = [\operatorname{currentLeft}]*x$\\
        
        $\operatorname{newLeftPart} = \operatorname{leftPart} + \operatorname{tempLeft}$	\\	
        $\operatorname{rightSize} = \operatorname{rightPart.Len} - x$	\\	
        $\operatorname{newRightPart} = list(\operatorname{rightPartSet})$	\\
        
       \If{$\operatorname{rightSize} > \operatorname{newRightPart.Len}$}{
       
            $\operatorname{lenDiff} = \operatorname{rightSize}-\operatorname{rightPartSet.Len}$	\\		
           $\operatorname{newRightPart} = [\operatorname{rightPartSet.getFirstElem}]*\operatorname{lenDiff}~+ list(\operatorname{rightPartSet})$\\
}		
        $\mathcal{C}^m = \operatorname{VALID\_CONFIGS}(\mathcal{C}^m, newLeftPart,\newline newRightPart)$\label{alg:valid-conf-recursive-call}
}\label{alg:valid-conf-end-recursive-case}
    \Return {$\mathcal{C}^m$}\label{alg:valid-config-return}
\caption{VALID\_CONFIGS($\mathcal{C}^m$, leftPart, rightPart)}
\label{alg:valid-config}
\end{algorithm}

\noindent $\triangleright$ {\bf Computational Complexity.} We recall that the problem of finding all valid configurations (Algorithm~\ref{alg:valid-config}) has been mapped to the multiset problem, which is known to have exponential complexity. \cite{stanley2011enumerative} has already shown that the number of multisets of cardinality $k$ to be taken from the set of $m$ elements is given by:
\[
     \frac{(k+m-1)!}{k!(m-1)!} %\binom{k+m-1}{m} =
\] 
We recall that each element of $\{1,2, \ldots, m\}$ must occur at least once in each multiset (see Section~\ref{sec:model-analysis-config:model}). This constraint reduces the number of elements whose order must be decided from $k$ to $k-m$. Substituting $k$ for $k-m$ gives the total number of valid configurations $|\mathcal{C}^m|$ for preemption $m$ with $k$ unique priorities in Equation~\ref{eqn:complexity}. 

\begin{equation}
    \label{eqn:complexity}
    |\mathcal{C}^m| =  \frac{(k-1)!}{(k-m)!(m-1)!}
\end{equation}
Algorithm~\ref{alg:assignment-of-preemption-levels} calls function $\operatorname{VALID \_CONFIGS}()$ until a solution is found or the maximum number of preemption levels is exceeded. Consequently, the maximum number of valid configurations to test is given by Equation~\ref{eqn:complexity-sum}.

\begin{equation}
    \label{eqn:complexity-sum}
    \sum_{m=1}^{P.Len -1} |\mathcal{C}^m|
\end{equation}


%\textcolor{red}{Putting Equations~\ref{eqn:complexity} and~\ref{eqn:complexity-sum} together, the computational complexity of the preemption class assignment solution is $\mathcal{O}(2^n)$ where \textit{n} is the number of unique priorities in $\mathcal{F}$. We note that while the complexity of this solution is exponential, the value of $n$ cannot exceed $8$, thus, making the complexity of this approach reasonable and bounded.}


%To this end purpose, we consider two different settings:~($1$)~a synthetic use-case; and ($2$)~two real-life use-cases from the literature -- SAE~\citep{gavriluct2020traffic} and Orion~\citep{zhao2017timing}.



==> sections/model-analysis-config/model-analysis-config.tex <==
\chapter{Model, Analysis, and Configuration}
\label{chap:model-analysis-configuration}

Meeting timing requirements is essential for any real-time communication medium. Therefore, formal timing analysis must be performed to provide safe temporal guarantees for frame transmission times when a new feature/scheme is proposed. In this chapter, we present results on the worst-case traversal time (WCTT) of frames under the assumption of multi-level preemption. As in most, if not all, real-time and/or time-critical preemptive systems, an appropriate priority allocation policy plays a central role in the resulting performance of both $1$-level and multi-level preemption schemes to avoid over-provisioning and/or sub-optimal utilization of hardware resources. In addition, multi-level preemption raises new configuration issues. In particular, the correct number of preemption levels to enable, and the synthesis of the assignment of flows to preemption classes remain open problems. In this chapter, we address these configuration challenges by providing a new configuration framework. The remainder of the chapter is organized as follows. First, in Section~\ref{sec:model-analysis-config:model}, we introduce the system model and enforce a set of rules for network and traffic management. Then we present the WCTT analysis and the configuration framework in  Sections~\ref{sec:model-analysis-config:analysis} and ~\ref{sec:model-analysis-config:configuration}, respectively.

%Finally, Section~\ref{sec:model-analysis-config:summary} concludes the chapter.

\section{Model}
\label{sec:model-analysis-config:model}
\input{feupphdteses/sections/model-analysis-config/model.tex}

\section{Analysis}
\label{sec:model-analysis-config:analysis}
\input{feupphdteses/sections/model-analysis-config/analysis.tex}

\section{Configuration}
\label{sec:model-analysis-config:configuration}
\input{feupphdteses/sections/model-analysis-config/configuration.tex}

\section*{Chapter summary}
\label{sec:model-analysis-config:summary}
In this chapter, we have provided formal and rigorous timing guarantees for each flow under a multi-level preemption scheme using a CPA-based approach and addressed the synthesis problem for multi-level frame preemption in TSN. Specifically, we first introduced the system model and assumptions and provided a background on the CPA model. Next, we identified the components of delay experienced by the flow and provided formal upper bounds for each of these components. Finally, we presented a configuration framework for multi-level preemption that addresses the unique configuration issues of the scheme. In particular, for a set of flows and the network topology, we have presented a framework for assigning priorities to the flows, determining which preemption level to enable, and assigning flows to preemption classes. Now that we have presented the formal timing analysis and configuration framework for determining priority assignment and a valid configuration for a given set of flows, we can demonstrate the applicability of the proposed framework and evaluate its performance in the next chapter.

==> sections/model-analysis-config/model.tex <==
In this section, we introduce all the parameters and assumptions that we will use in this chapter. In particular, we introduce the network, traffic, and configuration specifications in Section~\ref{sec:model:network}, Section~\ref{sec:model:traffic}, and Section~\ref{sec:model:configuration}. We assume that all timing characteristics are non-negative integers, i.e., they are multiples of a discrete time interval (e.g., the CPU tick).

\subsection{Network specification.}
\label{sec:model:network}
We assume an Ethernet backbone network for a distributed real-time embedded system. We represent the network as a directed graph $G \equals (\mathcal{N}, \mathcal{L})$, where $\mathcal{N}$ is the set of all nodes and $\mathcal{L}$ is the set of all physical links in the network. We assume that each link is bidirectional, full-duplex, and operates at a single reference speed, say~$s > 0$. The tuple~$G$ is given with the interpretation that: ($1$)~$\mathcal{N} = \operatorname{EP} \cup \operatorname{SW}$, where~$\operatorname{EP} \equals \{\operatorname{EP}_1, \operatorname{EP}_2, \ldots \}$ represents the set of all endpoints and~$\operatorname{SW} \equals \{\operatorname{SW}_1, \operatorname{SW}_2, \ldots\}$ is the set of all switches. Each $\operatorname{EP}_q$ (with $q \ge 1$) has a single input/output port and can receive and send network traffic, while $\operatorname{SW}$~ consists only of forwarding nodes, each with a finite number of input/output ports over which traffic is routed. Each $\operatorname{SW }_{\ell}$ (with $\ell \ge 1$) is equipped with a multi-level preemption capability and decides to which output port to forward a received frame based on its internal routing table. We also assume that each input/output port of the switch has $8$ priority queues and that each queue has flows of the appropriate priority level assigned to it. Finally, we assume that each $\operatorname{SW}_{\ell}$ supports multi-level preemption and Strict Priority (ST) transmission.
\begin{tcolorbox} 
According to the IEEE 802.1 Qbu standard, frame preemption can be implemented with or without the TSN shapers such as TAS and CBS. In this work, we choose the latter scenario (i.e., an implementation without shapers) to focus solely on evaluating multi-level preemption without the added complexity of other feature mechanisms.
\end{tcolorbox}


\subsection{Traffic specification.}
\label{sec:model:traffic}
We consider $\mathcal{F} \equals \{f_1, f_2, ..., f_n\}$ a network traffic with $n \ge 1$~flows. Each flow $f_i \equals \langle src_i, dst_i, T_i, D_i, S_i, P_i, \operatorname{ PC }_i \rangle$ consists of a potentially infinite number of instances (a.k.a. frames) and is characterized by: ($1$)~$src_i$, the source endpoint; ($2$)~$dst_i$, the destination endpoint; ($3$)~$T_i$, the minimum inter-arrival time between two consecutive frames of $f_i$, i.e., assuming that the first frame of~$f_i$ is released at~$src_i$ at time~ $a_{i,1} \ge 0$, then $a_{i,\lambda + 1} - a_{i,\lambda} \ge T_i$ for all $\lambda \ge 1$, where $a_{i,\lambda}$ is the release time of the $\lambda^{\operatorname{th}}$ frame; ($4$)~$D_i$, the relative deadline, i.e., $d_{i,\lambda} \equals a_{i,\lambda} + D_i$ is the latest time at which the $\lambda^{\operatorname{th}}$ frame of $f_i$ must reach $dst_i$; ($5$)~$S_i$, the size of $f_i$ (in bytes); ($6$)~$P_i$ (with $0 \leq P_i \leq 7$), the priority; and finally ($7$)~$\operatorname{ PC }_i$ the preemption class. For simplicity, we assume that $0$ is the highest priority and $7$ is the lowest. The specification in the standards suggests otherwise. However, we have chosen to keep both the frame priority and preemption class in the same format (ascending order, starting with $0$) to improve readability. For the preemption classes, we also assume that the smaller the value, the higher the preemption class. Flows with the same priority always belong to the same preemption class, but the converse is not true. In other words, flows with the same preemption class can have different priorities (see Figure~\ref{fig:configuration:preemption-class}). %Finally, the priority and the preemption class parameters lie at the core of the configuration problem addressed in this chapter and are determined in Section~\ref{sec:configuration:solution}. 


%\vspace{0.1cm}
\subsection{Flow configuration.}
\label{sec:model:configuration}
For a flow set $\mathcal{F}$, we denote by $\mathcal{C}^m \equals \{ \mathcal{C}_1^m, \mathcal{C}_2^m, \mathcal{C}_3^m, \ldots \}$ the set of all possible flow configurations under the assumption of an $m$-level preemption scheme (with $ 0 \leq m \leq 7$). We recall that an $m$-level preemption scheme implies $m+1$ preemption classes. Each configuration $\mathcal{C}_x^m$ (with $x \ge 1$) is an \textit{integer list} defining the preemption class of each priority level. Specifically, $\mathcal{C}_x^mis \equals [c_{x,0}^m, c_{x,1}^m, \ldots, c_{x,p-1}^m]$, where $p$ is the number of distinct priorities in $\mathcal{F}$ and $c_{x,\sigma}^m$ (with $ 0 \leq \sigma \leq p-1$) is the preemption class of all flows $f_i \in \mathcal{F}$ with priority $P_i = \sigma$. In other words, a preemption configuration is a nondecreasing and surjective function. Figure~\ref{fig:configuration:preemption-class} shows an example of a flow configuration $\mathcal{C}_x^3$ for a $3$-level preemption scheme (i.e., with $4$ preemption classes). 

\begin{figure}[htb]
\centering
\includegraphics[scale=0.7]{feupphdteses/sections/configuration/images/queue-preemption-class-config}
\caption{Preemption classes; priority queues and Configuration.}
\label{fig:configuration:preemption-class}
\end{figure}

\noindent In this figure, we assume that $x=1$ to refer to the ''first configuration'' from the set of all possible configurations $\mathcal{C}^3$. Flows with priorities $0$ and~$1$ are assigned to the preemption class~$0$, i.e., $c_{1,0}^3 = 0$ and $c_{1,1}^3 = 0$; flows with priority $2$ are assigned to preemption class~$1$; flows with priorities $3$, $4$ and~$5$ are assigned to preemption class~$2$; and finally, flows with priorities $6$ and~$7$ are assigned to preemption class~$3$. Thus, the resulting configuration is $\mathcal{C}_1^3 = [0,0,1,2,2,2,3,3]$. Note that we assume a network-wide configuration, i.e., $\mathcal{C}_1^3$ applies to all switches. Also, for any $m$-level preemption scheme, the following rules apply.
\begin{tcolorbox}
\begin{enumerate} \item [$R_1$--] Each flow $f_i$ can be assigned to one and only one preemption class; \item [$R_2$--] To reduce priority inversion, a flow, say $f_j$, with a lower priority than another flow, say $f_i$, cannot be assigned to a higher preemption class than that of $f_i$; \item[$R_3$--] To conserve hardware resources, at least one flow must be assigned to each preemption class. \item[$R_4$--] Any flow, say $f_i$, can preempt any other flow, say $f_j$, only if $\operatorname{ PC }_i < \operatorname{ PC }_j$, but flows in $\operatorname{ PC }_j$ cannot preempt flows in $\operatorname{ PC }_i$;
 
\item[$R_5$--] Following the TSN standard convention, flows in the same preemption class cannot preempt each other and are transmitted in a strict priority order;

\item[$R_6$--] Flows with the same priority are transmitted in a FIFO manner;

\item[$R_7$--] Flows with the same priority always belong to the same preemption class, but the converse is not true. In other words, flows with different priorities can be assigned to the same preemption class.
\end{enumerate}
\end{tcolorbox}

For ease of reading, an overview of the notations used in this chapter is provided in Table~\ref{tab:notations}.

%In additions to the notations defined in Chapter~\ref{chap:model}, an overview of notations used in this chapter is provided in Table~\ref{tab:notations}.
\begin{center}
\begin{table}[htb]
\caption{Overview of key variables}
\label{tab:notations}
\begin{longtable}{p{2.1cm}|p{6.5cm}}
\toprule
 $a_i^q$ & Arrival time of the $q^{th}$ frame ($f_i^q$) of flow~$f_i$\\
 $\mathcal{BP}$ & Set of best-effort preemptable flows\\
 $C_i^+$ & Maximum time to transmit any frame of $f_i$\\
 $\operatorname{PC}_i$ & Set of flows in the same preemption class as $f_i$\\
 $\delta^{+/-}_i$(q)& Latest/earliest arrival time of $f_i^q$\\
 $\mathcal{E}$ & Set of eMAC flows\\
 $F^{+}_i$ & Maximum number of fragments of $C_i^+$\\
 $hep(i)$ & Set of flows with a higher priority than or equal to $f_i$\\
 $\HPI_i$ & Higher-priority interference suffered by $f_i$\\
 $hp(i)$ &  Set of flows with a higher priority than $f_i$\\
 $lp(i)$ &  Set of flows with a lower priority than $f_i$\\
 $\LPB_i$ & Lower-priority blocking suffered by $f_i$ (including express frames)\\
 $\mWCTT$ & Maximum measured end-to-end delay\\
 $\eta^{+/-}_i(\Delta t)$ & Maximum/Minimum possible arrivals of a frame of $f_i$ within the period $\Delta t$\\
 $p^{+/-}_i$ & Maximum/Minimum payload of frames of $f_i$\\
 $\PB_i$ & Blocking suffered by $f_i$ due to the transmission of a lower-priority preemptable frame/frame fragment\\
 $PO_i( \Delta t, q, a_i^q)$ & Preemption overhead incurred by $f_i^q$\\
 $Q_i(q, a_i^q)$ & Queuing delay of $f_i^q$\\
 $rTX$ & Link data transmission rate\\
 $\SPB_i$ & Same-priority blocking suffered by $f_i$\\
 $sp(i)$ & Set of all flows with the same priority as $f_i$\\
 $\mathcal{TP}$ & Set of time-sensitive preemptable flows\\
 $\WCTT(q, a_i^q)$ & Worst-case traversal time of $f_i^q$\\
\bottomrule
\end{longtable}
\end{table}
\end{center}


% In addition to these three rules, we introduce the following definitions for any flow set $\mathcal{F}$ and network $\mathcal{G}$.

% \begin{definition}[Valid configuration]
% \label{def:valid-config}
% Any configuration will be stamped as ``valid'' if upon the flow-to-preemption-class assignment, it conforms to Rules $R_1$, $R_2$ and $R_3$.
% \end{definition}

% \begin{definition}[Solution]
% \label{def:solution}
% Any valid configuration will be considered a ``solution'' if all flows $f_i \in \mathcal{F}$ meet their deadlines.
% \end{definition}

% Rule~$R_2$ implies that $\mathcal{C}_x^m$ (with $x \ge 1$) is always sorted in an ascending order, i.e., $c_{x,\sigma}^m \le c_{x,\ell}^m$ for all $0 \le \sigma \le \ell \le p-1$. Rule~$R_3$ implies that each integer from $0$ to $m$ must appear \textit{at least once} in each valid configuration. Consequently, the task of generating all valid configurations $\mathcal{C}^m$ can be mapped to the problem of generating all ordered multisets~\citep{blizard1989multiset} of cardinality $p$ with elements taken from the set $\{0, \ldots, m\}$, where $p$ is the number of unique flow priorities in $\mathcal{F}$. Rule~$R_3$ also implies that all elements $\{0, \ldots, m\}$ must appear at least once in each multiset. 
% In the following section, we first provide a priority assignment scheme in Section~\ref{subsec:configuration:priority-assignment}, and then a preemption class assignment scheme in Section~\ref{subsec:configuration:preemption-class-assignment}

%\begin{definition}[Optimal solution]
%\label{def:optimal-solution}
%A solution is said to be ``optimal'' if it utilizes the minimum number of preemption levels.  %and where flows are assigned to the lowest possible preemption class
%\end{definition}

% Finally, for the sake of readability, an overview of notations used in this thesis is provided in Table~\ref{tab:notations}.
% \begin{center}
% \begin{table}[ht]
% \caption{Overview of key variables}
% \label{tab:notations}
% \begin{tabular}{p{1.7cm}|p{6.5cm}}
% \toprule
%  $a_i^q$ & Arrival time of the $q^{th}$ frame ($f_i^q$) of flow~$f_i$\\
%  $\mathcal{BP}$ & Set of best-effort preemptable flows\\
%  $C_i^+$ & Maximum time to transmit any frame of $f_i$\\
%  $\operatorname{PC}_i$ & Set of flows in the same preemption class as $f_i$\\
%  $\delta^{+/-}_i$(q)& Latest/earliest arrival time of $f_i^q$\\
%  $\mathcal{E}$ & Set of eMAC flows\\
%  $F^{+}_i$ & Maximum number of fragments of $C_i^+$\\
%  $hep(i)$ & Set of flows with a higher priority than or equal to $f_i$\\
%  $\HPI_i$ & Higher-priority interference suffered by $f_i$\\
%  $hp(i)$ &  Set of flows with a higher priority than $f_i$\\
%  $lp(i)$ &  Set of flows with a lower priority than $f_i$\\
%  $\LPB_i$ & Lower-priority blocking suffered by $f_i$ (including express frames)\\
%  $\mWCTT$ & Maximum measured end-to-end delay\\
%  $\eta^{+/-}_i(\Delta t)$ & Maximum/Minimum possible arrivals of a frame of $f_i$ within the period $\Delta t$\\
%  $p^{+/-}_i$ & Maximum/Minimum payload of frames of $f_i$\\
%  $\PB_i$ & Blocking suffered by $f_i$ due to the transmission of a lower-priority preemptable frame/frame fragment\\
%  $PO_i( \Delta t, q, a_i^q)$ & Preemption overhead incurred by $f_i^q$\\
%  $Q_i(q, a_i^q)$ & Queuing delay of $f_i^q$\\
%  $rTX$ & Link data transmission rate\\
%  $\SPB_i$ & Same-priority blocking suffered by $f_i$\\
%  $sp(i)$ & Set of all flows with the same priority as $f_i$\\
%  $\mathcal{TP}$ & Set of time-sensitive preemptable flows\\
%  $\WCTT(q, a_i^q)$ & Worst-case traversal time of $f_i^q$\\
% \bottomrule
% \end{tabular}
% \end{table}
% \end{center}



==> sections/model/system-model.tex <==
\chapter{System Model}
\label{chap:model}
In this chapter we introduce all the parameters that will be used in the quantitative aspect of this dissertation. We assume all timing
characteristics to be non-negative integers, i.e. they are multiples of some discrete time interval.

\section{ Network specification.}
\label{sec:model:network}
We assume an  Ethernet backbone network for a real-time distributed system. We represent the network as a directed graph $G \equals (\mathcal{N}, \mathcal{L})$, where $\mathcal{N}$ is the set of all nodes and $\mathcal{L}$ is the set of all physical links in the network. We assume that every link is bi-directional; full-duplex; and operates at a single reference speed, say~$s > 0$. The tuple~$G$ is given with the interpretation that: ($1$)~$\mathcal{N} = \operatorname{EP} \cup \operatorname{SW}$, where~$\operatorname{EP} \equals \{\operatorname{EP}_1, \operatorname{EP}_2, \ldots \}$ represents the set of all end-points and~$\operatorname{SW} \equals \{\operatorname{SW}_1, \operatorname{SW}_2, \ldots\}$ is the set of all switches. Each $\operatorname{EP}_q$ (with $q \ge 1$) has a single output port and can receive and send network traffic while $\operatorname{SW}$~consists only of forwarding nodes, each with a finite number of output ports, through which the traffic is routed. Each $\operatorname{SW}_{\ell}$ (with $\ell \ge 1$) is enabled with multi-level preemption capability and decides, based on its internal routing table, to which output port a received frame will be forwarded. We also assume that each switch Input/Output port has $8$ priority queues and that each queue is assigned to flows of the corresponding priority level. According to the IEEE 802.1 Qbu standard, frame preemption can be implemented with or without the TSN shapers such as TAS and CBS. In this work, we choose the latter scenario to focus purely on the evaluation of multi-level preemption without the added complexity of other protocol mechanisms. Therefore, each $\operatorname{SW}_{\ell}$ only supports multi-level preemption and Strict Priority (ST) transmission. 

\section{Traffic specification.}
\label{sec:model:traffic}
We consider $\mathcal{F} \equals \{f_1, f_2, ..., f_n\}$ a network traffic with $n \ge 1$~flows. Each flow $f_i \equals \langle src_i, dst_i, T_i, D_i,\\ S_i, P_i, \operatorname{PC}_i \rangle$ consists of a potentially infinite number of instances (a.k.a. frames) and is characterized by: ($1$)~$src_i$, the source endpoint; ($2$)~$dst_i$, the destination endpoint; ($3$)~$T_i$, the minimum inter-arrival time between two consecutive frames of $f_i$, i.e., by assuming that the first frame of~$f_i$ is released at~$src_i$ at time~ $a_{i,1} \ge 0$, then $a_{i,\lambda + 1} - a_{i,\lambda} \ge T_i$ for all $\lambda \ge 1$, where $a_{i,\lambda}$ is the release time of the $\lambda^{\operatorname{th}}$ frame; ($4$)~$D_i$, the relative deadline, i.e., $d_{i,\lambda} \equals a_{i,\lambda} + D_i$ is the latest time instant by which the $\lambda^{\operatorname{th}}$ frame of $f_i$ must reach $dst_i$; ($5$)~$S_i$, the size of $f_i$ (in bytes); ($6$)~$P_i$ (with $0 \leq P_i \leq 7$), the priority; and finally ($7$)~$\operatorname{PC}_i$ the preemption class. For the sake of convenience, we assume that $0$ is the highest priority and $7$ is the lowest\footnote{The specification in the standards suggests the opposite. However, we opted to keep both the frame priority and preemption class in the same format (ascending order starting from $0$) to improve readability.}. For preemption classes, we assume in the same vein that the smaller the value, the higher the preemption class. Flows with the same priority always belong to the same preemption class but the converse is not true. In other words, flows with the same preemption class may have different priorities (see Figure~\ref{fig:configuration:preemption-class}). %Finally, the priority and the preemption class parameters lie at the core of the configuration problem addressed in this chapter and are determined in Section~\ref{sec:configuration:solution}. 

\begin{figure}[htb]
\centering
\includegraphics[scale=0.7]{feupphdteses/sections/configuration/images/queue-preemption-class-config}
\caption{Preemption classes; priority queues and Configuration.}
\label{fig:configuration:preemption-class}
\vspace{-0.1in}
\end{figure}

%\vspace{0.1cm}
\section{ Flow configuration.}
\label{sec:model:configuration}
For a flow set $\mathcal{F}$, we denote by $\mathcal{C}^m \equals \{ \mathcal{C}_1^m, \mathcal{C}_2^m, \mathcal{C}_3^m, \ldots \}$ the set of all possible flow configurations, assuming an $m$-level preemption scheme\footnote{An $m$-level preemption scheme implies $m+1$ preemption classes.} (with $ 0 \leq m \leq 7$). Each configuration $\mathcal{C}_x^m$ (with $x \ge 1$) is an \textit{integer list} that defines the preemption class of each priority level. Concretely, $\mathcal{C}_x^m  \equals [c_{x,0}^m, c_{x,1}^m, \ldots, c_{x,p-1}^m]$, where $p$ is the number of different priorities in $\mathcal{F}$ and $c_{x,\sigma}^m$ (with $ 0 \leq \sigma \leq p-1$) is the preemption class of all flows $f_i \in \mathcal{F}$ with priority $P_i = \sigma$. In other words, a preemption configuration is a non-decreasing and surjective function. Figure~\ref{fig:configuration:preemption-class} illustrates an example of flow configuration $\mathcal{C}_x^3$ for a $3$-level preemption scheme (i.e., with $4$ preemption classes). Here, we assume that $x=1$ in order to refer to the ``first configuration'' out of the set of all possible configurations $\mathcal{C}^3$. Flows with priorities $0$ and~$1$ are assigned to the preemption class~$0$, i.e, $c_{1,0}^3 = 0$ and $c_{1,1}^3 = 0$; flows with priority $2$ are assigned to the preemption class~$1$; flows with priorities $3$, $4$ and~$5$ are assigned to the preemption class~$2$; and finally, flows with priorities $6$ and~$7$ are assigned to the preemption class~$3$. Therefore, the resulting  configuration is $\mathcal{C}_1^3 = [0,0,1,2,2,2,3,3]$. Note that we assume a network-wide configuration, i.e., $\mathcal{C}_1^3$ applies to all switches. Furthermore, for any $m$-level preemption scheme the following rules are enforced.

\begin{enumerate}
    \item [$R_1$--] Every flow $f_i$ can be assigned to one and only one preemption class;
    \item [$R_2$--] To reduce priority inversion, any flow, say $f_j$, with a lower priority than another flow, say $f_i$, cannot be assigned to a higher preemption class than that of $f_i$;
    \item[$R_3$--] To conserve hardware resources, every preemption class must have at least one flow assigned to it. 
    
    \item[$R_4$--] Every flow, say $f_i$, can preempt any other flow, say $f_j$, only if $\operatorname{PC}_i < \operatorname{PC}_j$, but flows in $\operatorname{PC}_j$ cannot preempt flows in $\operatorname{PC}_i$;
    
\item[$R_5$--] Following the TSN standards convention, flows in the same preemption class cannot preempt each other and are transmitted with a strict priority order;

\item[$R_6$--] Flows with the same priority are transmitted in a FIFO manner;

\item[$R_7$--] Flows with the same priority always belong to the same preemption class but the converse is not true. In other words, flows with different priorities can be assigned to the same preemption class.

\end{enumerate}
Finally, for the sake of readability, an overview of notations used in this chapter is provided in Table~\ref{tab:notations}.

%In additions to the notations defined in Chapter~\ref{chap:model}, an overview of notations used in this chapter is provided in Table~\ref{tab:notations}.
\begin{center}
\begin{table}[htb]
\caption{Overview of key variables}
\label{tab:notations}
\begin{longtable}{p{2.1cm}|p{6.5cm}}
\toprule
 $a_i^q$ & Arrival time of the $q^{th}$ frame ($f_i^q$) of flow~$f_i$\\
 $\mathcal{BP}$ & Set of best-effort preemptable flows\\
 $C_i^+$ & Maximum time to transmit any frame of $f_i$\\
 $\operatorname{PC}_i$ & Set of flows in the same preemption class as $f_i$\\
 $\delta^{+/-}_i$(q)& Latest/earliest arrival time of $f_i^q$\\
 $\mathcal{E}$ & Set of eMAC flows\\
 $F^{+}_i$ & Maximum number of fragments of $C_i^+$\\
 $hep(i)$ & Set of flows with a higher priority than or equal to $f_i$\\
 $\HPI_i$ & Higher-priority interference suffered by $f_i$\\
 $hp(i)$ &  Set of flows with a higher priority than $f_i$\\
 $lp(i)$ &  Set of flows with a lower priority than $f_i$\\
 $\LPB_i$ & Lower-priority blocking suffered by $f_i$ (including express frames)\\
 $\mWCTT$ & Maximum measured end-to-end delay\\
 $\eta^{+/-}_i(\Delta t)$ & Maximum/Minimum possible arrivals of a frame of $f_i$ within the period $\Delta t$\\
 $p^{+/-}_i$ & Maximum/Minimum payload of frames of $f_i$\\
 $\PB_i$ & Blocking suffered by $f_i$ due to the transmission of a lower-priority preemptable frame/frame fragment\\
 $PO_i( \Delta t, q, a_i^q)$ & Preemption overhead incurred by $f_i^q$\\
 $Q_i(q, a_i^q)$ & Queuing delay of $f_i^q$\\
 $rTX$ & Link data transmission rate\\
 $\SPB_i$ & Same-priority blocking suffered by $f_i$\\
 $sp(i)$ & Set of all flows with the same priority as $f_i$\\
 $\mathcal{TP}$ & Set of time-sensitive preemptable flows\\
 $\WCTT(q, a_i^q)$ & Worst-case traversal time of $f_i^q$\\
\bottomrule
\end{longtable}
\end{table}
\end{center}


% In addition to these three rules, we introduce the following definitions for any flow set $\mathcal{F}$ and network $\mathcal{G}$.

% \begin{definition}[Valid configuration]
% \label{def:valid-config}
% Any configuration will be stamped as ``valid'' if upon the flow-to-preemption-class assignment, it conforms to Rules $R_1$, $R_2$ and $R_3$.
% \end{definition}

% \begin{definition}[Solution]
% \label{def:solution}
% Any valid configuration will be considered a ``solution'' if all flows $f_i \in \mathcal{F}$ meet their deadlines.
% \end{definition}

% Rule~$R_2$ implies that $\mathcal{C}_x^m$ (with $x \ge 1$) is always sorted in an ascending order, i.e., $c_{x,\sigma}^m \le c_{x,\ell}^m$ for all $0 \le \sigma \le \ell \le p-1$. Rule~$R_3$ implies that each integer from $0$ to $m$ must appear \textit{at least once} in each valid configuration. Consequently, the task of generating all valid configurations $\mathcal{C}^m$ can be mapped to the problem of generating all ordered multisets~\citep{blizard1989multiset} of cardinality $p$ with elements taken from the set $\{0, \ldots, m\}$, where $p$ is the number of unique flow priorities in $\mathcal{F}$. Rule~$R_3$ also implies that all elements $\{0, \ldots, m\}$ must appear at least once in each multiset. 
% In the following section, we first provide a priority assignment scheme in Section~\ref{subsec:configuration:priority-assignment}, and then a preemption class assignment scheme in Section~\ref{subsec:configuration:preemption-class-assignment}

%\begin{definition}[Optimal solution]
%\label{def:optimal-solution}
%A solution is said to be ``optimal'' if it utilizes the minimum number of preemption levels.  %and where flows are assigned to the lowest possible preemption class
%\end{definition}

% Finally, for the sake of readability, an overview of notations used in this thesis is provided in Table~\ref{tab:notations}.
% \begin{center}
% \begin{table}[ht]
% \caption{Overview of key variables}
% \label{tab:notations}
% \begin{tabular}{p{1.7cm}|p{6.5cm}}
% \toprule
%  $a_i^q$ & Arrival time of the $q^{th}$ frame ($f_i^q$) of flow~$f_i$\\
%  $\mathcal{BP}$ & Set of best-effort preemptable flows\\
%  $C_i^+$ & Maximum time to transmit any frame of $f_i$\\
%  $\operatorname{PC}_i$ & Set of flows in the same preemption class as $f_i$\\
%  $\delta^{+/-}_i$(q)& Latest/earliest arrival time of $f_i^q$\\
%  $\mathcal{E}$ & Set of eMAC flows\\
%  $F^{+}_i$ & Maximum number of fragments of $C_i^+$\\
%  $hep(i)$ & Set of flows with a higher priority than or equal to $f_i$\\
%  $\HPI_i$ & Higher-priority interference suffered by $f_i$\\
%  $hp(i)$ &  Set of flows with a higher priority than $f_i$\\
%  $lp(i)$ &  Set of flows with a lower priority than $f_i$\\
%  $\LPB_i$ & Lower-priority blocking suffered by $f_i$ (including express frames)\\
%  $\mWCTT$ & Maximum measured end-to-end delay\\
%  $\eta^{+/-}_i(\Delta t)$ & Maximum/Minimum possible arrivals of a frame of $f_i$ within the period $\Delta t$\\
%  $p^{+/-}_i$ & Maximum/Minimum payload of frames of $f_i$\\
%  $\PB_i$ & Blocking suffered by $f_i$ due to the transmission of a lower-priority preemptable frame/frame fragment\\
%  $PO_i( \Delta t, q, a_i^q)$ & Preemption overhead incurred by $f_i^q$\\
%  $Q_i(q, a_i^q)$ & Queuing delay of $f_i^q$\\
%  $rTX$ & Link data transmission rate\\
%  $\SPB_i$ & Same-priority blocking suffered by $f_i$\\
%  $sp(i)$ & Set of all flows with the same priority as $f_i$\\
%  $\mathcal{TP}$ & Set of time-sensitive preemptable flows\\
%  $\WCTT(q, a_i^q)$ & Worst-case traversal time of $f_i^q$\\
% \bottomrule
% \end{tabular}
% \end{table}
% \end{center}



==> sections/routing/routing.tex <==
%\part{Bounding the Cache Related Contention in Single-core Platforms}
\chapter{On Smart Routing Schemes for Performance Improvement}
\label{chap:routing}

% \begin{center}
% 	\fbox{\bf
% 		\centering
% 		\begin{minipage}{\linewidth}
% 			\centering
% 			The outcome of the work that has been presented in this chapter titled ``Routing Heuristics for Load-balanced Transmission in TSN-Based Networks'' was accepted at the $17^{th}$ International Workshop on Real-Time Networks\footnote{https://www.ecrts.org/rtn/}, 
% 			(RTN'19) held at Stuttgart, Germany.   
% 	\end{minipage}}
% \end{center}



% \section{Introduction}
\label{sec3:intro}
\input{feupphdteses/sections/routing/sections/introduction.tex}

%
% \section{Time Sensitive Networking (TSN)}
% \label{sec:tsn}
% \input{sections/TSN.tex}
%
\section{Model of Computation}
\label{sec3:problem}
\input{feupphdteses/sections/routing/sections/problem_statement.tex}
%

%
% \section{Problem Statement}
% \label{sec:problem}
% \input{sections/formulation.tex}
%
\section{Proposed Solution}
\label{sec3:algorithms}
\input{feupphdteses/sections/routing/sections/approach.tex}

%
%\section{Congestion Recovery}
%\label{sec3:recovery}
%\input{sections/recovery.tex}
%
\section{Experimental Evaluation}
\label{sec3:experiment}
\input{feupphdteses/sections/routing/sections/experiment.tex}

%

% \section{Related Work}
% \label{sec3:related_work}
% \input{feupphdteses/sections/routing/sections/related_work.tex}

\section*{Chapter Summary}
\label{sec3:conclusion}
% % \input{feupphdteses/sections/chapter-2/sections/conclusion.tex}


% \subsection{Work Package 1 (WP1)}
% \textbf{To design and implement experiments that demonstrate the performance gains under multi-level preemption.}

% % \begin{itemize}
% % \item \textbf{Task1.1:} 
% % \item \textbf{Task1.2:} 

% % \item \textbf{Task1.3:} I

% % \end{itemize}

% \subsection{Work Package 2 (WP2)}

% \textbf{To further explore the impact of multi-level preemption on the worst-case latency analysis, especially in the presence of traffic shapers.}



% \subsection{Chapter Summary}

\label{C3:sec:summary}
\input{feupphdteses/sections/routing/sections/conclusion.tex}

==> sections/routing/sections/TSN.tex <==

The IEEE Time Sensitive Networking (TSN) group \cite{IEEE} is developing a new set of standards to introduce real-time features to Ethernet. Networks conforming to these standards are referred to  as  TSN networks. TSN is an emerging technology in real-time communication domains. The standards specify mechanisms for achieving not just a reliable transmission, but also a transmission with a bounded delay. For a given Ethernet network, it introduces features like ($i$)~global clock synchronization~\cite{Ieee2015802.1Qbv}; ($ii$)~frame replication and elimination~\cite{Ieee2017802.1CB}; ($iii$)~frame preemption~\cite{Ieee2016Preemption802.3br, IEEE802.1Qbu}; ($iv$)~path control and reservation~\cite{Ieee802.1Qca}; and finally ($v$)~network configuration~\cite{IEEE802QCC}. All these features put together to ensure reliable transmission and predictable end-to-end transmission delays. Specifically, global clock synchronization allows the clocks present at the network nodes to be precisely synchronized for accurate delay monitoring. Frame replication and elimination make it possible to achieve negligible packet losses. Frame preemption prevents non ``time-critical frames'' from blocking the transmission of ``time-critical frames''. Path control and reservation provide a mechanism to guarantee a Quality of service (QoS) level for streams before transmission~\cite{Ieee802.1Qca}. Finally, the network configuration features a centralized (re)-configuration capability to switched Ethernet networks. On another front, TSN provides mechanisms for defining different traffic classes for frames. 

The basic Ethernet standard ~\cite{IEEE2014} defines eight traffic classes, which can be grouped into three subcategories with TSN. These categories are referred to as (1) “Control data Traffic (CDT)”; (2) “Rate Constrained Traffic (RC)” (also corresponding to Audio Video Bridge Traffic (AVB)) and finally (3) “Best Effort Traffic (BE)”~\cite{IEEE802.1BA}. In a nutshell, CDT is traffic with real-time constraints; RC are traffic with predefined QoS constraints and BE is traffic with non-real-time requirements. As such, only CDT and RC traffics can have bounded end-to-end delays under TSN. For a comprehensive overview on TSN, we refer the interested reader to~\cite{Nasrallah2018}. In the context of this work, it is sufficient to mention that TSN extends the capabilities of Ethernet to traffic with stringent timing requirements. Also, we should mention that TSN ensures reliable and near-zero loss communication through its frame replication and elimination mechanism~\cite{Ieee2017802.1CB}. This involves each sending node making multiple copies of a frame and transmitting these on the network. The receiver nodes then will only receive one copy and discard (eliminate) the duplicated copies. Ideally, replicated frames should be transmitted on distinct paths without any overlap between the selected paths. But in reality, this is sometimes not feasible as some network topologies may not allow more than one distinct path from some source nodes to the destinations. In this case, it is important to design a routing mechanism that computes as distinct as possible alternative paths to replicated frames. TSN exhibits the potential to replace the current bus-based or Ethernet communication backbones in emerging application domains.

%Several research efforts  contributed to paving the way toward an efficient configuration of the traffic queues and computation of the dispatch tables. ~\cite{Gutierrez2015, Craciunas2016Qbv, Raagaard2017 } are a few examples. Some other contributions also provide enhancements to improve the QoS of non-CDT traffic ~\cite{Zhao2018, Nasrallah2018} and others estimate the Worst-Case Transmission Time (WCTT) of all traffic types ~\cite{Smirnov2017, Zhao2018, ThieleFormal}. Consequently, 

%TSN provides standards for achieving not just a reliable transmission, but also a transmission with a bounded delay. For a given Ethernet network, it introduces features like (i) global clock synchronization ~\cite{Ieee2015802.1Qbv};(ii) frame replication and elimination ~\cite{Ieee2017802.1CB}; (iii) frame preemption ~\cite{Ieee2016Preemption802.3br}, ~\cite{IEEE802.1Qbu}; (iv) path control and reservation ~\cite{Ieee802.1Qca}; and finally (v) network configuration ~\cite{IEEE802QCC}. All put together, these features ensure reliable transmission and predictable end-to-end transmission delays. Specifically, global clock synchronization allows the clocks present at the network nodes to be precisely synchronized for accurate delay monitoring. Frame replication and elimination make it possible to achieve negligible packet losses. Frame preemption prevents non “time-critical frames” from blocking the transmission of “time-critical frames”. Path control and reservation provide mechanisms to guarantee a Quality of service (QoS) level for streams before transmission ~\cite{Ieee802.1Qca}. Finally, network configuration provides a centralized (re-)configuration capability to switch Ethernet networks. On another front, TSN provides mechanisms for defining different traffic classes for frames. The basic Ethernet standard ~\cite{IEEE2014} defines eight traffic classes, which can be grouped into three different categories with TSN. These categories are referred to as (1) “Control data Traffic (CDT)”; (2) “Rate Constrained Traffic (RC)” (also corresponding to Audio Video Bridge Traffic (AVB)) and finally (3) “Best Effort Traffic (BE)”~\cite{IEEE802.1BA}. In a nutshell, CDT are traffic with real-time constraints; AVB are traffic with pre-defined QoS constraints and BE are traffic with non-real-time requirements. As such, only CDT and AVB traffics can have bounded end-to-end delays under TSN. The so-called “Time-Aware shapers (TAS)” ~\cite{Ieee2015802.1Qbv} has been introduced to meet this ambitious goal by ensuring that CDT and AVB traffics have guaranteed transmission slots in a cyclic and pre-computed dispatch schedule. 

%In addition to the TAS, TSN proposed the Burst Limiting Shaper (BLS) and the Peristatic Shaper (PS) ~\cite{Thiele2015Peristaltic}. Before these shapers,  AVB networks use the  Credit Based-shapers (CBS)~\cite{IEEE802.1BA} have been used to moderate the transmission bandwidth of AVB traffic classes and protect the whole network from burst effects. Under CBS, a transmission budget, also called a “credit”, is associated to each AVB traffic class in order to control its transmission rate. Here, the transmission of a frame belonging to an AVB class depends on the availability of the transmission credit of this class. The credit associated to each class at design time depletes as the frames from this class are being transmitted. Once the credit is exhausted, new frames from the class cannot be transmitted until the credit is replenished again. This offers a time window to frames belonging to other traffic classes to be transmitted. The replenishment modality of each budget is defined by the user, depending on the desired QoS. The BLS belongs to the class of CBS. However, BLS allows CDT traffic to make limited excess transmissions in transient overload (burst) conditions ~\cite{Thiele2016BLS}. Conversely, PS imposes an organization on the reception and transmission of frames at each node of the network by following well-defined equal time intervals. Here, every time window is divided into intervals (even and odd intervals) and all the frames that are received within an interval are transmitted in the next interval only. Figure \ref{fig:outputport} shows the schematic diagram of a TSN egress port.  

% \begin{figure}
%   \begin{center}
%     \includegraphics[width=\linewidth]{Images/tsnoutputport.PNG}
%     \caption { Schematic diagram of TSN frame forwarding at the egress port} 
%     \label{fig:outputport}
%   \end{center}
% \end{figure}

% In this figure, the gate control list for the TAS is shown in the table with entries $T_0, T_1,\ldots,  T_N$. Each entry $T_i$ consists of a sequence of zeros and ones representing the gate event at the output queues (Q1, …, Q8) of the port. A “1” indicates that the associated gate is open for transmission; whereas a “0” means that it is closed. The first row in the table, for example, indicates that at time $T_0$, the gate of Q1 is opened for transmission and all the others are closed. In the same vein, at time $T_1$, the gate of Q1 is closed for transmission and the gates of all the other queues (Q2 to Q8) are open. The last entry in the table says that the TAS schedule described in the table repeats in a cyclic manner. A frame on a queue can be transmitted only when its gate is opened at the time period. Note that each queue contains a unique class of frames, i.e., frames belonging to different traffic classes cannot share the same queue. Also, for AVB traffic classes (AVB 1 and AVB 2), a PS shaper, as described previously, is attached to the output gate to moderate the transmission of these traffic. Finally, the egress port selects the frame to be transmitted based on their respective priorities.



==> sections/routing/sections/abstract.tex <==
A carefully designed routing synthesis can help system designers achieve a better load balancing in TSN-based networks and avoid congestion. To this end purpose, this work proposes two heuristics referred to as ($1$)~$\lbdrr$, which aims at achieving a better load balancing and compute as much disjoint routing paths as possible for each replicated flow; and ($2$)~$\crdrr$, which recomputes paths for time-sensitive flows in congestion situations. Extensive simulations demonstrate that the proposed approach outperforms the classical Shortest Path (SPA) and the weighted Equal Cost Multi-path (wt-ECMP) algorithms in terms of the maximum load transmitted on a link by more than $70\%$ and $20\%$, respectively.


%In addition, they expect to achieve a reliable and near-zero loss transmission by introducing frame replication and elimination. This involves multiple copies of the same frame to be transmitted on the network via distinct paths. Unfortunately, congestion may occur in TSN networks due to temporary overload conditions or some node malfunctioning. To overcome this issue, a carefully designed routing synthesis can help avoid and/or deal with congestion situation. Ideally, replicated frames should have distinct paths but this is not the case in reality. In this work, we solve the above mentioned routing challenges by proposing two heuristic routing algorithms to achieve load balancing in TSN networks; compute as much disjoint routing paths as possible for replicated frames; and also recompute the paths for scheduled framed in overload conditions. 


==> sections/routing/sections/acknowledgment.tex <==
This work was partially supported by National Funds through FCT (Portuguese Foundation for Science and Technology) and co-financed by ERDF (European Regional Development Fund) under the Portugal2020 Program, within the CISTER Research Unit (CEC/04234).

==> sections/routing/sections/approach.tex <==
For the routing problem, we assume that all edges are homogeneous (i.e., they all have the same properties and are interchangeable). Before explaining our proposed routing strategy in detail, we should first define some terms so that the reader can better understand our approach.

\begin{definition}[Route]
\label{def:route}
A {\em route} $r_i$ of flow $f_i$ is defined as an ordered list of edges that can be traversed by $f_i$ from its source to its destination. Specifically: \[ r_i \equals \left\langle(src_i, v_{i, 1}), (v_{i, 1}, v_{i, 2}), \ldots, (v_{i, p}, dst_i)\right\rangle \]
\end{definition}

\begin{definition}[Valid route]
\label{def:valid_route}
A {\em valid route} for $f_i$ is defined as any route $r_i$ that meets its timing requirement~$D_i$.
\end{definition}

\begin{definition}[Length of a route]
\label{def:len_of_route}
The length of a route $r_i$ denoted by $len(r_i)$ is defined as the number of edges along the route.
\end{definition}

\begin{definition}[load of an edge]
\label{def:load}
For every edge $e = (v_1, v_2)\in \mathcal{V} \times \mathcal{V}$, we define the {\em load of~$e$}, denoted by $load(e)$, the sum of the sizes of all flows traversing $e$. Formally, the load of edge $e$ is defined by Equation~\ref{eqn:load}.
\begin{equation}
\label{eqn:load}
    load(e) \equals \sum_{f_i \: \operatorname{traversing} \: e} C_i
\end{equation}
\end{definition}

\begin{definition}[MaxLoad of a route]
\label{def:max_load}
The {\em MaxLoad} of a route $r_i$, denoted by $Maxload(r_i)$, is defined as the {\em maximum} load of all edges in $r_i$. Formally, the MaxLoad of route~$r_i$ is defined by Equation~\ref{eqn:maxload}.
\begin{equation}
\label{eqn:maxload}
    Maxload(r_i) \equals \max_{e \in r_i} \{load(e)\} 
\end{equation}
\end{definition}

% For the routing problem described in section ~\ref{sec:intro}, we are interested in designing algorithms that balances the transmission load in the network, while still meeting the timing requirements. In this scenario,
At this stage, we have all the tools we need to describe our proposed routing solution. The basic idea is as follows. Unlike traditional routing schemes (e.g., SPA, ECMP and wt-ECMP), where the underlying strategy is to find the shortest route for each flow, here we examine all valid routes. If we denote by $R_i$ the set of all valid routes for flow $f_i$, then our routing strategy is to select the route that leads to the best load distribution in $R_i$, i.e., the route that minimizes the cost function defined in Equation~\ref{eqn:cost}.
\begin{equation}
\label{eqn:cost}
    Cost(r_i, K) \equals Maxload(r_i) \: + K \cdot len(r_i)
\end{equation} 
\noindent In this Equation~\ref{eqn:cost}, the parameter $K > 0$ is a user-defined penalty constant. This parameter is meant to penalize the routes with longer length. 

\begin{tcolorbox}
   To make it short, parameter $K$ must be considered as a trade-off. It must be set so that the weight of $K \cdot len(r_i)$ in the cost function is significant and $Maxload(r_i)$ does not dominate it, and vice versa. 
\end{tcolorbox}
\noindent In the latter case, if $K \cdot len(r_i)$ dominates $Maxload(r_i)$, then the cost function would behave like wt-ECMP. On the other hand, {\em Maxload($r_i$)} is computed to penalize solutions where some edges in the route transmit a high number of flows, making these edges potential bottlenecks. Last but not least, if multiple routes provide the same lowest cost value, we select one of these routes in an arbitrary manner. Formally, for each flow $f_i$, its best route $Best(f_i)$ is defined by Equation~\ref{eqn:goal}.
\begin{equation}
\label{eqn:goal}
    Best(f_i) \equals \min_{r_i \in \operatorname{valid\_routes}} \left\{Cost(r_i, K)\right\} 
\end{equation}
From this equation, it follows that wt-ECMP is a special case of the proposed approach where the parameter $K$ is sufficiently large and $K \cdot len(r_i)$ dominates over $Maxload(r_i)$. Now we can proceed with the details of our proposed routing schemes.
\vspace{0.15cm}

\noindent $\triangleright \triangleleft$ {\bf On load-balancing (Algorithm~\ref{alg:lbdrr})}.
\label{subsec:load-bal}
The load balancing routing scheme ($\lbdrr$) takes three components as inputs, namely: ($1$)~the network topology $\mathcal{G}$; ($2$)~the set $\mathcal{F}$ of flows to be routed; and finally ($3$)~the user-defined penalty variable $K$. In the description of the algorithm, the notation $|A|$ refers to the cardinality of the set~$A$.

\begin{algorithm}[htb]
\SetAlgoLined
\KwData{Network topology $\mathcal{G}$; Set of flows $\mathcal{F}$; Constant $K$}
\KwResult{List of best routes for each flow in F}
$\operatorname{R} \gets empty \: list []$\;\label{alg:begin-init}
$\operatorname{edges} \gets$ Set of all edges in $G$\;
$\operatorname{load} \gets zeros [|edges|]$\;\label{alg:end-init}

\ForEach{$f_i \in F$}{
    $R_i \gets  [] $\;
    % $Maxload \gets \emptyset$\;
    % $Cost \gets \emptyset$\;
    % \ForEach{$r \in routes$}{ 
    %     $Maxload(r) \gets \max(load[e]$ for e in r\;
    %     $Cost(r) \gets Maxload(r) + k \cdot len(r)$\;
    % } %\ENDFOR
    Compute $r_i = Best(f_i)$ (see Equation~\ref{eqn:goal})\;\label{alg:best-route}
    %update the load(e) for each edge in $r_i$
  
    \ForEach{$e \in r_i$}{
        $load[e] = load[e] + C_i$\;\label{alg:update-edge-load}
    } %\ENDFOR \;  
    $R_i.append (r_i)$\;
    \If{$rep_i > 0$}{\label{alg:route-replicates}
        $used\_edges \gets \{e \in r_i\}$\;\label{alg:used-edges}
        $routes = \operatorname{valid\_routes}(G, src_i, dst_i)$\;\label{alg:valid-routes}
        \For{$j = 1\:  to \: rep_i$}{ 
            $r_{i,j} = \displaystyle\argmin_{r \in routes} {(|used\_edges \cap \{e \in r\}|)}$\;\label{alg:find-least-overlap}
            \ForEach{$egde \in r_{i,j} $}{ 
                $load[e] = load[e] + C_i$\;\label{alg:update-edge-load-rep}
            } %\ENDFOR \;
            $used\_edges = used\_edges \cup \{e \in r_{i,j}\}$\;\label{alg:update-used-edges}
            $R_i.append(r_{i,j})$\;\label{alg:update-R-i}
        } %\ENDFOR \;
        
   }\label{alg:end-route-replicates}
    $R.append(R_i)$\;\label{alg:update-R}
}
\Return{$R$} \label{alg:return-lbdrr}
\caption{LB-DRR.}
\label{alg:lbdrr}
\end{algorithm}

For each flow $f_i$, $\lbdrr$ computes the best route after the initialization phase (lines~\ref{alg:begin-init} to~\ref{alg:end-init}) using the Equation~\ref{eqn:goal} (line~\ref{alg:best-route}). Then, the load of all edges on this route is updated (line~\ref{alg:update-edge-load}) and the selected route is appended to the list of best routes $R_i$ of flow $f_i$. If the number of replicas of $f_i$ is strictly greater than zero, then all edges already traversed by the original flow $f_i$ are recorded in the variable $used\_edge$ (line~\ref{alg:used-edges}). Next, all valid routes are computed (line~\ref{alg:valid-routes}) and the route $r_{i,j}$ that has the least overlap with $used\_edges$ is selected for replica $f_{i,j}$ (with $j \in [1, rep_i]$) (line~\ref{alg:find-least-overlap}). If multiple routes return the same minimum overlap with $used\_edges$, then one of these routes is chosen arbitrarily and the load of all edges is updated to $r_{i,j}$ (line~\ref{alg:update-edge-load-rep}). Note that the edges belonging to $used\_edges$ are also updated to include those traversed by the replica $f_{i,j}$ (line~\ref{alg:update-used-edges}). Then, the route $r_{i,j}$ is appended to $R_i$ (line~\ref{alg:update-R-i}) and $R_i$, the list of selected routes for $f_i$ and its replicas, is appended to the list $R$ of selected routes for all flows (line~\ref{alg:update-R}). When this process is complete for all $f_i$ to be transmitted, the algorithm returns the list $R$ (line~\ref{alg:return-lbdrr}).

\begin{algorithm}[htb]
\SetAlgoLined
\KwData{Network topology $G$; Original routing configuration $R$; List  of loads on each edge ($load$); Congestion threshold $cgst\_threshold$; Constant $K$}
\KwResult{A new routing configuration $R_{new}$}

$ cgst\_edges  \gets \{e\:  in\:  \mathcal{G}\: |\:  load(e) >\:  cgst\_threshold\}$\;\label{alg:cgst_edges-comp}
$ New\_Topology  \gets \mathcal{G} \setminus cgst\_edges$\;\label{alg:init-new-topology}
$cgst\_routes \gets \{r \in R \: | \: r \cap cgst\_edges \neq \emptyset \}$\;\label{alg:cgst-edges}
$cgst\_flows \gets \{f_i\: traversing \: a\: route \: in \: cgst\_routes \}$\;\label{alg:cgst-flows}
$R_{new} \gets R \setminus cgst\_routes $\;\label{alg:init-R-new}
\ForEach{$f_i \in cgst\_flows$}{
    %$R_i \gets  [] $\;
    $routes \gets valid\_routes(New\_Topology, src_i, dst_i)$\;\label{alg:find-alternative-route}
    
    \eIf{$(routes \neq \emptyset)$ \label{alg:admissible}}{
    
     $r_i = \displaystyle\argmin_{r \in routes} (Cost(r, K))$\;\label{alg:best-alternative}
     \eIf{$(Maxload(r_i) \leq cgst\_threshold)$}{ \label{alg:admissible-upperbound}
     
     \ForEach{$e \in old\_r_i$}{\label{alg:loop-previous-route}
        $load[e] = load[e] - C_i$ \; \label{alg:sub-load-congested-route}
    } %\ENDFOR \;
    \ForEach{$e \in r_i$}{ 
        $load[e] =load[e] + C_i$ \;\label{alg:add-load-new-route}
    } %\ENDFOR \;
    %$R_i.append (r_i)$\;
    \ForEach{$e \in cgst\_edges$}{ \label{alg:begin-decongest}
        \If{($load(e) \leq cgst\_threshold$)}{ 
            $New\_Topology = New\_Topology.add(e)$\;
            $cgst\_edges = cgst\_edges \setminus \{e\}$\;
        } %\ENDIF \;
    }\label{alg:end-decongest} %\ENDFOR 

        
    }{ 
            $r_i = old\_r_i$\label{alg:no-alternative-threshold}
    }
   }{
         %$r_i = cgst\_routes(f_i)$ 
        $r_i = old\_r_i$\label{alg:no-alternative}    
   

   }
        $R_{new}.add(r_i)$\;\label{alg:update-R-new}
}
\Return{$R_{new}$} \label{alg:return-crdrr}
\caption{CR-DRR.}
\label{alg:crdrr}
\end{algorithm}

\vspace{0.1in}
\noindent $\triangleright \triangleleft$ {\bf On congestion recovery (Algorithm~\ref{alg:crdrr}).}
\label{subsec:Recovery}
This algorithm, referred to as $\crdrr$, is based on the {\em Tabu meta-heuristic}~\citep{glover1990tabu} and is reactive in that it aims to redirect flows that are in a congestion situation. In short, the main intuition behind any tabu-based meta-heuristic is to temporarily mark some moves as forbidden in order to force the algorithm to search for alternative solutions that may be better compared to the current solution with respect to a given metric. With this concept in mind, the $\crdrr$ scheme works as follows. It takes five components as input: ($1$)~the network topology $\mathcal{G}$; ($2$)~the initial routing configuration for all flows~$R$; ($3$)~the congestion threshold $cgst\_threshold$ which defines the upper limit of the allowed load on an edge before it is considered congested; ($4$)~the list of loads on each edge ($load$); and finally ($5$)~the user-defined penalty variable~$K$. All congested edges according to the $cgst\_threshold$ parameter are stored as ``tabu-edges'' ($csgt\_edges$) and temporarily removed from the network topology (line~\ref{alg:init-new-topology}).

\begin{tcolorbox}
    For each congestion situation, we initialize the set of congested routes $csgt\_routes$ (i.e., all routes that contain at least one congested edge), the set of flows ($csgt\_flows$) that traverse the congested routes, and the new set of routes $R_{new}$ that contains all routes in $R$ except the congested routes (lines~\ref{alg:cgst-edges} to~\ref{alg:init-R-new}). Then, for each congested flow $f_i \in cgst\_flows$, we search for alternative routes in the new topology (line~\ref{alg:find-alternative-route}).
\end{tcolorbox}
\noindent From these alternative routes, we choose the best route $r_i$ using Equation~\ref{eqn:cost} (line~\ref{alg:best-alternative}). Recall that if multiple routes yield the same minimum cost, we arbitrarily choose one of these routes. We check that the rerouting of the flow $f_i$ does not cause congestion on any edge in $r_i$ (line~\ref{alg:admissible-upperbound}). If this is the case, we leave $f_i$ on its original route $old\_r_i$ (line~\ref{alg:no-alternative-threshold}). At the end of this process, we update the list $load$ in two phases: ($i$)~on the old route $old\_r_i$: we subtract $C_i$ from all edges (line~\ref{alg:sub-load-congested-route}) and ($ii$)~on the new route $r_i$: we add $C_i$ to all edges (line~\ref{alg:add-load-new-route}). We update $cgst\_edges$ accordingly (lines~\ref{alg:begin-decongest} to~\ref{alg:end-decongest}). If there is no alternative route for $f_i$ in $New\_Topology$, it stays on its original route $old\_r_i$ (line~\ref{alg:no-alternative}). Finally, the computed route is appended to $R_{new}$ (line~\ref{alg:update-R-new}) and when all congested flows have been rerouted, the $R_{new}$ list is returned for all flows (line~\ref{alg:return-crdrr}).

==> sections/routing/sections/conclusion.tex <==
In this chapter,  we proposed two routing heuristics, referred to as $\lbdrr$ and $\crdrr$, to address the problems of load-balancing and congestion in TSN networks. We evaluated the performance of the proposed schemes against the popular SPA and wt-ECMP routing algorithms and showed an improvement of more than $70\%$ and $20\%$, respectively. This improvement has been observed w.r.t. the maximum load transmitted on an edge. On another front, the proposed heuristics exhibit high scalability w.r.t. an increase in the number of flows. 

% \subsection{Research Direction}
% \textbf{Given these promising results, we plan to investigate both the routing and scheduling of time-sensitive flows simultaneously in the preemptive TSN context. Also, we would like to develop techniques to reduce the search space of valid routes for better scalability, and quantify the impact of routing techniques on end-to-end timing requirements.}
% \vspace{0.15cm}
%relax the user-defined constant $K$ and seek for an optimal value

==> sections/routing/sections/experiment.tex <==
In this section, we report on the experiments we performed on synthetic workloads to evaluate the performance of the proposed heuristics ($\lbdrr$ and $\crdrr$) in terms of the maximum load transmitted on an edge compared to SPA and wt-ECMP. We then evaluate the scalability of the proposed algorithms to demonstrate their applicability.

\vspace{0.15cm}
\noindent $\triangleright$ \textbf{Setup}. We consider a TSN network with $50$ nodes and a connectivity degree falling in the interval $[0.15, 0.35]$, modeled as an {\em Erdős-Rényi} (ER) graph~\citep{erdHos2013spectral}. Such a graph can be generated by starting with a set of $n$ nodes and independently adding edges between them with probability $p$. The result is a graph with a random number of edges. The expected number of edges in an ER graph is equal to $n(n-1)/2 \times p$. Here $p$ is our predefined connectivity degree. We set $K = 100$ and randomly generate up to $1000$ real-time flows in window $[25,200]$, where the size of each flow is between $200$ and $1000$ bytes, the deadlines are between $2~ms$ and $5~ms$, and the replication level between $0$ and $2$. In the first set of experiments, we adopted the $\lbdrr$ routing scheme, and in the second set, we adopted the SPA routing scheme. In the latter case, we applied the algorithm $\crdrr$ to reroute the flows in case of congestion.

\vspace{0.15cm}
\noindent $\triangleright$ {\bf Results and discussion.}
In the first set of experiments, we found that $\lbdrr$ reduces the maximum load transmitted on an edge (Maxload) by an average of $70.3\%$ and $23.3\%$, respectively, compared to SPA and wt-ECMP. Figure~\ref{fig:load_balance} shows the Maxload for each routing scheme when the number of flows varies and $\lbdrr$ clearly dominates both SPA and wt-ECMP.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.8]{feupphdteses/sections/routing/Images/load_balance.pdf} 
    \caption{Load balancing: $\lbdrr$ vs. SPA and wt-ECMP.}
    \label{fig:load_balance}
\end{figure}

In Figure~\ref{fig:load_balance_c}, we observed that $\lbdrr$ performs better by varying the connectivity level of the network and its Maxload decreases significantly. 

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.8]{feupphdteses/sections/routing/Images/load_balance_c.pdf}
    \caption {Performance improvement w.r.t. network connectivity.}
    \label{fig:load_balance_c}
\end{figure}

Note that higher connectivity leads to longer runtime overhead due to the increasing number of routes to consider. Figure~\ref{fig:scale_f} illustrates the scalability of $\lbdrr$ as the number of flows increase.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.8]{feupphdteses/sections/routing/Images/scale_f.pdf} 
    \caption{Scalability w.r.t. number of flows.}
    \label{fig:scale_f}
    \end{figure}
 
As for increasing the number of flows, we found that $\lbdrr$ scales linearly, but very slowly (it took only $26$~seconds to compute routes for $1000$ flows). Now, if we increase the number of nodes, we set the connectivity level of the network to $0.2$ and consider $100$ real-time flows. Figure~\ref{fig:scale_n} shows that the execution time of $\lbdrr$ increases exponentially when the number of nodes exceeds $75$. However, it could still compute routes for $125$ nodes in $11$ minutes.

 \begin{figure}[htb]
        \centering
        \includegraphics[scale=0.8]{feupphdteses/sections/routing/Images/scale_n.pdf}
        \caption{Scalability w.r.t. number of nodes.}
        \label{fig:scale_n}
    \end{figure}
    

In the second set of experiments, we routed $750$ real-time flows with $SPA$, and observed tremendous congestion on the selected routes. Figures~\ref{fig:recovery_per_edge} and~\ref{fig:recovery_agg} show the results of congestion recovery and load redistribution.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.8]{feupphdteses/sections/routing/Images/congestion_r_n} 
    \caption{$\crdrr$ adopted to recover from congestion}
    \label{fig:recovery_per_edge}
\end{figure}

In Figure~\ref{fig:recovery_per_edge}, the network load was initially unbalanced (see the red curve), with multiple flows routed only a limited number of edges (see the leftmost peak), while several edges remained unused (see the rightmost long end). By applying the $\crdrr$ scheme, a significant improvement was observed (see the black curve). Figure~\ref{fig:recovery_agg} shows the load distribution of the congested network before and after applying $\crdrr$.
\begin{figure}[htb]
    \centering
       \includegraphics[scale=0.8]{feupphdteses/sections/routing/Images/congestion_r1.pdf}
    \caption{Load distribution under $\crdrr$.}
   \label{fig:recovery_agg}
\end{figure}
\begin{tcolorbox}
From Figure~\ref{fig:recovery_agg}, it can be seen that the load distribution curve of $\crdrr$ is close to the normal distribution.  Finally, $\crdrr$ shows the same behavior as $\lbdrr$ in terms of scalability.
\end{tcolorbox}


 

==> sections/routing/sections/introduction.tex <==
%In Chapter~\ref{chap:model-analysis-configuration} we analyzed the delay experienced by frames at the switch output ports of each transmission node. This delay increases with the number of nodes a frame traverses. Therefore, it is important to design routing mechanisms that reduce the number of links traversed. On the other hand, queuing delay components can increase significantly if frames are transmitted only over a few links on the shortest paths. In this chapter, we explore routing heuristics that balance the tradeoff between routing on the shortest path and ensuring that the transmission load is distributed as evenly as possible across the network.

%The TSN flow control mechanism can be considered from two perspectives: ($1$)~the scheduling (i.e., when each flow shall be transmitted); and ($2$)~the routing (i.e., on which path each flow shall be transmitted). D{\"u}rr et al.~\citep{durr2016no} demonstrated that the scheduling problem of real-time (a.k.a. time-sensitive) flows can be reduced to the No-Wait Job Shop Problem (NW-JSP), which is NP-Hard. On another front, Wang and Crowcroft~

%\citep{Wang1996QualityofServiceRF} proved that any routing problem that is subject to two or more independent additive or multiplicative tree constraints is NP-Hard. This is the case for time-sensitive flows. They are subject to timing, bandwidth, cost, and reliability constraints. Consequently, seeking an exact solution is very challenging and computationally expensive. Designing efficient heuristics is the only viable alternative. 

In the previous chapters, we implicitly assumed that for each flow there is a predefined and/or known route from the source node to the destination node, and that the routing strategy does not affect the performance of the network. \cite{Nayak2017}, \cite{Singh2017}, and \cite{gavrilut2017fault}, among others, have highlighted the importance of flow routing schemes for low latency, predictability, and reduced architectural cost in TSN, arguing that an inappropriate routing strategy may increase the number of transmission operations, leading to additional delays. In fact, an inappropriate routing scheme can increase the blocking time of flows in the network if too many flows attempt to traverse the same path at the same time. In this chapter, we focus on the routing problem of TSN flows. We believe that a strategy that minimizes the number of transmissions and the blocking time of each flow would help to avoid or mitigate these situations.

The TSN standard for path control and reservation~\citep{Ieee802.1Qca} recommends the \textit{Constrained Shortest Path First} (CSPF) routing scheme for transmission of time-sensitive flows (see page $71$). It specifies that this scheme 
\begin{tcolorbox} \enquote{
{\em essentially performs shortest-path routing on the topology that only contains the links meeting the constraint(s).}
}
\end{tcolorbox}

From this quote, it is clear that CSPF is similar in its operation to the \textit{Shortest Path Algorithm} (SPA). Consequently, this algorithm is also susceptible to congestion and longer blocking times for flows. To illustrate this claim, consider the network topology in Figure~\ref{fig:routing:topology}, in which six nodes ($N_1$ to $N_6$) and four switches ($\operatorname{SW}_1$ to $\operatorname{SW}_4$) are connected by full-duplex links. The nodes communicate through flow transmissions across the links and switches.

\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=1\linewidth]{feupphdteses/sections/routing/Images/topology}
    \caption {Congestion under CSPF routing policy.} 
    \label{fig:routing:topology}
  \end{center}
\end{figure}

In this example, we consider three flows -- flow $f_1$ (green) is transmitted from $N_1$ to $N_6$; $f_2$ (yellow) from $N_2$ to $N_5$; and finally, flow $f_3$ (brown) is transmitted from $N_3$ to $N_4$. We assume that the CSPF routing strategy is applied and that all valid paths from each source to each destination node allow each flow to satisfy its end-to-end timing requirement. Then, all these flows are transmitted over their shortest paths, which include the ``direct link'' (in red) between $\operatorname{SW}_1$ and $\operatorname{SW}_4$, thereby increasing the eventual blocking time over this link for each flow. This fact makes this link a potential single point of failure for the network and can cause congestion despite the high connectivity. The same limitation applies to the so-called \textit{Equal Cost Multi-Path} (ECMP) and the \textit{weighted Equal Cost Multi-Path} (wt-ECMP) routing schemes~\citep{Singh2017}. The basic idea of these two routing schemes is as follows. In ECMP, instead of computing a single shortest route, as is the case with SPA, multiple shortest routes are computed from which one or more routes are arbitrarily selected. The wt-ECMP scheme differs from ECMP only in the selection mechanism. Here, all computed shortest routes are assigned a ``weight'' to ensure that the selection is not arbitrary.
 
To circumvent the above hurdles and take full advantage of network connectivity, we propose a routing strategy that ensures load balancing, i.e., a strategy that distributes transmission operations as evenly as possible across links. In addition, this approach ensures that no link becomes the network's single potential point of failure.

\begin{tcolorbox}
 Two heuristics, referred to as \textit{Load-Balanced, Dynamic, and Replication-aware Routing algorithm} ($\lbdrr$) and \textit{Congestion Recovering, Dynamic and Replication-aware Routing} ($\crdrr$), are proposed in this framework with the following objectives:

\begin{itemize} \item[$\triangleright$] $\lbdrr$ aims to find a feasible route for each flow so that traffic on each link is minimized. This heuristic also ensures that replicated flows are transmitted on routes that are as disjoint as possible. \item[$\triangleright$] $\crdrr$ aims to compute alternative routes for each flow in a runtime congestion situation.
\end{itemize}
\end{tcolorbox}

The rest of this chapter is organized as follows. Section~\ref{sec3:problem} introduces the model of computation and introduces the notations adopted in this chapter. Our proposed heuristics ($\lbdrr$ and $\crdrr$) are explained in more detail in Section~\ref{sec3:algorithms}. Finally, Section~\ref{sec3:experiment} reports on the experiments performed and discussions about them.

%To achieve a reliable and near-zero loss transmission, TSN introduces frame replication and elimination to the Ethernet. This involves making multiple copies of the same frame and transmitting same on the network. The reciever nodes only recieve one copy of the frame and discards (eliminates) the duplicate copies. Ideally, replicated frames should be transmitted on distinct paths without any overlap. In reality, however,this is sometimes not feasible as some network topology may not have more than one distinct path from some sources to some destinations. In this case, what is achievable is to design a routing mechanism that achievs as much as possible distinct path computation for replicated streams.


==> sections/routing/sections/problem_statement.tex <==
In this section, we define the network topology and the flow specification that we assume in this chapter. We also introduce the notations and parameters that are necessary for a good understanding of our proposed heuristics.
\begin{tcolorbox}
    We note that the assumed model differs from the model presented in Section~\ref{sec:model-analysis-config:model} in that the connections here are not full-duplex and each flow may have replicas that are also transmitted over the network. This is because in this chapter we address the routing problem in a more general TSN context and are not limited to preemptive TSN networks only.
\end{tcolorbox}

\noindent $\triangleright$ {\bf Network topology specification.} We model the network as an undirected graph $\mathcal{G} \equals (\mathcal{V}, \mathcal{E})$, where the set $\mathcal{V} = N \cup \operatorname{ SW }_i$ of vertices in $\mathcal{G}$ consists of a finite set $N$ of endpoints and $\operatorname{ SW }_i$ of switches (see Figure~\ref{fig:routing:topology} for an example). The vertices are connected by a set $E$ of half-duplex links or edges. This means that each edge $e \in E$ is defined by a pair $(v_1, v_2) \in \mathcal{V} \times \mathcal{V}$ of two connected nodes, that allow data to be transmitted in only one direction at a time.

\vspace{0.15cm}

\noindent $\triangleright$ {\bf Flow specification.} We consider a set consisting of $n$ \emph{sporadic} time-sensitive flows $\mathcal{F} \equals \{f_1, f_2,\ldots, f_n \}$. Each flow $f_i \equals (src_i, dst_i, rep_i, C_i, T_i, D_i) \in \mathcal{F}$ is characterized by a \textbf{6-tuple,} where: ($1$)~$src_i$ is the source node of the flow; ($2$)~$dst_i$ is the destination node of the flow; ($3$)~$rep_i$ is the replication level of the flow (i.e., the number of replicas of $f_i$ that may be transmitted from $src_i$ to $dst_i$); ($4$)~$C_i$ is the size of the flow; ($5$)~$T_i$ is the minimum inter-arrival time of the flow (also known as the period); and finally, ($6$)~$D_i$ is the deadline of the flow, i.e., the latest time at which at least one copy (original or replicas) of $f_i$ must reach $dst_i$. We define the set of replicas of $f_i$ as $rep_{f_i} \equals \{f_{i,1}, f_{i,2},\ldots, f_{i, rep_i} \}$ and assume that each flow and all its replicas are transmitted {\em simultaneously} over the network.
% \footnote{Note that 1-to-m flows (with $m>1$) a.k.a. multi-cast flows can be captured in this model as $m$ 1-to-1 flows.}.
 
 



==> sections/routing/sections/related_work.tex <==
Traffic routing of time-sensitive (real-time) flows is non trivial~\citep{Nasrallah2018}. Routing optimization has been well studied in literature and sophisticated techniques have been proposed~\citep{wang2000multicast, grammatikakis1998packet}. However, contributions on TSN routing schemes have started less than a decade ago. In this context, both the rapid spanning tree protocol and shortest path bridging algorithms have widely been adopted in practice~\citep{Pop2016cyber}. On another front, the IEEE802.1 Qca standard~\citep{Ieee802.1Qca} specifies the Constrained Shortest Path First routing algorithm for TSN transmissions, but this algorithm does not prevent congestion situations and can increase contention in the network, unfortunately. Arif and Atia~\citep{arif2016load} proposed a methodology to evaluate the routes of a TSN end-to-end connection, but load-balancing was not part of their objectives.
\vspace{0.15cm}

Nayak et al.~\citep{Nayak2017} explored ILP-based algorithms for routing time-sensitive flows in TSN networks with Time Aware Shapers (a.k.a. IEEE-802.1Qbv). The proposed approach in their work differs from ours in that it does not address the congestion and load-balancing problems. Targeting a better load balancing for a TSN network, Singh~\citep{Singh2017} presented an algorithm, based on meta-heuristics, capable of routing new traffic flows at runtime with minimal overhead. But, the proposed approach adopts the shortest path algorithm (SPA) as an initial solution, and not all feasible routes are considered. This limits the solution search space, unfortunately. Gavrilut et al.~\citep{gavrilut2017fault} also took the same path and proposed heuristic methods for topology and routing synthesis. Their method tries to achieve optimal usage of the switches and links as well as an efficient routing of flows. However, they did not consider load-balancing. This paper fills this gap: it solves the problem of load-balancing, disjoint routing for duplicated flows, and dynamic re-routing in congestion situations.

%There are numerous contributions in the literature on the topic of timing analysis of deterministic Ethernet networks. In this section, we only report investigations in the context of IoT. 
%Serna et al ~\citep{oliver2014analysis} examined the suitability of an online incremental approach for the synthesis of time-triggered schedules in IIoT and profiled a number of metrics and trade-offs that had an impact on the efficiency, scalability, and feasibility. These metrics include the total number of schedulable requests; the link utilization and the effect of tight end-to-end latency on the schedulability. The simulation monitored the effects of traffic parameters like link utilization, end-to-end latency requirements, and period variations on online approaches of time-triggered schedule synthesis. Here, the end-to-end latency was assumed and given as part of the task parameters. However, the work does not contain any analysis for measuring it.

%Also, Simon et. al. in ~\citep{simon2017ethernet} showed, by simulation, how TSN protects express traffic (i.e., traffic with timing requirements) from lower priority traffic in Industrial Applications. The work promotes standard Ethernet, with a TSN feature, as a viable alternative to industrial networks in factory automation. In the same paper, the authors also highlighted the effects of factors such as packet size, link rate and source delay variation on overall packet delay variation. The work examines, by simulation, the packet transports in typical industrial network scenarios using TSN. However, it does not address the overall end-to-end delay. Simulation has been used in the study of network behavior. However, for deterministic Ethernet timing behavior, while it exhibits far less pessimism and is very useful for validating bounds provided by analytical approaches (e.g., the Compositional Performance Analysis (CPA) ~\citep{henia2005system, Rox2010}; the Network Calculus ~\citep{thiele2000real}, and the Transversal Approach ~\citep{bauer2012applying}), it fails to guarantee an exhaustive exploration of all possible scenarios~\citep{ThieleFormal}. As such, it holds true that a simple simulation is not enough for providing a safe upper bound on the WCTT of Ethernet frames. To date, we are not aware of any contribution in the state-of-the-art addressing in a formal and rigorous manner this problem, and this work is the first attempt in this direction.

%Several research efforts  contributed to paving the way toward an efficient configuration of the traffic queues and computation of the dispatch tables for TSN flows. ~\citep{Gutierrez2015, Craciunas2016Qbv, Raagaard2017 } are a few examples. Some other contributions also provide enhancements to improve the QoS of TSN traffic ~\citep{Zhao2018, Nasrallah2018} and others estimate the Worst-Case Transmission Time (WCTT) of all traffic types ~\citep{Smirnov2017, Zhao2018, ThieleFormal, Thiele2015Peristaltic}. 


